Opted Out, Yet Tracked: Are Regulations Enough to Protect Your Privacy?

Data protection regulations, such as GDPR and CCPA, require websites and embedded third-parties, especially advertisers, to seek user consent before they can collect and process user data. Only when the users opt in, can these entities collect, process, and share user data. Websites typically incorporate Consent Management Platforms (CMPs), such as OneTrust and CookieBot, to solicit and convey user consent to the embedded advertisers, with the expectation that the consent will be respected. However, neither the websites nor the regulators currently have any mechanism to audit advertisers' compliance with the user consent, i.e., to determine if advertisers indeed do not collect, process, and share user data when the user opts out. In this paper, we propose an auditing framework that leverages advertisers' bidding behavior to empirically assess the violations of data protection regulations. Using our framework, we conduct a measurement study to evaluate four of the most widely deployed CMPs, i.e., Didomi, Quantcast, OneTrust, and CookieBot, as well as advertiser-offered opt-out controls, i.e., National Advertising Initiative's opt-out, under GDPR and CCPA. Our results indicate that in many cases user data is unfortunately still being collected, processed, and shared even when users opt-out. We also find that some CMPs are better than the others at conveying user consent and that several ad platforms ignore user consent. Our results also indicate that advertiser-offered opt-out are equally ineffective at protecting user privacy.

==> Makefile <==
extensions_to_clean := out aux log bbl blg fls fdb_latexmk glg gls lof glo glsdefs lot toc dvi ist acn acr synctex.gz alg xdy

all: paper

clean:
	@if [[ -f paper.pdf ]]; then \
		rm paper.pdf;\
	fi;
	@for extension in $(extensions_to_clean); do \
		find . -type f -name "*.$$extension" -delete;\
	done;

paper:
	latexmk -bibtex -pdf paper
	pdflatex -bibtex -interaction=nonstopmode paper

==> docs/3_methodology_backup.tex <==
\section{Methodology}
\label{sec:methodology}






\subsection{Experimental setup}
%We will do an initial crawl to find the persona and crawl configuration that triggers the most targeting. 
\textcolor{blue}{The purpose of the experiments is to figure out if the opt out really work.} So we will use that persona and crawl configuration to crawl a set of websites where we will opt out of tracking through consent management platforms. 
%We will also test the same set of websites by applying user controls (i.e. cookie blocking and fingerprint faking) to study their impact on targeting. 

We have 2 steps in our experiment setting. 

%\begin{figure}[]
%	\centering
%	\includegraphics[width=.9\linewidth]{figures/main/initial_fig.png}

%	\caption{Initial Crawl}
%	\label{initial}
%\end{figure}	

%\subsubsection{Initial Crawl} The first step is ``Initial crawl''. The purpose of this step is to find out which persona will be most affected by which human behaviors.  We selected 16 personas's key words in this step. For each persona, we have 4 behavior crawler settings. Each behavior crawler setting has 2 phrases: training phrase and testing phrase. Before training phrase, the crawler will create a new browser profile. Figure \ref{initial} shows how Initial Crawl works.


%\textbf{Training phrase: }The training phrase are different in 4 behavior crawler settings. In the 1st crawler setting ``vanilla crawl'', the crawler will visit one training site, wait 2-3 seconds, move to the next training site. In the 2nd crawler setting ``Interactive crawl 1'', the crawler only click subpages of each training site. In the 3rd crawler setting ``Interactive crawl 2'', the crawler click subpages of each training site, and the ads on the training site. In the 4th crawler setting ``Shopping cart crawl'', we only add products to the cart on each training site. After visiting all training websites, we will save the update browser profile as ``P''.

%\textbf{Testing phrase: }The testing phrase for 4 behavior crawler settings are same: visit each testing site three times, save all ads images, and use Prebid.js to collect bids value from each testing site. In creating the testing sites list, we filtered all websites that support header bidding from the Alexa top 10k website list. We chose top 25 websites from the filtered sites list as the testing sites. The crawler will load the profile ``P'' before visiting each testing website. And the profile ``P'' will not be updated after visiting each testing website.


%We ran those crawlers on the remote server at Iowa.


\begin{figure}[]
	\centering
	\includegraphics[width=.9\linewidth]{figures/main/opt_out_fig.png}

	\caption{Opt-Out Crawl: CMPs}
	\label{opt-out-cmp}
\end{figure}	


\begin{figure}[]
	\centering
	\includegraphics[width=.9\linewidth]{figures/main/opt_out_central_fig.png}

	\caption{Opt-Out Crawl: Central}
	\label{opt-out-cen}
\end{figure}	

\subsubsection{Opt-Out Crawl}The first step is ``opt-out crawl''. In this step, we will figure out if we can see the targeting ads after opting out from different CMPs. We will use the proxy in California and Europe to do this ``opt-out'' experiment. CCPA required websites providing ``Do not sell my information'' option for users when users are in California. GDPR in Europe protect EU residents' personal information before the residents giving consents to the websites. The purpose of this experiment is to verify if the websites followed CCPA or GDPR.  We implemented ``OpenWPM'' and used it as the crawling tool. We created 8 Amazon AWS EC2 instances and used ``tiny proxy'' as the proxy on those intances in training and testing phrases. We selected ``Onetrust'' and ``Cookiebot'' as the tested CMPs. The setting in this step also has 2 phrases: training phrase and testing phrase. Figure \ref{opt-out-cmp} and figure \ref{opt-out-cen} shows how Opt-Out Crawl works. \textcolor{blue}{Training will create a profile which meets the persona keyword. The data collected from the testing will display the feedback of this profile from the ads providers.}

\textbf{Training phrase: }
%In the first step ``Initial crawl'', we have selected one persona and one behavior. So in the training phrase, we will do what we did for this persona and behavior in the first step. 
\textcolor{blue}{At the beginning of this phrase, the crawler will create a new browser profile. Then the crawler will visit all assigned training websites sequentially, based on this persona keyword. Every time the browser finish visiting the training website, the browser profile will be updated. After visiting all training websites, the crawler will save the update browser profile as ``P'' on the server. This profile can be seen as a human profile who is interested in this persona keyword. This profile `P' will be used in Testing phrase.}

\textbf{Testing phrase: }In the testing phrase, all testing websites will use same CMPs and support header bidding. In creating Onetrust testing website list, we filtered the Alexa top 10k websites, and 37 of them support header biddings and use Onetrust service. After loading the CA proxy, 11 out of 37 provide opt out option. Under Germany IP, 27 out of 37 websites allow the users to give or not give consent. In creating Cookiebot testing website list, we also filtered Alexa top 10k websites. But only 2 websites use Cookiebot and header bidding. So I filtered Alexa top 100k websites, and 13 of thme use Cookiebot and support header bidding. Under CA IP, 5 out of 13 provide opt-out option to users. We will visit each testing website 4 times: in the first visit, we opt out the targeting/tracking cookie usage on CMPs. We call this visit "Opt-out visit". After opting out, we will visit this site again three times to collect ads images, and use Prebid.js to collect bids value from each testing site. We call it "Collecting visit". The crawler will load the profile ``P'' before visiting each testing website. And the profile ``P'' will not be updated after visiting each testing website. 

We will also do the central opting out in ``opt-out crawl''. After the training phrase, the crawler will visit the site ``https://optout.networkadvertising.org/?c=1'' to opt-out all of listed advertisers, then visit each testing site three times, save all ads images, \textcolor{blue}{and use Prebid.js to collect bids value from each testing site. In creating the testing sites list, we filtered all websites that support header bidding from the Alexa top 10k website list. We chose top 25 websites from the filtered sites list as the testing sites. The crawler will load the profile ``P'' before visiting each testing website. And the profile ``P'' will not be updated after visiting each testing website.}



\subsubsection{User-Control Crawl}
The third step is ``user-control crawl''

\subsection{Pre Experiment Preparation}

\subsubsection{Proxy Setting}
In ``opt-out'' experiment, we need proxy to change our IP to California, US and other Europe countries such as Germany, France and United Kingdom. \textcolor{blue}{We do not know if the bids data are modified by third party proxy service, which may increase the risk of data inaccuracy.} We would like to build our proxy, because we need to guarantee all the bids data we collected are accurate. 

Tinyproxy is a small, efficient HTTP/SSL proxy. We can deploy it on cloud instances. AWS can provide service locations in US West (N. California), Europe (Frankfurt), Europe (Paris) and Europe (London), which meets ``opt-out'' experiment setting. So we deploy Tinyproxy on AWS ec2 as the proxy instance in ``opt-out'' experiment. We will manually connect to those proxy instances before running crawlers to make sure the proxy can work well. All crawlers will auto connect to those proxy instances.

\subsubsection{Persona Designing}
\textcolor{blue}{The purpose of creating different personas is to compare the performance of header bidding under different personas. The keywords of 16 personas are ``Adult, Art, Business, Computers, Games, Health, Home, Kids, News, Recreation, Reference, Regional, Science, Shopping, Society, Sports''. Those personas covered most aspects of human life. For each persona, we selected Alexa top 50 websites by catogory. \cite{alexa}}

\subsubsection{Bids Collecting}
\textcolor{blue}{We need methods to collect bids in our crawlers. Prebid.js provides code to improve header bidding to display ads\cite{prebid}. We can used it to receive all of the bids from the ads providers.}
%\subsection{Initial crawl}
%\begin{enumerate}
%    \item Browser: Firefox 
%    \item Personas: Sports, Fashion (2-3 personas selected)
%    \item Location: Use any location
%        \begin{enumerate}
%            \item CCPA is by default opt-out and consent is only required if the data is intended to be sold. Selecting California as a crawl location may introduce a bias, we avoid that by selecting locations outside california.
%        \end{enumerate}
%    \item Targeting: Measured on the basis of bid values and ad images
 %   \item Testing website list: Alexa top 1K websites 
%        \begin{enumerate}
%            \item Select websites that support HB by checking the presence of bids on the website
%        \end{enumerate}
%        \item Crawling configurations for training (use 100 websites for training)
%            \begin{enumerate}
%                \item Vanilla crawl
 %                   \begin{enumerate}
  %                      \item Visit a website, wait 2-3 seconds, move to the next website
%                    \end{enumerate}
%                \item Interactive crawl 1
%                    \begin{enumerate}
%                        \item Open subpages only. People likely don't click ads frequently
%                        \item Random scrolls and mouse movements on the page
%                        \item Wait 20-30 seconds on each page 
%                    \end{enumerate}
%                \item Interactive crawl 2
%                    \begin{enumerate}
%                        \item Open subpages and ads.
%                        \item Random scrolls and mouse movements on the page
%                        \item Wait 20-30 seconds on each page 
%                    \end{enumerate}
%                \item Shopping cart crawl
%                    \begin{enumerate}
%                        \item Select 100 websites that support shopping cart
%                        \item Fill shopping cart with some items
%                        \item Random scrolls and mouse movements on the page
%                    \end{enumerate}
%            \end{enumerate}
%\end{enumerate}


%\subsection{Opt-out crawl}
%\begin{enumerate}
%    \item Browser: Firefox 
%    \item Personas: Use the persona that triggered the most targeting in the initial crawl.
%    \item Location: California and EU. If we crawl from both California and EU, we will also be able to quantify the effectiveness of GDPR and CCPA.
%    \item CMPs: CookieBot, ... (2-3)
%    \item Websites with the selected CMPs: Extract a list from nerdydata. Rank them on the basis of their Alexa ranking. Select top N for each CMP.
%    \item Crawl configuration: Use the crawl configuration that triggered the most targeting in the initial crawl.
%    \item Targeting: Measured on the basis of bid values and ad images
%\end{enumerate}

%\subsection{User control crawl:}
%\begin{enumerate}
%    \item Browser: Firefox 
%    \item Personas: Use the persona that triggered the most targeting in the initial crawl.
%    \item Location: California and EU.
%    \item Websites with the selected CMPs: Use the same list of websites that was extracted for opt-out crawl. 
%    \item Crawl configuration: Use the crawl configuration that triggered the most targeting in the initial crawl.
%    \item Targeting: Measured on the basis of bid values ad images
%    \item User controls: 
%        \begin{enumerate}
%            \item Blocked cookies, Fake fingerprint
%            \item Blocked cookies, Original fingerprint
%            \item Unblocked cookies, Fake fingerprint
%        \end{enumerate}
%\end{enumerate}




==> docs/3_methodology_before_changing_structures_08102023.tex <==
\section{Our Framework for Auditing Advertising \& Tracking Services}
\label{sec:methodology}

%\begin{figure}[!t]
%    \centering
%        \subfloat[Consent management dialog for GDPR.]{
%        \includegraphics[width=0.8\columnwidth]{figures/GDPR-Cookiebot-1.png}
%        \label{fig:GDPR-CookieBot}
%        }
%        \hfill
%         \subfloat[Consent management dialog for CCPA.]{
%        \includegraphics[width=0.8\columnwidth]{figures/CCPA-Cookiebot-1.png}
%        \label{fig:CCPA-CookieBot}
%        }
%        \caption{Cookiebot's consent management dialog for GDPR and CCPA.}
%    \label{fig:CookieBot-CMPs}
%\end{figure}



%\begin{figure*}
%    \centering
%
%        \includegraphics[width=\textwidth]{figures/CMP_workflow.pdf}
%     
%        \caption{High level overview of our framework to audit regulatory compliance. (1) We use OpenWPM \cite{Englehardt16MillionSiteMeasurementCCS} to automatically visit top-50 websites from 16 different interest categories to simulate 16 user interest personas. (2) We filter top websites that support opt-outs through Didomi, Quantcast, OneTrust, and CookieBot under GDPR and CCPA and also support header bidding through \texttt{prebid.js} \cite{prebid}. (3) We then visit the filtered websites with user interest personas, opt-out of data processing and selling, and collect bids and network requests from advertisers. (4) We then analyze the collected bids and network requests to infer data processing and selling from advertisers.} % to audit advertisers' compliance with user consent.} 
%        \hl{Zengrui please update the text on top 50  Alexa webistes to top-100K websites in the top box.}
%        \label{fig:CMP}
%\end{figure*}

\begin{figure}
    \centering

        \includegraphics[width=0.4\textwidth]{figures/CMP_workflow_1008.pdf}
     
        \caption{High level overview of our framework to audit regulatory compliance. (1) We use OpenWPM \cite{Englehardt16MillionSiteMeasurementCCS} to automatically visit top-50 websites from 16 different interest categories to simulate 16 user interest personas. (2) We filter top websites that support opt-outs through Didomi, Quantcast, OneTrust, and CookieBot under GDPR and CCPA and also support header bidding through \texttt{prebid.js} \cite{prebid}. (3) We then visit the filtered websites with user interest personas, opt-out of data processing and selling, and collect bids and network requests from advertisers. (4) We then analyze the collected bids and network requests to infer data processing and selling from advertisers.} % to audit advertisers' compliance with user consent.} 
        \vspace{-1.2em}
        \label{fig:CMP}
\end{figure}



%%
% \subsection{Overview}
In this section, we describe our framework to audit advertising and tracking services under GDPR and CCPA. % compliance with the user consent. 
%
At a high level, we simulate synthetic user personas (profiles) with specific interests, intentionally leak those interests to advertisers and trackers, opt-out of processing and selling of user data, and analyze advertisers bidding behavior and network traffic to infer the usage and selling of leaked data. 
%
Figure \ref{fig:CMP} gives an overview of our approach. 



%%


% \hl{Describe how is non-compliance determined. }

% \begin{enumerate}
%     \item \textbf{\textit{Data processing non-compliance.}}
%     \item \textbf{\textit{Data sharing/selling non-compliance.}}
% \end{enumerate}



\subsection{Infrastructure}


\subsubsection{Web Crawling}
We rely on OpenWPM \cite{Englehardt16MillionSiteMeasurementCCS} to set up our auditing framework. 
%
OpenWPM is a widely used Firefox-based, open-source web measurement tool that has been used in numerous research studies \cite{openwpm_usage_stats}. 
%
OpenWPM by default provides functionality to automatically visit websites and capture network requests, among other things.
%
To adapt to our needs, we further extend OpenWPM to automatically opt-out of processing and selling of user data, and to capture advertisers bids on ad slots.\footnote{We will release our patch to OpenWPM at the time of publication.}



\subsubsection{Opting-out of Processing \& Selling of User Data}
\label{susub:opt-out}
We extend OpenWPM to programmatically opt-out of processing and selling of user data from Didomi, \cite{Didomi}, Quantcast \cite{Quantcast}, OneTrust \cite{OneTrust}, and CookieBot \cite{Cookiebot}, four of the widely used consent management platforms (CMPs) \cite{WebAlmanacStateofTheWebCMPs, hils2020measuring}. 
\textcolor{red}{Note that we also tested other CMPs. The other CMPs we have tested are TrustArc, Crownpeak, LiveRamp, CookieYes, Osano, AdRoll, iubenda and Usercentric. After we used Frankfurt, GE and Los Angeles, US IPs to filter if websites support Opt-out, Opt-in and prebid.js, CookieBot, Didomi, OneTrust and Quantcast have the top 4 highest number of websites from Alexa's top-100K websites list.}
\textcolor{blue}{We conducted assessments on alternative CMPs as well. Our evaluations encompassed TrustArc, Crownpeak, LiveRamp, CookieYes, Osano, AdRoll, iubenda, and Usercentric. Employing Frankfurt, GE and Los Angeles, US IPs, we filtered websites to verify their compatibility with Opt-out, Opt-in, and prebid.js. Notably, CookieBot, Didomi, OneTrust, and Quantcast emerged as the four CMPs with the greatest prevalence among the top 100K websites listed on Alexa.}
%
At a high level, we either trigger the JavaScript opt-out event or click the opt-out button of the CMP. 
%
Specifically, for Didomi, we check for the presence of consent dialog with \texttt{Didomi.notice.isVisible}, trigger \texttt{Didomi.setUserDisag-\\reeToAll} method to opt-out, and then hide the consent dialog by setting the display attributes of consent dialog markup to \texttt{none} \cite{didomi_api_docs}.
%
For OneTrust, we check for the presence of consent dialog with \texttt{window.OneTrust}, trigger \texttt{window.OneTrust.RejectAll} method to opt-out and hide the consent dialog \cite{OneTrust_api_docs}.
%
For CookieBot, we check for the presence of consent dialog with \texttt{window.Cookiebot}, traverse the DOM to find the opt-out button with id \texttt{CybotCookiebotD-\\ialogBodyButtonDecline} and click it. 
%
For Quantcast, we check for the presence of consent dialog by traversing the DOM to find the dialog with \texttt{qc-cmp2-summary-buttons} class name and click the button with \textit{Reject} or similar text.\footnote{Similar text candidates are manually compiled from the list of button text for all Quantcast consent dialogs.}
%
If the reject button is not present on the first page of consent dialog, we expand the dialog by clicking the button with \textit{more options} text and then click the \textit{Reject All} button. 
%
Figure \ref{fig:Quantcast-CMPs} shows the Quantcast dialog. % (in Appendix \ref{appendix:consent-dialog})
%
The full lists of websites used to test Opt-out/Opt-in are listed on Github \cite{16_lists_github}


\begin{figure}[!h]
    \centering
        \subfloat[Main page of consent dialog.]{
        \includegraphics[width=0.8\columnwidth]{figures/Quantcast-1.png}
        \label{fig:main-Quantcast}
        }
        \hfill
         \subfloat[Expanded consent dialog with all options.]{
        \includegraphics[width=0.8\columnwidth]{figures/Quantcast-2.png}
        \label{fig:selection-Quantcast}
        }
        \caption{Quantcast's consent management dialog for GDPR and CCPA.}
    \label{fig:Quantcast-CMPs}
\end{figure}




\subsubsection{Capturing Bidding by Advertisers}
\label{susub:bid-collection}
We treat advertisers bidding behavior as an indication of advertisers and trackers non-compliance with the user consent (as discussed in $\S$ \ref{subsection:non-compliance}).
%
To this end, we audit advertisers and trackers on websites that support header bidding, more specifically \texttt{prebid.js} --- a widely used implementation of header bidding protocol \cite{HB_usage}, primarily because header bidding occurs at the client side and allows us to intercept the bidding process \cite{HB_protocol}. 
\textcolor{red}{Other header bidding services like Amazon Transparent Ad Marketplace and Google Ad Manager (GAM) with EBDA (Exchange Bidding Dynamic Allocation) are server-side header biddings, so we can not get the bid data from the client side. Google had the client-side header bidding service before. However, the API googletag.pubads().getBidsReceived() is not available right now. }
\textcolor{blue}{Additional header bidding solutions such as Amazon Transparent Ad Marketplace and Google Ad Manager (GAM) featuring EBDA (Exchange Bidding Dynamic Allocation) operate through server-side mechanisms, preventing us from accessing bid data on the client side. Previously, Google offered a client-side header bidding service. Nevertheless, the current unavailability of the API googletag.pubads().getBidsReceived() has impacted this functionality.}
%
To capture the bids, we first identify header bidding supported websites.
%
We identify such websites by injecting a script on the webpage that probes the \texttt{prebid.js} version; if we receive a response, we consider the website as \texttt{prebid.js} supported website.
%
After identification, we capture the bids by calling the \texttt{getBidResponses} method which returns the bids CPMs\footnote{The bid values are expressed in CPM (cost per mille); which is the amount that an advertiser pays a website per one thousand visitors who see its advertisements.}. 
%
In case, we do not get any bids, we request the bids ourselves by calling the \texttt{requestBids} method.






\subsubsection{Capturing Cookie Syncing by Advertisers}
% \hl{Describe cookie syncing here. Might need to make other adjustments in Section 3 and may be other sections too}
Client side data sharing is a standard practice in the online advertising ecosystem. 
%
Advertisers most commonly share data through cookie syncing \cite{google_rtb_docs}.
%
Specifically, advertisers read their cookies (or other identifiers) from the browser and embed them in redirect requests which force the browser to send the embedded identifiers to the redirected advertiser. 
%
Since cookie syncing involves redirects from the browser, network traffic can be analyzed to detect cookie syncing events. 
%
To evaluate advertisers compliance, we measure whether opt-outs, under GDPR and CCPA, reduce cookie syncing.
%
We use the heuristic from prior work \cite{Iqbal22USENIXKhaleesi} to detect cookie syncing in network traffic when users opt-out and opt-in using CMPs.
%



\subsubsection{Simulating Measurements under GDPR \& CCPA}
We conduct our measurements from EU and California to audit third-party compliance under both GDPR and CCPA. 
%
We choose Frankfurt (Germany) and Northern California as representative jurisdictions under GDPR and CCPA, respectively.
%
We rely on Amazon EC2 to simulate web crawls through the respective locations.
%
We setup a new EC2 node, i.e., with a unique IP address, for each OpenWPM instance. 




%\input{docs/bids-table-germany.tex}
\input{docs/number-of-testing-sites.tex}
% \input{docs/bids-table-germany-new.tex}

\subsection{Methodology}

\subsubsection{Simulating Interest Personas}
\textcolor{red}{Since advertisers bidding behavior is different for different user interests, we simulate 16 user interest personas to capture a wide spectrum of bidding behavior. 
User personas are based on 16\footnote{Adult, Art, Business, Computers, Games, Health, Home, Kids, News, Recreation, Reference, Regional, Science, Shopping, Society, and Sports.} Alexa top websites by categories lists \cite{alexa}.\footnote{As of September 2020, Alexa does not provide a pre-compiled list of websites by category but instead provides an alternate service to search websites by keywords.} The full lists of websites used to train personas are listed on Github \cite{16_lists_github}. We got those lists before Alexa disabled them. To simulate each persona, we initialize a fresh browser profile in an OpenWPM instance, on a fresh EC2 node with a unique IP, iteratively visit top-50 websites in each category, and update browser profile after each visit. Note that we only visited the main page of each website. Our rationale in simulating personas is to convince advertisers and trackers of each persona's interests, so that the advertisers bid higher when they target personalized ads to each persona.In addition to the above-mentioned 16 personas, we also include a control persona, i.e., an empty browser profile. Control persona acts as a baseline and allows us to measure differences in bidding behavior. It is noteworthy that we also enable OpenWPM's bot mitigation and randomly wait between 10--30 seconds after loading each website in order to more accurately simulate user behavior. }

\textcolor{blue}{Recognizing the distinct bidding patterns exhibited by advertisers based on varying user interests, we undertake the simulation of 16 unique user interest personas. These personas are shaped by the categories of the top 16 Alexa-listed websites\footnote{Adult, Art, Business, Computers, Games, Health, Home, Kids, News, Recreation, Reference, Regional, Science, Shopping, Society, and Sports}\cite{alexa}. Notably, our selection approach compensates for Alexa's shift in offerings after September 2020\cite{16_lists_github}.The method of persona simulation involves initializing a fresh browser profile within an OpenWPM instance. This occurs on a pristine EC2 node, each furnished with an exclusive IP address. The process entails iterative visits to the top 50 websites within each category, with the browser profile being updated following each visit. Importantly, it is pertinent to highlight that our interactions were limited to the main pages of these websites. Our rationale for crafting these simulated personas rests upon their potential to persuade advertisers and trackers regarding the interests of each persona. The goal is to incentivize advertisers to submit higher bids when tailoring personalized ads for each persona. Inclusive of the aforementioned 16 personas, our study also introduces a control persona, represented by an empty browser profile. This control persona functions as a benchmark, facilitating the measurement of disparities in bidding behavior across personas. Noteworthy measures undertaken in our methodology encompass the activation of OpenWPM's bot mitigation features and the introduction of random delays ranging between 10 to 30 seconds subsequent to loading each website. These steps serve to enhance the authenticity of user behavior emulation.}


\textcolor{red}{We totally deployed 34 instances: 17 (16 personas + 1 Control) using 17 different IPs in Germany, and 17 (16 personas + 1 Control) using 17 different IPs in California. 
We automatically load selected web pages and simulate random user interactions, such as mouse movements and scrolls, with random delays between actions. We move the mouse a random amount in some directions, scroll in random intervals down the page, and randomly wait so page visits happen with irregularity. This approach aligns with prior web measurement research \cite{Iqbal22USENIXKhaleesi,Cook20HeaderBiddingPETS}.}

\textcolor{blue}{We deployed a total of 34 instances: 17 in Germany (16 personas + 1 Control) using 17 different IPs, and 17 in California (16 personas + 1 Control) using 17 different IPs.}

\textcolor{blue}{We automated the loading of selected web pages and simulated various user interactions, including mouse movements and scrolls, with random time gaps between actions. The mouse cursor is moved by varying amounts in different directions, scrolling occurs at unpredictable intervals down the page, and waiting periods are introduced randomly to create irregular patterns in page visits. This approach is consistent with previous research in web measurement \cite{Iqbal22USENIXKhaleesi,Cook20HeaderBiddingPETS}.}



\subsubsection{Measuring Targeting on Personas}
Next, we measure targeting received by our personas to infer compliance (or lack thereof) under GDPR and CCPA.
%
As mentioned earlier, we register negative user consent, i.e., opt-out of processing and selling of user data, through Didomi, Quantcast, OneTrust, and CookieBot and capture bids through \texttt{prebid.js}.
%
To this end, we shortlist websites that support opt-out through CMPs and also implement header bidding through \texttt{prebid.js}.
%
We identify such websites, by crawling Alexa top-100K websites, using OpenWPM, and probing for the presence of CMPs and \texttt{prebid.js} (as described in Section \ref{susub:opt-out} and \ref{susub:bid-collection}).
%
% To identify the websites that support \texttt{prebid.js}, we inject a script that probes the \texttt{prebid.js} version; if we receive a response, we mark the website as \texttt{prebid.js} supported website.
%
% We describe CMP identification process in Section \ref{susub:opt-out}.


%%
Table \ref{table:number-of-testing-websites} lists the presence of CMPs and \texttt{prebid.js} on Alexa top-100K websites. 
%
We note that a large number of websites deploy CMPs but not all of them deploy \texttt{prebid.js}.
%
However, scanning top-100K websites allows us to filter a meaningful number (i.e., 352) of websites that deploy CMPs and \texttt{prebid.js} under both GDPR and CCPA. 
%
After filtering the websites, we iteratively visit each website nine times from each of our 16 (+ control) personas under both GDPR and CCPA.
%
We visit the websites first time to opt-out of processing or selling of data and the next eight times to collect bids. 

%%
\textcolor{red}{We collect the bids from each website eight times to reduce the chance of outliers biasing our measurements. }
\textcolor{blue}{Occasionally, the internet connection might experience instability, causing the browser to miss out on receiving bids. The quantity of bids received by the browser during distinct visits can also vary. It is unfeasible to ensure that the framework or a typical browser captures bids from all potential advertisers within a single visit. Therefore, we configured our framework to access the website on 8 occasions. The choice of the number 8 isn't dictated by any particular rationale; rather, we opted for a relatively sizable number due to necessity.}
%
Specifically, additional factors, e.g., day/week and website popularity, may influence the bids \cite{Cook20HeaderBiddingPETS,Olejnik14SellingPrivacyNDSS,Papadopoulos17IMCYouAreTheProduct}. 
%
In addition, we also use identical hardware/software, collect bids at the same time, from the same location, and on the same websites, across all personas.
%
Overall, we expect that crawling websites several times and keeping conditions consistent will minimize the variability in bids. %, since all factors incorporated by advertisers cannot be trivially reverse engineered, 


% We minimize the variability by keeping conditions consistent across personas. 
% %
% Specifically, we used identical hardware/software, collected bids at the same time, from the same location, and on the same websites, across all personas (Section 3.2.4). Since it is non-trivial to reverse engineer and control all factors incorporated by advertisers, we crawled websites several times to further minimize the variability in bids.


% We note that OneTrust and Quantcast are the most widely deployed CMPs with presence on 3,046 and 2,563 websites under GDPR and 3,222 an 2,875 websites under CCPA, respectively. 
% %
% However, there are 96 and 234 websites under GDPR and 183 and 94 websites under CCPA that support both OneTrust and Quantcast, respectively.
% %
% CookieBot and Didomi are deployed on 756 and 52ewebsites under GDPR and 599 and 709 websites under CCPA, respectively. 

\subsubsection{Ensuring the Functionality of Selected CMPs}

\textcolor{red}{Before we move forward to further steps, we have to make sure how all selected CMPs work with advertisers before and after the user gives consent. CookieBot \cite{Cookiebot_blocking}, Didomi \cite{Didomi_blocking} and OneTrust \cite{Onetrust_blocking} all have official documents to explain how they handle 3rd party scripts loaded before the user gives consent. We did not find relative information about Quantcast. We manually tested all 4 CMPs under German IPs and calculated the number of HTTP requests from 3rd parties and 3rd party cookies. We used a Macbook device with a Chrome browser, and all data are monitored via Chrome DevTools. Table \ref{table:requests-cookies} contains the actual number of 3rd party HTTP requests and cookies before making a choice, after giving consent, or reject giving consent. Based on the number of requests and the number of cookies, 3rd parties seem not to be able to set trackers in cookies before the user gives consent under Cookiebot, Didomi, and Quantcast, and the number of requests is lower in Opt-out than in Opt-in. However, there is no such trend in Onetrust. Cookies from domain ``\textbf{googleads.g.doubleclick.net}'' and ``\textbf{agead2.googlesyndication.com}'' always appeared before and after giving/rejecting consent.}

\textcolor{blue}{We must ensure a comprehensive understanding of how each selected CMP interacts with advertisers both prior to and following user consent. CookieBot \cite{Cookiebot_blocking}, Didomi \cite{Didomi_blocking}, and OneTrust \cite{Onetrust_blocking} have official documentation outlining their procedures for managing 3rd party scripts that load prior to user consent. However, there is no available information pertaining to Quantcast. We conducted manual testing on all four CMPs using German IPs, calculating the quantity of HTTP requests generated by 3rd parties and the number of 3rd party cookies. Employing a Macbook device equipped with a Chrome browser, all data was monitored through Chrome DevTools. The exact counts of 3rd party HTTP requests and cookies are presented in Table \ref{table:requests-cookies}, depicting the figures before consent is given, after consent is granted, or after consent is denied. From the standpoint of request and cookie numbers, it appears that Cookiebot, Didomi, and Quantcast prevent 3rd parties from setting trackers in cookies before user consent. Additionally, the number of requests is lower in the Opt-out scenario compared to Opt-in. Conversely, such a trend is not evident in the case of OneTrust. Notably, cookies from domains ``\textbf{googleads.g.doubleclick.net}" and ``\textbf{agead2.googlesyndication.com}" consistently appear both before and after user consent or rejection.}

\textcolor{red}{All four CMPs also set consent cookies after the user gives or rejects giving consent. Cookiebot sets a new cookie ``CookieConsent'' after the user gives or rejects giving consent. Didomi uses two cookies ``didomi\_token'' and ``euconsent\-v2'' to store consent information. OneTrust sets the cookie ``OptanonConsent'' to remember the user's consent choice. In Quantcast, three cookies will be created after the user gives consent ``euconsent-v2'', ``\_pbjs\_userid\_consent\_data'', ``addtl\_consent''. Only ``euconsent-v2'' appeared if users reject giving consent. Note that all cookies are set as 1st party cookies, and do not belong to CMPs.}

\textcolor{blue}{Each of the four CMPs also establishes consent cookies following user decisions to either grant or deny consent. In the case of Cookiebot, a new cookie named ``CookieConsent" is created once the user makes a choice regarding consent. Didomi employs two cookies, namely ``didomi\_token" and ``euconsent-v2," to store consent-related information. OneTrust uses the ``OptanonConsent" cookie to retain the user's consent preference. In the context of Quantcast, three cookies are generated upon user consent: ``euconsent-v2," ``\_pbjs\_userid\_consent\_data," and ``addtl\_consent." If users opt to decline consent, only the ``euconsent-v2" cookie is present. It's important to note that all these cookies are designated as 1st party cookies and are not affiliated with the CMPs themselves.}

\input{tables/4CMPs_requests_cookies/summary.tex}




\subsubsection{Baseline Comparison with Opt-in}
To understand the impact of regulations, we also establish a baseline by opting in to the processing and selling of data. 
%
Our rationale for opting in is to get the upper bound on processing and selling of data, as inferred by advertisers bidding behavior.
%
To opt-in, we enable all cookie controls mentioned in Section \ref{susub:opt-out}.
%
For Didomi we call the \texttt{Didomi.setUserAgreeToAll}, for OneTrust we call \texttt{window. OneTrust.AllowAll}, for CookieBot we click the opt-in button with id \texttt{CybotCookiebotDialogBodyLevelButtonLevelOptinAl lowAll}, and for Quantcast we click the button with \textit{Accept} or similar text. 



\subsubsection{Comparison With Advertisers Self Regulations}
We also compare state-enforced regulations, i.e., GDPR and CCPA, with advertisers offered controls, i.e., with NAI's central opt-out \cite{nai_opt_out} in curbing the processing and selling of data.
%
We opt-out of NAI's offered controls by automatically navigating to their opt-out webpage \cite{nai_opt_out} and by clicking \textit{OPT OUT OF ALL} button.
%
To evaluate advertisers offered controls, we select a different set of websites that support \texttt{prebid.js} but do not support CMPs.
%
Specifically, we filter Alexa top-50 websites and identify 28 websites that support \texttt{prebid.js} but do not support any CMPs under both GDRP and CCPA.
%
It is important to select websites that do not support CMPs because otherwise we cannot distinguish between the impact of advertisers offered controls and state-enforced regulations. %facilitated by CMPs. 



\subsubsection{Statistical Analysis}
To evaluate if there are significant differences in advertisers bidding behavior when users opt-out under GDPR and CCPA, we conduct Mann-Whitney U test of statistical significance \cite{cohen1977statistical}.
%
Mann-Whitney U test is a nonparametric test to compare the differences between two distributions.
%
Since we perform multiple comparisons, i.e., compare bid values for all 16 personas, we also conduct Bonferroni correction on the statistical test. 
%
Our null hypothesis is that the bid distributions for opt-in and opt-out are similar to each other. 
%
We reject the null hypothesis, when the p-value (after correction, i.e., original value multiplied by 16) is less than 0.05 (reflecting a 95\% confidence interval), i.e., the distributions are statistically different. 
%We reject the null hypothesis, when the p-value is less than 0.05 (reflecting a 95\% confidence interval), i.e., the distributions are statistically different. %  (reflecting a 99.68\% confidence interval after Holm-Bonferroni correction)
%
We also measure the magnitude of the difference between bid values by calculating the effect size \cite{cohen1977statistical}. 
%
%Effect size less than 0.3, between 0.3 and 0.5, and greater than 0.5 is considered small, medium, and large, respectively.
Effect size less than 0.3, between 0.3 and 0.5, and greater than 0.5 is considered small, medium, and large, respectively. Effect sizes are reported only in cases where statistically significant differences are observed.
\textcolor{red}{Note that when there are no bids collected in opt-out or opt-in, we can not calculate p-value and effect size, as they need two datasets to do a comparison.}
\textcolor{blue}{In instances where no bids are accumulated under either opt-out or opt-in conditions, the calculation of p-value and effect size becomes unfeasible, as these measures necessitate two datasets for meaningful comparison.}

% calculate the effect size to measure the significance of difference. 



% To validate the hypothesis that the advertisers bidding behavior does not significantly change between opt-in and opt-out, 

% we conduct Mann-Whitney U test of statistical significance \cite{cohen1977statistical}.
% %

% %
% % Such a correction is essential in reducing value the baseline to determine the large difference.
% %
% Our null hypothesis is that the bid distributions for opt-in and opt-out are similar to each other. 
% %
% We reject the null hypothesis, when the \textit{p-value} is less than 0.05 (reflecting a 95\% confidence interval), i.e., the distributions are statistically different. %  (reflecting a 99.68\% confidence interval after Holm-Bonferroni correction)
% %
% Table \ref{table:statistical-test-gdpr-ccpa} presents the result for the statistical test. 
% %
% As compared to opt-in, the advertisers bidding behavior does not significantly change for opt-out under both GDPR and CCPA,


% \hl{discuss effect size.}



% \hl{We  analyze bids from advertisers who we did not explicitly leak user interests to, i.e., the advertisers who did not appear in the persona simulation phase but appeared when we opted-out and measured targeting on those personas.
%
% Higher bid values from advertisers, who we did not explicitly leak user interests to will highlight the potential selling and sharing of user data from at least one of the advertisers who we leaked user data in the persona simulation phase.}

==> docs/4_2_evaluation.tex <==

% \subsection{Advertiser-Offered NAI's Opt-Out Controls are not very Effective Either}
% We also analyze advertisers bidding behavior by exercising advertisers offered opt-out controls.
% %
% Specifically, we opt-out through National Advertising Initiative (NAI) -- an advertising consortium -- provided controls to opt-out of targeted advertising \cite{nai_opt_out}.
% %
% Similar to state-enforced regulations, i.e., GDPR and CCPA, we evaluate whether (a) opt-out through NAI reduces targeting, (b) whether the reduction is statistically different, and (c) whether advertisers share data without user consent. 


% \textit{Similar to GDPR and CCPA, most personas receive higher bids as compared to control when user opt-out through NAI.}
% %
% \textcolor{red}{NAI columns in Table \ref{table:GDPR-bidding-mean}  and \ref{table:CCPA-bidding-mean}}
% \textcolor{blue}{Table \ref{table:NAI-bidding-mean}} presents bids from advertisers who support opt-outs under the NAI's opt-out controls. 
% %
% To make a comparison with GDPR and CCPA, we opt-out of targeted advertising in both EU and California. 
% %

% \textcolor{red}{In EU, when we opt-out of targeted advertising, 9 and 3 personas receive bids higher than the average and higher than the sum of average and standard deviation, respectively, as compared to the control persona. }
% \textcolor{blue}{In EU, when we opt-out of targeted advertising, 14 personas receive bids higher than the average, and all of 14 personas receive bids higher than the sum of average and standard deviation, respectively, as compared to the control persona. }

% %
% \textcolor{red}{In California, when we opt-out of targeted advertising, 8 and 1 personas receive bids higher than the average and higher than the sum of average and standard deviation, respectively, as compared to the control persona. }
% \textcolor{blue}{In California, when we opt-out of targeted advertising, 6 and 1 personas receive bids higher than the average and higher than the sum of average and standard deviation, respectively, as compared to the control persona. }


% %
% \textcolor{red}{In comparison to the opt-out facilitated by OneTrust and CookieBot under GDPR, 4 and 7 few personas receive bid values that are higher than the average bid values of control.}
% \textcolor{blue}{In comparison to the opt-out facilitated by CookieBot and Quantcast under GDPR, 8, and 1 few personas receive bid values that are higher than the average bid values of control. Comparing to Didomi, NAI has 3 more personas receive bids values that are higher than the average bid values of control. There are no difference of number of personas between Onetrust and NAI under GDPR. }

% %  
% \textcolor{red}{In comparison to the opt-out facilitated by OneTrust under CCPA, 2 personas receive bid values that are higher than the average bid values of control; for CookieBot in both cases equal number of personas receive bids that are higher than the average bid values of control.}
% \textcolor{blue}{In comparison to the opt-out facilitated by Cookiebot, Didomi, OneTrust and Quantcast under CCPA, 10, 2, 8, and 10 less personas receive bid values that are higher than the average bid values of control.}



% \textit{Similar to GDPR and CCPA, opt-out is statistically similar to opt-in (no-action).}
% %
% Since advertisers assume default opt-in without explicit user consent to opt-out, we do not take any action to explicitly opt-in for NAI. 
% %
% \textcolor{red}{It can be seen from the NAI columns in Table \ref{table:u-test}, that for 10 and 9 personas in EU and California, there is no significant difference in advertisers bidding behavior for opt-in and opt-out. }
% \textcolor{blue}{It can be seen from the NAI columns in Table \ref{table:u-test-gdpr} and Table \ref{table:u-test-ccpa}, that for 16 and 11 personas in EU and California, there is no significant difference in advertisers bidding behavior for opt-in and opt-out.}
% %
% For the remaining personas in both GDPR and CCPA, we note that bidding distributions are different for opt-out and opt-in configurations but the effect size is small.
% %

% \textcolor{red}{In comparison to opt-out facilitated by OneTrust and CookieBot under GDPR, 5 more and 3 few personas are statistically similar to opt-in, respectively.} 
% \textcolor{blue}{In comparison to opt-out facilitated by Didomi, Onetrust and Quantcast under GDPR, 6,6 and 9 few personas are statistically similar to opt-in, respectively. This number is same as by Cookiebot.} 
% %  
% \textcolor{red}{In comparison to opt-out facilitated by OneTrust under CCPA, 1 more persona is statistically similar to opt-in; for CookieBot in both cases equal number of personas are statistically similar. }
% \textcolor{blue}{In comparison to opt-out facilitated by Cookiebot and Quantcast under CCPA, 3 and 1 less personas is statistically similar to opt-in; for Didomi and Onetrust, 11 and 4more personas are statistically similar to opt-in. }


%\input{docs/cookie-syncing-events-table_CCPA-new.tex}

%\input{docs/cookie-syncing-events-table_NAI-new.tex}


% \textit{Similar to GDPR and CCPA, advertisers share data without user consent.}
% %
% \textbf{\textit{(a) Server side sharing:}} Table \ref{table:in_test_not_in_train} presents the bids from NAI member advertisers who we did not explicitly leak user interests in both EU and California. 
% %
% In EU, when we opt-out of targeted advertising, 12 and 11 personas receive bids higher than the average and higher than the sum of average and standard deviation, respectively, as compared to the control persona. 
% %
% In California, when we opt-out of targeted advertising, 7 personas receive bids higher than the average and none of the personas receive higher than the sum of average and standard deviation as compared to the control persona. 
% %
% In comparison to the opt-out facilitated by OneTrust and CookieBot under GDPR, 4 few personas receive bid values that are higher than the average bid values of control.
% %  
% In comparison to the opt-out facilitated by OneTrust under CCPA, 1 more and 6 few personas personas receive bid values that are higher than the average bid values of control.


%%
% \textbf{\textit{(b) Client side sharing:}}
% \textcolor{red}{Table \ref{tbl:GDPR_cookie_syncing} and \ref{tbl:CCPA_cookie_syncing}} \textcolor{blue}{Table \ref{tbl:NAI_cookie_syncing}}show cookie syncing statistics for NAI, under GDPR and CCPA, respectively.
% %

% \textcolor{red}{When we opt-out, we note that the percentage of advertisers participating in cookie syncing decreases by 9.6\% under GDPR and increase by 0.7\% under CCPA.}
% \textcolor{blue}{When we opt-out, we note that the percentage of advertisers participating in cookie syncing increases by 23.54\% under GDPR and decrease by 14.41\% under CCPA. The number of events increases 3 under GDPR and decease 22 under CCPA. }
% %
% \textcolor{red}{In comparison to opt-out through OneTrust under GDPR, 8.2\% few advertisers participate in cookie syncing.}
% \textcolor{blue}{In comparison to opt-out through Cookiebot, Didomi and Quantcast under GDPR, 46.63\%, 10.42\%, and 3.3\% more advertisers participate in cookie syncing. 42.71\% few advertisers participate in cookie syncing in NAI than in Onetrust.}

% %
% \textcolor{red}{We do not make a comparison with CookieBot because cookie syncing increases when we opt-out through CookieBot under GDPR.}

% %
% \textcolor{red}{In comparison to opt-out through OneTrust and CookieBot under CCPA, 8.6\% few and 5.8\% more advertisers participate in cookie syncing.}

% \textcolor{blue}{In comparison to opt-out through Cookiebot, Didomi Onetrust under CCPA, 40.61\% more, 13.2, 4.3\% less, and 0.9\% more advertisers participate in cookie syncing.}


%


% %%
% \textbf{\textit{Takeaway \#4:}}  
% We note that the advertiser-offered opt-out controls are also ineffective in curbing the processing and selling of user data despite user consent to opt-out. 
% %
% While advertisers at large do not honor their own opt-out controls, they slightly reduce targeting and share less data as compared to the state-enforced regulations.
% %


==> docs/4_4_compliance_conveyence.tex <==
\subsection{Consent Handling by CMPs}
At a high level, CMPs block or allow cookies to enforce user consent \cite{cookiebot_functions,  didomi_cookies_storage}. 
%
As a first step, CMPs scan the website and identify all first and third-party cookies.
%
After identifying the cookies, CMPs classify them into essential (i.e., necessary for websites to operate) and non-essential (e.g., advertising, tracking, marketing, etc.) cookies. 
%
To identify necessary cookies, CMPs rely on information from the website developers 
%
To identify non-essential cookies, CMPs do not clearly disclose their techniques, but they might just be relying on information shared by advertising and tracking services about the purpose of their cookies (e.g., Google declares the purpose of their cookies \cite{google_ads_cookies}).
%
% However, they might be relying on information shared by advertising and tracking services about the purpose of their cookies (e.g., Google declares the purpose of their cookies \cite{https://business.safety.google/adscookies/})
% Since many advertising and tracking services declare the purpose of their cookies (e.g., Google declares the purpose of their cookies \cite{https://business.safety.google/adscookies/}), CMPs might rely on that information to identify non-essential cookies. 
%
Many CMPs, such as OneTrust and Cookiebot, consolidate the information across websites and maintain database of cookies and their purposes \cite{onetrust_zero_code_cookie_block, cookiebot_functions}. 
%
Consolidating information allows CMPs to automatically identify essential and non-essential cookies on new websites. 



%%
CMPs typically take user consent and store it at the client side in first-party cookies.
%
In addition to blocking cookies, CMPs also block execution of elements (e.g., scripts, iframes, videos, images) that might exfiltrate non-essential cookies before user consent is stored. 
%
To give website developers more control in order to accurately enforce user consent and avoid breakage by blocking essential cookies, CMPs allow website developers to block or allow cookies. 


%%
There are two main ways in which advertisers might be able to process and share user information despite negative consent. 
%
One, website developers may inaccurately deploy CMPs. 
%
For example, tracking code may execute first before CMPs even have a chance to block cookies or website developers may inaccurately list non-essential cookies as essential. 
%
Two, advertisers may rely on side channel information to circumvent enforcement by CMPs. 
%
For example, advertisers may routinely change their cookies to avoid detection or they may rely on browser fingerprinting to track users \cite{Iqbal21FPInspectorSP}.
%
Recently, Toth et al. \cite{toth-pets22} found that CMPs themselves may violate regulations and that their configuration options may lead to non-compliance.


% user consent may not be enforced 

% It is important to note that advertisers and trackers could use side channels to avoid blocking by CMPs or website accurately developers may not deploy CMPs as per

% could use undeclared cookies to avoid blocking by CMPs all together


% some CMPs periodically generate reports about new cookies and require developers to 

% To provide your users with the best possible experience and to ensure that informed consent is given, please make sure to routinely categorize your unclassified cookies. Use your monthly report to see new cookies we've identified since last scan, and to check that everything is categorized appropriately.}





% two resources to classify cookies: (i) information from the website developers, (ii) external information documentation about the cookies. 
% %
% Some CMPs such as Didomi, also claim to partner with 



% CMPs typically take user consent and store it at the client side in first-party cookies \cite{https://www.cookiebot.com/en/functions/ ,  https://developers.didomi.io/cmp/web-sdk/consent-notice/cookies}
% %
% Based on the consent, CMPs either allow or block exfiltration of non-essential cookies.
% %
% CMPs identify the purpose of cookies by relying on self declaration by the website vendors or from the documentation of prominent online services. 
% %
% Many CMPs, such as OneTrust and Cookiebot, maintain a database of cookies and their purpose \cite{https://www.onetrust.com/blog/introducing-onetrust-zero-code-cookie-auto-blocking, https://www.cookiebot.com/en/functions/}. 
% %
% In addition to blocking cookies, CMPs also block elements/requests on the webpage that might exfiltrate non-essential cookies. 


% %%
% CMPs also personalize the consent management for each website. 
% %
% Specifically, if they identify a new cookie for which the CMP has no information, they will ask the website developer for details. 
% %


% Cookiebot CMP maintains a global cookie repository with descriptions of the purpose of commonly used third party cookies.

% When Cookiebot CMP identifies a known cookie on your website it uses the information from the knowledge base to describe the purpose of the cookie to your website visitors.

% From the global repository Cookiebot CMP creates a local repository after the first scan of your website.

% In the local repository you can change any applied description and set purpose descriptions on all cookies identified by the scanner.

% On subsequent scans Cookiebot CMP reuses information from the local repository to describe both first and third party cookies.



% Cookiebot CMP can automatically block all first-party and third-party cookies and trackers on your website. Alternatively, you can manually mark up scripts to be held back until the user has consented. 


% The consent state is stored on the user's browser as a persistent cookie with a JSON-formatted value that can also be read server side to evaluate the user's consent before setting cookies.

% In the Cookie Manager you can see on which URL a cookie was first discovered which makes it easy for you to identify the scripts setting cookies



% The Cookiebot Scanner scans your website and identifies all cookies being set AND the scripts, iframes, videos, images etc. setting them, as well as a number of other methods used to track users and set cookies (Including pixels, among others - See: What kinds of cookies and tracking technologies does the Cookiebot scanner find?)

% Based on the scan and paired with the classification of cookies in our manager, a configuration file is automatically built and made available to the consent banner implemented on your website.

% Every time we scan your website and every time you make a changes to your settings in the Cookiebot Manager, your configuration file is updated and the latest information is applied when automatically blocking cookies on your website.

% \hl{To provide your users with the best possible experience and to ensure that informed consent is given, please make sure to routinely categorize your unclassified cookies. Use your monthly report to see new cookies we've identified since last scan, and to check that everything is categorized appropriately.}


% The way it technically works is that each cookie setting script and element is identified and registered in a way that it can be uniquely identified again at a later stage. Our algorithm includes a number of steps to identify and verify the script, among them content checksum, file, path and keyword matching, and more.

% If one script has been assessed to be the initiator of several cookies and these cookies belong to different categories, then the script will be blocked unless all categories the cookies belong to have been consented to.




% When our solution is implemented correctly it disables elements that set cookies. To enable these elements certain rules determine whether the element should be enabled based on a visitor's consent.

% If an element sets cookies in only a single category, the conditions that need to be met for the element to be allowed to load are very simple; If a visitor has accepted that category of cookies (or all categories), the element will be allowed to load. If the opposite is true the element will remain blocked.

% Things become more complicated when a single element sets cookies in multiple categories. This is particularly true for script bundles. These are files that essentially contain a collection of scripts that fulfill a variety of functions and can potentially set cookies in multiple categories.





% ONETRUST 

% https://www.onetrust.com/blog/introducing-onetrust-zero-code-cookie-auto-blocking/

% ScanYourWebsite \& Categorize Cookies
% SelectYourConsent Model(s)
% Publish and Add OneTrust Script toYourWebsite
% How It Works:

% Takes the category of the cookie and matches it with the cookie source
%  Automatically blocks the source from firing
% Defines a list of the most common third-party trackers (Google Analytics, Facebook, LinkedIn, etc.)
% Blocksthese scripts from loading based on how a user categorizes cookies and chooses consent model(s) for a website


% The tool constantly scans your website for cookies and tracking technologies and auto-categorizes these technologies into consent groups by mapping to CookiepediaTM, a database of over 11 million pre-categorized technologies. Once the cookies are categorized, it is easy to customize your consent model(s) to determine which groups of cookies are loaded by default vs. blocked by default.

% We'll walk you through an easy step-by-step process to set up your consent notice and auto-block cookies in order to reach true compliance.



% Here are the steps to add a cookie notice to your website:

% Scan for cookies and tracking technologies.
% Auto-categorize scan results with Cookiepedia – our database of over 11 million cookies.
% Style consent notice. Update the colors, logo, layout and behaviors using our easy-to-use design center.
% Customize consent model(s). You can use several models at the same time for visitors in different regions using OneTrust's Consent by Geolocation feature.
% Add the OneTrust Cookie Consent and Website Scanning script to your website.



% Auto-Blocking

% This method is the easiest to use by using OneTrust's Auto-Blocking technology. Simply add the script onto your site and auto-block all key tracking technologies that are not categorized as Strictly Necessary until the user has provided consent. We have defined a list of the most common trackers (Google Analytics, Facebook, LinkedIn, etc.) and auto-block these scripts from loading based on how you have categorized your cookies and your chosen consent model(s).


% Tag Manager Integrations

% Using Google Tag Manger or Adobe Dynamic Tag Manager, simply create triggers in your tag management solution that only fire tags that set cookies if that category of cookies is accepted.

% JavaScript Wrapper

% Update the existing scripts on your website with our JavaScript Wrapper that adds a group identifier to ensure those cookies are not fired until the visitor accepts that group of cookies.

% Learn more about OneTrust PreferenceChoice Cookie Consent and Website Scanning, the most mature and trusted solution for cookie consent.

==> docs/ads_images.tex <==
\begin{figure}
    \centering
        \includegraphics[width=\columnwidth]{figures/ads_images/opt-out.png}
        
        \caption{ \textbf{Tower General Contractors} ads image in Opt-out in persona: Home, with setting: CCPA-Onetrust.}
        \label{fig:image_out}
\end{figure}

\begin{figure}
    \centering
        \includegraphics[width=\columnwidth]{figures/ads_images/opt-in.png}
          
        \caption{ \textbf{Framing With TimberStrand LSL} ads image in Opt-in in persona: Home, with setting: CCPA-Onetrust.}
        \label{fig:image_in}   
\end{figure}

\begin{figure}
    \centering
        \includegraphics[width=\columnwidth]{figures/ads_images/control.png}
        \caption{ \textbf{Buydrcleanspray.com} ads image in Control, with setting: CCPA-Onetrust.}
        \label{fig:image_control}     
\end{figure}

==> docs/bid_tables.tex <==
\begin{table*}[!h]
    \centering
    \begin{tabular}{l?{0.3mm}rr|rr|rr?{0.3mm}rr|rr|rr?{0.3mm}rr|rr} 
    \toprule
     & \multicolumn{6}{c?{0.3mm}}{\textbf{OneTrust}} & \multicolumn{6}{c?{0.3mm}}{\textbf{CookieBot}}& \multicolumn{4}{c}{\textbf{NAI}}    \\ 
     & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c}{\textbf{Opt-in}}  & \multicolumn{2}{c?{0.3mm}}{\textbf{No-action}}   & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c}{\textbf{Opt-in}}  & \multicolumn{2}{c?{0.3mm}}{\textbf{No action}}   & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c}{\textbf{No action}}   \\ 
    \textbf{Personas}     & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c}{\textbf{Std.}}  \\ 
    \toprule
    \textbf{Adult}  & 0.45$^{\textcolor{red}{\uparrow}}$ & 0.89   & 1.80$^{\textcolor{red}{\uparrow}}$ 
    & 3.56   & 0.27$^{\textcolor{red}{\uparrow}}$ 
    & 0.14   & 2.5E-3$^{\textcolor{red}{\uparrow}}$   & 0.00   & 1.4E-5$^{\textcolor{red}{\downarrow}}$ & 0.00   & 1.4E-5$^{\textcolor{red}{\downarrow}}$ & 0.00   & 0.29$^{\downarrow}$  & 0.61   & 0.51$^{\textcolor{red}{\uparrow}}$  & 0.87    \\ 
    
    \textbf{Arts}  & 0.16$^{\textcolor{red}{\uparrow}}$& 0.22   & 0.36$^{\textcolor{red}{\uparrow}}$
    & 0.21   & 0.24$^{\textcolor{red}{\uparrow}}$   
    & 0.17   & 0.07$^{\textcolor{red}{\uparrow}}$  & 0.00   & 0.03$^{\textcolor{red}{\uparrow}}$ 
    & 0.03   & 0.01$^{\textcolor{red}{\downarrow}}$& 0.00   & 0.17$^{\downarrow}$  & 0.26   & 0.13$^{\downarrow}$    & 0.18    \\ 
    
    \textbf{Business}     & 0.05$^{\textcolor{red}{\uparrow}}$ & 0.04   & 0.28$^{\textcolor{red}{\uparrow}}$ 
    & 0.17   & 0.17$^{\uparrow}$    & 0.16   & 0.04$^{\textcolor{red}{\uparrow}}$  & 0.03   & 0.08$^{\textcolor{red}{\uparrow}}$ 
    & 0.06   & 1.3E-5$^{\textcolor{red}{\downarrow}}$& 0.00   & 0.56$^{\uparrow}$& 0.74   & 0.18$^{\downarrow}$   & 0.13    \\ 
    
    \textbf{Computers}    & 0.08$^{\textcolor{red}{\uparrow}}$  
    & 0.05   & 0.27$^{\textcolor{red}{\uparrow}}$ 
    & 0.13   & 0.04$^{\downarrow}$    & 0.00   & 0.12$^{\textcolor{red}{\uparrow}}$    & 0.06   & 0.15$^{\textcolor{red}{\uparrow}}$ 
    & 0.06   & 0.16$^{\textcolor{red}{\uparrow}}$   & 0.03   & 0.37$^{\uparrow}$& 0.69   & 0.57$^{\textcolor{red}{\uparrow}}$  & 0.86    \\ 
    
    \textbf{Games} & 0.16$^{\textcolor{red}{\uparrow}}$ & 0.00   & 1.6E-5$^{\textcolor{red}{\downarrow}}$ 
    & 0.00   & - $^{\downarrow}$ 
    & - & 1.3E-5
    & 0.00   & 1.3E-5$^{\textcolor{red}{\downarrow}}$& 0.00   & 0.04$^{\textcolor{red}{\downarrow}}$  & 0.03   & 0.42$^{\uparrow}$& 0.68   & 0.12$^{\downarrow}$    & 0.11    \\ 
    
    \textbf{Health}& 1.23$^{\textcolor{red}{\uparrow}}$  & 1.21   & -$^{\textcolor{red}{\downarrow}}$ 
    & - & - $^{\downarrow}$ 
    & - & 0.08$^{\textcolor{red}{\uparrow}}$   & 0.07   & 0.07$^{\textcolor{red}{\uparrow}}$ 
    & 0.05   & 1.3E-5$^{\textcolor{red}{\downarrow}}$  & 0.00   & 0.48$^{\uparrow}$& 0.89   & 0.47$^{\textcolor{red}{\uparrow}}$    & 0.85    \\ 
    
    \textbf{Home}  & 0.07$^{\textcolor{red}{\uparrow}}$ & 0.07   & 0.47$^{\textcolor{red}{\uparrow}}$ 
    & 0.51   & 0.25$^{\textcolor{red}{\uparrow}}$   & 0.18   & 0.69$^{\textcolor{red}{\uparrow}}$ 
    & 0.49   & 0.48$^{\textcolor{red}{\uparrow}}$ & 0.49   & 0.11$^{\uparrow}$  & 0.06   & 0.22$^{\downarrow}$  & 0.19   & 0.13$^{\downarrow}$  & 0.20    \\ 
    
    \textbf{Kids}  & 0.05$^{\textcolor{red}{\uparrow}}$ & 0.05   & 0.15$^{\textcolor{red}{\uparrow}}$ 
    & 0.10   & 0.04$^{\downarrow}$  & 0.02   & 0.11$^{\textcolor{red}{\uparrow}}$ 
    & 0.05   & 0.14$^{\textcolor{red}{\uparrow}}$& 0.05   & 0.12$^{\uparrow}$  & 0.06   & 0.18$^{\downarrow}$  & 0.17   & 0.37$^{\uparrow}$  & 0.69    \\ 
    
    \textbf{News}  & 0.04$^{\textcolor{red}{\uparrow}}$& 0.05   & 0.37$^{\textcolor{red}{\uparrow}}$ 
    & 0.46   & 0.24$^{\textcolor{red}{\uparrow}}$   & 0.16   & 0.17$^{\textcolor{red}{\uparrow}}$ 
    & 0.03   & 0.17$^{\textcolor{red}{\uparrow}}$& 0.03   & 0.15$^{\textcolor{red}{\uparrow}}$  & 0.04   & 0.42$^{\uparrow}$& 0.77   & 0.16$^{\downarrow}$    & 0.19    \\ 
    
    \textbf{Recreation}   & 0.04$^{\textcolor{red}{\uparrow}}$  & 0.04   & 0.29$^{\textcolor{red}{\uparrow}}$ 
    & 0.11   & 0.11$^{\downarrow}$& 0.00   & 0.05$^{\textcolor{red}{\uparrow}}$ 
    & 0.04   & 7.3E-4$^{\textcolor{red}{\downarrow}}$ & 0.00   & 1.3E-5$^{\textcolor{red}{\downarrow}}$ & 0.00   & 0.45$^{\uparrow}$& 0.68   & 0.13$^{\downarrow}$    & 0.20    \\ 
    
    \textbf{Reference}    & 0.04$^{\textcolor{red}{\uparrow}}$  & 0.04   & 0.42$^{\textcolor{red}{\uparrow}}$ 
    & 0.33   & 0.12$^{\uparrow}$ & 0.07   & 0.16$^{\textcolor{red}{\uparrow}}$
    & 0.03   & 0.17$^{\textcolor{red}{\uparrow}}$   & 0.05   & 0.16$^{\textcolor{red}{\uparrow}}$   & 0.02   & 0.71$^{\textcolor{red}{\uparrow}}$
    & 0.83   & 0.64$^{\textcolor{red}{\uparrow}}$& 0.88    \\ 
    
    \textbf{Regional}     & 0.03$^{\textcolor{red}{\uparrow}}$  & 0.03   & 0.21$^{\textcolor{red}{\uparrow}}$ 
    & 0.17   & 0.08$^{\downarrow}$      & 0.00   & 0.07$^{\textcolor{red}{\uparrow}}$ 
    & 0.01   & 0.11$^{\textcolor{red}{\uparrow}}$  & 0.05   & 0.01$^{\textcolor{red}{\downarrow}}$   & 0.00   & 0.88$^{\textcolor{red}{\uparrow}}$
    & 0.95   & 0.14$^{\downarrow}$      & 0.14    \\ 
    
    \textbf{Science}      & 0.07$^{\textcolor{red}{\uparrow}}$& 0.01   & 0.07$^{\uparrow}$ & 0.01   & 0.49$^{\textcolor{red}{\uparrow}}$  & 0.00   & 1.4E-5$^{\textcolor{red}{\uparrow}}$ & 0.00   & 0.04$^{\textcolor{red}{\uparrow}}$    & 0.04   & 1.4E-5$^{\textcolor{red}{\downarrow}}$   & 0.00   & 0.57$^{\uparrow}$& 0.85   & 0.31$^{\uparrow}$ & 0.31    \\ 
    
    \textbf{Shopping}     & 0.05$^{\textcolor{red}{\uparrow}}$ & 0.04   & 0.05$^{\uparrow}$ & 0.03   & 0.07$^{\downarrow}$ & 3.8E-3   & 1.3E-5   & 0.00   & 0.06$^{\textcolor{red}{\uparrow}}$ & 0.04   & 0.10$^{\uparrow}$    & 0.09   & 0.26$^{\downarrow}$  & 0.29   & 0.64$^{\textcolor{red}{\uparrow}}$  & 0.87    \\ 
    
    \textbf{Society}      & 0.19$^{\textcolor{red}{\uparrow}}$    & 0.15   & 0.38$^{\textcolor{red}{\uparrow}}$ 
    & 0.15   & 0.32$^{\textcolor{red}{\uparrow}}$ & 0.17   & 0.17$^{\textcolor{red}{\uparrow}}$ 
    & 0.03   & 0.16$^{\textcolor{red}{\uparrow}}$& 0.02   & 0.17$^{\textcolor{red}{\uparrow}}$    & 0.03   & 0.14$^{\downarrow}$  & 0.19   & 0.16$^{\downarrow}$  & 0.19    \\ 
    
    \textbf{Sports}& 0.16$^{\textcolor{red}{\uparrow}}$ & 0.29   & 0.17$^{\textcolor{red}{\uparrow}}$ 
    & 0.13   & 0.09$^{\downarrow}$  & 0.03   & 0.12$^{\textcolor{red}{\uparrow}}$ 
    & 0.04   & 0.10$^{\textcolor{red}{\uparrow}}$& 0.08   & 0.09$^{\downarrow}$  & 0.04   & 0.39$^{\uparrow}$& 0.71   & 0.26$^{\uparrow}$   & 0.25    \\
    
    \midrule
    \textbf{Control} & 1.4E-5   & 0.00   & 0.06   & 0.05   & 0.12   & 0.08   & 1.3E-5   & 0.00   & 0.0014   & 0.00   & 0.10   & 0.03   & 0.29   & 0.29   & 0.19   & 0.19    \\ 
    
    \bottomrule
    % \hline
    % \textbf{Avg.}   & 0.177     & 0.080     & 0.168     & 0.187     & 0.334     & 0.382     & 0.071     & 0.025     & 0.109     & 0.052     & 0.104     & 0.062     & 0.300     & 0.418     & 0.400     & 0.576      \\ 
    % \hline
    % \textbf{Std.}   & 0.124     & 0.076     & 0.292     & 0.337     & 0.418     & 0.859     & 0.067     & 0.026     & 0.161     & 0.116     & 0.115     & 0.113     & 0.193     & 0.325     & 0.201     & 0.276      \\
    % \hline
\end{tabular}
\caption{Ad bidding under GDPR in Germany. Avg. column represents the average of each advertiser's median bid value. Std. represents the standard deviation of each advertiser's median bid value. Opt-out, opt-in, and no action represent the bids when we opt-out, opt-in, and do no take any action on selling of user data, respectively.  $\uparrow$ and $\downarrow$ indicate bid values that are higher and lower than Control's avg., respectively. $\textcolor{red}{\uparrow}$ and $\textcolor{red}{\downarrow}$ indicate bid values that are Control's avg. $\pm$ std., respectively.}
\label{table:GDPR-bidding}
\end{table*}


\begin{table*}[!h]
    \centering
    \begin{tabular}{l?{0.3mm}rr|rr|rr?{0.3mm}rr|rr|rr?{0.3mm}rr|rr} 
    \toprule
    \multirow{3}{*}{\textbf{Personas}}
     & \multicolumn{6}{c?{0.3mm}}{\textbf{OneTrust}} & \multicolumn{6}{c?{0.3mm}}{\textbf{CookieBot}}& \multicolumn{4}{c}{\textbf{NAI}}    \\ 
     & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c}{\textbf{Opt-in}}  & \multicolumn{2}{c?{0.3mm}}{\textbf{No-action}}   & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c}{\textbf{Opt-in}}  & \multicolumn{2}{c?{0.3mm}}{\textbf{No action}}   & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c}{\textbf{No action}}   \\ 
    
        & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c}{\textbf{Std.}}  \\ 
    \toprule
    \textbf{Adult}& 0.38$^{\textcolor{red}{\uparrow}}$ 
    & 0.60   & 0.51$^{\textcolor{red}{\uparrow}}$    & 0.69   & 0.09$^{\downarrow}$    & 0.02   & 0.26$^{\uparrow}$    & 0.26   & 0.12$^{\downarrow}$ & 0.15   & 0.67$^{\textcolor{red}{\uparrow}}$ & 1.69   & 0.32$^{\downarrow}$& 0.26   & 0.54$^{\uparrow}$& 0.66    \\ 
    
    \textbf{Arts} & 0.27$^{\uparrow}$    & 0.30   & 0.20$^{\downarrow}$    & 0.12   & 0.22$^{\uparrow}$    & 0.24   & 0.22$^{\uparrow}$    & 0.29   & 0.33$^{\uparrow}$ & 0.33   & 0.30$^{\uparrow}$ & 0.31   & 0.35$^{\downarrow}$& 0.28   & 0.47$^{\downarrow}$  & 0.59    \\ 
    
    \textbf{Business}    & 0.36$^{\textcolor{red}{\uparrow}}$    & 0.31   & 0.62$^{\textcolor{red}{\uparrow}}$    & 0.47   & 0.60$^{\textcolor{red}{\uparrow}}$    & 0.40   & 0.21$^{\uparrow}$    & 0.26   & 0.27$^{\uparrow}$ & 0.24   & 0.15$^{\downarrow}$& 0.16   & 0.46$^{\downarrow}$& 0.51   & 0.24$^{\downarrow}$  & 0.23    \\ 
    
    \textbf{Computers}   & 0.34$^{\uparrow}$    & 0.29   & 0.65$^{\textcolor{red}{\uparrow}}$    & 0.86   & 0.30$^{\uparrow}$    & 0.32   & 0.26$^{\uparrow}$    & 0.29   & 0.16$^{\downarrow}$ & 0.16   & 0.15$^{\downarrow}$& 0.15   & 0.41$^{\downarrow}$& 0.57   & 0.29$^{\downarrow}$  & 0.52    \\ 
    
    \textbf{Games}& 0.55$^{\textcolor{red}{\uparrow}}$    & 0.39   & 0.32$^{\uparrow}$    & 0.32   & 0.39$^{\uparrow}$    & 0.19   & 0.24$^{\uparrow}$    & 0.35   & 0.23$^{\uparrow}$ & 0.29   & 0.14$^{\downarrow}$& 0.16   & 0.64$^{\uparrow}$& 1.02   & 0.46$^{\downarrow}$  & 0.57    \\ 
    
    \textbf{Health}      & 0.35$^{\uparrow}$    & 0.35   & 0.83$^{\textcolor{red}{\uparrow}}$    & 0.90   & 0.44$^{\textcolor{red}{\uparrow}}$    & 0.38   & 0.97$^{\textcolor{red}{\uparrow}}$    & 1.84   & 0.22$^{\uparrow}$ & 0.34   & 0.18$^{\uparrow}$ & 0.22   & 0.51$^{\uparrow}$& 0.83   & 0.31$^{\downarrow}$  & 0.27    \\ 
    
    \textbf{Home} & 0.97$^{\textcolor{red}{\uparrow}}$    & 1.63   & 0.38$^{\uparrow}$    & 0.30   & 0.41$^{\textcolor{red}{\uparrow}}$    & 0.32   & 0.18$^{\downarrow}$    & 0.25   & 0.22$^{\uparrow}$ & 0.23   & 0.14$^{\downarrow}$& 0.17   & 0.71$^{\uparrow}$& 0.88   & 0.42$^{\downarrow}$  & 0.58    \\ 
    
    \textbf{Kids} & 0.30$^{\uparrow}$    & 0.38   & 0.41$^{\uparrow}$    & 0.33   & 0.61$^{\textcolor{red}{\uparrow}}$    & 0.72   & 0.27$^{\uparrow}$    & 0.25   & 0.22$^{\uparrow}$ & 0.26   & 0.20$^{\uparrow}$ & 0.27   & 0.19$^{\downarrow}$& 0.21   & 0.40$^{\downarrow}$  & 0.95    \\ 
    
    \textbf{News} & 0.31$^{\uparrow}$    & 0.27   & 0.37$^{\uparrow}$    & 0.41   & 0.44$^{\textcolor{red}{\uparrow}}$    & 0.34   & 0.25$^{\uparrow}$    & 0.22   & 0.20$^{\uparrow}$ & 0.21   & 0.17$^{\uparrow}$ & 0.20   & 0.66$^{\uparrow}$& 0.67   & 0.96$^{\uparrow}$& 1.62    \\ 
    
    \textbf{Recreation}  & 0.29$^{\uparrow}$    & 0.43   & 0.68$^{\textcolor{red}{\uparrow}}$    & 1.04   & 0.25$^{\uparrow}$    & 0.32   & 0.16$^{\downarrow}$ & 0.20   & 0.14$^{\downarrow}$ & 0.19   & 0.16$^{\uparrow}$ & 0.18   & 0.35$^{\downarrow}$ & 0.50   & 0.16$^{\downarrow}$  & 0.20    \\ 
    
    \textbf{Reference}   & 1.52$^{\textcolor{red}{\uparrow}}$    & 2.68   & 0.32$^{\uparrow}$    & 0.28   & 0.36$^{\uparrow}$    & 0.19   & 0.79$^{\textcolor{red}{\uparrow}}$    & 1.38   & 0.22$^{\uparrow}$ & 0.26   & 0.23$^{\uparrow}$ & 0.29   & 0.68$^{\uparrow}$& 0.96   & 0.38$^{\downarrow}$  & 0.27    \\ 
    
    \textbf{Regional}    & 0.82$^{\textcolor{red}{\uparrow}}$    & 1.14   & 0.29$^{\uparrow}$    & 0.32   & 0.59$^{\textcolor{red}{\uparrow}}$    & 0.58   & 0.17$^{\downarrow}$ & 0.18   & 0.20$^{\uparrow}$ & 0.18   & 0.16$^{\uparrow}$ & 0.18   & 0.33$^{\downarrow}$& 0.26   & 0.82$^{\uparrow}$& 0.91    \\ 
    
    \textbf{Science}     & 0.35$^{\uparrow}$    & 0.22   & 0.31$^{\uparrow}$    & 0.24   & 0.37$^{\uparrow}$    & 0.38   & 0.27$^{\uparrow}$    & 0.27   & 0.16$^{\downarrow}$ & 0.17   & 0.16$^{\uparrow}$ & 0.23   & 0.35$^{\downarrow}$& 0.35   & 0.45$^{\downarrow}$  & 0.41    \\ 
    
    \textbf{Shopping}    & 0.32$^{\uparrow}$    & 0.23   & 1.35$^{\textcolor{red}{\uparrow}}$    & 1.43   & 0.30$^{\uparrow}$    & 0.20   & 0.16$^{\downarrow}$ & 0.17   & 0.27$^{\uparrow}$ & 0.36   & 0.15$^{\downarrow}$& 0.15   & 0.63$^{\uparrow}$& 0.83   & 0.36$^{\downarrow}$  & 0.26    \\ 
    
    \textbf{Society}     & 0.43$^{\textcolor{red}{\uparrow}}$    & 0.31   & 0.45$^{\uparrow}$    & 0.29   & 0.62$^{\textcolor{red}{\uparrow}}$    & 0.77   & 0.13$^{\downarrow}$    & 0.16   & 0.17$^{\uparrow}$ & 0.17   & 0.12$^{\downarrow}$& 0.15   & 0.54$^{\uparrow}$& 0.46   & 0.43$^{\downarrow}$  & 0.56    \\ 
    
    \textbf{Sports}      & 0.37$^{\textcolor{red}{\uparrow}}$    & 0.30   & 0.38$^{\uparrow}$    & 0.33   & 0.40$^{\textcolor{red}{\uparrow}}$    & 0.31   & 0.19$^{\uparrow}$    & 0.17   & 0.14$^{\downarrow}$ & 0.15   & 0.20$^{\uparrow}$ & 0.27   & 0.23$^{\downarrow}$& 0.25   & 0.55$^{\uparrow}$  & 0.86    \\ 
    
    
    \midrule
    \textbf{Control} & 0.23   & 0.13   & 0.26   & 0.21   & 0.19   & 0.20   & 0.19   & 0.18   & 0.16   & 0.18   & 0.15   & 0.17   & 0.47   & 0.59   & 0.49   & 0.61    \\ 
    
    \bottomrule
    % \textbf{Avg.}   & 0.388     & 0.346     & 0.481     & 0.587     & 0.490     & 0.501     & 0.203     & 0.290     & 0.290     & 0.395     & 0.202     & 0.228     & 0.454     & 0.592     & 0.461     & 0.554      \\ 
    % \textbf{Std.}   & 0.157     & 0.191     & 0.333     & 0.657     & 0.279     & 0.357     & 0.128     & 0.364     & 0.227     & 0.467     & 0.055     & 0.069     & 0.195     & 0.354     & 0.162     & 0.269      \\
    % \bottomrule
    \end{tabular}
    \caption{Ad bidding under CCPA. Avg. column represents the average of each advertiser's median bid value. Std. represents the standard deviation of each advertiser's median bid value. Opt-out, opt-in, and no action represent the bids when we opt-out, opt-in, and do no take any action on selling of user data, respectively. $\uparrow$ and $\downarrow$ indicate bid values that are higher and lower than Control's avg., respectively. $\textcolor{red}{\uparrow}$ and $\textcolor{red}{\downarrow}$ indicate bid values that are Control's avg. $\pm$ std., respectively.}
    \label{table:CCPA-bidding}
    \end{table*}


\begin{table*}
    \centering
    \begin{tabular}{l?{0.3mm}ll|ll|ll?{0.3mm}ll|ll|ll} 
    \toprule

    & \multicolumn{6}{c?{0.3mm}}{\textbf{GDPR}} & \multicolumn{6}{c}{\textbf{CCPA}} \\ 
    
    \textbf{Personas} & \multicolumn{2}{c}{\textbf{OneTrsut}}& \multicolumn{2}{c}{\textbf{CookieBot}}  & \multicolumn{2}{c?{0.3mm}}{\textbf{NAI}}  & \multicolumn{2}{c}{\textbf{OneTrsut}}& \multicolumn{2}{c}{\textbf{CookieBot}}  & \multicolumn{2}{c}{\textbf{NAI}}  \\ 

    \multicolumn{1}{c?{0.3mm}}{}  & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \textbf{Avg.} & \textbf{Std.}   & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c}{\textbf{Std.}}  \\ 
    \toprule
    \textbf{Adult}  & 0.08$^{\textcolor{red}{\uparrow}}$      & 0.00  & \multicolumn{1}{c}{---}& \multicolumn{1}{c|}{---}& 0.66$^{\textcolor{red}{\uparrow}}$ & 0.96& 0.16$^{\downarrow}$    & 0.00  & 0.27$^{\uparrow}$    & 0.20  & 0.29$^{\downarrow}$    & 0.30     \\ 
    
    \textbf{Arts}  & 0.07$^{\textcolor{red}{\uparrow}}$      & 0.00  & \multicolumn{1}{c}{---}& \multicolumn{1}{c|}{---}& 0.05$^{\downarrow}$      & 0.00 & \multicolumn{1}{c}{---}   & \multicolumn{1}{c|}{---} & 0.28$^{\uparrow}$    & 0.20  & 0.18$^{\downarrow}$    & 0.22     \\ 
    
    \textbf{Business}  & 0.08$^{\textcolor{red}{\uparrow}}$      & 0.00  & 0.07$^{\textcolor{red}{\uparrow}}$    & 0.00 & 0.33$^{\uparrow}$ & 0.28& 0.22$^{\downarrow}$    & 0.00  & 0.25$^{\uparrow}$    & 0.22  & 0.25$^{\downarrow}$    & 0.28     \\ 
    
    \textbf{Computers} & \multicolumn{1}{c}{---}   & \multicolumn{1}{c|}{---} & 0.06$^{\textcolor{red}{\uparrow}}$    & 0.00 & 1.20$^{\textcolor{red}{\uparrow}}$ & 1.13& 0.41$^{\textcolor{red}{\uparrow}}$    & 0.00  & 0.38$^{\textcolor{red}{\uparrow}}$    & 0.17  & 0.72$^{\uparrow}$      & 0.87     \\ 
    
    \textbf{Games}  & 0.16$^{\textcolor{red}{\uparrow}}$      & 0.00  & \multicolumn{1}{c}{---}& \multicolumn{1}{c|}{---}& 0.92$^{\textcolor{red}{\uparrow}}$ & 0.84& 0.68$^{\textcolor{red}{\uparrow}}$    & 0.49  & 0.25$^{\uparrow}$    & 0.22  & 0.23$^{\downarrow}$    & 0.22     \\ 
    
    \textbf{Health} & 2.43$^{\textcolor{red}{\uparrow}}$      & 0.00  & 0.05$^{\textcolor{red}{\uparrow}}$    & 0.00 & 0.74$^{\textcolor{red}{\uparrow}}$ & 1.03& 0.09$^{\textcolor{red}{\downarrow}}$    & 0.01  & 2.27$^{\textcolor{red}{\uparrow}}$    & 2.68  & 0.89$^{\uparrow}$      & 1.07     \\ 
    
    \textbf{Home}   & \multicolumn{1}{c}{---}   & \multicolumn{1}{c|}{---} & \multicolumn{1}{c}{---}    & \multicolumn{1}{c|}{---}    & 0.33$^{\uparrow}$ & 0.28& 0.58$^{\textcolor{red}{\uparrow}}$    & 0.37  & 0.25$^{\uparrow}$    & 0.22  & 0.69$^{\uparrow}$      & 0.72     \\ 
    
    \textbf{Kids}   & 0.07$^{\textcolor{red}{\uparrow}}$      & 0.00  & 0.05$^{\textcolor{red}{\uparrow}}$    & 0.00 & 0.07$^{\downarrow}$      & 0.00& 0.30$^{\uparrow}$    & 0.21  & 0.44$^{\textcolor{red}{\uparrow}}$    & 0.17  & 0.06$^{\downarrow}$    & 0.05     \\ 
    
    \textbf{News}   & \multicolumn{1}{c}{---}   & \multicolumn{1}{c|}{---} & \multicolumn{1}{c}{---}& \multicolumn{1}{c|}{---}& 1.53$^{\textcolor{red}{\uparrow}}$ & 0.86& 0.32$^{\uparrow}$    & 0.30  & 0.19$^{\downarrow}$      & 0.00  & 0.74$^{\uparrow}$      & 0.80     \\ 
    
    \textbf{Recreation}& \multicolumn{1}{c}{---}   & \multicolumn{1}{c|}{---} & 0.05$^{\textcolor{red}{\uparrow}}$    & 0.00 & 1.02$^{\textcolor{red}{\uparrow}}$ & 0.77& 0.14$^{\downarrow}$      & 0.00  & 0.37$^{\uparrow}$    & 0.18  & 0.05$^{\downarrow}$    & 0.02     \\ 
    
    \textbf{Reference} & 0.08$^{\textcolor{red}{\uparrow}}$      & 0.01  & \multicolumn{1}{c}{---}& \multicolumn{1}{c|}{---}& 1.47$^{\textcolor{red}{\uparrow}}$ & 0.85& 1.16$^{\textcolor{red}{\uparrow}}$    & 1.12  & 0.37$^{\uparrow}$    & 0.17  & 0.65$^{\uparrow}$      & 0.74     \\ 
    
    \textbf{Regional}  & 0.08$^{\textcolor{red}{\uparrow}}$      & 0.00  & 0.06$^{\textcolor{red}{\uparrow}}$    & 0.00 & 1.78$^{\textcolor{red}{\uparrow}}$ & 0.82& 0.14$^{\downarrow}$      & 0.00  & 0.37$^{\uparrow}$    & 0.18  & 0.62$^{\uparrow}$      & 0.00     \\ 
    
    \textbf{Science}& 0.07$^{\textcolor{red}{\uparrow}}$      & 0.00  & \multicolumn{1}{c}{---}& \multicolumn{1}{c|}{---}& 0.67$^{\textcolor{red}{\uparrow}}$ & 0.90& 0.35$^{\uparrow}$      & 0.28  & 0.39$^{\textcolor{red}{\uparrow}}$    & 0.14  & 0.33$^{\downarrow}$    & 0.20     \\ 
    
    \textbf{Shopping}  & 0.09$^{\textcolor{red}{\uparrow}}$      & 0.02  & \multicolumn{1}{c}{---}& \multicolumn{1}{c|}{---}& 0.75$^{\textcolor{red}{\uparrow}}$ & 0.00& 0.19$^{\downarrow}$      & 0.02  & 0.19$^{\downarrow}$      & 0.22  & 1.11$^{\textcolor{red}{\uparrow}}$      & 1.03     \\ 
    
    \textbf{Society}& \multicolumn{1}{c}{---}   & \multicolumn{1}{c|}{---} & \multicolumn{1}{c}{---}& \multicolumn{1}{c|}{---}& 0.08$^{\downarrow}$      & 0.03& 0.52$^{\textcolor{red}{\uparrow}}$      & 0.42  & 0.25$^{\uparrow}$    & 0.22  & 0.57$^{\uparrow}$      & 0.45     \\ 
    
    \textbf{Sports} & 0.09$^{\textcolor{red}{\uparrow}}$      & 0.02  & \multicolumn{1}{c}{---}& \multicolumn{1}{c|}{---}& 1.01$^{\textcolor{red}{\uparrow}}$ & 0.96& 0.27$^{\uparrow}$      & 0.11  & 0.31$^{\uparrow}$    & 0.17  & 0.22$^{\downarrow}$    & 0.27     \\ 
    
    \midrule

    \textbf{Control}& 0.00    & 0.00  & 0.00 & 0.00 & 0.29    & 0.29& 0.23    & 0.13  & 0.19    & 0.18  & 0.47    & 0.59     \\
    
    \bottomrule

\end{tabular}
\caption{Ad bidding under CCPA and GDPR from advertisers who did not bid or appear when we simulated personas but appeared and bid after we opted opt-out under of processing and selling of data. Avg. column represents the average of each advertiser's median bid value. Std. represents the standard deviation of each advertiser's median bid value. $\uparrow$ and $\downarrow$ indicate bid values that are higher and lower than Control's avg., respectively. $\textcolor{red}{\uparrow}$ and $\textcolor{red}{\downarrow}$ indicate bid values that are Control's avg. $\pm$ std., respectively. \hl{@Zengrui, please swap GDPR and CCPA columns. We discuss GDPR first.}}
\label{table:in_test_not_in_train}
\end{table*}
    





==> docs/bidders_appeared_percentage.tex <==
%
%
%\begin{table}[h]
%\centering
%\caption{Top 5 most prevalent advertisers that participate in bidding when we opt-out through OneTrust and CookieBot under GDPR and CCPA. GDPR and CCPA columns represent the average number of personas in which the advertiser appear as a bidder across both OneTrust and CookieBot, under GDPR and CCPA, respectively.}
%    \begin{tabular}{l?{0.3mm}r?{0.3mm}r} 
%    \toprule
%     \textbf{Advertisers}& \textbf{GDPR} & \textbf{CCPA}    \\ 
%    \toprule
%
%
%\textbf{AppNexus}      & 93.75\%       & 71.88\%  \\
%\textbf{PubMatic}      & 62.50\%       & 100.00\%   \\
%\textbf{IndexExchange} & 46.88\%    & 90.63\%   \\
%\textbf{Rubicon}       & 34.38\% &  78.13\%   \\
%% \textbf{Nobid}         & 21.88\% & 31.25\%       \\
%\textbf{TripleLift} &6.25\% & 81.25\% \\
%\bottomrule
%\end{tabular}
%\vspace{-3mm}
%\label{tbl:prevalent-advertisers}
%\end{table}
%
%
%% Most prevalent advertisers that participate in cookie syncing, when we opt-out under GDPR and CCPA. These advertiser appear in all personas across OneTrust, CookieBot, and NAI configurations. OT, CB, and NAI columns represent the count of cookie syncing events under OneTrust, CookieBot, and NAI for each advertiser.







\begin{table}[h]
\centering
\caption{\textcolor{blue}{Top 5 most prevalent advertisers that participate in bidding when we opt-out through Cookiebot, Didomia, Onetrust and Quantcast under GDPR and CCPA. GDPR and CCPA columns represent the average number of personas in which the advertiser appear as a bidder across at least two times of all Cookiebot, Didomia, Onetrust and Quantcast, under GDPR and CCPA, respectively.}}
    \begin{tabular}{l?{0.3mm}r?{0.3mm}r} 
    \toprule
     \textbf{Advertisers}& \textbf{GDPR} & \textbf{CCPA}    \\ 
    \toprule

\textbf{Adpone}      & 100.00\% & 100.00\%        \\
\textbf{PubMatic}      & 25.00\% & 68.75\%        \\
%\textbf{TheMediaGrid}      & -- & 37.50\%        \\
\textbf{TripleLift} & 12.50\% & 12.50\%     \\
\textbf{VerizonMedia}       & 25.00\% & 12.50\%   \\
% \textbf{Nobid}         & 21.88\% & 31.25\%       \\
\textbf{AT\&T} & 6.25\% &12.50\% \\
\bottomrule
\end{tabular}
\vspace{-3mm}
\label{tbl:prevalent-advertisers}
\end{table}


==> docs/bids-table-NAI-interval.tex <==
\begin{table}
\tiny
%\adjustbox{max width=\textwidth}{
    \centering
    \caption{Ad bidding under GDPR in Germany and CCPA in California after 1 month since training and opt-out/opt-in, using NAI service. Avg. column represents the mean of all bid value. Std. represents the standard deviation of all bid value. Opt-out and opt-in represent the bids when we opt-out and opt-in the selling of user data, respectively.  \textcolor{highbids}{Light red} and \textcolor{lowbids}{Light blue} indicate bid values that are higher and lower than Control's avg., respectively. \textcolor{higherbids}{Dark red} and \textcolor{lowerbids}{Dark blue} indicate bid values that are Control's avg. $\pm$ std., respectively. }   
        \begin{tabular}{l?{0.3mm}ll|ll?{0.3mm}ll|ll} 
    \toprule
     & \multicolumn{4}{c?{0.3mm}}{\textbf{GDPR}} & \multicolumn{4}{c}{\textbf{CCPA}}  \\ 
     & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c?{0.3mm}}{\textbf{Opt-in}}     & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c}{\textbf{Opt-in}} \\ 
    \textbf{Persona}     & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c}{\textbf{Std.}}  \\ 
    \toprule
    
    
    
\textbf{Adult}      & 0.03 {\cellcolor{lowbids}}                                                                                                           & 0.13 & 0.01 {\cellcolor{lowbids}}                                                                                                              & 0.05 & 0.09  {\cellcolor{lowbids}}                                                                                                             & 0.17 & 0.07 {\cellcolor{lowbids}}                                                                                                             & 0.15  \\
\textbf{Arts}       & 0.01 {\cellcolor{lowbids}}                                                                                                              & 0.03 & 0.02  {\cellcolor{lowbids}}                                                                                                             & 0.06 & 0.09  {\cellcolor{lowbids}}                                                                                                             & 0.15 & 0.06 {\cellcolor{lowbids}}                                                                                                             & 0.12  \\
\textbf{Business}   & 0.01  {\cellcolor{lowbids}}                                                                                                             & 0.03 & 0.01 {\cellcolor{lowbids}}                                                                                                              & 0.04 & 0.09 {\cellcolor{lowbids}}                                                                                                              & 0.26 & 0.03 {\cellcolor{lowbids}}                                                                                                             & 0.07  \\
\textbf{Computers}  & 3.9E-3 {\cellcolor{lowbids}}                                                                                                          & 0.02 & 0.02  {\cellcolor{lowbids}}                                                                                                             & 0.06 & 0.08   {\cellcolor{lowbids}}                                                                                                            & 0.17 & 0.08  & 0.22  \\
\textbf{Games}      & 0.01 {\cellcolor{lowbids}}                                                                                                              & 0.02 & 0.01   {\cellcolor{lowbids}}                                                                                                            & 0.03 & 0.05 {\cellcolor{lowbids}}                                                                                                              & 0.11 & 0.07 {\cellcolor{lowbids}}                                                                                                             & 0.17  \\
\textbf{Health}     & 2.2E-3{\cellcolor{lowbids}}                                                                                                           & 0.01 & 0.01  {\cellcolor{lowbids}}                                                                                                             & 0.02 & 0.08  {\cellcolor{lowbids}}                                                                                                             & 0.15 & 0.06 {\cellcolor{lowbids}}                                                                                                             & 0.19  \\
\textbf{Home}       & 0.01  {\cellcolor{lowbids}}                                                                                                             & 0.02 & 4.3E-3 {\cellcolor{lowbids}}                                                                                                              & 0.01 & 0.08 {\cellcolor{lowbids}}                                                                                                                 & 0.15 & 0.06 {\cellcolor{lowbids}}                                                                                                                & 0.18  \\
\textbf{Kids}       & 0.01 {\cellcolor{lowbids}}                                                                                                                 & 0.02 & 0.02   {\cellcolor{lowbids}}                                                                                                               & 0.04 & 0.07   {\cellcolor{lowbids}}                                                                                                               & 0.23 & 0.07 {\cellcolor{lowbids}}                                                                                                                & 0.14  \\
\textbf{News}       & 0.01   {\cellcolor{lowbids}}                                                                                                               & 0.03 & 0.01  {\cellcolor{lowbids}}                                                                                                                & 0.03 & 0.11 {\cellcolor{highbids}}                                                                                                         & 0.27 & 0.04 {\cellcolor{lowbids}}                                                                                                                & 0.12  \\
\textbf{Recreation} & 2.3E-3 {\cellcolor{lowbids}}                                                                                                             & 0.01 & 0.01 {\cellcolor{lowbids}}                                                                                                                 & 0.03 & 0.10  & 0.18 & 0.09  {\cellcolor{highbids}}                                                                                                       & 0.22  \\
\textbf{Reference}  & 0.01  {\cellcolor{lowbids}}                                                                                                                & 0.04 & 0.01 {\cellcolor{lowbids}}                                                                                                                 & 0.01 & 0.07 {\cellcolor{lowbids}}                                                                                                                 & 0.16 & 0.08  & 0.21  \\
\textbf{Regional}   & 0.01   {\cellcolor{lowbids}}                                                                                                               & 0.02 & 0.01 {\cellcolor{lowbids}}                                                                                                                 & 0.03 & 0.12     {\cellcolor{highbids}}                                                                                                     & 0.41 & 0.04 {\cellcolor{lowbids}}                                                                                                                & 0.06  \\
\textbf{Science}    & 0.03  {\cellcolor{lowbids}}                                                                                                                & 0.11 & 0.01   {\cellcolor{lowbids}}                                                                                                               & 0.01 & 0.14 {\cellcolor{highbids}}                                                                                                         & 0.25 & 0.09  {\cellcolor{highbids}}                                                                                                       & 0.19  \\
\textbf{Shopping}   & 0.03   {\cellcolor{lowbids}}                                                                                                               & 0.13 & 0.01 {\cellcolor{lowbids}}                                                                                                                 & 0.02 & 0.13   {\cellcolor{highbids}}                                                                                                       & 0.25 & 0.05 {\cellcolor{lowbids}}                                                                                                                & 0.16  \\
\textbf{Society}    & 0.00  {\cellcolor{lowbids}}                                                                                                                & 0.00 & 3.1E-3{\cellcolor{lowbids}}                                                                                                              & 0.02 & 0.15  {\cellcolor{highbids}}                                                                                                        & 0.21 & 0.05 {\cellcolor{lowbids}}                                                                                                                & 0.11  \\
\textbf{Sports}     & 0.01 {\cellcolor{lowbids}}                                                                                                                 & 0.04 & 0.01  {\cellcolor{lowbids}}                                                                                                                & 0.02 & 0.15 {\cellcolor{highbids}}                                                                                                         & 0.51 & 0.07  {\cellcolor{lowbids}}                                                                                                               & 0.26  \\


\midrule
\textbf{Control}    & 0.04     & 0.12 & 0.03     & 0.12 & 0.10     & 0.17 & 0.08    & 0.13  \\


    \bottomrule

\end{tabular}

%\vspace{-5mm}
\label{table:NAI-bidding-mean}
\end{table}



==> docs/bids-table-NAI.tex <==
\begin{table}
\scriptsize
%\adjustbox{max width=\textwidth}{
    \centering
    \caption{\textcolor{blue}{Ad bidding under GDPR in Germany and CCPA in California. Avg. column represents the mean of all bid value. Std. represents the standard deviation of all bid value using NAI service. Opt-out and opt-in represent the bids when we opt-out and opt-in the selling of user data, respectively.  Color \textcolor{pink}{pink} and \textcolor{cyan}{cyan} indicate bid values that are higher and lower than Control's avg., respectively. Color \textcolor{red}{red} and \textcolor{blue}{blue} indicate bid values that are Control's avg. $\pm$ std., respectively.}}
    \begin{tabular}{l?{0.3mm}ll|ll?{0.3mm}ll|ll} 
    \toprule
     & \multicolumn{4}{c?{0.3mm}}{\textbf{GDPR}} & \multicolumn{4}{c}{\textbf{CCPA}}  \\ 
     & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c?{0.3mm}}{\textbf{Opt-in}}     & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c}{\textbf{Opt-in}} \\ 
    \textbf{Persona}     & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c}{\textbf{Std.}}  \\ 
    \toprule
    
    
    
\textbf{Adult}       & 0.00   {\cellcolor{red}}                                                                                                      & 0.01                                           & 0.00 {\cellcolor{pink}}                                                                                                         & 0.03                                           & 0.10                                          {\cellcolor{pink}}                                                               & 0.26                                           & 0.07                                          {\cellcolor{pink}}                                                               & 0.12                                            \\ 

\textbf{Arts}        & 0.00          {\cellcolor{red}}                                                                                                      & 0.00                                           & 0.00                                          {\cellcolor{cyan}}                                                               & 0.01                                           & 0.06                                          {\cellcolor{cyan}}                                                               & 0.14                                           & 0.07                                          {\cellcolor{pink}}                                                               & 0.15                                            \\ 

\textbf{Business}    & 0.00       {\cellcolor{red}}                                                                                                      & 0.01                                           & 0.01                                          {\cellcolor{pink}}                                                               & 0.04                                           & 0.02                                          {\cellcolor{cyan}}                                                               & 0.06                                           & 0.08                                          {\cellcolor{pink}}                                                               & 0.21                                            \\ 

\textbf{Computers}   & 0.00                                          {\cellcolor{red}}                                                                                                      & 0.03                                           & 0.01                                          {\cellcolor{pink}}                                                               & 0.03                                           & 0.03                                          {\cellcolor{cyan}}                                                               & 0.14                                           & 0.03                                          {\cellcolor{cyan}}                                                               & 0.07                                            \\ 

\textbf{Games}       & 0.00       {\cellcolor{red}}                                                                                                      & 0.00                                           & 0.00                                          {\cellcolor{cyan}}                                                               & 0.00                                           & 0.09                                          {\cellcolor{pink}}                                                               & 0.18                                           & 0.03                                          {\cellcolor{cyan}}                                                               & 0.07                                            \\ 

\textbf{Health}      & 0.00   {\cellcolor{red}}                                                                                                      & 0.00                                           & 0.01                                          {\cellcolor{pink}}                                                               & 0.04                                           & 0.16                                          {\cellcolor{pink}}                                                               & 0.33                                           & 0.20                                          {\cellcolor{red}}                                                                                                      & 0.40                                            \\ 

\textbf{Home}        & 0.00  {\cellcolor{cyan}}                                                                                                       & 0.00                                           & 0.00                                          {\cellcolor{cyan}}                                                               & 0.00                                           & 0.03                                          {\cellcolor{cyan}}                                                               & 0.10                                           & 0.05                                          {\cellcolor{pink}}                                                               & 0.11                                            \\ 

\textbf{Kids}        & 0.00      {\cellcolor{red}}                                                                                                      & 0.00                                           & 0.00                                          {\cellcolor{pink}}                                                               & 0.03                                           & 0.07                                          {\cellcolor{cyan}}                                                               & 0.12                                           & 0.08                                          {\cellcolor{pink}}                                                               & 0.16                                            \\ 

\textbf{News}        & 0.00      {\cellcolor{red}}                                                                                                      & 0.00                                           & 0.00                                          {\cellcolor{cyan}}                                                               & 0.01                                           & 0.03                                          {\cellcolor{cyan}}                                                               & 0.09                                           & 0.06                                          {\cellcolor{pink}}                                                               & 0.15                                            \\ 

\textbf{Recreation}  & 0.00                                          {\cellcolor{red}}                                                                                                      & 0.01                                           & 0.00                                          {\cellcolor{cyan}}                                                               & 0.01                                           & 0.02                                          {\cellcolor{cyan}}                                                               & 0.05                                           & 0.08                                          {\cellcolor{pink}}                                                               & 0.12                                            \\ 

\textbf{Reference}   & 0.00                                          {\cellcolor{red}}                                                                                                      & 0.01                                           & 0.00                                          {\cellcolor{cyan}}                                                               & 0.00                                           & 0.02                                          {\cellcolor{cyan}}                                                               & 0.04                                           & 0.07                                          {\cellcolor{pink}}                                                               & 0.17                                            \\ 

\textbf{Regional}    & 0.00      {\cellcolor{red}}                                                                                                      & 0.01                                           & 0.00                                          {\cellcolor{cyan}}                                                               & 0.00                                           & 0.22                                          {\cellcolor{red}}                                                                                                      & 0.57                                           & 0.09                                          {\cellcolor{pink}}                                                               & 0.21                                            \\ 

\textbf{Science}     & 0.00             {\cellcolor{red}}                                                                                                      & 0.00                                           & 0.01                                          {\cellcolor{pink}}                                                               & 0.04                                           & 0.02                                          {\cellcolor{cyan}}                                                               & 0.07                                           & 0.03                                          {\cellcolor{cyan}}                                                               & 0.07                                            \\ 

\textbf{Shopping}    & 0.00                                          {\cellcolor{red}}                                                                                                      & 0.01                                           & 0.00                                          {\cellcolor{cyan}}                                                               & 0.00                                           & 0.07                                          {\cellcolor{pink}}                                                               & 0.16                                           & 0.07                                          {\cellcolor{pink}}                                                               & 0.16                                            \\ 

\textbf{Society}     & 0.00              {\cellcolor{cyan}}                                                                                           & 0.00                                           & 0.01                                          {\cellcolor{pink}}                                                               & 0.04                                           & 0.05                                          {\cellcolor{cyan}}                                                               & 0.12                                           & 0.11                                          {\cellcolor{pink}}                                                               & 0.21                                            \\ 

\textbf{Sports}      & 0.01               {\cellcolor{red}}                                                                                                      & 0.04                                           & 0.01                                          {\cellcolor{pink}}                                                               & 0.04                                           & 0.09                                          {\cellcolor{pink}}                                                               & 0.17                                           & 0.14                                          {\cellcolor{pink}}                                                               & 0.23                                            \\ 

\midrule
\textbf{Control}     & 0.00                                           & 0.00                                           & 0.00                                           & 0.02                                           & 0.07                                           & 0.15                                           & 0.05                                           & 0.12                                            \\


    \bottomrule

\end{tabular}

%\vspace{-5mm}
\label{table:NAI-bidding-mean}
\end{table}



==> docs/bids-table-california-new-interval.tex <==
\begin{table*}
\footnotesize
%\adjustbox{max width=\textwidth}{
    \centering
    \caption{Ad bidding under CCPA in California after 1 month since training and opt-out/opt-in. Avg. column represents the mean of all bid value. Std. represents the standard deviation of all bid value. Opt-out and opt-in represent the bids when we opt-out and opt-in the selling of user data, respectively.  \textcolor{highbids}{Light red} and \textcolor{lowbids}{Light blue} indicate bid values that are higher and lower than Control's avg., respectively. \textcolor{higherbids}{Dark red} and \textcolor{lowerbids}{Dark blue} indicate bid values that are Control's avg. $\pm$ std., respectively. } \begin{tabular}{l?{0.3mm}ll|ll?{0.3mm}ll|ll?{0.3mm}ll|ll?{0.3mm}ll|ll} 
    \toprule
     & \multicolumn{4}{c?{0.3mm}}{\textbf{Cookiebot}} & \multicolumn{4}{c?{0.3mm}}{\textbf{Didomi}}& \multicolumn{4}{c?{0.3mm}}{\textbf{Onetrust}}& \multicolumn{4}{c}{\textbf{Quantcast}}      \\ 
     & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c?{0.3mm}}{\textbf{Opt-in}}     & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c?{0.3mm}}{\textbf{Opt-in}}    & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c?{0.3mm}}{\textbf{Opt-in}}& \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c}{\textbf{Opt-in}}     \\ 
    \textbf{Persona}     & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}}  & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}}&  \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c}{\textbf{Std.}} \\ 
    \toprule
    
    
    
\textbf{Adult}      & 0.44  {\cellcolor{highbids}}                                                                                         & 0.13 & 0.97   {\cellcolor{lowbids}}                                                                                                  & 1.53 & 0.41  {\cellcolor{highbids}}                                                                                                    & 0.74 & 0.17  {\cellcolor{highbids}}                                                                                                   & 0.26 & 1.38    {\cellcolor{lowbids}}                                                                                                           & 1.40 & 1.00    {\cellcolor{lowbids}}                                                                                                          & 1.36 & 0.35              {\cellcolor{highbids}}                                                                                         & 0.86 & 0.34    {\cellcolor{lowbids}}                                                                                                          & 0.44  \\

\textbf{Arts}       & 0.36   {\cellcolor{lowbids}}                                                                                                             & 0.22 & 1.93    {\cellcolor{highbids}}                                                                                                 & 1.70 & 0.39  {\cellcolor{highbids}}                                                                                                    & 0.75 & 0.13       & 0.22 & 1.18      {\cellcolor{lowbids}}                                                                                                         & 1.27 & 0.87     {\cellcolor{lowbids}}                                                                                                         & 1.17 & 0.33  {\cellcolor{highbids}}                                                                                                     & 0.75 & 0.38     {\cellcolor{lowbids}}                                                                                                         & 0.51  \\

\textbf{Business}   & 0.29   {\cellcolor{lowbids}}                                                                                                             & 0.24 & 1.70   {\cellcolor{highbids}}                                                                                                  & 1.93 & 0.32 {\cellcolor{highbids}}                                                                                                     & 0.25 & 0.14   {\cellcolor{highbids}}                                                                                                  & 0.24 & 1.52    {\cellcolor{lowbids}}                                                                                                           & 1.52 & 1.07  {\cellcolor{highbids}}                                                                                                   & 1.59 & 0.29 {\cellcolor{highbids}}                                                                                                      & 0.70 & 0.42    & 0.52  \\

\textbf{Computers}  & 0.51  {\cellcolor{highbids}}                                                                                                     & 0.12 & 1.16   {\cellcolor{highbids}}                                                                                                  & 1.53 & 0.56  {\cellcolor{highbids}}                                                                                                    & 0.86 & 0.14   {\cellcolor{highbids}}                                                                                                  & 0.22 & 1.42     {\cellcolor{lowbids}}                                                                                                          & 1.28 & 0.85    {\cellcolor{lowbids}}                                                                                                          & 1.30 & 0.33              {\cellcolor{highbids}}                                                                                         & 0.73 & 0.43    {\cellcolor{highbids}}                                                                                                 & 0.50  \\

\textbf{Games}      & 0.30   {\cellcolor{lowbids}}                                                                                                             & 0.22 & 1.10  {\cellcolor{lowbids}}                                                                                                            & 1.61 & 0.34   {\cellcolor{highbids}}                                                                                                   & 0.26 & 0.15 {\cellcolor{highbids}}                                                                                                    & 0.43 & 1.51    {\cellcolor{lowbids}}                                                                                                           & 1.19 & 0.79    {\cellcolor{lowbids}}                                                                                                          & 0.92 & 0.28    & 0.77 & 0.43   {\cellcolor{highbids}}                                                                                                  & 0.56  \\

\textbf{Health}     & 0.44  {\cellcolor{highbids}}                                                                                                     & 0.22 & 0.95   {\cellcolor{lowbids}}                                                                                                           & 1.51 & 0.36    {\cellcolor{highbids}}                                                                                                  & 0.58 & 0.11   {\cellcolor{lowbids}}                                                                                                           & 0.17 & 1.59  {\cellcolor{highbids}}                                                                                                    & 1.29 & 0.86    {\cellcolor{lowbids}}                                                                                                          & 1.21 & 0.30   {\cellcolor{highbids}}                                                                                                    & 0.80 & 0.40    {\cellcolor{lowbids}}                                                                                                          & 0.48  \\

\textbf{Home}       & 0.30   {\cellcolor{lowbids}}                                                                                                             & 0.22 & 1.11    {\cellcolor{lowbids}}                                                                                                          & 1.54 & 0.23    {\cellcolor{lowbids}}                                                                                                           & 0.21 & 0.14   {\cellcolor{highbids}}                                                                                                  & 0.27 & 1.10    {\cellcolor{lowbids}}                                                                                                           & 1.10 & 1.29   {\cellcolor{highbids}}                                                                                                  & 1.17 & 0.34  {\cellcolor{highbids}}                                                                                                     & 0.83 & 0.41   {\cellcolor{lowbids}}                                                                                                           & 0.49  \\

\textbf{Kids}       & 0.41   {\cellcolor{highbids}}                                                                                                    & 0.21 & 1.61   {\cellcolor{highbids}}                                                                                                  & 1.69 & 0.78    {\cellcolor{higherbids}}                                                                             & 1.66 & 0.25    {\cellcolor{highbids}}                                                                                                 & 0.95 & 1.56   {\cellcolor{lowbids}}                                                                                                            & 1.53 & 0.93     {\cellcolor{lowbids}}                                                                                                         & 1.11 & 0.27     {\cellcolor{lowbids}}                                                                                                           & 0.78 & 0.41    {\cellcolor{lowbids}}                                                                                                          & 0.54  \\

\textbf{News}       & 0.47  {\cellcolor{highbids}}                                                                                                     & 0.14 & 2.60 {\cellcolor{highbids}}                                                                                                    & 1.71 & 0.41  {\cellcolor{highbids}}                                                                                                    & 0.66 & 0.14   {\cellcolor{highbids}}                                                                                                  & 0.23 & 1.44   {\cellcolor{lowbids}}                                                                                                            & 1.42 & 0.74    {\cellcolor{lowbids}}                                                                                                          & 1.12 & 0.30              {\cellcolor{highbids}}                                                                                         & 0.73 & 0.41      {\cellcolor{lowbids}}                                                                                                        & 0.63  \\

\textbf{Recreation} & 0.44 {\cellcolor{highbids}}                                                                                                       & 0.16 & 2.01  {\cellcolor{highbids}}                                                                                                   & 1.83 & 1.54   {\cellcolor{higherbids}}                                                                                       & 8.18 & 0.27   {\cellcolor{highbids}}                                                                                                  & 0.98 & 1.64   {\cellcolor{highbids}}                                                                                                   & 1.72 & 1.08   {\cellcolor{highbids}}                                                                                                  & 1.34 & 0.29    {\cellcolor{highbids}}                                                                                                   & 0.78 & 0.32    {\cellcolor{lowbids}}                                                                                                          & 0.44  \\

\textbf{Reference}  & 0.37    {\cellcolor{lowbids}}                                                                                                            & 0.17 & 2.27  {\cellcolor{highbids}}                                                                                                   & 1.79 & 0.26     {\cellcolor{lowbids}}                                                                                                          & 0.22 & 0.13    & 0.23 & 1.18      {\cellcolor{lowbids}}                                                                                                         & 1.07 & 1.02      {\cellcolor{lowbids}}                                                                                                        & 1.32 & 0.33   {\cellcolor{highbids}}                                                                                                    & 0.88 & 0.38     {\cellcolor{lowbids}}                                                                                                         & 0.47  \\

\textbf{Regional}   & 0.31  {\cellcolor{lowbids}}                                                                                                              & 0.26 & 1.13  {\cellcolor{highbids}}                                                                                                   & 1.54 & 0.40  {\cellcolor{highbids}}                                                                                                    & 0.68 & 0.12    {\cellcolor{lowbids}}                                                                                                          & 0.32 & 1.15    {\cellcolor{lowbids}}                                                                                                           & 1.25 & 1.11            {\cellcolor{highbids}}                                                                                         & 1.36 & 0.41   {\cellcolor{highbids}}                                                                                                    & 1.06 & 0.38    {\cellcolor{lowbids}}                                                                                                          & 0.52  \\

\textbf{Science}    & 0.48   {\cellcolor{highbids}}                                                                                                    & 0.14 & 2.23  {\cellcolor{highbids}}                                                                                                   & 1.77 & 0.30  {\cellcolor{highbids}}                                                                                                    & 0.42 & 0.14  {\cellcolor{highbids}}                                                                                                   & 0.22 & 1.18    {\cellcolor{lowbids}}                                                                                                           & 1.21 & 0.67     {\cellcolor{lowbids}}                                                                                                         & 0.95 & 0.42 {\cellcolor{highbids}}                                                                                                       & 1.06 & 0.34    {\cellcolor{lowbids}}                                                                                                          & 0.49  \\

\textbf{Shopping}   & 0.39   {\cellcolor{lowbids}}                                                                                                             & 0.20 & 1.32   {\cellcolor{highbids}}                                                                                                  & 1.68 & 0.29     {\cellcolor{highbids}}                                                                                                 & 0.37 & 0.12     {\cellcolor{lowbids}}                                                                                                         & 0.16 & 1.29    {\cellcolor{lowbids}}                                                                                                           & 1.41 & 0.69     {\cellcolor{lowbids}}                                                                                                         & 1.07 & 0.38     {\cellcolor{highbids}}                                                                                                  & 1.01 & 0.40    {\cellcolor{lowbids}}                                                                                                          & 0.49  \\

\textbf{Society}    & 0.42  {\cellcolor{highbids}}                                                                                                     & 0.20 & 1.62   {\cellcolor{highbids}}                                                                                                  & 1.72 & 0.36  {\cellcolor{highbids}}                                                                                                    & 0.49 & 0.12  {\cellcolor{lowbids}}                                                                                                            & 0.17 & 1.47   {\cellcolor{lowbids}}                                                                                                            & 1.43 & 0.93     {\cellcolor{lowbids}}                                                                                                         & 1.33 & 0.30  {\cellcolor{highbids}}                                                                                                     & 0.77 & 0.41   {\cellcolor{lowbids}}                                                                                                           & 0.57  \\

\textbf{Sports}     & 0.30    {\cellcolor{lowbids}}                                                                                                            & 0.25 & 1.85   {\cellcolor{highbids}}                                                                                                  & 1.82 & 0.26    {\cellcolor{lowbids}}                                                                                                           & 0.39 & 0.18     {\cellcolor{highbids}}                                                                                                & 0.53 & 2.80   {\cellcolor{highbids}}                                                                                                   & 3.03 & 0.95  {\cellcolor{lowbids}}                                                                                                            & 1.31 & 0.29   {\cellcolor{highbids}}                                                                                                    & 0.83 & 0.43   {\cellcolor{highbids}}                                                                                                  & 0.55  \\

\midrule
\textbf{Control}    & 0.40               & 0.21 & 1.12             & 1.53 & 0.28              & 0.49 & 0.13             & 0.29 & 1.57              & 1.49 & 1.06             & 1.34 & 0.28               & 0.68 & 0.42             & 0.53 \\


    \bottomrule

\end{tabular}

%\vspace{-5mm}
\label{table:CCPA-bidding-mean-interval}
\end{table*}



==> docs/bids-table-california-new.tex <==
\begin{table*}
\footnotesize
%\adjustbox{max width=\textwidth}{
    \centering
    \caption{Ad bidding under CCPA in California. Avg. column represents the mean of all bid value. Std. represents the standard deviation of all bid value. Opt-out and opt-in represent the bids when we opt-out and opt-in the selling of user data, respectively. \textcolor{highbids}{Light red} and \textcolor{lowbids}{Light blue} indicate bid values that are higher and lower than Control's avg., respectively. \textcolor{higherbids}{Dark red} and \textcolor{lowerbids}{Dark blue} indicate bid values that are Control's avg. $\pm$ std., respectively. \hl{the ordering should be Didomi, Quantcast, OneTrust, Cookiebot.}}
    \begin{tabular}{l?{0.3mm}ll|ll?{0.3mm}ll|ll?{0.3mm}ll|ll?{0.3mm}ll|ll} 
    \toprule
     & \multicolumn{4}{c?{0.3mm}}{\textbf{Cookiebot}} & \multicolumn{4}{c?{0.3mm}}{\textbf{Didomi}}& \multicolumn{4}{c?{0.3mm}}{\textbf{Onetrust}}& \multicolumn{4}{c}{\textbf{Quantcast}}      \\ 
     & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c?{0.3mm}}{\textbf{Opt-in}}     & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c?{0.3mm}}{\textbf{Opt-in}}    & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c?{0.3mm}}{\textbf{Opt-in}}& \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c}{\textbf{Opt-in}}     \\ 
    \textbf{Persona}     & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}}  & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}}&  \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c}{\textbf{Std.}} \\ 
    \toprule
    
    
    
\textbf{Adult}      & 0.37 {\cellcolor{highbids}}                                         & 0.20                     & 0.34   {\cellcolor{highbids}}                                       & 0.21                     & 0.17   {\cellcolor{lowbids}}                                       & 0.28                     & 0.17    {\cellcolor{highbids}}                                      & 0.35                     & 1.09    {\cellcolor{highbids}}                                      & 0.98                     & 0.46   {\cellcolor{lowbids}}                                       & 0.64                     & 0.25   {\cellcolor{highbids}}                                       & 0.58                     & 0.16   {\cellcolor{lowbids}}                                       & 0.18                      \\
\textbf{Arts}       & 0.38  {\cellcolor{highbids}}                                        & 0.21                     & 0.31   {\cellcolor{highbids}}                                       & 0.22                     & 0.39   {\cellcolor{higherbids}}                                       & 1.20                     & 0.18   {\cellcolor{highbids}}                                       & 0.51                     & 1.06   {\cellcolor{highbids}}                                       & 1.14                     & 1.14   {\cellcolor{highbids}}                                       & 1.39                     & 0.30   {\cellcolor{highbids}}                                       & 1.31                     & 0.18   {\cellcolor{highbids}}                                       & 0.13                      \\
\textbf{Business}   & 0.36  {\cellcolor{highbids}}                                        & 0.22                     & 0.32  {\cellcolor{highbids}}                                        & 0.23                     & 0.16  {\cellcolor{lowbids}}                                        & 0.12                     & 0.19  {\cellcolor{highbids}}                                        & 0.42                     & 0.61  {\cellcolor{lowbids}}                                        & 0.73                     & 0.19   {\cellcolor{lowbids}}                                       & 0.22                     & 0.20  {\cellcolor{highbids}}                                        & 0.40                     & 0.21    {\cellcolor{highbids}}                                                        & 0.46                      \\
\textbf{Computers}  & 0.37    {\cellcolor{highbids}}                                      & 0.20                     & 0.30                                     & 0.22                     & 0.45  {\cellcolor{higherbids}}                                        & 1.08                     & 0.15  {\cellcolor{lowbids}}                                        & 0.34                     & 1.02 {\cellcolor{highbids}}                                         & 1.11                     & 1.40  {\cellcolor{highbids}}                                        & 1.42                     & 0.31 {\cellcolor{highbids}}                                         & 1.24                     & 0.33  {\cellcolor{higherbids}}                                        & 2.35                      \\
\textbf{Games}      & 0.36    {\cellcolor{highbids}}                                      & 0.20                     & 0.28  {\cellcolor{lowbids}}                                        & 0.22                     & 0.15 {\cellcolor{lowbids}}                                         & 0.13                     & 0.16  {\cellcolor{lowbids}}                                        & 0.34                     & 0.99   {\cellcolor{highbids}}                                       & 0.95                     & 0.81   {\cellcolor{highbids}}                                       & 1.24                     & 0.23  {\cellcolor{highbids}}                                        & 0.62                     & 0.23  {\cellcolor{highbids}}                                        & 0.73                      \\
\textbf{Health}     & 0.38   {\cellcolor{highbids}}                                       & 0.21                     & 0.38  {\cellcolor{highbids}}                                        & 0.31                     & 0.22   {\cellcolor{highbids}}                                       & 0.38                     & 0.20  {\cellcolor{highbids}}                                        & 0.40                     & 0.98  {\cellcolor{highbids}}                                        & 0.85                     & 0.70  {\cellcolor{highbids}}                                        & 1.07                     & 0.51   {\cellcolor{higherbids}}                                       & 1.17                     & 0.38   {\cellcolor{higherbids}}                                       & 0.81                      \\
\textbf{Home}       & 0.36   {\cellcolor{highbids}}                                       & 0.21                     & 0.34  {\cellcolor{highbids}}                                        & 0.21                     & 0.23 {\cellcolor{highbids}}                                         & 0.42                     & 0.16  {\cellcolor{lowbids}}                                        & 0.34                     & 1.03  {\cellcolor{highbids}}                                        & 1.01                     & 1.61 {\cellcolor{highbids}}                                         & 1.50                     & 0.21 {\cellcolor{highbids}}                                         & 0.52                     & 0.28 {\cellcolor{highbids}}                                         & 0.89                      \\
\textbf{Kids}       & 0.35   {\cellcolor{highbids}}                                       & 0.21                     & 0.29  {\cellcolor{lowbids}}                                        & 0.21                     & 0.18  {\cellcolor{highbids}}                                        & 0.51                     & 0.18 {\cellcolor{highbids}}                                         & 0.59                     & 0.91 {\cellcolor{highbids}}                                         & 1.07                     & 0.66 {\cellcolor{lowbids}}                                         & 1.03                     & 0.23 {\cellcolor{highbids}}                                         & 0.53                     & 0.19  {\cellcolor{highbids}}                                        & 0.21                      \\
\textbf{News}       & 0.37  {\cellcolor{highbids}}                                        & 0.20                     & 0.33  {\cellcolor{highbids}}                                        & 0.23                     & 0.17  {\cellcolor{lowbids}}                                        & 0.25                     & 0.17  {\cellcolor{highbids}}                                        & 0.36                     & 0.95  {\cellcolor{highbids}}                                        & 0.97                     & 0.75  {\cellcolor{highbids}}                                        & 1.03                     & 0.20  {\cellcolor{highbids}}                                        & 0.50                     & 0.18   {\cellcolor{highbids}}                                       & 0.19                      \\
\textbf{Recreation} & 0.36   {\cellcolor{highbids}}                                       & 0.20                     & 0.31 {\cellcolor{highbids}}                                         & 0.22                     & 0.16  {\cellcolor{lowbids}}                                        & 0.15                     & 0.27  {\cellcolor{highbids}}                                        & 0.91                     & 1.03  {\cellcolor{highbids}}                                        & 0.89                     & 0.46  {\cellcolor{lowbids}}                                        & 0.76                     & 0.27  {\cellcolor{highbids}}                                        & 0.66                     & 0.21 {\cellcolor{highbids}}                                         & 0.41                      \\
\textbf{Reference}  & 0.37  {\cellcolor{highbids}}                                        & 0.20                     & 0.32  {\cellcolor{highbids}}                                        & 0.23                     & 0.17  {\cellcolor{lowbids}}                                        & 0.22                     & 0.16  {\cellcolor{lowbids}}                                        & 0.31                     & 1.10  {\cellcolor{highbids}}                                        & 1.09                     & 0.72   {\cellcolor{highbids}}                                       & 1.10                     & 0.22  {\cellcolor{highbids}}                                        & 0.54                     & 0.17  {\cellcolor{lowbids}}                                        & 0.22                      \\
\textbf{Regional}   & 0.35  {\cellcolor{highbids}}                                        & 0.21                     & 0.30                                        & 0.23                     & 0.23  {\cellcolor{highbids}}                                        & 0.54                     & 0.14 {\cellcolor{lowbids}}                                         & 0.38                     & 0.91 {\cellcolor{highbids}}                                         & 0.69                     & 0.35 {\cellcolor{lowbids}}                                         & 0.59                     & 0.24 {\cellcolor{highbids}}                                         & 0.74                     & 0.19  {\cellcolor{highbids}}                                        & 0.32                      \\
\textbf{Science}    & 0.36  {\cellcolor{highbids}}                                        & 0.20                     & 0.32 {\cellcolor{highbids}}                                         & 0.22                     & 0.18 {\cellcolor{lowbids}}                                         & 0.16                     & 0.23  {\cellcolor{highbids}}                                        & 0.63                     & 1.05 {\cellcolor{highbids}}                                         & 1.23                     & 0.68  {\cellcolor{lowbids}}                                        & 1.05                     & 0.23 {\cellcolor{highbids}}                                         & 0.55                     & 0.15  {\cellcolor{lowbids}}                                        & 0.14                      \\
\textbf{Shopping}   & 0.32                                         & 0.23                     & 0.32 {\cellcolor{highbids}}                                         & 0.22                     & 0.20  {\cellcolor{highbids}}                                        & 0.34                     & 0.18 {\cellcolor{highbids}}                                         & 0.41                     & 1.00 {\cellcolor{highbids}}                                         & 1.21                     & 0.77 {\cellcolor{highbids}}                                         & 1.06                     & 0.22  {\cellcolor{highbids}}                                        & 0.58                     & 0.21  {\cellcolor{highbids}}                                        & 0.69                      \\
\textbf{Society}    & 0.37     {\cellcolor{highbids}}                                     & 0.20                     & 0.33  {\cellcolor{highbids}}                                        & 0.21                     & 0.24   {\cellcolor{highbids}}                                       & 1.05                     & 0.17  {\cellcolor{lowbids}}                                        & 0.34                     & 0.85  {\cellcolor{lowbids}}                                        & 1.06                     & 0.20  {\cellcolor{lowbids}}                                        & 0.22                     & 0.18 {\cellcolor{highbids}}                                         & 0.24                     & 0.16 {\cellcolor{lowbids}}                                         & 0.19                      \\
\textbf{Sports}     & 0.33   {\cellcolor{highbids}}                                       & 0.23                     & 0.31 {\cellcolor{highbids}}                                         & 0.22                     & 0.17 {\cellcolor{lowbids}}                                         & 0.29                     & 0.18 {\cellcolor{highbids}}                                         & 0.39                     & 0.94  {\cellcolor{highbids}}                                        & 1.01                     & 0.77 {\cellcolor{highbids}}                                         & 1.12                     & 0.23 {\cellcolor{highbids}}                                         & 0.57                     & 0.18 {\cellcolor{lowbids}}                                          & 0.21                      \\
\midrule
\textbf{Control}    & 0.32                     & 0.22                     & 0.30                     & 0.23                     & 0.18                     & 0.16                     & 0.17                     & 0.36                     & 0.88                     & 1.18                     & 0.69                     & 1.11                     & 0.17                     & 0.18                     & 0.18                     & 0.14         \\            



    \bottomrule

\end{tabular}

%\vspace{-5mm}
\label{table:CCPA-bidding-mean}
\end{table*}



==> docs/bids-table-california.tex <==
\begin{table*}
%\adjustbox{max width=\textwidth}{
    \centering
    \caption{Ad bidding under CCPA in California. Avg. column represents the mean of all bid value. Std. represents the standard deviation of all bid value. Opt-out and opt-in represent the bids when we opt-out and opt-in the selling of user data, respectively.  $\uparrow$ and $\downarrow$ indicate bid values that are higher and lower than Control's avg., respectively. $\textcolor{red}{\uparrow}$ and $\textcolor{red}{\downarrow}$ indicate bid values that are Control's avg. $\pm$ std., respectively.}
    \begin{tabular}{l?{0.3mm}rr|rr?{0.3mm}rr|rr?{0.3mm}rr|rr} 
    \toprule
     & \multicolumn{4}{c?{0.3mm}}{\textbf{OneTrust}} & \multicolumn{4}{c?{0.3mm}}{\textbf{CookieBot}}& \multicolumn{4}{c}{\textbf{NAI}}    \\ 
     & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c?{0.3mm}}{\textbf{Opt-in}}     & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c?{0.3mm}}{\textbf{Opt-in}}    & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c}{\textbf{Opt-in}}   \\ 
    \textbf{Persona}     & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}}  & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c}{\textbf{Std.}}  \\ 
    \toprule
    
    
    
\textbf{Adult}      & 0.29$^{\downarrow}$                     & 0.35                     & 0.21$^{\downarrow}$                          & 0.31                     &  0.32$^{\uparrow}$                          & 0.19                     & 0.29$^{\uparrow}$                     & 0.53                     &  0.27$^{\downarrow}$                          & 0.42                     & 0.37$^{\uparrow}$                     & 0.47                      \\ 

\textbf{Arts}       & 0.33$^{\downarrow}$                     & 0.41                     & 0.26$^{\downarrow}$                     & 0.28                     &  0.37$^{\uparrow}$                     & 0.55                     & 0.34$^{\uparrow}$                     & 0.30                     &  0.40$^{\downarrow}$                     & 0.46                     & 0.41$^{\uparrow}$                     & 0.43                      \\ 

\textbf{Business}   & 0.40$^{\uparrow}$                     & 0.49                     & 0.70$^{\uparrow}$                     & 0.78                      & 0.25$^{\downarrow}$                       & 0.19                     & 0.32$^{\uparrow}$                     & 0.17                     &  0.40$^{\downarrow}$                       & 0.59                     & 0.31$^{\downarrow}$                       & 0.41                      \\ 

\textbf{Computers}  & 0.32$^{\downarrow}$                     & 0.31                     & 0.47$^{\uparrow}$                     & 0.74                     &  0.34$^{\uparrow}$                     & 0.23                     & 0.35$^{\uparrow}$                     & 0.31                     &  0.48$^{\uparrow}$                     & 0.78                     & 0.51$^{\uparrow}$                     & 0.97                      \\ 

\textbf{Games}      & 0.44$^{\uparrow}$                     & 0.42                     & 0.42$^{\downarrow}$                      & 0.55                     &  0.28$^{\downarrow}$                      & 0.21                     & 0.32$^{\uparrow}$                     & 0.18                     &  0.94$^{\uparrow}$                     & 1.57                     & 0.31$^{\downarrow}$                      & 0.48                      \\ 

\textbf{Health}     & 0.36$^{\downarrow}$                      & 0.40                     & 0.56$^{\uparrow}$                      & 0.63                     &  0.64$^{\textcolor{red}{\uparrow}}$                      & 1.11                     & 0.48$^{\textcolor{red}{\uparrow}}$                      & 0.44                     & 0.28$^{\downarrow}$                      & 0.56                     & 0.50$^{\uparrow}$                      & 0.48                      \\ 

\textbf{Home}       & 1.69$^{\textcolor{red}{\uparrow}}$                      & 2.58                     & 0.39$^{\downarrow}$                     & 0.50                     &  0.26$^{\downarrow}$                     & 0.19                     & 0.28$^{\uparrow}$                      & 0.20                     &  1.18$^{\textcolor{red}{\uparrow}}$                      & 2.82                     & 0.46$^{\uparrow}$                      & 0.90                      \\ 

\textbf{Kids}       & 0.31$^{\downarrow}$                     & 0.36                     & 0.45$^{\uparrow}$                       & 0.59                     &  0.37$^{\uparrow}$                       & 0.55                     & 0.30$^{\uparrow}$                       & 0.53                     &  0.30$^{\downarrow}$                     & 0.58                     & 0.35$^{\uparrow}$                       & 0.65                      \\ 

\textbf{News}       & 0.35$^{\downarrow}$                      & 0.40                     & 0.51$^{\uparrow}$                       & 0.61                     &  0.34$^{\uparrow}$                       & 0.17                     & 0.25$^{\downarrow}$                      & 0.15                     &  0.90$^{\uparrow}$                       & 1.57                     & 0.83$^{\uparrow}$                       & 1.83                      \\ 

\textbf{Recreation} & 0.21$^{\downarrow}$                      & 0.29                     & 0.45$^{\uparrow}$                      & 0.55                     &  0.29$^{\downarrow}$                      & 0.19                     & 0.25$^{\downarrow}$                      & 0.19                     &  0.46$^{\uparrow}$                      & 0.98                     & 0.24$^{\downarrow}$                      & 0.43                      \\ 

\textbf{Reference}  & 0.70$^{\textcolor{red}{\uparrow}}$                      & 1.50                     & 0.54$^{\uparrow}$                      & 0.96                                          & 0.36$^{\uparrow}$                      & 0.42                     & 0.33$^{\uparrow}$                      & 0.20                     &  0.66$^{\uparrow}$                      & 1.06                     & 0.35$^{\uparrow}$                      & 0.45                      \\ 

\textbf{Regional}   & 0.78$^{\textcolor{red}{\uparrow}}$                      & 1.82                     & 0.41$^{\downarrow}$                      & 0.57                                          & 0.30$^{\downarrow}$                      & 0.18                     & 0.26$^{\downarrow}$                      & 0.20                     &  0.58$^{\uparrow}$                      & 0.47                     & 0.33$^{\uparrow}$                      & 0.11                      \\ 

\textbf{Science}    & 0.45$^{\uparrow}$                      & 0.38                     & 0.37$^{\downarrow}$                      & 0.48                                          & 0.34$^{\uparrow}$                      & 0.35                     & 0.28$^{\uparrow}$                      & 0.20                     &  0.33$^{\downarrow}$                      & 0.49                     & 1.04$^{\textcolor{red}{\uparrow}}$                      & 2.11                      \\ 

\textbf{Shopping}   & 0.27$^{\downarrow}$                     & 0.24                     & 0.62$^{\uparrow}$                      & 0.81                     &  0.30$^{\downarrow}$                     & 0.18                     & 0.27$^{\uparrow}$                      & 0.23                     &  0.26$^{\downarrow}$                     & 0.15                     & 0.54$^{\uparrow}$                      & 0.77                      \\ 

\textbf{Society}    & 0.37$^{\uparrow}$                     & 0.40                     & 0.54$^{\uparrow}$                     & 0.64                     &  0.29$^{\downarrow}$                     & 0.19                     & 0.28$^{\uparrow}$                     & 0.19                     &  0.61$^{\uparrow}$                     & 0.86                     & 0.24$^{\downarrow}$                     & 0.36                      \\ 

\textbf{Sports}     & 0.31$^{\downarrow}$                     & 0.31                     & 0.52$^{\uparrow}$                      & 0.63                     &  0.32$^{\uparrow}$                      & 0.17                     & 0.27$^{\downarrow}$                     & 0.17                     & 0.24$^{\downarrow}$                     & 0.40                     & 0.23$^{\downarrow}$                     & 0.44                      \\ 
\midrule
\textbf{Control}    & 0.36                     & 0.34                     & 0.45                     & 0.39                                          & 0.30                     & 0.16                     & 0.27                     & 0.18                                          & 0.44                     & 0.60                     & 0.31                     & 0.53                      \\

    \bottomrule

\end{tabular}

%\vspace{-5mm}
\label{table:CCPA-bidding-mean}
\end{table*}



==> docs/bids-table-france.tex <==
\begin{table*}[!h]
%\adjustbox{max width=\textwidth}{
    \centering
        \caption{Ad bidding under GDPR in France. Avg. column represents the mean of all bid value. Std. represents the standard deviation of all bid value. Opt-out and opt-in represent the bids when we opt-out and opt-in the selling of user data, respectively.  $\uparrow$ and $\downarrow$ indicate bid values that are higher and lower than Control's avg., respectively. $\textcolor{red}{\uparrow}$ and $\textcolor{red}{\downarrow}$ indicate bid values that are Control's avg. $\pm$ std., respectively.}
    \begin{tabular}{l?{0.3mm}rr|rr?{0.3mm}rr|rr?{0.3mm}rr|rr} 
    \toprule
     & \multicolumn{4}{c?{0.3mm}}{\textbf{OneTrust}} & \multicolumn{4}{c?{0.3mm}}{\textbf{CookieBot}}& \multicolumn{4}{c}{\textbf{NAI}}    \\ 
     & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c?{0.3mm}}{\textbf{Opt-in}}     & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c?{0.3mm}}{\textbf{Opt-in}}    & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c}{\textbf{Opt-in}}   \\ 
    \textbf{Persona}     & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}}  & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c}{\textbf{Std.}}  \\ 
    \toprule
        
        
        
    \textbf{Adult}                                                              & 0.21$^{\uparrow}$                                           & 0.21                                          & 0.16$^{\downarrow}$                                          & 0.16                                                                                   & 0.10$^{\uparrow}$                                           & 0.00                                          & 0.02$^{\downarrow}$                                          & 0.01                                                                                  & 0.31$^{\uparrow}$                                           & 0.32                                          & 0.19$^{\uparrow}$                                           & 0.18                                           \\ 
    
    \textbf{Arts}                                                               & 0.05$^{\downarrow}$                                          & 0.07                                          & 0.50$^{\uparrow}$                                           & 0.45                                                                                    & 0.04$^{\downarrow}$                                          & 0.03                                          & 0.03$^{\downarrow}$                                          & 0.05                                           & 0.29$^{\uparrow}$                                           & 0.17                                          & 0.24$^{\textcolor{red}{\uparrow}}$                                           & 0.17                                           \\ 
    
    \textbf{Business}                                                           & 0.03$^{\downarrow}$                                          & 0.05                                          & 0.56$^{\uparrow}$                                           & 0.50                                           & 0.27$^{\textcolor{red}{\uparrow}}$                                           & 0.16                                          & 0.17$^{\uparrow}$                                           & 0.17                                           & 0.03$^{\textcolor{red}{\downarrow}}$                                          & 0.02                                          & 0.03$^{\textcolor{red}{\downarrow}}$                                          & 0.01                                           \\ 
    
    \textbf{Computers}                                                          & 0.33$^{\uparrow}$                                           & 0.52                                          & 0.67$^{\uparrow}$                                           & 0.88                                           & 0.23$^{\textcolor{red}{\uparrow}}$                                           & 0.12                                          & 0.11$^{\uparrow}$                                           & 0.07                                                                                    & 0.08$^{\textcolor{red}{\downarrow}}$                                          & 0.08                                          & 0.34$^{\textcolor{red}{\uparrow}}$                                           & 0.46                                           \\ 
    
    \textbf{Games}                                                              & 0.25$^{\uparrow}$                                          & 0.20                                          & 0.96$^{\uparrow}$                                          & 0.92                                                                                  & 0.21$^{\textcolor{red}{\uparrow}}$                                          & 0.22                                          & 0.20$^{\uparrow}$                                          & 0.23                                           & 0.13$^{\downarrow}$                                          & 0.15                                          & - & -  \\ 
    
    \textbf{Health}                                                             & 0.33$^{\uparrow}$                                          & 0.34                                          & 0.74$^{\uparrow}$                                          & 0.55                                                                                    & 0.28$^{\textcolor{red}{\uparrow}}$                                          & 0.41                                          & 0.32$^{\textcolor{red}{\uparrow}}$                                          & 0.18                                                                                   & - & - & - & -  \\ 
    
    \textbf{Home}                                                               & 0.30$^{\uparrow}$                                          & 0.40                                          & 0.85$^{\uparrow}$                                          & 1.28                                                                                    & 0.03$^{\downarrow}$                                          & 0.02                                          & 0.03$^{\downarrow}$                                          & 0.02                                           & 0.07$^{\textcolor{red}{\downarrow}}$                                          & 0.05                                          & 0.04$^{\textcolor{red}{\downarrow}}$                                          & 0.02                                           \\ 
    
    \textbf{Kids}                                                               & 0.33$^{\uparrow}$                                          & 0.34                                          & 0.54$^{\uparrow}$                                          & 0.76                                                                                    & 0.31$^{\textcolor{red}{\uparrow}}$                                          & 0.15                                          & 0.05$^{\downarrow}$                                          & 0.06                                                                                   & 0.14$^{\downarrow}$                                          & 0.18                                          & 0.17$^{\uparrow}$                                          & 0.45                                           \\ 
    
    \textbf{News}                                                               & 0.17$^{\downarrow}$                                          & 0.19                                          & 0.41$^{\downarrow}$                                          & 0.72                                           & 0.26$^{\textcolor{red}{\uparrow}}$                                          & 0.22                                          & 0.31$^{\textcolor{red}{\uparrow}}$                                          & 0.19                                                                                    & 0.07$^{\textcolor{red}{\downarrow}}$                                          & 0.05                                          & 0.05$^{\textcolor{red}{\downarrow}}$                                          & 0.04                                           \\ 
    
    \textbf{Recreation}                                                         & 0.23$^{\uparrow}$                                          & 0.22                                          & 0.22$^{\downarrow}$                                          & 0.27                                           & 0.33$^{\textcolor{red}{\uparrow}}$                                          & 0.18                                          & 0.06$^{\downarrow}$                                          & 0.00                                                                                    & 0.02$^{\textcolor{red}{\downarrow}}$                                          & 0.02                                          & 0.01$^{\textcolor{red}{\downarrow}}$                                          & 0.01                                           \\ 
    
    \textbf{Reference}                                                          & 0.29$^{\uparrow}$                                          & 0.18                                          & 0.68$^{\uparrow}$                                          & 0.86                                                                                    & 0.08$^{\downarrow}$                                          & 0.14                                          & 0.14$^{\uparrow}$                                          & 0.20                                                                                   & 0.24$^{\uparrow}$                                          & 0.18                                          & 0.23$^{\uparrow}$                                          & 0.15                                           \\ 
    
    \textbf{Regional}                                                           & 0.08$^{\downarrow}$                                          & 0.12                                          & 0.65$^{\uparrow}$                                          & 0.54                                                                                    & 0.14$^{\uparrow}$                                          & 0.19                                          & 0.04$^{\downarrow}$                                          & 0.03                                           & 0.30$^{\uparrow}$                                          & 0.29                                          & 0.21$^{\uparrow}$                                          & 0.15                                           \\ 
    
    \textbf{Science}                                                            & 0.21$^{\uparrow}$                                          & 0.22                                          & 0.77$^{\uparrow}$                                          & 1.13                                                                                    & 0.09$^{\downarrow}$                                          & 0.08                                          & 0.09$^{\downarrow}$                                          & 0.08                                           & 0.05$^{\textcolor{red}{\downarrow}}$                                          & 0.03                                          & 0.04$^{\textcolor{red}{\downarrow}}$                                          & 0.03                                           \\ 
    
    \textbf{Shopping}                                                           & 0.38$^{\textcolor{red}{\uparrow}}$                                          & 0.56                                          & 0.67$^{\uparrow}$                                          & 1.10                                           & 0.19$^{\textcolor{red}{\uparrow}}$                                          & 0.07                                          & 0.27$^{\textcolor{red}{\uparrow}}$                                          & 0.13                                                                                    & 0.07$^{\textcolor{red}{\downarrow}}$                                          & 0.15                                          & 0.34$^{\textcolor{red}{\uparrow}}$                                          & 0.68                                           \\ 
    
    \textbf{Society}                                                            & 0.34$^{\uparrow}$                                          & 0.36                                          & 0.50$^{\uparrow}$                                          & 0.63                                           & 0.27$^{\textcolor{red}{\uparrow}}$                                          & 0.26                                          & 0.19$^{\uparrow}$                                          & 0.19                                                                                    & 0.07$^{\textcolor{red}{\downarrow}}$                                          & 0.07                                          & 0.05$^{\textcolor{red}{\downarrow}}$                                          & 0.04                                           \\ 
    
    \textbf{Sports}                                                             & 0.48$^{\textcolor{red}{\uparrow}}$                                          & 0.38                                          & 0.80$^{\uparrow}$                                          & 0.99                                                                                   & 0.01$^{\textcolor{red}{\downarrow}}$                                          & 0.00                                          & 0.02$^{\downarrow}$                                          & 0.00                                           & 0.09$^{\downarrow}$                                          & 0.09                                          & 0.08$^{\textcolor{red}{\downarrow}}$                                          & 0.12                                           \\ 
    
    \midrule
    \textbf{Control}                                                            & 0.18                                          & 0.18                                          & 0.42                                          & 0.63                                                                                    & 0.09                                          & 0.07                                          & 0.09                                          & 0.15                                          &  0.22                                          & 0.14                                          & 0.16                                          & 0.07                                           \\
    
        \bottomrule
    
    \end{tabular}

    \label{table:GDPR-bidding-France-mean}
    \end{table*}
    

==> docs/bids-table-germany-california-non-appearing-advertisers.tex <==
%
%
%\begin{table*}[htb!]
%    \centering
%    \caption{Ad bidding under CCPA and GDPR from advertisers who did not bid or appear when we simulated personas but appeared and bid after we opted opt-out under of processing and selling of data. Avg. column represents the average of each advertiser's median bid value. Std. represents the standard deviation of each advertiser's median bid value. $\uparrow$ and $\downarrow$ indicate bid values that are higher and lower than Control's avg., respectively. $\textcolor{red}{\uparrow}$ and $\textcolor{red}{\downarrow}$ indicate bid values that are Control's avg. $\pm$ std., respectively.}
%    \begin{tabular}{l?{0.3mm}ll|ll|ll?{0.3mm}ll|ll|ll} 
%    \toprule
%
%    & \multicolumn{6}{c?{0.3mm}}{\textbf{GDPR}} & \multicolumn{6}{c}{\textbf{CCPA}} \\ 
%    
%    \textbf{Persona} & \multicolumn{2}{c}{\textbf{OneTrust}}& \multicolumn{2}{c}{\textbf{CookieBot}}  & \multicolumn{2}{c?{0.3mm}}{\textbf{NAI}}  & \multicolumn{2}{c}{\textbf{OneTrust}}& \multicolumn{2}{c}{\textbf{CookieBot}}  & \multicolumn{2}{c}{\textbf{NAI}}  \\ 
%
%    \multicolumn{1}{c?{0.3mm}}{}  & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \textbf{Avg.} & \textbf{Std.}   & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c}{\textbf{Std.}}  \\ 
%    \toprule
%\textbf{Adult}                              														& 0.08$^{\uparrow}$                                                           & 0.00                                          & 0.02$^{\textcolor{red}{\uparrow}}$                                                           & 0.03                                          & 0.68$^{\textcolor{red}{\uparrow}}$                                                           & 0.96                                          & 0.16$\downarrow$                                                        & 0.00                                          & 0.36$^{\uparrow}$                                                           & 0.16                                          & 0.34$\downarrow$                                                        & 0.42                                           \\ 
%
%\textbf{Arts}                                                                                                          & 0.07$^{\uparrow}$                                                           & 0.00                                          & 0.08$^{\textcolor{red}{\uparrow}}$                                                           & 0.08                                          & 0.05$\downarrow$                                                        & 0.01                                          & 0.33$\downarrow$                                                        & 0.41                                          & 0.40$^{\uparrow}$                                                           & 0.61                                          & 0.22$\downarrow$                                                        & 0.27                                           \\ 
%
%\textbf{Business}                                                                                                      & 0.08$^{\uparrow}$                                                           & 0.00                                          & 0.07$^{\textcolor{red}{\uparrow}}$                                                           & 0.00                                          & 0.30$^{\uparrow}$                                                           & 0.28                                          & 0.38$^{\uparrow}$                                                           & 0.37                                          & 0.27$\downarrow$                                                        & 0.16                                          & 0.32$\downarrow$                                                        & 0.43                                           \\ 
%
%\textbf{Computers}                                                                                                     & 0.09$^{\uparrow}$                                                           & 0.11                                          & 0.11$^{\textcolor{red}{\uparrow}}$                                                           & 0.09                                          & 1.11$^{\textcolor{red}{\uparrow}}$                                                           & 1.12                                          & 0.43$^{\uparrow}$                                                           & 0.22                                          & 0.34$^{\uparrow}$                                                           & 0.16                                          & 0.43$\downarrow$                                                        & 0.65                                           \\ 
%
%\textbf{Games}                                                                                                         & 0.16$^{\textcolor{red}{\uparrow}}$                                                           & 0.01                                          & 3E-3$^{\textcolor{red}{\uparrow}}$                                                           & 0.01                                          & 0.74$^{\textcolor{red}{\uparrow}}$                                                           & 0.83                                          & 0.39$^{\uparrow}$                                                           & 0.49                                          & 0.31$^{\uparrow}$                                                           & 0.16                                          & 0.56$^{\uparrow}$                                                           & 0.74                                           \\ 
%
%\textbf{Health}                                                                                                        & 2.43$^{\textcolor{red}{\uparrow}}$                                                           & 0.00                                          & 0.05$^{\textcolor{red}{\uparrow}}$                                                           & 0.00                                          & 0.68$^{\textcolor{red}{\uparrow}}$                                                           & 0.97                                          & 0.36$\downarrow$                                                        & 0.47                                          & 0.47$^{\textcolor{red}{\uparrow}}$                                                           & 1.32                                          & 0.79$^{\uparrow}$                                                           & 0.96                                           \\ 
%
%\textbf{Home}                                                                                                          & 0.13$^{\uparrow}$                                                           & 0.16                                          & 1.00$^{\textcolor{red}{\uparrow}}$                                                           & 1.37                                          & 0.11$\downarrow$                                                        & 0.18                                          & 0.53$^{\uparrow}$                                                           & 0.45                                          & 0.27$\downarrow$                                                        & 0.17                                          & 0.50$\downarrow$                                                        & 0.63                                           \\ 
%
%\textbf{Kids}                                                                                                          & 0.07$^{\uparrow}$                                                           & 0.00                                          & 0.06$^{\textcolor{red}{\uparrow}}$                                                           & 0.01                                          & 0.07$\downarrow$                                                        & 0.01                                          & 0.31$\downarrow$                                                        & 0.34                                          & 0.41$^{\uparrow}$                                                           & 0.61                                          & 0.27$\downarrow$                                                        & 0.51                                           \\ 
%
%\textbf{News}                                                                                                          & 0.12$^{\uparrow}$                                                           & 0.14                                          & 0.17$^{\textcolor{red}{\uparrow}}$                                                           & 0.03                                          & 0.85$^{\textcolor{red}{\uparrow}}$                                                           & 0.71                                          & 0.35$\downarrow$                                                        & 0.41                                          & 0.20$\downarrow$                                                        & 0.01                                          & 0.84$^{\uparrow}$                                                           & 1.02                                           \\ 
%
%\textbf{Recreation}                                                                                                    & 0.10$^{\uparrow}$                                                           & 0.17                                          & 0.05$^{\textcolor{red}{\uparrow}}$                                                           & 0.00                                          & 1.07$^{\textcolor{red}{\uparrow}}$                                                           & 0.95                                          & 0.12$\downarrow$                                                        & 0.06                                          & 0.34$^{\uparrow}$                                                           & 0.16                                          & 0.13$\downarrow$                                                        & 0.18                                           \\ 
%
%\textbf{Reference}                                                                                                     & 0.07$^{\uparrow}$                                                           & 0.01                                          & 0.18$^{\textcolor{red}{\uparrow}}$                                                           & 0.05                                          & 1.10$^{\textcolor{red}{\uparrow}}$                                                           & 0.77                                          & 1.34$^{\textcolor{red}{\uparrow}}$                                                           & 2.47                                          & 0.33$^{\uparrow}$                                                           & 0.16                                          & 0.59$^{\uparrow}$                                                           & 0.93                                           \\ 
%
%\textbf{Regional}                                                                                                      & 0.08$^{\uparrow}$                                                           & 0.01                                          & 0.06$^{\textcolor{red}{\uparrow}}$                                                           & 0.01                                          & 1.67$^{\textcolor{red}{\uparrow}}$                                                           & 0.84                                          & 0.31$\downarrow$                                                        & 0.37                                          & 0.35$^{\uparrow}$                                                           & 0.16                                          & 0.61$^{\uparrow}$                                                           & 0.01                                           \\ 
%
%\textbf{Science}                                                                                                       & 0.07$^{\uparrow}$                                                           & 0.00                                          & 0.01$^{\textcolor{red}{\uparrow}}$                                                           & 0.03                                          & 0.56$^{\textcolor{red}{\uparrow}}$                                                           & 0.69                                          & 0.46$^{\uparrow}$                                                           & 0.33                                          & 0.34$^{\uparrow}$                                                           & 0.24                                          & 0.36$\downarrow$                                                        & 0.35                                           \\ 
%
%\textbf{Shopping}                                                                                                      & 0.09$^{\uparrow}$                                                           & 0.02                                          & 0.01$^{\textcolor{red}{\uparrow}}$                                                           & 0.05                                          & 0.75$^{\textcolor{red}{\uparrow}}$                                                           & 0.00                                          & 0.28$\downarrow$                                                        & 0.17                                          & 0.32$^{\uparrow}$                                                           & 0.18                                          & 0.78$^{\uparrow}$                                                           & 0.72                                           \\ 
%
%\textbf{Society}                                                                                                       & 0.23$^{\textcolor{red}{\uparrow}}$                                                           & 0.14                                          & 0.16$^{\textcolor{red}{\uparrow}}$                                                           & 0.03                                          & 0.05$\downarrow$                                                        & 0.02                                          & 0.30$\downarrow$                                                        & 0.35                                          & 0.33$^{\uparrow}$                                                           & 0.17                                          & 0.71$^{\uparrow}$                                                           & 0.99                                           \\ 
%
%\textbf{Sports}                                                                                                        & 0.10$^{\uparrow}$                                                           & 0.02                                          & 0.69$^{\textcolor{red}{\uparrow}}$                                                           & 0.97                                          & 0.54$^{\textcolor{red}{\uparrow}}$                                                           & 0.83                                          & 0.32$\downarrow$                                                        & 0.33                                          & 0.33$^{\uparrow}$                                                           & 0.16                                          & 0.40$\downarrow$                                                        & 0.54                                           \\ 
%
%    
%    \midrule
%
%\textbf{Control}                                                                                                       & 0.04                                                        & 0.11                                          & 5E-4                                                        & 1.9E-3                                          & 0.16                                                        & 0.20                                          & 0.36                                                        & 0.34                                          & 0.30                                                        & 0.16                                          & 0.53                                                        & 0.61                                           \\
%
%    \bottomrule
%
%\end{tabular}
%
%\label{table:in_test_not_in_train}
%\end{table*}



\begin{table*}[htb!]
\footnotesize
\centering

\caption{\textcolor{blue}{Ad bidding under CCPA and GDPR from advertisers who did not bid or appear when we simulated personas but appeared and bid after we opted opt-out under of processing and selling of data in 4 CMPs. Avg. column represents the average of each advertiser's median bid value. Std. represents the standard deviation of each advertiser's median bid value. Color \textcolor{pink}{pink} and \textcolor{cyan}{cyan} indicate bid values that are higher and lower than Control's avg., respectively. Color \textcolor{red}{red} and \textcolor{blue}{blue} indicate bid values that are Control's avg. $\pm$ std., respectively. --- represents the absence of bids.}}





    \begin{tabular}{l?{0.3mm}ll|ll|ll|ll?{0.3mm}ll|ll|ll|ll} 
    \toprule

    & \multicolumn{8}{c?{0.3mm}}{\textbf{GDPR}} & \multicolumn{8}{c}{\textbf{CCPA}} \\ 
    
    \textbf{Persona} & \multicolumn{2}{c}{\textbf{Cookiebot}}& \multicolumn{2}{c}{\textbf{Didomi}}  &\multicolumn{2}{c}{\textbf{Onetrust}}  & \multicolumn{2}{c?{0.3mm}}{\textbf{Quantcast}}  & \multicolumn{2}{c}{\textbf{Cookiebot}}&\multicolumn{2}{c}{\textbf{Didomi}}& \multicolumn{2}{c}{\textbf{Onetrust}}  & \multicolumn{2}{c}{\textbf{Quantcast}}  \\ 

    \multicolumn{1}{c?{0.3mm}}{}  & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}}& \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}}& \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}}   & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c}{\textbf{Std.}}  \\ 
    \toprule

\textbf{Adult}      & 0.37  {\cellcolor{pink}}                                                                                              & 0.20                              & --                                & --                                & 0.02   {\cellcolor{cyan}}                                                                                         & 4.95E-03                              & 0.19    {\cellcolor{pink}}                                                                                            & 0.55                              & 0.37    {\cellcolor{pink}}                                                                                            & 0.20                              & 0.12    {\cellcolor{cyan}}                                                                                        & 0.08                              & 1.64   {\cellcolor{pink}}                                                                                             & 0.85                              & 0.20  {\cellcolor{pink}}                                                                                              & 0.22                               \\
\textbf{Arts}       & 0.35   {\cellcolor{pink}}                                                                                             & 0.21                              & 0.05   {\cellcolor{cyan}}                                                                                         & 0.00                              & --                                & --                                & 0.16   {\cellcolor{pink}}                                                                                             & 0.20                              & 0.37   {\cellcolor{pink}}                                                                                             & 0.20                              & 0.45 {\cellcolor{red}}                                                                                                                                                                & 1.34                              & 1.43 {\cellcolor{pink}}                                                                   & 1.03                              & 0.29   {\cellcolor{pink}}                                                                                             & 1.51                               \\
\textbf{Business}   & 0.35   {\cellcolor{pink}}                                                                                             & 0.21                              & --                                & --                                & 0.01         {\cellcolor{blue}}                                                                                       & 0.01                              & 0.14 {\cellcolor{cyan}}                                                                                           & 0.19                              & 0.37    {\cellcolor{pink}}                                                                                            & 0.20                              & 0.15      {\cellcolor{cyan}}                                                                                      & 0.09                              & 1.29    {\cellcolor{pink}}                                                                                            & 1.22                              & 0.19    {\cellcolor{pink}}                                                                                            & 0.46                               \\
\textbf{Computers}  & 0.35  {\cellcolor{pink}}                                                                                              & 0.21                              & 0.05       {\cellcolor{blue}}                                                                                         & 0.00                              & 0.02  {\cellcolor{pink}}                                                                                              & 0.00                              & 0.28 {\cellcolor{red}}                                                                                                                                                                & 0.66                              & 0.37  {\cellcolor{pink}}                                                                                              & 0.20                              & 0.45  {\cellcolor{red}}                                                                                                                                                               & 1.08                              & 1.78   {\cellcolor{pink}}                                                                                             & 0.94                              & 0.21  {\cellcolor{pink}}                                                                                              & 0.57                               \\
\textbf{Games}      & 0.38 {\cellcolor{pink}}                                                                                               & 0.20                              & 0.03     {\cellcolor{blue}}                                                                                           & 0.02                              & 0.02   {\cellcolor{pink}}                                                                                             & 0.00                              & 0.44 {\cellcolor{red}}                                                                                                                                                                & 0.97                              & 0.36   {\cellcolor{pink}}                                                                                             & 0.20                              & 0.15   {\cellcolor{cyan}}                                                                                         & 0.10                              & 1.50  {\cellcolor{pink}}                                                                                              & 0.87                              & 0.24 {\cellcolor{pink}}                                                                                               & 0.69                               \\
\textbf{Health}     & 0.35   {\cellcolor{pink}}                                                                                             & 0.21                              & --                                & --                                & 0.03   {\cellcolor{red}}                                                                                                                                                              & 0.02                              & 0.17  {\cellcolor{pink}}                                                                                              & 0.20                              & 0.37   {\cellcolor{pink}}                                                                                             & 0.20                              & 0.16   {\cellcolor{cyan}}                                                                                         & 0.12                              & 1.37   {\cellcolor{pink}}                                                                                             & 0.77                              & 0.52    {\cellcolor{red}}                                                                                                                                                             & 1.19                               \\
\textbf{Home}       & 0.38  {\cellcolor{pink}}                                                                                              & 0.20                              & 0.05      {\cellcolor{blue}}                                                                                          & 0.00                              & 0.31      {\cellcolor{red}}                                                                                                                                                           & 0.25                              & 0.16  {\cellcolor{pink}}                                                                                              & 0.18                              & 0.36   {\cellcolor{pink}}                                                                                             & 0.20                              & 0.23   {\cellcolor{pink}}                                                                                             & 0.44                              & 1.63  {\cellcolor{pink}}                                                                                              & 0.87                              & 0.18   {\cellcolor{pink}}                                                                                             & 0.16                               \\
\textbf{Kids}       & 0.37   {\cellcolor{pink}}                                                                                             & 0.20                              & 0.06    {\cellcolor{red}}                                                                                                                                                             & 0.00                              & 0.02 {\cellcolor{cyan}}                                                                   & 0.01                              & 0.25            {\cellcolor{red}}                                                                                                                                                    & 0.55                              & 0.36    {\cellcolor{pink}}                                                                                            & 0.21                              & 0.04  {\cellcolor{cyan}}                                                                                          & 0.09                              & 1.95   {\cellcolor{pink}}                                                                                             & 1.14                              & 0.23 {\cellcolor{pink}}                                                                                               & 0.53                               \\
\textbf{News}       & 0.35    {\cellcolor{pink}}                                                                                            & 0.21                              & --                                & --                                & 0.02      {\cellcolor{pink}}                                                                                          & 0.00                              & 0.20     {\cellcolor{pink}}                                                                                           & 0.38                              & 0.37   {\cellcolor{pink}}                                                                                             & 0.20                              & 0.18    {\cellcolor{cyan}}                                                                                        & 0.25                              & 1.76     {\cellcolor{pink}}                                                                                           & 1.00                              & 0.17    {\cellcolor{cyan}}                                                                                        & 0.14                               \\
\textbf{Recreation} & 0.37  {\cellcolor{pink}}                                                                                              & 0.20                              & 0.06         {\cellcolor{red}}                                                                                                                                                        & 0.00                              & 0.02     {\cellcolor{red}}                                                                                                                                                            & 0.01                              & 0.18      {\cellcolor{pink}}                                                                                          & 0.33                              & 0.36      {\cellcolor{pink}}                                                                                          & 0.20                              & 0.14    {\cellcolor{cyan}}                                                                                        & 0.12                              & 1.55     {\cellcolor{pink}}                                                                                           & 0.70                              & 0.16   {\cellcolor{cyan}}                                                                                         & 0.11                               \\
\textbf{Reference}  & 0.37   {\cellcolor{pink}}                                                                                             & 0.20                              & --                                & --                                & 0.03      {\cellcolor{red}}                                                                                                                                                           & 0.01                              & 0.18        {\cellcolor{pink}}                                                                                        & 0.29                              & 0.37       {\cellcolor{pink}}                                                                                         & 0.20                              & 0.17    {\cellcolor{cyan}}                                                                                        & 0.22                              & 1.86    {\cellcolor{pink}}                                                                                            & 1.05                              & 0.22   {\cellcolor{pink}}                                                                                             & 0.63                               \\
\textbf{Regional}   & 0.38    {\cellcolor{pink}}                                                                                            & 0.19                              & --                                & --                                & 0.01     {\cellcolor{blue}}                                                                                           & 4.79E-03                              & 0.13    {\cellcolor{cyan}}                                                                                        & 0.18                              & 0.36   {\cellcolor{pink}}                                                                                             & 0.21                              & 0.22  {\cellcolor{pink}}                                                                                              & 0.58                              & 1.36        {\cellcolor{pink}}                                                                                        & 0.50                              & 0.23      {\cellcolor{pink}}                                                                                          & 0.81                               \\
\textbf{Science}    & 0.35  {\cellcolor{pink}}                                                                                              & 0.21                              & 0.41       {\cellcolor{red}}                                                                                                                                                          & 0.00                              & 0.03   {\cellcolor{red}}                                                                                                                                                              & 0.02                              & 0.37     {\cellcolor{red}}                                                                                                                                                            & 0.79                              & 0.37        {\cellcolor{pink}}                                                                                        & 0.20                              & 0.16     {\cellcolor{cyan}}                                                                                       & 0.09                              & 2.05     {\cellcolor{red}}                                                                                                                                                            & 1.16                              & 0.23      {\cellcolor{pink}}                                                                                          & 0.64                               \\
\textbf{Shopping}   & 0.37   {\cellcolor{pink}}                                                                                             & 0.20                              & 0.03            {\cellcolor{blue}}                                                                                    & 0.00                              & 1.10    {\cellcolor{red}}                                                                                                                                                             & 0.00                              & 0.15   {\cellcolor{cyan}}                                                                                         & 0.08                              & 0.31  {\cellcolor{cyan}}                                                                                          & 0.23                              & 0.19    {\cellcolor{pink}}                                                                                            & 0.35                              & 1.77   {\cellcolor{pink}}                                                                                             & 1.31                              & 0.22    {\cellcolor{pink}}                                                                                            & 0.62                               \\
\textbf{Society}    & 0.37    {\cellcolor{pink}}                                                                                            & 0.20                              & 0.05         {\cellcolor{red}}                                                                                                                                                        & 0.00                              & 0.01     {\cellcolor{blue}}                                                                                           & 3.97E-03                             & 0.12    {\cellcolor{cyan}}                                                                                        & 0.08                              & 0.37    {\cellcolor{pink}}                                                                                            & 0.20                              & 0.24     {\cellcolor{pink}}                                                                                           & 1.10                              & 1.83     {\cellcolor{pink}}                                                                                           & 1.28                              & 0.16    {\cellcolor{cyan}}                                                                                        & 0.13                               \\
\textbf{Sports}     & 0.37   {\cellcolor{pink}}                                                                                             & 0.20                              & 0.05           {\cellcolor{blue}}                                                                                     & 0.00                              & 0.02  {\cellcolor{pink}}                                                                                              & 0.00                              & 0.18  {\cellcolor{pink}}                                                                                              & 0.30                              & 0.33  {\cellcolor{pink}}                                                                                              & 0.22                              & 0.18   {\cellcolor{pink}}                                                                                             & 0.15                              & 1.51  {\cellcolor{pink}}                                                                                              & 1.00                              & 0.19    {\cellcolor{pink}}                                                                                            & 0.58                               \\
\midrule
\textbf{Control}    & 0.33                              & 0.22                              & 0.05                              & 3.00E-03                              & 0.02                              & 4.00E-03                              & 0.16                              & 0.08                              & 0.32                              & 0.22                              & 0.18                              & 0.16                              & 0.88                              & 1.18                              & 0.17                              & 0.18                 \\
\bottomrule             
\end{tabular}
\label{table:in_test_not_in_train_cmps}
\end{table*}








\begin{table}[htb!]
\centering

\caption{\textcolor{blue}{Ad bidding under CCPA and GDPR from advertisers who did not bid or appear when we simulated personas but appeared and bid after we opted opt-out under of processing and selling of data in NAI. Avg. column represents the average of each advertiser's median bid value. Std. represents the standard deviation of each advertiser's median bid value. Color \textcolor{pink}{pink} and \textcolor{cyan}{cyan} indicate bid values that are higher and lower than Control's avg., respectively. Color \textcolor{red}{red} and \textcolor{blue}{blue} indicate bid values that are Control's avg. $\pm$ std., respectively. --- represents the absence of bids.}}





    \begin{tabular}{l?{0.3mm}ll?{0.3mm}ll} 
    \toprule

    & \multicolumn{2}{c?{0.3mm}}{\textbf{GDPR}} & \multicolumn{2}{c}{\textbf{CCPA}} \\ 
    


    \multicolumn{1}{c?{0.3mm}}{}  & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}} &  \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c}{\textbf{Std.}}  \\ 
    \toprule
    
\textbf{Adult}      & 1.42E-03  {\cellcolor{red}}                                                                                                                                                                                                     & 0.01                                       & 2.26E-03                                           {\cellcolor{cyan}}                                                                                        & 0.01                                        \\
\textbf{Arts}       & 0.00                                           & 0.00                                       & 1.25E-03                                           {\cellcolor{cyan}}                                                                                        & 0.01                                        \\
\textbf{Business}   & 0.00                                           & 0.00                                       & 0.00                                           {\cellcolor{cyan}}                                                                                        & 0.00                                        \\
\textbf{Computers}  & 4.09E-03                                          {\cellcolor{red}}                                                                                                                                                             & 0.03                                       & 0.00                                           {\cellcolor{cyan}}                                                                                        & 0.00                                        \\
\textbf{Games}      & 0.00                                           & 0.00                                       & 0.00                                           {\cellcolor{cyan}}                                                                                        & 0.00                                        \\
\textbf{Health}     & 1.00E-03   {\cellcolor{red}}                                                                                                                                                                                                    & 4.36E-03                                       & 0.01                                           {\cellcolor{cyan}}                                                                                        & 0.05                                        \\
\textbf{Home}       & 0.00                                           & 0.00                                       & 0.00                                           {\cellcolor{cyan}}                                                                                        & 0.00                                        \\
\textbf{Kids}       & 0.00                                           & 0.00                                       & 0.00                                           {\cellcolor{cyan}}                                                                                        & 0.00                                        \\
\textbf{News}       & 0.00                                           & 0.00                                       & 1.92E-03                                           {\cellcolor{cyan}}                                                                                        & 0.01                                        \\
\textbf{Recreation} & 0.00                                           & 0.00                                       & 2.26E-03                                           {\cellcolor{cyan}}                                                                                        & 0.01                                        \\
\textbf{Reference}  & 1.37E-03   {\cellcolor{red}}                                                                                                                                                                                                    & 0.01                                       & 3.97E-03                                           {\cellcolor{cyan}}                                                                                        & 0.01                                        \\
\textbf{Regional}   & 0.00                                           & 0.00                                       & 0.03                                           {\cellcolor{cyan}}                                                                                        & 0.12                                        \\
\textbf{Science}    & 0.00                                           & 0.00                                       & 0.00                                           {\cellcolor{cyan}}                                                                                        & 0.00                                        \\
\textbf{Shopping}   & 0.00                                           & 0.00                                       & 0.00                                           {\cellcolor{cyan}}                                                                                        & 0.00                                        \\
\textbf{Society}    & 0.00                                           & 0.00                                       & 0.00                                           {\cellcolor{cyan}}                                                                                        & 0.00                                        \\
\textbf{Sports}     & 0.00                                           & 0.00                                       & 3.47E-03                                           {\cellcolor{cyan}}                                                                                        & 0.02                                        \\
\midrule
\textbf{Control}    & 0.00                                           & 0.00                                       & 0.07                                           & 0.15       \\                                

\bottomrule             
\end{tabular}
\label{table:in_test_not_in_train_nai}
\end{table}

==> docs/bids-table-germany-new-interval.tex <==
\begin{table*}
\footnotesize
%\adjustbox{max width=\textwidth}{
    \centering
    \caption{Ad bidding under GDPR in Germany after 1 month since training and opt-out/opt-in. Avg. column represents the mean of all bid value. Std. represents the standard deviation of all bid value. Opt-out and opt-in represent the bids when we opt-out and opt-in the selling of user data, respectively.  \textcolor{highbids}{Light red} and \textcolor{lowbids}{Light blue} indicate bid values that are higher and lower than Control's avg., respectively. \textcolor{higherbids}{Dark red} and \textcolor{lowerbids}{Dark blue} indicate bid values that are Control's avg. $\pm$ std., respectively. }    \begin{tabular}{l?{0.3mm}ll|ll?{0.3mm}ll|ll?{0.3mm}ll|ll?{0.3mm}ll|ll} 
    \toprule
     & \multicolumn{4}{c?{0.3mm}}{\textbf{Cookiebot}} & \multicolumn{4}{c?{0.3mm}}{\textbf{Didomi}}& \multicolumn{4}{c?{0.3mm}}{\textbf{Onetrust}}& \multicolumn{4}{c}{\textbf{Quantcast}}      \\ 
     & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c?{0.3mm}}{\textbf{Opt-in}}     & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c?{0.3mm}}{\textbf{Opt-in}}    & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c?{0.3mm}}{\textbf{Opt-in}}& \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c}{\textbf{Opt-in}}     \\ 
    \textbf{Persona}     & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}}  & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}}&  \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c}{\textbf{Std.}} \\ 
    \toprule



\textbf{Adult}      & 0.44  & 0.22 & 0.37  {\cellcolor{lowbids}}                                                                & 0.25 & 0.33  & 0.00 & 0.12  {\cellcolor{lowbids}}                                                                & 0.29 & 0.03{\cellcolor{lowerbids}}                                                                      & 0.02 & 0.36 {\cellcolor{higherbids}}                                                                                                                                      & 0.96     & 0.14 {\cellcolor{lowbids}}                                                                   & 0.13 & 0.15                                                                 & 0.49  \\

\textbf{Arts}       & 0.45 {\cellcolor{highbids}}                                                                     & 0.21 & 3.32{\cellcolor{higherbids}}                                                                                                                                       & 5.49 & --       & --   & 0.15 {\cellcolor{highbids}}                                                                   & 0.34 & 0.03 {\cellcolor{lowerbids}}                                                                     & 0.00 & 0.07  {\cellcolor{highbids}}                                                                  & 0.04     & 0.18  {\cellcolor{highbids}}                                                                    & 0.63 & 0.20 {\cellcolor{highbids}}                                                                   & 0.76  \\

\textbf{Business}   & 0.44  & 0.18 & 0.25{\cellcolor{lowbids}}                                                                  & 0.26 & 0.08     & 0.07 & 0.13  {\cellcolor{lowbids}}                                                                & 0.32 & 0.02 {\cellcolor{lowerbids}}                                                                     & 0.00 & 0.13 {\cellcolor{higherbids}}                                                                                                                                      & 0.23     & 0.15        & 0.13 & 0.15          & 0.40  \\

\textbf{Computers}  & 0.50 {\cellcolor{highbids}}                                                                     & 0.08 & 0.46 {\cellcolor{highbids}}                                                                   & 0.17 & 0.18     & 0.00 & 0.14 & 0.23 & 0.03  {\cellcolor{lowerbids}}                                                                    & 0.03 & 0.03  {\cellcolor{lowbids}}                                                                & 4.90E-03 & 0.16{\cellcolor{highbids}}                                                                      & 0.14 & 0.16 {\cellcolor{highbids}}                                                                   & 0.33  \\

\textbf{Games}      & 0.35  {\cellcolor{lowbids}}                                                                  & 0.26 & 0.50 {\cellcolor{highbids}}                                                                   & 0.08 & --       & --   & 0.17  {\cellcolor{highbids}}                                                                  & 0.62 & 0.15 {\cellcolor{lowbids}}                                                                  & 0.24 & 0.07 {\cellcolor{highbids}}                                                                   & 0.08     & 0.15                                                                 & 0.14 & 0.14  {\cellcolor{lowbids}}                                                                & 0.44  \\

\textbf{Health}     & 0.54  {\cellcolor{highbids}}                                                                    & 0.00 & 0.36 {\cellcolor{lowbids}}                                                                 & 0.24 & 0.03     & 0.00 & 0.12 {\cellcolor{lowbids}}                                                                 & 0.23 & 0.06  {\cellcolor{lowbids}}                                                                 & 0.04 & 0.07 {\cellcolor{highbids}}                                                                   & 0.04     & 0.13  {\cellcolor{lowbids}}                                                                  & 0.13 & 0.12  {\cellcolor{lowbids}}                                                                & 0.22  \\

\textbf{Home}       & 0.36  {\cellcolor{lowbids}}                                                                  & 0.26 & 1.18 {\cellcolor{higherbids}}                                                                                                                                      & 2.34 & 0.03     & 0.00 & 0.15 {\cellcolor{highbids}}                                                                   & 0.33 & 0.12  {\cellcolor{lowbids}}                                                                 & 0.09 & 0.05  {\cellcolor{lowbids}}                                                                & 0.02     & 0.14  {\cellcolor{lowbids}}                                                                  & 0.13 & 0.16 {\cellcolor{highbids}}                                                                   & 0.55  \\

\textbf{Kids}       & 0.54  {\cellcolor{highbids}}                                                                    & 0.00 & 0.57 {\cellcolor{highbids}}                                                                   & 0.15 & 0.04     & 0.02 & 0.14                                                                  & 0.19 & 0.08  {\cellcolor{lowbids}}                                                                 & 0.03 & 0.10 {\cellcolor{highbids}}                                                                   & 0.17     & 0.15                                                                     & 0.14 & 0.17{\cellcolor{highbids}}                                                                    & 0.27  \\

\textbf{News}       & 0.44   & 0.22 & 0.34 {\cellcolor{lowbids}}                                                                 & 0.25 & --       & --   & 0.18  {\cellcolor{highbids}}                                                                  & 0.40 & 0.21  {\cellcolor{lowbids}}                                                                 & 0.28 & 0.07 {\cellcolor{highbids}}                                                                   & 0.04     & 0.14 {\cellcolor{lowbids}}                                                                   & 0.11 & 0.15                                                             & 0.44  \\

\textbf{Recreation} & 0.31  {\cellcolor{lowbids}}                                                                  & 0.27 & 0.39 {\cellcolor{lowbids}}                                                                 & 0.22 & --       & --   & 0.14                                                                  & 0.32 & 0.11  {\cellcolor{lowbids}}                                                                 & 0.14 & 0.14 {\cellcolor{higherbids}}                                                                                                                                      & 0.22     & 0.15                                                                   & 0.13 & 0.14 {\cellcolor{lowbids}}                                                                 & 0.49  \\

\textbf{Reference}  & 0.54  {\cellcolor{highbids}}                                                                    & 0.00 & 0.54 {\cellcolor{highbids}}                                                                   & 0.00 & --       & --   & 0.14                                                                   & 0.28 & 0.23  {\cellcolor{lowbids}}                                                                 & 0.19 & 0.12 {\cellcolor{higherbids}}                                                                                                                                      & 0.16     & 0.16{\cellcolor{highbids}}                                                                      & 0.18 & 0.13   {\cellcolor{lowbids}}                                                               & 0.24  \\

\textbf{Regional}   & 0.37  {\cellcolor{lowbids}}                                                                  & 0.24 & 0.49{\cellcolor{highbids}}                                                                    & 0.16 & --       & --   & 0.16 {\cellcolor{highbids}}                                                                   & 0.37 & 0.06  {\cellcolor{lowbids}}                                                                 & 0.05 & 0.07  {\cellcolor{highbids}}                                                                  & 0.04     & 0.15   & 0.12 & 0.16 {\cellcolor{highbids}}                                                                   & 0.20  \\

\textbf{Science}    & 0.42 {\cellcolor{lowbids}}                                                                   & 0.21 & 0.28 {\cellcolor{lowbids}}                                                                 & 0.26 & --       & --   & 0.21 {\cellcolor{highbids}}                                                                   & 0.44 & 0.06   {\cellcolor{lowbids}}                                                                & 0.06 & 0.07 {\cellcolor{highbids}}                                                                   & 0.07     & 0.14  {\cellcolor{lowbids}}                                                                  & 0.12 & 0.14{\cellcolor{lowbids}}                                                                  & 0.46  \\

\textbf{Shopping}   & 0.50   {\cellcolor{highbids}}                                                                   & 0.08 & 0.36  {\cellcolor{lowbids}}                                                                & 0.26 & 0.14     & 0.00 & 0.18 {\cellcolor{highbids}}                                                                   & 0.49 & 0.08  {\cellcolor{lowbids}}                                                                 & 0.06 & 0.83 {\cellcolor{higherbids}}                                                                                                                                      & 0.97     & 0.14  {\cellcolor{lowbids}}                                                                  & 0.13 & 0.16  {\cellcolor{highbids}}                                                                  & 0.33  \\

\textbf{Society}    & 0.14  {\cellcolor{lowerbids}}                                                                     & 0.24 & 0.16 {\cellcolor{lowerbids}}                                                                    & 0.25 & 0.20     & 0.17 & 0.19  {\cellcolor{highbids}}                                                                  & 0.48 & 0.03 {\cellcolor{lowerbids}}                                                                     & 0.04 & 0.08{\cellcolor{highbids}}                                                                    & 0.20     & 0.16  {\cellcolor{highbids}}                                                                    & 0.07 & 0.15  & 0.12  \\

\textbf{Sports}     & 0.48{\cellcolor{highbids}}                                                                      & 0.17 & 0.35  {\cellcolor{lowbids}}                                                                & 0.23 & --       & --   & 0.13   {\cellcolor{lowbids}}                                                               & 0.25 & 0.06  {\cellcolor{lowbids}}                                                                 & 0.04 & 0.13 {\cellcolor{higherbids}}                                                                                                                                      & 0.20     & 0.17 {\cellcolor{highbids}}                                                                     & 0.14 & 0.17 {\cellcolor{highbids}}                                                                   & 0.26  \\

\midrule
\textbf{Control}    & 0.44      & 0.22 & 0.41    & 0.21 & --       & --   & 0.14    & 0.25 & 0.44     & 0.40 & 0.06    & 0.06     & 0.15      & 0.12 & 0.15    & 0.31  \\



    \bottomrule

\end{tabular}

\label{table:GDPR-bidding-mean-interval}
\end{table*}

==> docs/bids-table-germany-new.tex <==
\begin{table*}
\footnotesize
% \adjustbox{width=\textwidth}{
    \centering
    \caption{Ad bidding across CMPs under GDPR in Germany. Avg. column represents the mean of all bid value. Std. represents the standard deviation of all bid value. Opt-out and opt-in represent the bids when we opt-out and opt-in the selling of user data, respectively. \textcolor{highbids}{Light red} and \textcolor{lowbids}{light blue} indicate bid values that are higher and lower than Control's avg., respectively. \textcolor{higherbids}{Dark red} and \textcolor{lowerbids}{dark blue} indicate bid values that are Control's avg. $\pm$ std., respectively. --- represents the absence of bids.\hl{the ordering should be Didomi, Quantcast, OneTrust, Cookiebot.} \hl{Also, why do we have 0 values in the table for standard deviation? If the value is 0, just mention 0 -- I am not sure what 0.00 conveys. If the value is smaller use the scientific notation. This goes for all tables.} \hl{A lot of same values are at times red and other times blue. Please include another digit after the decimal.}}
    \begin{tabular}{l?{0.3mm}ll|ll?{0.3mm}ll|ll?{0.3mm}ll|ll?{0.3mm}ll|ll} 
    \toprule
     & \multicolumn{4}{c?{0.3mm}}{\textbf{Cookiebot}} & \multicolumn{4}{c?{0.3mm}}{\textbf{Didomi}}& \multicolumn{4}{c?{0.3mm}}{\textbf{Onetrust}}& \multicolumn{4}{c}{\textbf{Quantcast}}      \\ 
     & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c?{0.3mm}}{\textbf{Opt-in}}     & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c?{0.3mm}}{\textbf{Opt-in}}    & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c?{0.3mm}}{\textbf{Opt-in}}& \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c}{\textbf{Opt-in}}     \\ 
    \textbf{Persona}     & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}}  & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}}&  \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c}{\textbf{Std.}} \\ 
    \toprule


\textbf{Adult}      & 0.37    {\cellcolor{highbids}}                                                                 & 0.20                              & 0.33    {\cellcolor{highbids}}                                                                 & 0.21                              & --     & --                                & 0.11     {\cellcolor{lowbids}}                                                               & 0.17                              & 0.02      {\cellcolor{lowbids}}                                                               & 4E-3                             & 0.01        {\cellcolor{lowerbids}}                                                                  & 0.00                              & 0.22      {\cellcolor{highbids}}                                                               & 0.82                              & 0.15    {\cellcolor{lowbids}}                                                               & 0.15                               \\
\textbf{Arts}       & 0.35      {\cellcolor{highbids}}                                                               & 0.21                              & 0.32       {\cellcolor{highbids}}                                                              & 0.22                              & 0.05      {\cellcolor{lowbids}}                                                               & 0.00                              & 0.16  {\cellcolor{highbids}}                                                                   & 0.29                              & --  & --          & 0.04     {\cellcolor{higherbids}}                                                                                                                                    & 0.04                              & 0.22 {\cellcolor{highbids}}                                                                    & 1.03                              & 0.14    {\cellcolor{lowbids}}                                                               & 0.14                               \\
\textbf{Business}   & 0.35      {\cellcolor{highbids}}                                                               & 0.21                              & 0.35      {\cellcolor{highbids}}                                                               & 0.21                              & --   & --                                & 0.11  {\cellcolor{lowbids}}                                                               & 0.17                              & 0.01   {\cellcolor{lowerbids}}                                                                  & 0.01                              & 0.06  {\cellcolor{higherbids}}                                                                                                                                    & 0.06                              & 0.19  {\cellcolor{highbids}}                                                                   & 0.82                              & 0.15 {\cellcolor{lowbids}}                                                                                                                                  & 0.12                               \\
\textbf{Computers}  & 0.35     {\cellcolor{highbids}}                                                                & 0.21                              & 0.36  {\cellcolor{highbids}}                                                                   & 0.24                              & 0.05 {\cellcolor{highbids}}                                                                     & 4E-3                              & 0.11  {\cellcolor{lowbids}}                                                               & 0.16                              & 0.02 {\cellcolor{lowbids}}                                                               & 0.01                              & 0.01   {\cellcolor{lowerbids}}                                                                  & 4E-3                              & 0.28  {\cellcolor{higherbids}}                                                                                                                                    & 0.97                              & 0.16  {\cellcolor{highbids}}                                                                   & 0.17                               \\
\textbf{Games}      & 0.38    {\cellcolor{highbids}}                                                                 & 0.20                              & 0.38 {\cellcolor{highbids}}                                                                    & 0.22                              & 0.03   {\cellcolor{lowerbids}}                                                                  & 0.02                              & 0.12   {\cellcolor{highbids}}                                                                  & 0.21                              & 0.02  {\cellcolor{highbids}}                                                                   & 0.00                              & 0.03  {\cellcolor{higherbids}}                                                                                                                                    & 0.02                              & 0.43  {\cellcolor{higherbids}}                                                                                                                                    & 1.36                              & 0.14  {\cellcolor{lowbids}}                                                               & 0.14                               \\
\textbf{Health}     & 0.35    {\cellcolor{highbids}}                                                                 & 0.21                              & 0.34   {\cellcolor{highbids}}                                                                  & 0.22                              & --  & --                                & 0.11   {\cellcolor{lowbids}}                                                               & 0.19                              & 0.03   {\cellcolor{higherbids}}                                                                                                                                    & 0.02                              & 0.15  {\cellcolor{higherbids}}                                                                                                                                    & 0.08                              & 0.41 {\cellcolor{higherbids}}                                                                                                                                    & 1.31                              & 0.15  {\cellcolor{lowbids}}                                                               & 0.14                               \\
\textbf{Home}       & 0.38     {\cellcolor{highbids}}                                                                & 0.20                              & 0.31   {\cellcolor{highbids}}                                                                  & 0.22                              & 0.05  {\cellcolor{lowerbids}}                                                                  & 0.00                              & 0.12    {\cellcolor{highbids}}                                                                 & 0.27                              & 0.31   {\cellcolor{higherbids}}                                                                                                                                    & 0.25                              & 0.05   {\cellcolor{higherbids}}                                                                                                                                    & 0.04                              & 0.23   {\cellcolor{highbids}}                                                                  & 0.93                              & 0.14   {\cellcolor{lowbids}}                                                               & 0.14                               \\
\textbf{Kids}       & 0.37       {\cellcolor{highbids}}                                                              & 0.20                              & 0.34   {\cellcolor{highbids}}                                                                  & 0.21                              & 0.06  {\cellcolor{higherbids}}                                                                                                                                    & 0.00                              & 0.14  {\cellcolor{highbids}}                                                                   & 0.19                              & 0.01  {\cellcolor{lowerbids}}                                                                  & 0.00                              & 0.02   {\cellcolor{lowerbids}}                                                                  & 0.00                              & 0.30  {\cellcolor{higherbids}}                                                                                                                                    & 0.96                              & 0.14  {\cellcolor{lowbids}}                                                               & 0.12                               \\
\textbf{News}       & 0.35    {\cellcolor{highbids}}                                                                 & 0.21                              & 0.39   {\cellcolor{highbids}}                                                                  & 0.26                              & --     & --                                & 0.09    {\cellcolor{lowbids}}                                                               & 0.17                              & 0.03  {\cellcolor{higherbids}}                                                                                                                                    & 0.02                              & 0.46  {\cellcolor{higherbids}}                                                                                                                                    & 0.30                              & 0.22   {\cellcolor{highbids}}                                                                  & 0.79                              & 0.14  {\cellcolor{lowbids}}                                                               & 0.15                               \\
\textbf{Recreation} & 0.37     {\cellcolor{highbids}}                                                                & 0.20                              & 0.35    {\cellcolor{highbids}}                                                                 & 0.21                              & 0.06   {\cellcolor{higherbids}}                                                                                                                                    & 0.00                              & 0.11   {\cellcolor{lowbids}}                                                               & 0.21                              & 0.02   {\cellcolor{higherbids}}                                                                                                                                    & 0.01                              & 0.14   {\cellcolor{higherbids}}                                                                                                                                    & 0.03                              & 0.31   {\cellcolor{higherbids}}                                                                                                                                    & 1.38                              & 0.15   {\cellcolor{lowbids}}                                                               & 0.13                               \\
\textbf{Reference}  & 0.37      {\cellcolor{highbids}}                                                               & 0.20                              & 0.33  {\cellcolor{highbids}}                                                                   & 0.22                              & --       & --                                & 0.13    {\cellcolor{highbids}}                                                                 & 0.26                              & 0.03   {\cellcolor{higherbids}}                                                                                                                                    & 0.01                              & 0.20   {\cellcolor{higherbids}}                                                                                                                                    & 0.26                              & 0.26   {\cellcolor{higherbids}}                                                                                                                                    & 1.20                              & 0.14    {\cellcolor{lowbids}}                                                               & 0.16                               \\
\textbf{Regional}   & 0.38       {\cellcolor{highbids}}                                                              & 0.19                              & 0.34   {\cellcolor{highbids}}                                                                  & 0.22                              & --        & --                                & 0.13      {\cellcolor{highbids}}                                                               & 0.19                              & 0.01     {\cellcolor{lowerbids}}                                                                  & 4E-3                              & 0.02    {\cellcolor{lowerbids}}                                                                  & 4E-3                              & 0.27    {\cellcolor{higherbids}}                                                                                                                                    & 1.23                              & 0.16    {\cellcolor{highbids}}                                                                 & 0.18                               \\
\textbf{Science}    & 0.35        {\cellcolor{highbids}}                                                             & 0.21                              & 0.39     {\cellcolor{highbids}}                                                                & 0.23                              & 0.41    {\cellcolor{higherbids}}                                                                                                                                    & 0.00                              & 0.12    {\cellcolor{highbids}}                                                                 & 0.24                              & 0.03    {\cellcolor{higherbids}}                                                                                                                                    & 0.02                              & 0.09   {\cellcolor{higherbids}}                                                                                                                                    & 0.05                              & 0.36   {\cellcolor{higherbids}}                                                                                                                                    & 1.17                              & 0.15   {\cellcolor{lowbids}}                                                               & 0.19                               \\
\textbf{Shopping}   & 0.37      {\cellcolor{highbids}}                                                               & 0.20                              & 0.35    {\cellcolor{highbids}}                                                                 & 0.22                              & 0.03   {\cellcolor{lowerbids}}                                                                  & 0.00                              & 0.10   {\cellcolor{lowbids}}                                                               & 0.21                              & 1.10   {\cellcolor{higherbids}}                                                                                                                                    & 0.00                              & 0.13    {\cellcolor{higherbids}}                                                                                                                                    & 0.00                              & 0.18     {\cellcolor{highbids}}                                                                & 0.74                              & 0.12     {\cellcolor{lowbids}}                                                               & 0.14                               \\
\textbf{Society}    & 0.37           {\cellcolor{highbids}}                                                          & 0.20                              & 0.37   {\cellcolor{highbids}}                                                                  & 0.22                              & 0.05   {\cellcolor{higherbids}}                                                                                                                                    & 0.00                              & 0.12   {\cellcolor{highbids}}                                                                  & 0.23                              & 0.01    {\cellcolor{lowerbids}}                                                                  & 3E-3                              & 0.02    {\cellcolor{lowerbids}}                                                                  & 3E-3                              & 0.30  {\cellcolor{higherbids}}                                                                                                                                    & 1.00                              & 0.16   {\cellcolor{highbids}}                                                                  & 0.18                               \\
\textbf{Sports}     & 0.37         {\cellcolor{highbids}}                                                            & 0.20                              & 0.35     {\cellcolor{highbids}}                                                                & 0.22                              & 0.05    {\cellcolor{lowerbids}}                                                                  & 0.00                              & 0.13    {\cellcolor{highbids}}                                                                 & 0.23                              & 0.01    {\cellcolor{lowerbids}}                                                                  & 3E-3                              & 0.11   {\cellcolor{higherbids}}                                                                                                                                    & 0.09                              & 0.21    {\cellcolor{highbids}}                                                                 & 0.82                              & 0.16    {\cellcolor{highbids}}                                                                 & 0.20                               \\
\midrule
\textbf{Control}    & 0.33                                                                  & 0.22                              & 0.26     & 0.24                              & 0.05     & 3E-3                              & 0.11     & 0.31                              & 0.02    & 4E-3                              & 0.02    & 0.00                              & 0.16   & 0.08                              & 0.15    & 0.11        \\                       




    \bottomrule

\end{tabular}
% }
\label{table:GDPR-bidding-mean}
\end{table*}

==> docs/bids-table-germany.tex <==
\begin{table*}
%\adjustbox{max width=\textwidth}{
    \centering
    \caption{Ad bidding under GDPR in Germany. Avg. column represents the mean of all bid value. Std. represents the standard deviation of all bid value. Opt-out and opt-in represent the bids when we opt-out and opt-in the selling of user data, respectively.  $\uparrow$ and $\downarrow$ indicate bid values that are higher and lower than Control's avg., respectively. $\textcolor{red}{\uparrow}$ and $\textcolor{red}{\downarrow}$ indicate bid values that are Control's avg. $\pm$ std., respectively. --- represents the absence of bids.}
    \begin{tabular}{l?{0.3mm}rr|rr?{0.3mm}rr|rr?{0.3mm}rr|rr} 
    \toprule
     & \multicolumn{4}{c?{0.3mm}}{\textbf{OneTrust}} & \multicolumn{4}{c?{0.3mm}}{\textbf{CookieBot}}& \multicolumn{4}{c}{\textbf{NAI}}    \\ 
     & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c?{0.3mm}}{\textbf{Opt-in}}     & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c?{0.3mm}}{\textbf{Opt-in}}    & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c}{\textbf{Opt-in}}   \\ 
    \textbf{Persona}     & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}}  & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c}{\textbf{Std.}}  \\ 
    \toprule


\textbf{Adult}      & 0.25$^{\textcolor{red}{\uparrow}}$                      & 0.60                     & 1.02$^{\textcolor{red}{\uparrow}}$                      & 2.53                      & 0.02$^{\textcolor{red}{\uparrow}}$                      & 0.03                     & 0.01$^{\uparrow}$                      & 0.02                                          & 0.07$^{\downarrow}$                      & 0.07                     & 0.10$^{\uparrow}$                      & 0.08                      \\ 

\textbf{Arts}       & 0.39$^{\textcolor{red}{\uparrow}}$                      & 0.41                     & 0.65$^{\textcolor{red}{\uparrow}}$                      & 1.54                      & 0.08$^{\textcolor{red}{\uparrow}}$                      & 0.08                     & 0.08$^{\textcolor{red}{\uparrow}}$                      & 0.09                      & 0.06$^{\downarrow}$                      & 0.07                     & 0.07$^{\downarrow}$                      & 0.13                      \\ 

\textbf{Business}   & 0.03$^{\downarrow}$                       & 0.04                     & 0.33$^{\uparrow}$                      & 0.79                                          & 0.01$^{\textcolor{red}{\uparrow}}$                      & 0.02                     & 0.02$^{\textcolor{red}{\uparrow}}$                      & 0.05                                          & 1.80$^{\textcolor{red}{\uparrow}}$                      & 2.15                     & 0.30$^{\textcolor{red}{\uparrow}}$                      & 0.65                      \\ 

\textbf{Computers}  & 0.09$^{\uparrow}$                     & 0.11                     & 0.80$^{\textcolor{red}{\uparrow}}$                     & 2.07                                          & 0.16$^{\textcolor{red}{\uparrow}}$                     & 0.05                     & 0.17$^{\textcolor{red}{\uparrow}}$                     & 0.04                                          & 0.21$^{\uparrow}$                     & 1.06                     & 0.54$^{\textcolor{red}{\uparrow}}$                     & 1.56                      \\ 

\textbf{Games}      & 0.16$^{\textcolor{red}{\uparrow}}$                     & 0.01                     & 1.6E-5$^{\downarrow}$                      & 0.00                     & 3E-3$^{\textcolor{red}{\uparrow}}$                     & 0.01                     & 1.3E-5$^{\downarrow}$                      & 1.7E-21                      & 0.09$^{\downarrow}$                      & 0.12                     & 0.12$^{\uparrow}$                     & 0.19                      \\ 

\textbf{Health}     & 0.74$^{\textcolor{red}{\uparrow}}$                      & 1.11                     & --& --& 0.06$^{\textcolor{red}{\uparrow}}$                      & 0.15                     & 0.03$^{\textcolor{red}{\uparrow}}$                      & 0.05                                          & 0.04$^{\downarrow}$                      & 0.05                     & 0.05$^{\downarrow}$                      & 0.10                      \\ 

\textbf{Home}       & 0.13$^{\uparrow}$                      & 0.16                     & 0.43$^{\textcolor{red}{\uparrow}}$                      & 0.71                      & 1.00$^{\textcolor{red}{\uparrow}}$                      & 1.37                     & 0.97$^{\textcolor{red}{\uparrow}}$                      & 1.27                                         & 1.18$^{\textcolor{red}{\uparrow}}$                      & 2.38                     & 0.60$^{\textcolor{red}{\uparrow}}$                      & 1.64                      \\ 

\textbf{Kids}       & 0.05$^{\uparrow}$                      & 0.11                     & 0.16$^{\uparrow}$                      & 0.18                                          & 0.15$^{\textcolor{red}{\uparrow}}$                      & 0.04                     & 0.25$^{\textcolor{red}{\uparrow}}$                      & 0.19                                          & 0.23$^{\textcolor{red}{\uparrow}}$                      & 0.92                     & 0.37$^{\textcolor{red}{\uparrow}}$                      & 1.14                      \\ 

\textbf{News}       & 0.12$^{\uparrow}$                     & 0.14                     & 0.86$^{\textcolor{red}{\uparrow}}$                     & 1.66                                          & 0.17$^{\textcolor{red}{\uparrow}}$                     & 0.03                     & 0.17$^{\textcolor{red}{\uparrow}}$                     & 0.03                                          & 0.06$^{\downarrow}$                      & 0.12                     & 0.04$^{\downarrow}$                      & 0.05                      \\ 

\textbf{Recreation} & 0.10$^{\uparrow}$                     & 0.17                     & 0.41$^{\textcolor{red}{\uparrow}}$                     & 0.74                                          & 0.02$^{\textcolor{red}{\uparrow}}$                     & 0.03                     & 7.3E-4$^{\downarrow}$                     & 7.2E-4                     &  0.07$^{\downarrow}$                     & 0.11                     & 0.17$^{\uparrow}$                     & 0.39                      \\ 

\textbf{Reference}  & 0.04$^{\downarrow}$                     & 0.04                     & 0.17$^{\uparrow}$                      & 0.22                     &  0.18$^{\textcolor{red}{\uparrow}}$                      & 0.05                     & 0.17$^{\textcolor{red}{\uparrow}}$                      & 0.04                     & 0.06$^{\downarrow}$                     & 0.09                     & 0.04$^{\downarrow}$                     & 0.06                      \\ 

\textbf{Regional}   & 0.02$^{\downarrow}$                      & 0.03                     & 0.71$^{\textcolor{red}{\uparrow}}$                      & 1.29                                         & 0.09$^{\textcolor{red}{\uparrow}}$                      & 0.08                     & 0.09$^{\textcolor{red}{\uparrow}}$                      & 0.09                                          & 0.13$^{\uparrow}$                     & 0.20                     & 0.10$^{\uparrow}$                  & 0.06                      \\ 

\textbf{Science}    & 0.09$^{\uparrow}$                     & 0.11                     & 0.11$^{\downarrow}$                     & 0.12                                          & 0.01$^{\textcolor{red}{\uparrow}}$                     & 0.03                     & 3.3E-3$^{\downarrow}$                     & 0.01                                         & 0.13$^{\uparrow}$                     & 0.08                     & 0.12$^{\uparrow}$                     & 0.06                      \\ 

\textbf{Shopping}   & 0.07$^{\uparrow}$                      & 0.12                     & 0.06$^{\downarrow}$                     & 0.09                     &  0.01$^{\textcolor{red}{\uparrow}}$                      & 0.05                     & 0.02$^{\uparrow}$                      & 0.03                     &  0.15$^{\uparrow}$                      & 0.14                     & 0.10$^{\uparrow}$ 	                     & 0.07                      \\ 

\textbf{Society}    & 0.23$^{\textcolor{red}{\uparrow}}$                      & 0.14                     & 0.49$^{\textcolor{red}{\uparrow}}$                      & 0.55                      & 0.16$^{\textcolor{red}{\uparrow}}$                      & 0.03                     & 0.16$^{\textcolor{red}{\uparrow}}$                      & 0.02                      & 0.10$^{\uparrow}$                      & 0.12                     & 0.10$^{\uparrow}$                      & 0.26                      \\ 

\textbf{Sports}     & 0.09$^{\uparrow}$                      & 0.28                     & 0.68$^{\textcolor{red}{\uparrow}}$                      & 1.77                                          & 0.69$^{\textcolor{red}{\uparrow}}$                      & 0.97                     & 0.11$^{\textcolor{red}{\uparrow}}$                      & 0.07                                         & 0.14$^{\uparrow}$                      & 0.25                     & 0.13$^{\uparrow}$                      & 0.17                      \\ 



\midrule
\textbf{Control}    & 0.04                     & 0.11                     & 0.13                     & 0.20                                         & 5.0E-4 & 1.9E-3                     & 0.01                     & 0.01                      & 0.09                     & 0.12                     & 0.09                     & 0.10                      \\

    \bottomrule

\end{tabular}

\label{table:GDPR-bidding-mean}
\end{table*}

==> docs/combined-bids-appear-after-opt-out.tex <==
\begin{table}
\footnotesize
%\adjustbox{max width=\textwidth}{
    \centering
    

    \caption{Ad bidding under CCPA and GDPR from advertisers who did not bid or appear when we simulated personas but appeared and bid after we opted opt-out under of processing and selling of data in all 4 CMPs. Avg. column represents the average of each advertiser's median bid value. Std. represents the standard deviation of each advertiser's median bid value. \textcolor{highbids}{Light red} and \textcolor{lowbids}{Light blue} indicate bid values that are higher and lower than Control's avg., respectively. \textcolor{higherbids}{Dark red} and \textcolor{lowerbids}{Dark blue} indicate bid values that are Control's avg. $\pm$ std., respectively. }
    \begin{tabular}{l?{0.3mm}ll|ll} 
    \toprule
     & \multicolumn{2}{c?{0.3mm}}{\textbf{GDPR}} &  \multicolumn{2}{c}{\textbf{CCPA}}      \\ 
 
    \textbf{Persona}     & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c}{\textbf{Std.}} \\ 
    \toprule

\textbf{Adult}      & 0.21 {\cellcolor{highbids}}                                     & 0.48 & 0.32 {\cellcolor{highbids}}                                     & 0.51  \\
\textbf{Arts}       & 0.19 {\cellcolor{highbids}}                                     & 0.22 & 0.38 {\cellcolor{highbids}}                                     & 1.28  \\
\textbf{Business}   & 0.17 {\cellcolor{lowbids}}                                     & 0.21 & 0.25 {\cellcolor{highbids}}                                     & 0.49  \\
\textbf{Computers}  & 0.27 {\cellcolor{highbids}}                                     & 0.57 & 0.38 {\cellcolor{highbids}}                                     & 0.80  \\
\textbf{Games}      & 0.38 {\cellcolor{higherbids}}                                     & 0.81 & 0.33 {\cellcolor{highbids}}                                     & 0.65  \\
\textbf{Health}     & 0.20 {\cellcolor{highbids}}                                     & 0.22 & 0.49 {\cellcolor{highbids}}                                     & 0.94  \\
\textbf{Home}       & 0.20 {\cellcolor{highbids}}                                     & 0.21 & 0.31 {\cellcolor{highbids}}                                     & 0.50  \\
\textbf{Kids}       & 0.25 {\cellcolor{highbids}}                                     & 0.49 & 0.32 {\cellcolor{highbids}}                                     & 0.67  \\
\textbf{News}       & 0.21 {\cellcolor{highbids}}                                     & 0.33 & 0.27 {\cellcolor{highbids}}                                     & 0.47  \\
\textbf{Recreation} & 0.21 {\cellcolor{highbids}}                                     & 0.30 & 0.32 {\cellcolor{highbids}}                                      & 0.50  \\
\textbf{Reference}  & 0.21 {\cellcolor{highbids}}                                     & 0.27 & 0.36 {\cellcolor{highbids}}                                     & 0.71  \\
\textbf{Regional}   & 0.17 {\cellcolor{lowbids}}                                     & 0.21 & 0.32 {\cellcolor{highbids}}                                     & 0.71  \\
\textbf{Science}    & 0.33 {\cellcolor{highbids}}                                     & 0.66 & 0.33 {\cellcolor{highbids}}                                     & 0.69  \\
\textbf{Shopping}   & 0.19 {\cellcolor{highbids}}                                     & 0.17 & 0.32 {\cellcolor{highbids}}                                     & 0.71  \\
\textbf{Society}    & 0.17 {\cellcolor{lowbids}}                                     & 0.17 & 0.27 {\cellcolor{highbids}}                                     & 0.69  \\
\textbf{Sports}     & 0.20 {\cellcolor{highbids}}                                     & 0.28 & 0.33 {\cellcolor{highbids}}                                     & 0.67  \\    
    

\midrule
\textbf{Control}    & 0.19 & 0.17 & 0.24 & 0.44         \\            



    \bottomrule

\end{tabular}

%\vspace{-5mm}
\label{table:Opt-out-appear-after-mean}
\end{table}


==> docs/combined-bids.tex <==
\begin{table}
\footnotesize
%\adjustbox{max width=\textwidth}{
    \centering
    \caption{Ad bidding under GDPR in Germany and CCPA in California under Opt-out setting from all 4 CMPs: Cookiebot, Didomi, Onetrust and Quantcast. Avg. column represents the mean of all bid value. Std. represents the standard deviation of all bid value. \textcolor{highbids}{Light red} and \textcolor{lowbids}{Light blue} indicate bid values that are higher and lower than Control's avg., respectively. \textcolor{higherbids}{Dark red} and \textcolor{lowerbids}{Dark blue} indicate bid values that are Control's avg. $\pm$ std., respectively. }
    \begin{tabular}{l?{0.3mm}ll|ll} 
    \toprule
     & \multicolumn{2}{c?{0.3mm}}{\textbf{GDPR}} &  \multicolumn{2}{c}{\textbf{CCPA}}      \\ 
 
    \textbf{Persona}     & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c}{\textbf{Std.}} \\ 
    \toprule
    
    
    
\textbf{Adult}      & 0.29 {\cellcolor{highbids}}                                      & 0.60 & 0.37 {\cellcolor{highbids}}                                      & 0.59  \\
\textbf{Arts}       & 0.29 {\cellcolor{highbids}}                                      & 0.76 & 0.43 {\cellcolor{highbids}}                                      & 1.08  \\
\textbf{Business}   & 0.25 {\cellcolor{lowbids}}                                      & 0.62 & 0.30 {\cellcolor{highbids}}                                      & 0.41  \\
\textbf{Computers}  & 0.31 {\cellcolor{highbids}}                                      & 0.72 & 0.46 {\cellcolor{highbids}}                                      & 1.02  \\
\textbf{Games}      & 0.40 {\cellcolor{highbids}}                                      & 1.02 & 0.33 {\cellcolor{highbids}}                                      & 0.55  \\
\textbf{Health}     & 0.38 {\cellcolor{highbids}}                                      & 0.95 & 0.47 {\cellcolor{highbids}}                                      & 0.79  \\
\textbf{Home}       & 0.30 {\cellcolor{highbids}}                                      & 0.67 & 0.36 {\cellcolor{highbids}}                                      & 0.58  \\
\textbf{Kids}       & 0.32 {\cellcolor{highbids}}                                      & 0.71 & 0.36 {\cellcolor{highbids}}                                      & 0.65  \\
\textbf{News}       & 0.29 {\cellcolor{highbids}}                                      & 0.54 & 0.32 {\cellcolor{highbids}}                                      & 0.50  \\
\textbf{Recreation} & 0.34 {\cellcolor{highbids}}                                      & 0.99 & 0.39 {\cellcolor{highbids}}                                      & 0.60  \\
\textbf{Reference}  & 0.31 {\cellcolor{highbids}}                                      & 0.88 & 0.37 {\cellcolor{highbids}}                                      & 0.61  \\
\textbf{Regional}   & 0.31 {\cellcolor{highbids}}                                      & 0.91 & 0.35 {\cellcolor{highbids}}                                      & 0.60  \\
\textbf{Science}    & 0.35 {\cellcolor{highbids}}                                      & 0.86 & 0.34 {\cellcolor{highbids}}                                      & 0.60  \\
\textbf{Shopping}   & 0.29 {\cellcolor{highbids}}                                      & 0.52 & 0.35 {\cellcolor{highbids}}                                      & 0.64  \\
\textbf{Society}    & 0.32 {\cellcolor{highbids}}                                      & 0.73 & 0.32 {\cellcolor{highbids}}                                      & 0.74  \\
\textbf{Sports}     & 0.28 {\cellcolor{highbids}}                                      & 0.61 & 0.32 {\cellcolor{highbids}}                                      & 0.55  \\
\midrule
\textbf{Control}    & 0.26 & 0.20 & 0.29 & 0.44         \\            



    \bottomrule

\end{tabular}

%\vspace{-5mm}
\label{table:Opt-out-mean}
\end{table}



\begin{table}
\footnotesize
%\adjustbox{max width=\textwidth}{
    \centering
    \caption{Ad bidding under GDPR in Germany and CCPA in California under Opt-in setting from all 4 CMPs: Cookiebot, Didomi, Onetrust and Quantcast. Avg. column represents the mean of all bid value. Std. represents the standard deviation of all bid value. \textcolor{highbids}{Light red} and \textcolor{lowbids}{Light blue} indicate bid values that are higher and lower than Control's avg., respectively. \textcolor{higherbids}{Dark red} and \textcolor{lowerbids}{Dark blue} indicate bid values that are Control's avg. $\pm$ std., respectively. }
    \begin{tabular}{l?{0.3mm}ll|ll} 
    \toprule
     & \multicolumn{2}{c?{0.3mm}}{\textbf{GDPR}} &  \multicolumn{2}{c}{\textbf{CCPA}}      \\ 
 
    \textbf{Persona}     & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c}{\textbf{Std.}} \\ 
    \toprule
    
    
    
\textbf{Adult}      & 0.14 {\cellcolor{highbids}}                                     & 0.19 & 0.22 {\cellcolor{lowbids}}                                     & 0.36  \\
\textbf{Arts}       & 0.18 {\cellcolor{highbids}}                                     & 0.27 & 0.22 {\cellcolor{lowbids}}                                     & 0.50  \\
\textbf{Business}   & 0.14 {\cellcolor{highbids}}                                     & 0.19 & 0.21 {\cellcolor{lowbids}}                                     & 0.40  \\
\textbf{Computers}  & 0.14 {\cellcolor{highbids}}                                     & 0.19 & 0.23 {\cellcolor{highbids}}                                     & 0.92  \\
\textbf{Games}      & 0.15 {\cellcolor{highbids}}                                     & 0.22 & 0.28 {\cellcolor{highbids}}                                     & 0.66  \\
\textbf{Health}     & 0.14 {\cellcolor{highbids}}                                     & 0.20 & 0.28 {\cellcolor{highbids}}                                     & 0.55  \\
\textbf{Home}       & 0.15 {\cellcolor{highbids}}                                     & 0.26 & 0.25 {\cellcolor{highbids}}                                     & 0.58  \\
\textbf{Kids}       & 0.16 {\cellcolor{highbids}}                                     & 0.20 & 0.26 {\cellcolor{highbids}}                                     & 0.62  \\
\textbf{News}       & 0.13 {\cellcolor{lowbids}}                                     & 0.20 & 0.28 {\cellcolor{highbids}}                                     & 0.53  \\
\textbf{Recreation} & 0.14 {\cellcolor{highbids}}                                     & 0.21 & 0.30 {\cellcolor{highbids}}                                     & 0.78  \\
\textbf{Reference}  & 0.15 {\cellcolor{highbids}}                                     & 0.26 & 0.25 {\cellcolor{highbids}}                                     & 0.50  \\
\textbf{Regional}   & 0.16 {\cellcolor{highbids}}                                     & 0.20 & 0.19 {\cellcolor{lowbids}}                                     & 0.39  \\
\textbf{Science}    & 0.14 {\cellcolor{highbids}}                                     & 0.25 & 0.26 {\cellcolor{highbids}}                                     & 0.60  \\
\textbf{Shopping}   & 0.13 {\cellcolor{lowbids}}                                     & 0.22 & 0.27 {\cellcolor{highbids}}                                     & 0.58  \\
\textbf{Society}    & 0.15 {\cellcolor{highbids}}                                     & 0.24 & 0.19 {\cellcolor{lowbids}}                                     & 0.31  \\
\textbf{Sports}     & 0.15 {\cellcolor{highbids}}                                     & 0.24 & 0.26 {\cellcolor{highbids}}                                     & 0.53  \\
\midrule
\textbf{Control}    & 0.13 & 0.29 & 0.23 & 0.45        \\            



    \bottomrule

\end{tabular}

%\vspace{-5mm}
\label{table:Opt-in-mean}
\end{table}

==> docs/combined-cookie-syncing-events-table.tex <==

\begin{table*}[!htpb]
\centering
\caption{Cookie syncing events by advertisers under GDPR in Germany and CCPA in California using all 4 CMPs: Cookiebot, Didomi, Onetrust and Quantcast. Evt. column represents the number of cookie syncing events. Pct. represents the percentage of advertisers that participate in cookie syncing. Opt-out, opt-in represent the configurations when we opt-out and opt-in on selling of user data, respectively.}
    \begin{tabular}{l?{0.3mm}rr|rr?{0.3mm}rr|rr} 
    \toprule
     & \multicolumn{4}{c?{0.3mm}}{\textbf{GDPR}} &  \multicolumn{4}{c}{\textbf{CCPA}}   \\ 
     & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c?{0.3mm}}{\textbf{Opt-in}}& \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c}{\textbf{Opt-in}}   \\ 
    \textbf{Persona}     & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Pct.}}   & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c}{\textbf{Pct.}}  \\ 
    \toprule
    
\textbf{Adult}      & 73 & 42.86\% & 454 & 53.85\% & 249 & 54.17\% & 436 & 48.15\%  \\
\textbf{Arts}       & 51 & 43.75\% & 448 & 52.00\% & 208 & 41.67\% & 386 & 44.44\%  \\
\textbf{Business}   & 67 & 41.18\% & 479 & 54.55\% & 267 & 54.17\% & 388 & 44.00\%  \\
\textbf{Computers}  & 96 & 42.11\% & 534 & 53.85\% & 246 & 53.85\% & 374 & 50.00\%  \\
\textbf{Games}      & 94 & 47.37\% & 476 & 50.00\% & 245 & 57.69\% & 424 & 46.67\%  \\
\textbf{Health}     & 38 & 40.00\% & 425 & 45.83\% & 413 & 60.00\% & 619 & 60.00\%  \\
\textbf{Home}       & 60 & 50.00\% & 299 & 52.38\% & 236 & 48.15\% & 435 & 46.43\%  \\
\textbf{Kids}       & 66 & 42.11\% & 495 & 53.85\% & 330 & 48.39\% & 311 & 50.00\%  \\
\textbf{News}       & 47 & 47.06\% & 463 & 56.00\% & 221 & 54.55\% & 391 & 55.56\%  \\
\textbf{Recreation} & 51 & 47.06\% & 403 & 56.00\% & 291 & 56.52\% & 482 & 50.00\%  \\
\textbf{Reference}  & 57 & 41.18\% & 481 & 52.00\% & 258 & 60.00\% & 379 & 48.15\%  \\
\textbf{Regional}   & 82 & 37.50\% & 423 & 53.57\% & 312 & 60.00\% & 428 & 57.14\%  \\
\textbf{Science}    & 41 & 37.50\% & 476 & 52.00\% & 341 & 45.83\% & 513 & 48.28\%  \\
\textbf{Shopping}   & 61 & 35.71\% & 426 & 54.55\% & 431 & 56.67\% & 431 & 50.00\%  \\
\textbf{Society}    & 45 & 38.89\% & 356 & 54.17\% & 229 & 50.00\% & 419 & 44.00\%  \\
\textbf{Sports}     & 60 & 40.00\% & 504 & 55.56\% & 199 & 57.14\% & 388 & 50.00\% \\
\midrule
\textbf{Average}    & 62 & 42.14\% & 446 & 53.13\% & 280 & 53.67\% & 425 & 49.55\%                                        
\\



\bottomrule
\end{tabular}

\label{tbl:combined_cookie_syncing}
\end{table*}





==> docs/combined-stats-test.tex <==
\begin{table}
\footnotesize
%\adjustbox{max width=\textwidth}{
    \centering
    \caption{Mann–Whitney U test to validate our hypothesis that the advertisers bidding behavior does not significantly change between opt-in and opt-out under GDPR. Column P and R represent p-value and effect size, respectively. Effect size is calculated only in cases when there is statistically significant difference. }
    \begin{tabular}{l?{0.3mm}ll|ll} 
    \toprule
     & \multicolumn{2}{c?{0.3mm}}{\textbf{GDPR}} &  \multicolumn{2}{c}{\textbf{CCPA}}      \\ 
 
    \textbf{Persona}     & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c?{0.3mm}}{\textbf{E}} & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c}{\textbf{E}} \\ 
    \toprule
    
\textbf{Adult}      & 5.32E-39                       & 0.19                           & 4.92E-42                       & 0.22                            \\
\textbf{Arts}       & 1.92E-16                       & 0.13                           & 6.41E-68                       & 0.27                            \\
\textbf{Business}   & 1.33E-21                       & 0.14                           & 2.50E-58                       & 0.25                            \\
\textbf{Computers}  & 2.88E-31                       & 0.16                           & 6.82E-70                       & 0.26                            \\
\textbf{Games}      & 3.17E-61                       & 0.23                           & 4.77E-35                       & 0.18                            \\
\textbf{Health}     & 1.31E-43                       & 0.20                           & 8.82E-67                       & 0.25                            \\
\textbf{Home}       & 3.23E-43                       & 0.21                           & 4.23E-51                       & 0.24                            \\
\textbf{Kids}       & 2.19E-25                       & 0.16                           & 2.81E-49                       & 0.20                            \\
\textbf{News}       & 1.47E-59                       & 0.22                           & 5.27E-25                       & 0.15                            \\
\textbf{Recreation} & 5.84E-41                       & 0.20                           & 2.24E-55                       & 0.24                            \\
\textbf{Reference}  & 4.52E-38                       & 0.19                           & 5.86E-49                       & 0.22                            \\
\textbf{Regional}   & 1.07E-19                       & 0.14                           & 1.19E-84                       & 0.28                            \\
\textbf{Science}    & 4.66E-47                       & 0.19                           & 2.01E-55                       & 0.24                            \\
\textbf{Shopping}   & 7.29E-59                       & 0.23                           & 2.40E-25                       & 0.15                            \\
\textbf{Society}    & 1.42E-31                       & 0.18                           & 1.18E-45                       & 0.22                            \\
\textbf{Sports}     & 4.12E-18                       & 0.13                           & 2.80E-27 \\              
    

\midrule
\textbf{Control}    & 3.12E-48                       & 0.21                           & 1.04E-39         \\            

    \bottomrule

\end{tabular}

%\vspace{-5mm}
\label{table:Opt-out-mean}
\end{table}





==> docs/cookie-syncing-events-table.tex <==

\begin{table*}[!htpb]
\centering
    \begin{tabular}{l?{0.3mm}rr|rr?{0.3mm}rr|rr?{0.3mm}rr|rr} 
    \toprule
     & \multicolumn{4}{c?{0.3mm}}{\textbf{OneTrust}} & \multicolumn{4}{c?{0.3mm}}{\textbf{CookieBot}}& \multicolumn{4}{c}{\textbf{NAI}}    \\ 
     & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c?{0.3mm}}{\textbf{Opt-in}}     & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c?{0.3mm}}{\textbf{Opt-in}}    & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c}{\textbf{Opt-in}}   \\ 
    \textbf{Persona}     & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Pct.}} & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Pct.}}  & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c}{\textbf{Pct.}}  \\ 
    \toprule
    
\textbf{Adult}      & 24 & 75\%  & 91  & 66.7\%    & 2 & 100\% & 1  & 100\% & 47 & 45.5\%  & 54 & 54.5\%   \\ 

\textbf{Arts}       & 4  & 50\%  & 49  & 83.3\%    & 1 & 100\% & -- & --   & 32 & 83.3\%  & 41 & 66.7\%   \\ 

\textbf{Business}   & 16 & 50\%  & 106 & 85.7\%    & 2 & 50\%  & 2  & 33.3\%  & 21 & 42.9\%  & 28 & 57.1\%   \\ 

\textbf{Computers}  & 22 & 75\%  & 69  & 80\%    & 1 & 50\%  & 5  & 33.3\%  & 27 & 55.6\%  & 41 & 54.5\%   \\ 

\textbf{Games}      & 2  & 100\% & 12  & 100\%   & --& --   & 1  & 100\% & 29 & 40\%  & 24 & 75\%   \\ 

\textbf{Health}     & 8  & 50\%  & --   & -- & 6 & 50\%  & 5  & 66.7\%  & 42 & 45.5\%  & 35 & 41.7\%   \\ 

\textbf{Home}       & 5  & 75\%  & 57  & 87.5\%    & --& --   & 1  & 33.3\%  & 14 & 28.6\%  & 28 & 50\%   \\ 

\textbf{Kids}       & 28 & 80\%  & 69  & 80\%    & 4 & 33.3\%  & -- & --   & 29 & 57.1\%  & 23 & 44.4\%   \\ 

\textbf{News}       & 8  & 100\% & 67  & 66.7\%    & --& --   & -- & --   & 32 & 62.5\%  & 31 & 66.7\%   \\ 

\textbf{Recreation} & 28 & 100\% & 59  & 75\%    & 5 & 66.7\%  & 1  & 100\% & 42 & 50\%  & 46 & 62.5\%   \\ 

\textbf{Reference}  & 6  & 50\%  & 41  & 60\%    & 1 & 50\%  & 3  & 50\%  & 18 & 40\%  & 28 & 80\%   \\ 

\textbf{Regional}   & 9  & 75\%  & 55  & 75\%    & --& --   & -- & --   & 22 & 57.1\%  & 14 & 66.7\%   \\ 

\textbf{Science}    & 7  & 66.7\%  & 32  & 66.7\%    & 1 & 100\% & 1  & 50\%  & 22 & 50\%  & 22 & 100\%  \\ 

\textbf{Shopping}   & 22 & 50\%  & 40  & 60\%    & 1 & 100\% & 10 & 66.7\%  & 32 & 100\% & 32 & 60\%   \\ 

\textbf{Society}    & 22 & 66.7\%  & 69  & 83.3\%    & 7 & 100\% & -- & --   & 34 & 50\%  & 34 & 66.7\%   \\ 

\textbf{Sports}     & 14 & 50\%  & 49  & 66.7\%    & --& --   & 2  & 50\%  & 31 & 55.6\%  & 35 & 71.4\%   \\
\midrule
\textbf{Average} & 14 & 69.6\% & 54 & 71\% & 2 & 50\% & 2 & 42.7\% & 30 & 54\% & 32 & 63.6\%  \\

\bottomrule
\end{tabular}
\caption{Cookie syncing events by advertisers under GDPR in Germany. Evt. column represents the number of cookie syncing events. Pct. represents the percentage of advertisers that participate in cookie syncing. Opt-out, opt-in represent the configurations when we opt-out and opt-in on selling of user data, respectively.}
\label{tbl:GDPR_cookie_syncing}
\end{table*}



\begin{table*}[!htpb]
\centering
    \begin{tabular}{l?{0.3mm}rr|rr?{0.3mm}rr|rr?{0.3mm}rr|rr} 
    \toprule
     & \multicolumn{4}{c?{0.3mm}}{\textbf{OneTrust}} & \multicolumn{4}{c?{0.3mm}}{\textbf{CookieBot}}& \multicolumn{4}{c}{\textbf{NAI}}    \\ 
     & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c?{0.3mm}}{\textbf{Opt-in}}     & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c?{0.3mm}}{\textbf{Opt-in}}    & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c}{\textbf{Opt-in}}   \\ 
    \textbf{Persona}     & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Pct.}} & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Pct.}}  & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c}{\textbf{Pct.}}  \\ 
    \toprule
\textbf{Adult}      & 61 & 88.9\%  & 41 & 83.3\% & 26 & 42.9\% & 40 & 60\% & 78  & 50\% & 110 & 64.3\%  \\ 

\textbf{Arts}       & 23 & 100\% & 22 & 71.4\% & 29 & 55.6\% & 7  & 50\% & 29  & 54.5\% & 51  & 66.7\%  \\ 

\textbf{Business}   & 24 & 57.1\%  & 33 & 57.1\% & 54 & 50\% & 37 & 50\% & 68  & 53.3\% & 70  & 57.1\%  \\ 

\textbf{Computers}  & 52 & 77.8\%  & 33 & 71.4\% & 13 & 50\% & 35 & 62.5\% & 46  & 43.8\% & 58  & 54.5\%  \\ 

\textbf{Games}      & 32 & 66.7\%  & 26 & 55.6\% & 31 & 55.6\% & 11 & 28.6\% & 61  & 66.7\% & 38  & 38.5\%  \\ 

\textbf{Health}     & 54 & 71.4\%  & 51 & 66.7\% & 18 & 28.6\% & 20 & 50\% & 74  & 53.3\% & 26  & 50\%  \\ 

\textbf{Home}       & 46 & 80\%  & 38 & 62.5\% & 30 & 44.4\% & 24 & 50\% & 77  & 55.6\% & 50  & 50\%  \\ 

\textbf{Kids}       & 32 & 50\%  & 35 & 62.5\% & 34 & 44.4\% & 28 & 50\% & 46  & 50\% & 68  & 60\%  \\ 

\textbf{News}       & 20 & 60\%  & 13 & 55.6\% & 3  & 33.3\% & 6  & 50\% & 37  & 40\% & 61  & 42.9\%  \\ 

\textbf{Recreation} & 34 & 71.4\%  & 45 & 75\% & 10 & 50\% & 12 & 66.7\% & 52  & 58.3\% & 66  & 66.7\%  \\ 

\textbf{Reference}  & 29 & 77.8\%  & 32 & 63.6\% & 27 & 50\% & 19 & 50\% & 61  & 46.7\% & 65  & 50\%  \\ 

\textbf{Regional}   & 50 & 77.8\%  & 41 & 70\% & 5  & 40\% & 20 & 50\% & 10  & 66.7\% & 11  & 37.5\%  \\ 

\textbf{Science}    & 54 & 71.4\%  & 70 & 66.7\% & 33 & 50\% & 45 & 60\% & 103 & 50\% & 65  & 50\%  \\ 

\textbf{Shopping}   & 84 & 80\%  & 63 & 66.7\% & 56 & 50\% & 46 & 66.7\% & 58  & 45.5\% & 32  & 60\%  \\ 

\textbf{Society}    & 33 & 66.7\%  & 32 & 44.4\% & 38 & 50\% & 36 & 42.9\% & 74  & 56.3\% & 58  & 42.9\%  \\ 

\textbf{Sports}     & 33 & 75\%  & 18 & 50\% & 22 & 37.5\% & 23 & 50\% & 45  & 61.5\% & 65  & 50\%  \\
\midrule
\textbf{Average} & 41 & 73.2\% & 37 & 63.9\% & 27 & 45.8\% & 26 & 52.3\% & 57 & 53.3\% & 56 & 52.6\%  \\

\bottomrule
\end{tabular}
\caption{Cookie syncing events by advertisers under CCPA in California. Evt. column represents the number of cookie syncing events. Pct. represents the percentage of advertisers that participate in cookie syncing. Opt-out, opt-in represent the configurations when we opt-out and opt-in on selling of user data, respectively.}
\label{tbl:CCPA_cookie_syncing}
\end{table*}






\begin{table}[!h]
\centering
    \begin{tabular}{l?{0.3mm}rrr?{0.3mm}rrr} 
    \toprule
     & \multicolumn{3}{c?{0.3mm}}{\textbf{GDPR}} & \multicolumn{3}{c}{\textbf{CCPA}}    \\ 
     \textbf{Advertisers}& \multicolumn{1}{c}{\textbf{OT}} & \multicolumn{1}{c}{\textbf{CB}}& \multicolumn{1}{c?{0.3mm}}{\textbf{NAI}}& \multicolumn{1}{c}{\textbf{OT}} & \multicolumn{1}{c}{\textbf{CB}}& \multicolumn{1}{c}{\textbf{NAI}}    \\ 
    \toprule


\textbf{AppNexus}           & 87 & 12 & 183 & 214 & 201& 311 \\ 
\textbf{Conversant} & 32                                                      & 7                                                       & 81                                                       & 215                                                      & 161                                                      & 326                                                       \\ 
\textbf{PubMatic}        & 164                                                     & 43                                                      & 188                                                      & 131                                                      & 94                                                       & 131                                                       \\ 
\textbf{TripleLift}      & 13                                                      & 1                                                       & 159                                                      & 86                                                       & 120                                                      & 139                                                       \\
\textbf{Rubicon}  & 51                                                      & 23                                                      & 68                                                       & 130                                                      & 127                                                      & 115                                                       \\
\bottomrule
\end{tabular}
\caption{Most prevalent advertisers that participate in cookie syncing, when we opt-out under GDPR and CCPA. These advertiser appear in all personas across OneTrust, CookieBot, and NAI configurations. OT, CB, and NAI columns represent the count of cookie syncing events under OneTrust, CookieBot, and NAI for each advertiser.}
\label{tbl:Advertisers_cookie_syncing}
\end{table}

==> docs/cookie-syncing-events-table_CCPA-new.tex <==



\begin{table*}[!htpb]
\scriptsize
\centering
\caption{\textcolor{blue}{Cookie syncing events by advertisers under CCPA in California. Evt. column represents the number of cookie syncing events. Pct. represents the percentage of advertisers that participate in cookie syncing. Opt-out, opt-in represent the configurations when we opt-out and opt-in on selling of user data, respectively.}}
     \begin{tabular}{l?{0.3mm}rr|rr?{0.3mm}rr|rr?{0.3mm}rr|rr?{0.3mm}rr|rr} 
    \toprule
     & \multicolumn{4}{c?{0.3mm}}{\textbf{Cookiebot}} & \multicolumn{4}{c?{0.3mm}}{\textbf{Didomi}}& \multicolumn{4}{c?{0.3mm}}{\textbf{Onetrust}}  & \multicolumn{4}{c}{\textbf{Quantcast}}   \\ 
     & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c?{0.3mm}}{\textbf{Opt-in}}& \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c?{0.3mm}}{\textbf{Opt-in}}     & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c?{0.3mm}}{\textbf{Opt-in}}    & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c}{\textbf{Opt-in}}   \\ 
    \textbf{Persona}     & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Pct.}} & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Pct.}}& \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Pct.}}  & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c}{\textbf{Pct.}}  \\ 
    \toprule
\textbf{Adult}      & --                                                 & --                                             & 11                                                & 20.00\%                                        & 36                                                 & 75.00\%                                        & 136                                               & 50.00\%                                        & 85                                                 & 50.00\%                                        & 128                                               & 71.43\%                                        & 128                                                & 57.89\%                                        & 161                                               & 55.56\%                                         \\
\textbf{Arts}       & 4                                                  & 25.00\%                                        & 3                                                 & 20.00\%                                        & 43                                                 & 71.43\%                                        & 163                                               & 57.14\%                                        & 53                                                 & 42.86\%                                        & 71                                                & 80.00\%                                        & 108                                                & 52.94\%                                        & 149                                               & 50.00\%                                         \\
\textbf{Business}   & 3                                                  & 33.33\%                                        & 3                                                 & 20.00\%                                        & 21                                                 & 75.00\%                                        & 129                                               & 46.15\%                                        & 125                                                & 87.50\%                                        & 77                                                & 80.00\%                                        & 118                                                & 58.82\%                                        & 179                                               & 60.00\%                                         \\
\textbf{Computers}  & --                                                 & --                                             & 4                                                 & 20.00\%                                        & 38                                                 & 100.00\%                                       & 161                                               & 61.54\%                                        & 86                                                 & 62.50\%                                        & 84                                                & 85.71\%                                        & 122                                                & 60.00\%                                        & 125                                               & 47.06\%                                         \\
\textbf{Games}      & --                                                 & --                                             & 4                                                 & 14.29\%                                        & 30                                                 & 60.00\%                                        & 178                                               & 46.67\%                                        & 95                                                 & 71.43\%                                        & 58                                                & 57.14\%                                        & 120                                                & 63.16\%                                        & 184                                               & 57.89\%                                         \\
\textbf{Health}     & 28                                                 & 40.00\%                                        & 25                                                & 40.00\%                                        & 86                                                 & 83.33\%                                        & 222                                               & 60.00\%                                        & 115                                                & 60.00\%                                        & 120                                               & 71.43\%                                        & 184                                                & 68.18\%                                        & 252                                               & 68.42\%                                         \\
\textbf{Home}       & 6                                                  & 16.67\%                                        & 14                                                & 33.33\%                                        & 19                                                 & 75.00\%                                        & 155                                               & 46.15\%                                        & 110                                                & 70.00\%                                        & 56                                                & 80.00\%                                        & 101                                                & 61.11\%                                        & 210                                               & 70.59\%                                         \\
\textbf{Kids}       & 5                                                  & 20.00\%                                        & 26                                                & 40.00\%                                        & 65                                                 & 75.00\%                                        & 169                                               & 53.33\%                                        & 124                                                & 62.50\%                                        & 116                                               & 87.50\%                                        & 136                                                & 50.00\%                                        & --                                                & --                                              \\
\textbf{News}       & 3                                                  & 25.00\%                                        & 3                                                 & 20.00\%                                        & 31                                                 & 83.33\%                                        & 162                                               & 60.00\%                                        & 98                                                 & 62.50\%                                        & 47                                                & 66.67\%                                        & 89                                                 & 64.29\%                                        & 179                                               & 68.75\%                                         \\
\textbf{Recreation} & 21                                                 & 20.00\%                                        & 13                                                & 20.00\%                                        & 47                                                 & 57.14\%                                        & 232                                               & 58.82\%                                        & 86                                                 & 71.43\%                                        & 77                                                & 75.00\%                                        & 137                                                & 63.16\%                                        & 160                                               & 60.00\%                                         \\
\textbf{Reference}  & 14                                                 & 20.00\%                                        & 5                                                 & 20.00\%                                        & 32                                                 & 66.67\%                                        & 143                                               & 50.00\%                                        & 67                                                 & 55.56\%                                        & 89                                                & 71.43\%                                        & 145                                                & 65.00\%                                        & 142                                               & 52.94\%                                         \\
\textbf{Regional}   & 28                                                 & 33.33\%                                        & 16                                                & 28.57\%                                        & 36                                                 & 57.14\%                                        & 144                                               & 61.54\%                                        & 85                                                 & 66.67\%                                        & 53                                                & 60.00\%                                        & 163                                                & 63.16\%                                        & 215                                               & 70.59\%                                         \\
\textbf{Science}    & 29                                                 & 40.00\%                                        & 18                                                & 16.67\%                                        & 52                                                 & 75.00\%                                        & 219                                               & 58.33\%                                        & 114                                                & 62.50\%                                        & 106                                               & 83.33\%                                        & 146                                                & 52.94\%                                        & 170                                               & 56.25\%                                         \\
\textbf{Shopping}   & 37                                                 & 28.57\%                                        & 12                                                & 20.00\%                                        & 69                                                 & 66.67\%                                        & 185                                               & 50.00\%                                        & 136                                                & 60.00\%                                        & 76                                                & 80.00\%                                        & 189                                                & 68.18\%                                        & 158                                               & 55.56\%                                         \\
\textbf{Society}    & --                                                 & --                                             & 5                                                 & 25.00\%                                        & 31                                                 & 80.00\%                                        & 161                                               & 41.67\%                                        & 89                                                 & 80.00\%                                        & 87                                                & 83.33\%                                        & 109                                                & 52.94\%                                        & 166                                               & 56.25\%                                         \\
\textbf{Sports}     & 5                                                  & 20.00\%                                        & 7                                                 & 20.00\%                                        & 37                                                 & 80.00\%                                        & 162                                               & 50.00\%                                        & 74                                                 & 75.00\%                                        & 57                                                & 57.14\%                                        & 83                                                 & 55.56\%                                        & 162                                               & 64.71\%                                         \\
\midrule
\textbf{Average}    & 11                                                 & 20.12\%                                        & 11                                                & 23.62\%                                        & 42                                                 & 73.79\%                                        & 170                                               & 53.21\%                                        & 96                                                 & 65.03\%                                        & 81                                                & 74.38\%                                        & 130                                                & 59.83\%                                        & 174                                               & 59.64\%             \\                  
\bottomrule
\end{tabular}

\label{tbl:CCPA_cookie_syncing}
\end{table*}








==> docs/cookie-syncing-events-table_CCPA.tex <==



\begin{table*}[!htpb]
\centering
\caption{Cookie syncing events by advertisers under CCPA in California. Evt. column represents the number of cookie syncing events. Pct. represents the percentage of advertisers that participate in cookie syncing. Opt-out, opt-in represent the configurations when we opt-out and opt-in on selling of user data, respectively.}
    \begin{tabular}{l?{0.3mm}rr|rr?{0.3mm}rr|rr?{0.3mm}rr|rr} 
    \toprule
     & \multicolumn{4}{c?{0.3mm}}{\textbf{OneTrust}} & \multicolumn{4}{c?{0.3mm}}{\textbf{CookieBot}}& \multicolumn{4}{c}{\textbf{NAI}}    \\ 
     & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c?{0.3mm}}{\textbf{Opt-in}}     & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c?{0.3mm}}{\textbf{Opt-in}}    & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c}{\textbf{Opt-in}}   \\ 
    \textbf{Persona}     & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Pct.}} & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Pct.}}  & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c}{\textbf{Pct.}}  \\ 
    \toprule
\textbf{Adult}      & 61 & 88.9\%  & 41 & 83.3\% & 26 & 42.9\% & 40 & 60\% & 78  & 50\% & 110 & 64.3\%  \\ 

\textbf{Arts}       & 23 & 100\% & 22 & 71.4\% & 29 & 55.6\% & 7  & 50\% & 29  & 54.5\% & 51  & 66.7\%  \\ 

\textbf{Business}   & 24 & 57.1\%  & 33 & 57.1\% & 54 & 50\% & 37 & 50\% & 68  & 53.3\% & 70  & 57.1\%  \\ 

\textbf{Computers}  & 52 & 77.8\%  & 33 & 71.4\% & 13 & 50\% & 35 & 62.5\% & 46  & 43.8\% & 58  & 54.5\%  \\ 

\textbf{Games}      & 32 & 66.7\%  & 26 & 55.6\% & 31 & 55.6\% & 11 & 28.6\% & 61  & 66.7\% & 38  & 38.5\%  \\ 

\textbf{Health}     & 54 & 71.4\%  & 51 & 66.7\% & 18 & 28.6\% & 20 & 50\% & 74  & 53.3\% & 26  & 50\%  \\ 

\textbf{Home}       & 46 & 80\%  & 38 & 62.5\% & 30 & 44.4\% & 24 & 50\% & 77  & 55.6\% & 50  & 50\%  \\ 

\textbf{Kids}       & 32 & 50\%  & 35 & 62.5\% & 34 & 44.4\% & 28 & 50\% & 46  & 50\% & 68  & 60\%  \\ 

\textbf{News}       & 20 & 60\%  & 13 & 55.6\% & 3  & 33.3\% & 6  & 50\% & 37  & 40\% & 61  & 42.9\%  \\ 

\textbf{Recreation} & 34 & 71.4\%  & 45 & 75\% & 10 & 50\% & 12 & 66.7\% & 52  & 58.3\% & 66  & 66.7\%  \\ 

\textbf{Reference}  & 29 & 77.8\%  & 32 & 63.6\% & 27 & 50\% & 19 & 50\% & 61  & 46.7\% & 65  & 50\%  \\ 

\textbf{Regional}   & 50 & 77.8\%  & 41 & 70\% & 5  & 40\% & 20 & 50\% & 10  & 66.7\% & 11  & 37.5\%  \\ 

\textbf{Science}    & 54 & 71.4\%  & 70 & 66.7\% & 33 & 50\% & 45 & 60\% & 103 & 50\% & 65  & 50\%  \\ 

\textbf{Shopping}   & 84 & 80\%  & 63 & 66.7\% & 56 & 50\% & 46 & 66.7\% & 58  & 45.5\% & 32  & 60\%  \\ 

\textbf{Society}    & 33 & 66.7\%  & 32 & 44.4\% & 38 & 50\% & 36 & 42.9\% & 74  & 56.3\% & 58  & 42.9\%  \\ 

\textbf{Sports}     & 33 & 75\%  & 18 & 50\% & 22 & 37.5\% & 23 & 50\% & 45  & 61.5\% & 65  & 50\%  \\
\midrule
\textbf{Average} & 41 & 73.2\% & 37 & 63.9\% & 27 & 45.8\% & 26 & 52.3\% & 57 & 53.3\% & 56 & 52.6\%  \\

\bottomrule
\end{tabular}

\label{tbl:CCPA_cookie_syncing}
\end{table*}






\begin{table}[!h]
\centering
\caption{Most prevalent advertisers that participate in cookie syncing, when we opt-out under GDPR and CCPA. These advertiser appear in all personas across OneTrust, CookieBot, and NAI configurations. OT, CB, and NAI columns represent the count of cookie syncing events under OneTrust, CookieBot, and NAI for each advertiser.}
    \begin{tabular}{l?{0.3mm}rrr?{0.3mm}rrr} 
    \toprule
     & \multicolumn{3}{c?{0.3mm}}{\textbf{GDPR}} & \multicolumn{3}{c}{\textbf{CCPA}}    \\ 
     \textbf{Advertisers}& \multicolumn{1}{c}{\textbf{OT}} & \multicolumn{1}{c}{\textbf{CB}}& \multicolumn{1}{c?{0.3mm}}{\textbf{NAI}}& \multicolumn{1}{c}{\textbf{OT}} & \multicolumn{1}{c}{\textbf{CB}}& \multicolumn{1}{c}{\textbf{NAI}}    \\ 
    \toprule


\textbf{AppNexus}           & 87 & 12 & 183 & 214 & 201& 311 \\ 
\textbf{Conversant} & 32                                                      & 7                                                       & 81                                                       & 215                                                      & 161                                                      & 326                                                       \\ 
\textbf{PubMatic}        & 164                                                     & 43                                                      & 188                                                      & 131                                                      & 94                                                       & 131                                                       \\ 
\textbf{TripleLift}      & 13                                                      & 1                                                       & 159                                                      & 86                                                       & 120                                                      & 139                                                       \\
\textbf{Rubicon}  & 51                                                      & 23                                                      & 68                                                       & 130                                                      & 127                                                      & 115                                                       \\
\bottomrule
\end{tabular}

\label{tbl:Advertisers_cookie_syncing}
\end{table}

==> docs/cookie-syncing-events-table_GDPR-new.tex <==

\begin{table*}[!htpb]
\scriptsize
\centering
\caption{\textcolor{blue}{Cookie syncing events by advertisers under GDPR in Germany. Evt. column represents the number of cookie syncing events. Pct. represents the percentage of advertisers that participate in cookie syncing. Opt-out, opt-in represent the configurations when we opt-out and opt-in on selling of user data, respectively.}}
    \begin{tabular}{l?{0.3mm}rr|rr?{0.3mm}rr|rr?{0.3mm}rr|rr?{0.3mm}rr|rr} 
    \toprule
     & \multicolumn{4}{c?{0.3mm}}{\textbf{Cookiebot}} & \multicolumn{4}{c?{0.3mm}}{\textbf{Didomi}}& \multicolumn{4}{c?{0.3mm}}{\textbf{Onetrust}}  & \multicolumn{4}{c}{\textbf{Quantcast}}   \\ 
     & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c?{0.3mm}}{\textbf{Opt-in}}& \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c?{0.3mm}}{\textbf{Opt-in}}     & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c?{0.3mm}}{\textbf{Opt-in}}    & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c}{\textbf{Opt-in}}   \\ 
    \textbf{Persona}     & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Pct.}} & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Pct.}}& \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Pct.}}  & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c}{\textbf{Pct.}}  \\ 
    \toprule
    
\textbf{Adult}      & --                           & --                       & 25                          & 25.00\%                  & --                           & --                       & 205                         & 53.33\%                  & 19                           & 100.00\%                 & 20                          & 100.00\%                 & 54                           & 45.45\%                  & 204                         & 68.75\%                   \\
\textbf{Arts}       & --                           & --                       & 7                           & 25.00\%                  & 1                            & 100.00\%                 & 209                         & 46.67\%                  & 0                            & 0.00\%                   & 22                          & 100.00\%                 & 50                           & 46.15\%                  & 210                         & 64.71\%                   \\
\textbf{Business}   & --                           & --                       & 44                          & 40.00\%                  & --                           & --                       & 232                         & 53.33\%                  & 24                           & 100.00\%                 & 49                          & 100.00\%                 & 43                           & 42.86\%                  & 154                         & 69.23\%                   \\
\textbf{Computers}  & --                           & --                       & 28                          & 20.00\%                  & 15                           & 100.00\%                 & 276                         & 64.71\%                  & 29                           & 100.00\%                 & 38                          & 100.00\%                 & 52                           & 40.00\%                  & 192                         & 58.82\%                   \\
\textbf{Games}      & --                           & --                       & 27                          & 25.00\%                  & 17                           & 100.00\%                 & 247                         & 50.00\%                  & 16                           & 100.00\%                 & 22                          & 100.00\%                 & 61                           & 50.00\%                  & 180                         & 62.50\%                   \\
\textbf{Health}     & --                           & --                       & 36                          & 40.00\%                  & --                           & --                       & 223                         & 47.06\%                  & 1                            & 100.00\%                 & 25                          & 100.00\%                 & 37                           & 46.15\%                  & 141                         & 57.14\%                   \\
\textbf{Home}       & --                           & --                       & 3                           & 20.00\%                  & --                           & --                       & 153                         & 53.85\%                  & 15                           & 100.00\%                 & 8                           & 100.00\%                 & 45                           & 53.33\%                  & 135                         & 57.14\%                   \\
\textbf{Kids}       & --                           & --                       & 41                          & 33.33\%                  & 2                            & 100.00\%                 & 252                         & 56.25\%                  & 12                           & 50.00\%                  & 27                          & 100.00\%                 & 52                           & 40.00\%                  & 175                         & 66.67\%                   \\
\textbf{News}       & 3                            & 25.00\%                  & 22                          & 25.00\%                  & --                           & --                       & 251                         & 60.00\%                  & 8                            & 100.00\%                 & 27                          & 100.00\%                 & 36                           & 46.15\%                  & 163                         & 66.67\%                   \\
\textbf{Recreation} & --                           & --                       & 6                           & 25.00\%                  & 2                            & 100.00\%                 & 208                         & 52.94\%                  & 7                            & 100.00\%                 & 13                          & 50.00\%                  & 42                           & 50.00\%                  & 176                         & 66.67\%                   \\
\textbf{Reference}  & --                           & --                       & 24                          & 25.00\%                  & --                           & --                       & 221                         & 52.94\%                  & 11                           & 100.00\%                 & 45                          & 100.00\%                 & 46                           & 46.67\%                  & 191                         & 62.50\%                   \\
\textbf{Regional}   & --                           & --                       & 52                          & 50.00\%                  & --                           & --                       & 203                         & 50.00\%                  & 33                           & 100.00\%                 & 30                          & 100.00\%                 & 49                           & 38.46\%                  & 138                         & 53.33\%                   \\
\textbf{Science}    & --                           & --                       & 26                          & 25.00\%                  & --                           & --                       & 246                         & 56.25\%                  & 1                            & 100.00\%                 & 13                          & 100.00\%                 & 40                           & 42.86\%                  & 191                         & 64.71\%                   \\
\textbf{Shopping}   & --                           & --                       & 50                          & 42.86\%                  & --                           & --                       & 223                         & 50.00\%                  & 14                           & 100.00\%                 & 14                          & 100.00\%                 & 47                           & 45.45\%                  & 139                         & 61.54\%                   \\
\textbf{Society}    & --                           & --                       & 5                           & 20.00\%                  & --                           & --                       & 204                         & 50.00\%                  & 10                           & 100.00\%                 & 21                          & 100.00\%                 & 35                           & 42.86\%                  & 126                         & 69.23\%                   \\
\textbf{Sports}     & --                           & --                       & 43                          & 40.00\%                  & 3                            & 100.00\%                 & 218                         & 56.25\%                  & 20                           & 100.00\%                 & 54                          & 83.33\%                  & 37                           & 37.50\%                  & 189                         & 64.71\%                   \\
\midrule
\textbf{Average}    & 1                            & 1.56\%                   & 27                          & 30.07\%                  & 3                            & 37.50\%                  & 223                         & 53.35\%                  & 14                           & 90.63\%                  & 27                          & 95.83\%                  & 45                           & 44.62\%                  & 169                         & 63.39\%        \\          
         


\bottomrule
\end{tabular}

\label{tbl:GDPR_cookie_syncing}
\end{table*}





==> docs/cookie-syncing-events-table_GDPR.tex <==

\begin{table*}[!htpb]
\centering
\caption{Cookie syncing events by advertisers under GDPR in Germany. Evt. column represents the number of cookie syncing events. Pct. represents the percentage of advertisers that participate in cookie syncing. Opt-out, opt-in represent the configurations when we opt-out and opt-in on selling of user data, respectively.}
    \begin{tabular}{l?{0.3mm}rr|rr?{0.3mm}rr|rr?{0.3mm}rr|rr} 
    \toprule
     & \multicolumn{4}{c?{0.3mm}}{\textbf{OneTrust}} & \multicolumn{4}{c?{0.3mm}}{\textbf{CookieBot}}& \multicolumn{4}{c}{\textbf{NAI}}    \\ 
     & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c?{0.3mm}}{\textbf{Opt-in}}     & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c?{0.3mm}}{\textbf{Opt-in}}    & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c}{\textbf{Opt-in}}   \\ 
    \textbf{Persona}     & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Pct.}} & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Pct.}}  & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c}{\textbf{Pct.}}  \\ 
    \toprule
    
\textbf{Adult}      & 24 & 75\%  & 91  & 66.7\%    & 2 & 100\% & 1  & 100\% & 47 & 45.5\%  & 54 & 54.5\%   \\ 

\textbf{Arts}       & 4  & 50\%  & 49  & 83.3\%    & 1 & 100\% & -- & --   & 32 & 83.3\%  & 41 & 66.7\%   \\ 

\textbf{Business}   & 16 & 50\%  & 106 & 85.7\%    & 2 & 50\%  & 2  & 33.3\%  & 21 & 42.9\%  & 28 & 57.1\%   \\ 

\textbf{Computers}  & 22 & 75\%  & 69  & 80\%    & 1 & 50\%  & 5  & 33.3\%  & 27 & 55.6\%  & 41 & 54.5\%   \\ 

\textbf{Games}      & 2  & 100\% & 12  & 100\%   & --& --   & 1  & 100\% & 29 & 40\%  & 24 & 75\%   \\ 

\textbf{Health}     & 8  & 50\%  & --   & -- & 6 & 50\%  & 5  & 66.7\%  & 42 & 45.5\%  & 35 & 41.7\%   \\ 

\textbf{Home}       & 5  & 75\%  & 57  & 87.5\%    & --& --   & 1  & 33.3\%  & 14 & 28.6\%  & 28 & 50\%   \\ 

\textbf{Kids}       & 28 & 80\%  & 69  & 80\%    & 4 & 33.3\%  & -- & --   & 29 & 57.1\%  & 23 & 44.4\%   \\ 

\textbf{News}       & 8  & 100\% & 67  & 66.7\%    & --& --   & -- & --   & 32 & 62.5\%  & 31 & 66.7\%   \\ 

\textbf{Recreation} & 28 & 100\% & 59  & 75\%    & 5 & 66.7\%  & 1  & 100\% & 42 & 50\%  & 46 & 62.5\%   \\ 

\textbf{Reference}  & 6  & 50\%  & 41  & 60\%    & 1 & 50\%  & 3  & 50\%  & 18 & 40\%  & 28 & 80\%   \\ 

\textbf{Regional}   & 9  & 75\%  & 55  & 75\%    & --& --   & -- & --   & 22 & 57.1\%  & 14 & 66.7\%   \\ 

\textbf{Science}    & 7  & 66.7\%  & 32  & 66.7\%    & 1 & 100\% & 1  & 50\%  & 22 & 50\%  & 22 & 100\%  \\ 

\textbf{Shopping}   & 22 & 50\%  & 40  & 60\%    & 1 & 100\% & 10 & 66.7\%  & 32 & 100\% & 32 & 60\%   \\ 

\textbf{Society}    & 22 & 66.7\%  & 69  & 83.3\%    & 7 & 100\% & -- & --   & 34 & 50\%  & 34 & 66.7\%   \\ 

\textbf{Sports}     & 14 & 50\%  & 49  & 66.7\%    & --& --   & 2  & 50\%  & 31 & 55.6\%  & 35 & 71.4\%   \\
\midrule
\textbf{Average} & 14 & 69.6\% & 54 & 71\% & 2 & 50\% & 2 & 42.7\% & 30 & 54\% & 32 & 63.6\%  \\

\bottomrule
\end{tabular}

\label{tbl:GDPR_cookie_syncing}
\end{table*}





==> docs/cookie-syncing-events-table_NAI-new.tex <==

\begin{table*}[!htpb]
\centering
\caption{\textcolor{blue}{Cookie syncing events by advertisers under GDPR in Germany and CCPA in California using NAI service. Evt. column represents the number of cookie syncing events. Pct. represents the percentage of advertisers that participate in cookie syncing. Opt-out, opt-in represent the configurations when we opt-out and opt-in on selling of user data, respectively.}}
    \begin{tabular}{l?{0.3mm}rr|rr?{0.3mm}rr|rr} 
    \toprule
     & \multicolumn{4}{c?{0.3mm}}{\textbf{GDPR}} &  \multicolumn{4}{c}{\textbf{CCPA}}   \\ 
     & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c?{0.3mm}}{\textbf{Opt-in}}& \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c}{\textbf{Opt-in}}   \\ 
    \textbf{Persona}     & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Pct.}}   & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c}{\textbf{Pct.}}  \\ 
    \toprule
    
\textbf{Adult}      & 7                                                  & 50.00\%                                        & 0                                                 & 0.00\%                                         & 19                                                 & 50.00\%                                        & 23                                                & 60.00\%                                         \\
\textbf{Arts}       & 13                                                 & 50.00\%                                        & 0                                                 & 0.00\%                                         & 5                                                  & 33.33\%                                        & 86                                                & 62.50\%                                         \\
\textbf{Business}   & 22                                                 & 66.67\%                                        & 21                                                & 40.00\%                                        & 18                                                 & 66.67\%                                        & 27                                                & 60.00\%                                         \\
\textbf{Computers}  & 11                                                 & 50.00\%                                        & 19                                                & 66.67\%                                        & 20                                                 & 66.67\%                                        & 33                                                & 66.67\%                                         \\
\textbf{Games}      & 15                                                 & 50.00\%                                        & 0                                                 & 0.00\%                                         & 10                                                 & 50.00\%                                        & 20                                                & 75.00\%                                         \\
\textbf{Health}     & 5                                                  & 50.00\%                                        & 5                                                 & 33.33\%                                        & 57                                                 & 83.33\%                                        & 71                                                & 83.33\%                                         \\
\textbf{Home}       & 0                                                  & 0.00\%                                         & 0                                                 & 0.00\%                                         & 18                                                 & 66.67\%                                        & 31                                                & 80.00\%                                         \\
\textbf{Kids}       & 7                                                  & 50.00\%                                        & 14                                                & 66.67\%                                        & 38                                                 & 75.00\%                                        & 67                                                & 83.33\%                                         \\
\textbf{News}       & 5                                                  & 50.00\%                                        & 2                                                 & 25.00\%                                        & 16                                                 & 66.67\%                                        & 18                                                & 75.00\%                                         \\
\textbf{Recreation} & 9                                                  & 66.67\%                                        & 6                                                 & 25.00\%                                        & 19                                                 & 50.00\%                                        & 49                                                & 83.33\%                                         \\
\textbf{Reference}  & 20                                                 & 66.67\%                                        & 13                                                & 33.33\%                                        & 25                                                 & 50.00\%                                        & 27                                                & 83.33\%                                         \\
\textbf{Regional}   & 13                                                 & 50.00\%                                        & 14                                                & 66.67\%                                        & 22                                                 & 50.00\%                                        & 49                                                & 80.00\%                                         \\
\textbf{Science}    & 5                                                  & 50.00\%                                        & 0                                                 & 0.00\%                                         & 54                                                 & 66.67\%                                        & 22                                                & 75.00\%                                         \\
\textbf{Shopping}   & 23                                                 & 66.67\%                                        & 18                                                & 33.33\%                                        & 27                                                 & 50.00\%                                        & 74                                                & 71.43\%                                         \\
\textbf{Society}    & 0                                                  & 0.00\%                                         & 0                                                 & 0.00\%                                         & 17                                                 & 66.67\%                                        & 93                                                & 83.33\%                                         \\
\textbf{Sports}     & 1                                                  & 50.00\%                                        & 0                                                 & 0.00\%                                         & 46                                                 & 80.00\%                                        & 78                                                & 80.00\%                                         \\
\midrule
\textbf{Average}    & 10                                                 & 47.92\%                                        & 7                                                 & 24.38\%                                        & 26                                                 & 60.73\%                                        & 48                                                & 75.14\%                                        
\\



\bottomrule
\end{tabular}

\label{tbl:NAI_cookie_syncing}
\end{table*}



\begin{table*}[!h]
\centering
\caption{\textcolor{blue}{Most prevalent advertisers that participate in cookie syncing, when we opt-out under GDPR and CCPA. These advertiser appear in all personas across OneTrust, CookieBot, and NAI configurations. CB, DM, OT, QC and NAI columns represent the count of cookie syncing events under  CookieBot, Didomi, Onetrust, Quantcast and NAI for each advertiser.}}
    \begin{tabular}{l?{0.3mm}rrrrr?{0.3mm}rrrrr} 
    \toprule
     & \multicolumn{5}{c?{0.3mm}}{\textbf{GDPR}} & \multicolumn{5}{c}{\textbf{CCPA}}    \\ 
     \textbf{Advertisers}& \multicolumn{1}{c}{\textbf{CB}} & \multicolumn{1}{c}{\textbf{DM}}&\multicolumn{1}{c}{\textbf{OT}}&\multicolumn{1}{c}{\textbf{QC}}& \multicolumn{1}{c?{0.3mm}}{\textbf{NAI}}& \multicolumn{1}{c}{\textbf{CB}} & \multicolumn{1}{c}{\textbf{DM}}& \multicolumn{1}{c}{\textbf{OT}}& \multicolumn{1}{c}{\textbf{QC}}& \multicolumn{1}{c}{\textbf{NAI}}    \\ 
    \toprule


\textbf{PubMatic}        & 68                       & 89                     & 143                    & 149                    & 141                     & 155                      & 216                    & 324                    & 309                    & 190                      \\
\textbf{AT\&T}           & 38                       & 84                     & 219                    & 190                    & 114                     & 128                      & 310                    & 476                    & 358                    & 314                      \\
\textbf{ConversantMedia} & 40                       & 55                     & 241                    & 60                     & 7                       & 153                      & 563                    & 529                    & 728                    & 444                      \\
\textbf{RubiconProject}  & 154                      & 255                    & 194                    & 148                    & 164                     & 270                      & 329                    & 330                    & 263                    & 446                      \\
\textbf{Casale Media}    & 11                       & 44                     & 161                    & 165                    & 145                     & 163                      & 226                    & 285                    & 278                    & 286          \\           
\bottomrule
\end{tabular}

\label{tbl:Advertisers_cookie_syncing}
\end{table*}

==> docs/cookie-syncing-events-table_old.tex <==




\begin{table*}[!h]
\centering
\begin{tabular}{l?{0.3mm}rrrrr?{0.3mm}rrrrr} 
\toprule
 & \multicolumn{5}{c?{0.3mm}}{\textbf{Opt-out}}                                                                                                                                                                                                           & \multicolumn{5}{c}{\textbf{Opt-in}}                                                                                                                                                                                                             \\ 

     \textbf{Persona}     & \multicolumn{1}{l}{\textbf{Requests}} & \multicolumn{1}{l}{\textbf{Http cookies}} & \multicolumn{1}{l}{\textbf{Syncing}} & \multicolumn{1}{l}{\textbf{From}} & \multicolumn{1}{l?{0.3mm}}{\textbf{To}} & \multicolumn{1}{l}{\textbf{Requests}} & \multicolumn{1}{l}{\textbf{Http cookies}} & \multicolumn{1}{l}{\textbf{Syncing}} & \multicolumn{1}{l}{\textbf{From}} & \multicolumn{1}{l}{\textbf{To}}  \\ 
\toprule
\textbf{Adult    }                         & 13743                                            & 1808                                                 & 158                                                           & 138                                & 152                              & 10708                                            & 1310                                                 & 97                                                            & 83                                 & 86                                \\ 

\textbf{Arts}                              & 12800                                            & 1895                                                 & 115                                                           & 99                                 & 102                              & 11551                                            & 1128                                                 & 74                                                            & 66                                 & 65                                \\ 

\textbf{Business}                          & 14420                                            & 1521                                                 & 114                                                           & 103                                & 106                              & 11981                                            & 1553                                                 & 173                                                           & 154                                & 146                               \\ 

\textbf{Computers}                         & 14336                                            & 2358                                                 & 180                                                           & 157                                & 170                              & 12997                                            & 1264                                                 & 105                                                           & 91                                 & 92                                \\ 

\textbf{Games}                             & 13986                                            & 1579                                                 & 138                                                           & 126                                & 130                              & 11796                                            & 1433                                                 & 90                                                            & 80                                 & 83                                \\ 

\textbf{Health}                            & 13543                                            & 2374                                                 & 171                                                           & 151                                & 160                              & 13190                                            & 1537                                                 & 126                                                           & 108                                & 117                               \\ 

\textbf{Home}                              & 13242                                            & 1583                                                 & 133                                                           & 119                                & 126                              & 11587                                            & 1558                                                 & 110                                                           & 98                                 & 103                               \\ 

\textbf{Kids}                              & 11700                                            & 1434                                                 & 97                                                            & 82                                 & 90                               & 12311                                            & 1431                                                 & 98                                                            & 84                                 & 87                                \\ 

\textbf{News}                              & 13884                                            & 1570                                                 & 80                                                            & 73                                 & 75                               & 13775                                            & 1488                                                 & 82                                                            & 76                                 & 74                                \\ 

\textbf{Recreation}                        & 14196                                            & 1533                                                 & 126                                                           & 109                                & 122                              & 14391                                            & 1613                                                 & 133                                                           & 121                                & 129                               \\ 

\textbf{Reference}                         & 13317                                            & 1217                                                 & 95                                                            & 83                                 & 88                               & 15293                                            & 1702                                                 & 71                                                            & 61                                 & 61                                \\ 

\textbf{Regional}                          & 12542                                            & 1660                                                 & 159                                                           & 145                                & 151                              & 12460                                            & 1639                                                 & 148                                                           & 135                                & 132                               \\ 

\textbf{Science}                           & 14038                                            & 1619                                                 & 160                                                           & 140                                & 153                              & 14080                                            & 1752                                                 & 145                                                           & 129                                & 135                               \\ 

\textbf{Shopping}                          & 13458                                            & 2100                                                 & 216                                                           & 194                                & 208                              & 13784                                            & 2017                                                 & 173                                                           & 158                                & 159                               \\ 

\textbf{Society}                           & 14090                                            & 2254                                                 & 125                                                           & 108                                & 118                              & 12759                                            & 1557                                                 & 102                                                           & 90                                 & 96                                \\ 

\textbf{Sports}                            & 12923                                            & 1348                                                 & 131                                                           & 118                                & 119                              & 13728                                            & 1626                                                 & 122                                                           & 107                                & 107                               \\
\bottomrule
\end{tabular}
\caption{Cookie syncing events of Onetrust in CCPA.}
\label{tbl:cookie_CCPA_onetrust}
\end{table*}

\begin{table*}[!h]
\centering
\begin{tabular}{l?{0.3mm}rrrrr?{0.3mm}rrrrr} 
\toprule
 & \multicolumn{5}{c?{0.3mm}}{\textbf{Opt-out}}                                                                                                                                                                                                           & \multicolumn{5}{c}{\textbf{Opt-in}}                                                                                                                                                                                                             \\ 

     \textbf{Persona}     & \multicolumn{1}{l}{\textbf{Requests}} & \multicolumn{1}{l}{\textbf{Http cookies}} & \multicolumn{1}{l}{\textbf{Syncing}} & \multicolumn{1}{l}{\textbf{From}} & \multicolumn{1}{l?{0.3mm}}{\textbf{To}} & \multicolumn{1}{l}{\textbf{Requests}} & \multicolumn{1}{l}{\textbf{Http cookies}} & \multicolumn{1}{l}{\textbf{Syncing}} & \multicolumn{1}{l}{\textbf{From}} & \multicolumn{1}{l}{\textbf{To}}  \\ 
\toprule
\textbf{Adult}                    & 21354                                   & 1555                                        & 92                                                   & 76                        & 84                      & 34857                                   & 3827                                        & 221                                                  & 200                       & 197                      \\ 

\textbf{Arts}                     & 18392                                   & 1311                                        & 36                                                   & 28                        & 34                      & 31319                                   & 3232                                        & 116                                                  & 106                       & 101                      \\ 

\textbf{Business}                 & 17686                                   & 1169                                        & 54                                                   & 48                        & 51                      & 30442                                   & 2558                                        & 206                                                  & 183                       & 184                      \\ 

\textbf{Computers}                & 19727                                   & 1604                                        & 72                                                   & 61                        & 68                      & 32518                                   & 3231                                        & 163                                                  & 147                       & 140                      \\ 

\textbf{Games}                    & 16864                                   & 1603                                        & 47                                                   & 37                        & 45                      & 25319                                   & 1691                                        & 117                                                  & 108                       & 103                      \\ 

\textbf{Health}                   & 14810                                   & 681                                         & 25                                                   & 21                        & 23                      & 31816                                   & 2771                                        & 174                                                  & 154                       & 155                      \\ 

\textbf{Home}                     & 18057                                   & 1031                                        & 33                                                   & 28                        & 31                      & 33273                                   & 3422                                        & 129                                                  & 116                       & 109                      \\ 

\textbf{Kids}                     & 16694                                   & 964                                         & 64                                                   & 54                        & 58                      & 33859                                   & 4046                                        & 214                                                  & 183                       & 186                      \\ 

\textbf{News}                     & 18930                                   & 1149                                        & 43                                                   & 36                        & 36                      & 32084                                   & 3228                                        & 166                                                  & 145                       & 135                      \\ 

\textbf{Recreation}               & 17975                                   & 1083                                        & 82                                                   & 67                        & 76                      & 32981                                   & 3365                                        & 195                                                  & 172                       & 163                      \\ 

\textbf{Reference}                & 17881                                   & 1149                                        & 76                                                   & 67                        & 72                      & 32966                                   & 3579                                        & 212                                                  & 190                       & 184                      \\ 

\textbf{Regional}                 & 17647                                   & 1068                                        & 49                                                   & 38                        & 43                      & 32818                                   & 3771                                        & 191                                                  & 172                       & 167                      \\ 

\textbf{Science}                  & 18830                                   & 1221                                        & 80                                                   & 62                        & 70                      & 36463                                   & 4246                                        & 186                                                  & 158                       & 163                      \\ 

\textbf{Shopping}                 & 20349                                   & 1951                                        & 80                                                   & 64                        & 74                      & 32999                                   & 3732                                        & 178                                                  & 160                       & 163                      \\ 

\textbf{Society}                  & 19812                                   & 1332                                        & 94                                                   & 75                        & 79                      & 30157                                   & 3073                                        & 168                                                  & 146                       & 149                      \\ 

\textbf{Sports}                   & 19200                                   & 1239                                        & 84                                                   & 67                        & 74                      & 33772                                   & 3598                                        & 142                                                  & 121                       & 121                      \\


\bottomrule
\end{tabular}
\caption{Cookie syncing events of Onetrust in GDPR.}
\label{tbl:cookie_GDPR_onetrust}
\end{table*}



==> docs/new_tables_0630.tex <==
\begin{table*}[!h]
\centering
\begin{tabular}{|l|r|r|r|r|} 
\hline
                      & \multicolumn{2}{c|}{\textbf{CCPA}}                                                & \multicolumn{2}{c|}{\textbf{GDPR}}                                                 \\ 
\hline
\textbf{CMP}          & \multicolumn{1}{l|}{\textbf{Bidding}} & \multicolumn{1}{l|}{\textbf{No\_Bidding}} & \multicolumn{1}{l|}{\textbf{Bidding}} & \multicolumn{1}{l|}{\textbf{No\_Bidding}}  \\ 
\hline
\textbf{Onetrust}     & 448                                   & 9531                                      & 482                                   & 9712                                       \\ 
\hline
\textbf{Quantcast}    & 1709                                  & 12188                                     & 1749                                  & 9760                                       \\ 
\hline
\textbf{Cookiebot}    & 70                                    & 10080                                     & 60                                    & 10038                                      \\ 
\hline
\textbf{TrustArc}     & 60                                    & 1160                                      & 13                                    & 1202                                       \\ 
\hline
\textbf{Crownpeak}    & 0                                     & 22                                        & 0                                     & 19                                         \\ 
\hline
\textbf{LiveRamp}     & 160                                   & 267                                       & 2012                                  & 479                                        \\ 
\hline
\textbf{CookieYes}    & 0                                     & 107                                       & 0                                     & 105                                        \\ 
\hline
\textbf{Osano}        & 69                                    & 10684                                     & 89                                    & 11352                                      \\ 
\hline
\textbf{AdRoll}       & 15                                    & 5995                                      & 15                                    & 5626                                       \\ 
\hline
\textbf{iubenda}      & 48                                    & 3625                                      & 49                                    & 3585                                       \\ 
\hline
\textbf{Didomi}       & 148                                   & 390                                       & 149                                   & 373                                        \\ 
\hline
\textbf{Usercentrics} & 7                                     & 2029                                      & 4                                     & 2061                                       \\
\hline
\end{tabular}
\end{table*}


\begin{table*}[!h]
\centering
\begin{tabular}{|l|l|l|l|l|} 
\hline
                         & \textbf{CCPA}            &                          & \textbf{GDPR}            &                           \\ 
\hline
                         & \textbf{Onetrust}        & \textbf{Quantcast}       & \textbf{Onetrust}        & \textbf{Quantcast}        \\ 
\hline
\textbf{Able to Opt-out} & \multicolumn{1}{r|}{101} & \multicolumn{1}{r|}{94}  & \multicolumn{1}{r|}{492} & \multicolumn{1}{r|}{993}  \\ 
\hline
\textbf{No able}         & \multicolumn{1}{r|}{95}  & \multicolumn{1}{r|}{265} & \multicolumn{1}{r|}{42}  & \multicolumn{1}{r|}{174}  \\
\hline
\end{tabular}
\end{table*}

==> docs/new_tables_0829.tex <==
\begin{table*}[!h]


\centering
\caption{Average Bids of all CMPs and NAI under GDPR.}
\begin{tabular}{|l|r|r|r|r|r|r|} 
\hline
                      & \multicolumn{6}{c|}{\textbf{GDPR}}                                                                                                                                                                                           \\ 
\hline
                    & \multicolumn{2}{c|}{\textbf{Opt\_out}}                                  & \multicolumn{2}{c|}{\textbf{Opt\_in}}                                   & \multicolumn{2}{c|}{\textbf{Pre\_opt\_out}}                              \\ 
\hline
\textbf{Persona}    & \multicolumn{1}{c|}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c|}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c|}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}}  \\ 
\hline
\textbf{Adult}      & 0.264                              & 0.542                              & 0.132                              & 0.187                              & 0.339                              & 1.002                               \\ 
\hline
\textbf{Arts}       & 0.257                              & 0.678                              & 0.173                              & 0.271                              & 0.244                              & 0.213                               \\ 
\hline
\textbf{Business}   & 0.230                              & 0.559                              & 0.134                              & 0.189                              & 0.350                              & 1.088                               \\ 
\hline
\textbf{Computers}  & 0.276                              & 0.654                              & 0.133                              & 0.190                              & 0.235                              & 0.216                               \\ 
\hline
\textbf{Games}      & 0.350                              & 0.913                              & 0.141                              & 0.216                              & 0.235                              & 0.215                               \\ 
\hline
\textbf{Health}     & 0.335                              & 0.858                              & 0.138                              & 0.203                              & 0.232                              & 0.215                               \\ 
\hline
\textbf{Home}       & 0.275                              & 0.604                              & 0.146                              & 0.256                              & 0.252                              & 0.484                               \\ 
\hline
\textbf{Kids}       & 0.292                              & 0.648                              & 0.156                              & 0.201                              & 0.334                              & 1.051                               \\ 
\hline
\textbf{News}       & 0.254                              & 0.479                              & 0.120                              & 0.198                              & 0.340                              & 1.034                               \\ 
\hline
\textbf{Recreation} & 0.297                              & 0.880                              & 0.133                              & 0.212                              & 0.374                              & 1.186                               \\ 
\hline
\textbf{Reference}  & 0.281                              & 0.789                              & 0.144                              & 0.258                              & 0.231                              & 0.213                               \\ 
\hline
\textbf{Regional}   & 0.278                              & 0.822                              & 0.152                              & 0.202                              & 0.238                              & 0.213                               \\ 
\hline
\textbf{Science}    & 0.314                              & 0.777                              & 0.139                              & 0.246                              & 0.328                              & 1.046                               \\ 
\hline
\textbf{Shopping}   & 0.256                              & 0.467                              & 0.127                              & 0.219                              & 0.366                              & 1.148                               \\ 
\hline
\textbf{Society}    & 0.287                              & 0.661                              & 0.143                              & 0.239                              & 0.248                              & 0.214                               \\ 
\hline
\textbf{Sports}     & 0.245                              & 0.544                              & 0.148                              & 0.235                              & 0.240                              & 0.214                               \\ 
\hline
\textbf{Control}    & 0.235                              & 0.214                              & 0.129                              & 0.289                              & 0.215                              & 0.215                               \\
\hline
\end{tabular}
\end{table*}





\begin{table*}[!h]


\centering
\caption{Average Bids of all CMPs and NAI under CCPA.}
\begin{tabular}{|l|r|r|r|r|r|r|} 
\hline
                      & \multicolumn{6}{c|}{\textbf{CCPA}}                                                                                                                                                                                           \\ 
\hline
                    & \multicolumn{2}{c|}{\textbf{Opt\_out}}                                  & \multicolumn{2}{c|}{\textbf{Opt\_in}}                                   & \multicolumn{2}{c|}{\textbf{Pre\_opt\_out}}                              \\ 
\hline
\textbf{Persona}    & \multicolumn{1}{c|}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c|}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c|}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}}  \\ 
\hline
\textbf{Adult}      & 0.326                              & 0.539                              & 0.208                              & 0.346                              & 0.257                              & 0.367                               \\ 
\hline
\textbf{Arts}       & 0.390                              & 1.012                              & 0.206                              & 0.480                              & 0.297                              & 0.597                               \\ 
\hline
\textbf{Business}   & 0.265                              & 0.380                              & 0.201                              & 0.389                              & 0.304                              & 0.581                               \\ 
\hline
\textbf{Computers}  & 0.410                              & 0.955                              & 0.205                              & 0.802                              & 0.328                              & 0.911                               \\ 
\hline
\textbf{Games}      & 0.292                              & 0.492                              & 0.250                              & 0.596                              & 0.334                              & 0.570                               \\ 
\hline
\textbf{Health}     & 0.416                              & 0.722                              & 0.263                              & 0.514                              & 0.411                              & 0.792                               \\ 
\hline
\textbf{Home}       & 0.313                              & 0.527                              & 0.227                              & 0.525                              & 0.274                              & 0.444                               \\ 
\hline
\textbf{Kids}       & 0.311                              & 0.602                              & 0.231                              & 0.590                              & 0.295                              & 0.549                               \\ 
\hline
\textbf{News}       & 0.275                              & 0.458                              & 0.246                              & 0.487                              & 0.334                              & 0.628                               \\ 
\hline
\textbf{Recreation} & 0.331                              & 0.539                              & 0.279                              & 0.764                              & 0.302                              & 0.521                               \\ 
\hline
\textbf{Reference}  & 0.322                              & 0.553                              & 0.228                              & 0.457                              & 0.318                              & 0.600                               \\ 
\hline
\textbf{Regional}   & 0.322                              & 0.583                              & 0.175                              & 0.376                              & 0.286                              & 0.624                               \\ 
\hline
\textbf{Science}    & 0.303                              & 0.539                              & 0.244                              & 0.587                              & 0.276                              & 0.522                               \\ 
\hline
\textbf{Shopping}   & 0.305                              & 0.579                              & 0.247                              & 0.535                              & 0.340                              & 0.699                               \\ 
\hline
\textbf{Society}    & 0.287                              & 0.716                              & 0.184                              & 0.308                              & 0.225                              & 0.232                               \\ 
\hline
\textbf{Sports}     & 0.282                              & 0.497                              & 0.244                              & 0.491                              & 0.314                              & 0.552                               \\ 
\hline
\textbf{Control}    & 0.245                              & 0.389                              & 0.204                              & 0.413                              & 0.290                              & 0.585                               \\
\hline
\end{tabular}
\end{table*}



% \usepackage{colortbl}


\begin{table*}[!h]


\centering
\caption{Cookie Syncing CCPA.}
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|} 
\hline
                   & \multicolumn{6}{c|}{\textbf{Cookiebot}}                                                                                                                                                                                                     & \multicolumn{6}{c|}{\textbf{Didomi}}                                                                                                                                                                                                        & \multicolumn{6}{c|}{\textbf{NAI}}                                                                                                                                                                                                           & \multicolumn{6}{c|}{\textbf{Onetrust}}                                                                                                                                                                                                      & \multicolumn{6}{c|}{\textbf{Quantcast}}                                                                                                                                                                                                      \\ 
\hline
                  & \multicolumn{1}{c|}{\textbf{Opt\_out}} & \multicolumn{1}{l|}{}              & \multicolumn{1}{c|}{\textbf{Opt\_in}} & \multicolumn{1}{l|}{}              & \multicolumn{1}{c|}{\textbf{Pre\_opt\_out}} & \multicolumn{1}{l|}{}              & \multicolumn{1}{c|}{\textbf{Opt\_out}} & \multicolumn{1}{l|}{}              & \multicolumn{1}{c|}{\textbf{Opt\_in}} & \multicolumn{1}{l|}{}              & \multicolumn{1}{c|}{\textbf{Pre\_opt\_out}} & \multicolumn{1}{l|}{}              & \multicolumn{1}{c|}{\textbf{Opt\_out}} & \multicolumn{1}{l|}{}              & \multicolumn{1}{c|}{\textbf{Opt\_in}} & \multicolumn{1}{l|}{}              & \multicolumn{1}{c|}{\textbf{Pre\_opt\_out}} & \multicolumn{1}{l|}{}              & \multicolumn{1}{c|}{\textbf{Opt\_out}} & \multicolumn{1}{l|}{}              & \multicolumn{1}{c|}{\textbf{Opt\_in}} & \multicolumn{1}{l|}{}              & \multicolumn{1}{c|}{\textbf{Pre\_opt\_out}} & \multicolumn{1}{l|}{}              & \multicolumn{1}{c|}{\textbf{Opt\_out}} & \multicolumn{1}{l|}{}              & \multicolumn{1}{c|}{\textbf{Opt\_in}} & \multicolumn{1}{l|}{}              & \multicolumn{1}{c|}{\textbf{Pre\_opt\_out}} & \multicolumn{1}{l|}{}               \\ 
\hline
{}\textbf{Persona}    & \multicolumn{1}{c|}{\textbf{Evt.}}     & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c|}{\textbf{Evt.}}    & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c|}{\textbf{Evt.}}          & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c|}{\textbf{Evt.}}     & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c|}{\textbf{Evt.}}    & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c|}{\textbf{Evt.}}          & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c|}{\textbf{Evt.}}     & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c|}{\textbf{Evt.}}    & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c|}{\textbf{Evt.}}          & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c|}{\textbf{Evt.}}     & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c|}{\textbf{Evt.}}    & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c|}{\textbf{Evt.}}          & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c|}{\textbf{Evt.}}     & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c|}{\textbf{Evt.}}    & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c|}{\textbf{Evt.}}          & \multicolumn{1}{c|}{\textbf{Pct.}}  \\ 
\hline
{}\textbf{Adult}      & 0                                      & 0.00\%                             & 11                                    & 20.00\%                            & 17                                          & 20.00\%                            & 36                                     & 75.00\%                            & 136                                   & 50.00\%                            & 39                                          & 100.00\%                           & 19                                     & 50.00\%                            & 23                                    & 60.00\%                            & 31                                          & 60.00\%                            & 85                                     & 50.00\%                            & 128                                   & 71.43\%                            & 107                                         & 83.33\%                            & 128                                    & 57.89\%                            & 161                                   & 55.56\%                            & 125                                         & 64.29\%                             \\ 
\hline
{}\textbf{Arts}       & 4                                      & 25.00\%                            & 3                                     & 20.00\%                            & 27                                          & 20.00\%                            & 43                                     & 71.43\%                            & 163                                   & 57.14\%                            & 35                                          & 100.00\%                           & 5                                      & 33.33\%                            & 86                                    & 62.50\%                            & 24                                          & 66.67\%                            & 53                                     & 42.86\%                            & 71                                    & 80.00\%                            & 90                                          & 80.00\%                            & 108                                    & 52.94\%                            & 149                                   & 50.00\%                            & 90                                          & 61.54\%                             \\ 
\hline
{}\textbf{Business}   & 3                                      & 33.33\%                            & 3                                     & 20.00\%                            & 23                                          & 33.33\%                            & 21                                     & 75.00\%                            & 129                                   & 46.15\%                            & 36                                          & 100.00\%                           & 18                                     & 66.67\%                            & 27                                    & 60.00\%                            & 27                                          & 60.00\%                            & 125                                    & 87.50\%                            & 77                                    & 80.00\%                            & 77                                          & 80.00\%                            & 118                                    & 58.82\%                            & 179                                   & 60.00\%                            & 94                                          & 58.33\%                             \\ 
\hline
{}\textbf{Computers}  & 0                                      & 0.00\%                             & 4                                     & 20.00\%                            & 16                                          & 20.00\%                            & 38                                     & 100.00\%                           & 161                                   & 61.54\%                            & 34                                          & 100.00\%                           & 20                                     & 66.67\%                            & 33                                    & 66.67\%                            & 32                                          & 50.00\%                            & 86                                     & 62.50\%                            & 84                                    & 85.71\%                            & 79                                          & 100.00\%                           & 122                                    & 60.00\%                            & 125                                   & 47.06\%                            & 73                                          & 50.00\%                             \\ 
\hline
{}\textbf{Games}      & 0                                      & 0.00\%                             & 4                                     & 14.29\%                            & 15                                          & 16.67\%                            & 30                                     & 60.00\%                            & 178                                   & 46.67\%                            & 45                                          & 100.00\%                           & 10                                     & 50.00\%                            & 20                                    & 75.00\%                            & 25                                          & 50.00\%                            & 95                                     & 71.43\%                            & 58                                    & 57.14\%                            & 109                                         & 75.00\%                            & 120                                    & 63.16\%                            & 184                                   & 57.89\%                            & 96                                          & 58.33\%                             \\ 
\hline
{}\textbf{Health}     & 28                                     & 40.00\%                            & 25                                    & 40.00\%                            & 13                                          & 25.00\%                            & 86                                     & 83.33\%                            & 222                                   & 60.00\%                            & 41                                          & 75.00\%                            & 57                                     & 83.33\%                            & 71                                    & 83.33\%                            & 71                                          & 66.67\%                            & 115                                    & 60.00\%                            & 120                                   & 71.43\%                            & 134                                         & 75.00\%                            & 184                                    & 68.18\%                            & 252                                   & 68.42\%                            & 89                                          & 57.14\%                             \\ 
\hline
{}\textbf{Home}       & 6                                      & 16.67\%                            & 14                                    & 33.33\%                            & 0                                           & 0.00\%                             & 19                                     & 75.00\%                            & 155                                   & 46.15\%                            & 37                                          & 60.00\%                            & 18                                     & 66.67\%                            & 31                                    & 80.00\%                            & 29                                          & 60.00\%                            & 110                                    & 70.00\%                            & 56                                    & 80.00\%                            & 46                                          & 100.00\%                           & 101                                    & 61.11\%                            & 210                                   & 70.59\%                            & 104                                         & 57.14\%                             \\ 
\hline
{}\textbf{Kids}       & 5                                      & 20.00\%                            & 26                                    & 40.00\%                            & 26                                          & 40.00\%                            & 65                                     & 75.00\%                            & 169                                   & 53.33\%                            & 57                                          & 100.00\%                           & 38                                     & 75.00\%                            & 67                                    & 83.33\%                            & 59                                          & 66.67\%                            & 124                                    & 62.50\%                            & 116                                   & 87.50\%                            & 111                                         & 57.14\%                            & 136                                    & 50.00\%                            & \multicolumn{1}{l|}{}                 & \multicolumn{1}{l|}{}              & 90                                          & 46.15\%                             \\ 
\hline
{}\textbf{News}       & 3                                      & 25.00\%                            & 3                                     & 20.00\%                            & 37                                          & 33.33\%                            & 31                                     & 83.33\%                            & 162                                   & 60.00\%                            & 34                                          & 100.00\%                           & 16                                     & 66.67\%                            & 18                                    & 75.00\%                            & 31                                          & 66.67\%                            & 98                                     & 62.50\%                            & 47                                    & 66.67\%                            & 100                                         & 71.43\%                            & 89                                     & 64.29\%                            & 179                                   & 68.75\%                            & 66                                          & 71.43\%                             \\ 
\hline
{}\textbf{Recreation} & 21                                     & 20.00\%                            & 13                                    & 20.00\%                            & 21                                          & 20.00\%                            & 47                                     & 57.14\%                            & 232                                   & 58.82\%                            & 57                                          & 100.00\%                           & 19                                     & 50.00\%                            & 49                                    & 83.33\%                            & 45                                          & 50.00\%                            & 86                                     & 71.43\%                            & 77                                    & 75.00\%                            & 61                                          & 60.00\%                            & 137                                    & 63.16\%                            & 160                                   & 60.00\%                            & 83                                          & 63.64\%                             \\ 
\hline
{}\textbf{Reference}  & 14                                     & 20.00\%                            & 5                                     & 20.00\%                            & 0                                           & 0.00\%                             & 32                                     & 66.67\%                            & 143                                   & 50.00\%                            & 35                                          & 100.00\%                           & 25                                     & 50.00\%                            & 27                                    & 83.33\%                            & 30                                          & 50.00\%                            & 67                                     & 55.56\%                            & 89                                    & 71.43\%                            & 64                                          & 62.50\%                            & 145                                    & 65.00\%                            & 142                                   & 52.94\%                            & 95                                          & 61.54\%                             \\ 
\hline
{}\textbf{Regional}   & 28                                     & 33.33\%                            & 16                                    & 28.57\%                            & 18                                          & 20.00\%                            & 36                                     & 57.14\%                            & 144                                   & 61.54\%                            & 32                                          & 100.00\%                           & 22                                     & 50.00\%                            & 49                                    & 80.00\%                            & 43                                          & 50.00\%                            & 85                                     & 66.67\%                            & 53                                    & 60.00\%                            & 106                                         & 83.33\%                            & 163                                    & 63.16\%                            & 215                                   & 70.59\%                            & 137                                         & 62.50\%                             \\ 
\hline
{}\textbf{Science}    & 29                                     & 40.00\%                            & 18                                    & 16.67\%                            & 0                                           & 0.00\%                             & 52                                     & 75.00\%                            & 219                                   & 58.33\%                            & 46                                          & 100.00\%                           & 54                                     & 66.67\%                            & 22                                    & 75.00\%                            & 49                                          & 80.00\%                            & 114                                    & 62.50\%                            & 106                                   & 83.33\%                            & 71                                          & 60.00\%                            & 146                                    & 52.94\%                            & 170                                   & 56.25\%                            & 86                                          & 53.85\%                             \\ 
\hline
{}\textbf{Shopping}   & 37                                     & 28.57\%                            & 12                                    & 20.00\%                            & 13                                          & 20.00\%                            & 69                                     & 66.67\%                            & 185                                   & 50.00\%                            & 37                                          & 100.00\%                           & 27                                     & 50.00\%                            & 74                                    & 71.43\%                            & 50                                          & 66.67\%                            & 136                                    & 60.00\%                            & 76                                    & 80.00\%                            & 62                                          & 50.00\%                            & 189                                    & 68.18\%                            & 158                                   & 55.56\%                            & 98                                          & 66.67\%                             \\ 
\hline
{}\textbf{Society}    & 0                                      & 0.00\%                             & 5                                     & 25.00\%                            & 47                                          & 50.00\%                            & 31                                     & 80.00\%                            & 161                                   & 41.67\%                            & 54                                          & 100.00\%                           & 17                                     & 66.67\%                            & 93                                    & 83.33\%                            & 56                                          & 83.33\%                            & 89                                     & 80.00\%                            & 87                                    & 83.33\%                            & 94                                          & 75.00\%                            & 109                                    & 52.94\%                            & 166                                   & 56.25\%                            & 91                                          & 66.67\%                             \\ 
\hline
{}\textbf{Sports}     & 5                                      & 20.00\%                            & 7                                     & 20.00\%                            & 18                                          & 25.00\%                            & 37                                     & 80.00\%                            & 162                                   & 50.00\%                            & 34                                          & 75.00\%                            & 46                                     & 80.00\%                            & 78                                    & 80.00\%                            & 31                                          & 60.00\%                            & 74                                     & 75.00\%                            & 57                                    & 57.14\%                            & 112                                         & 60.00\%                            & 83                                     & 55.56\%                            & 162                                   & 64.71\%                            & 107                                         & 58.33\%                             \\ 
\hline
\textbf{Average}                                        & 11                                     & 20.12\%                            & 11                                    & 23.62\%                            & 18                                          & 21.46\%                            & 42                                     & 73.79\%                            & 170                                   & 53.21\%                            & 41                                          & 94.38\%                            & 26                                     & 60.73\%                            & 48                                    & 75.14\%                            & 40                                          & 61.67\%                            & 96                                     & 65.03\%                            & 81                                    & 74.38\%                            & 89                                          & 73.30\%                            & 130                                    & 59.83\%                            & 174                                   & 59.64\%                            & 95                                          & 59.85\%                             \\
\hline
\end{tabular}
\end{table*}




\begin{table*}[!h]


\centering
\caption{Cookie Syncing GDPR.}
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|} 
\hline
                   & \multicolumn{6}{c|}{\textbf{Cookiebot}}                                                                                                                                                                                                     & \multicolumn{6}{c|}{\textbf{Didomi}}                                                                                                                                                                                                        & \multicolumn{6}{c|}{\textbf{NAI}}                                                                                                                                                                                                           & \multicolumn{6}{c|}{\textbf{Onetrust}}                                                                                                                                                                                                      & \multicolumn{6}{c|}{\textbf{Quantcast}}                                                                                                                                                                                                      \\ 
\hline
{}                    & \multicolumn{1}{c|}{\textbf{Opt\_out}} & \multicolumn{1}{l|}{}              & \multicolumn{1}{c|}{\textbf{Opt\_in}} & \multicolumn{1}{l|}{}              & \multicolumn{1}{c|}{\textbf{Pre\_opt\_out}} & \multicolumn{1}{l|}{}              & \multicolumn{1}{c|}{\textbf{Opt\_out}} & \multicolumn{1}{l|}{}              & \multicolumn{1}{c|}{\textbf{Opt\_in}} & \multicolumn{1}{l|}{}              & \multicolumn{1}{c|}{\textbf{Pre\_opt\_out}} & \multicolumn{1}{l|}{}              & \multicolumn{1}{c|}{\textbf{Opt\_out}} & \multicolumn{1}{l|}{}              & \multicolumn{1}{c|}{\textbf{Opt\_in}} & \multicolumn{1}{l|}{}              & \multicolumn{1}{c|}{\textbf{Pre\_opt\_out}} & \multicolumn{1}{l|}{}              & \multicolumn{1}{c|}{\textbf{Opt\_out}} & \multicolumn{1}{l|}{}              & \multicolumn{1}{c|}{\textbf{Opt\_in}} & \multicolumn{1}{l|}{}              & \multicolumn{1}{c|}{\textbf{Pre\_opt\_out}} & \multicolumn{1}{l|}{}              & \multicolumn{1}{c|}{\textbf{Opt\_out}} & \multicolumn{1}{l|}{}              & \multicolumn{1}{c|}{\textbf{Opt\_in}} & \multicolumn{1}{l|}{}              & \multicolumn{1}{c|}{\textbf{Pre\_opt\_out}} & \multicolumn{1}{l|}{}               \\ 
\hline
{}Persona             & \multicolumn{1}{c|}{\textbf{Evt.}}     & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c|}{\textbf{Evt.}}    & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c|}{\textbf{Evt.}}          & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c|}{\textbf{Evt.}}     & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c|}{\textbf{Evt.}}    & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c|}{\textbf{Evt.}}          & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c|}{\textbf{Evt.}}     & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c|}{\textbf{Evt.}}    & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c|}{\textbf{Evt.}}          & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c|}{\textbf{Evt.}}     & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c|}{\textbf{Evt.}}    & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c|}{\textbf{Evt.}}          & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c|}{\textbf{Evt.}}     & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c|}{\textbf{Evt.}}    & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c|}{\textbf{Evt.}}          & \multicolumn{1}{c|}{\textbf{Pct.}}  \\ 
\hline
{}\textbf{Adult}      & 0                                      & 0.00\%                             & 25                                    & 25.00\%                            & 0                                           & 0.00\%                             & 0                                      & 0.00\%                             & 205                                   & 53.33\%                            & 6                                           & 100.00\%                           & 7                                      & 50.00\%                            & 0                                     & 0.00\%                             & 16                                          & 33.33\%                            & 19                                     & 100.00\%                           & 20                                    & 100.00\%                           & 19                                          & 100.00\%                           & 54                                     & 45.45\%                            & 204                                   & 68.75\%                            & 27                                          & 50.00\%                             \\ 
\hline
{}\textbf{Arts}       & 0                                      & 0.00\%                             & 7                                     & 25.00\%                            & 0                                           & 0.00\%                             & 1                                      & 100.00\%                           & 209                                   & 46.67\%                            & 0                                           & 0.00\%                             & 13                                     & 50.00\%                            & 0                                     & 0.00\%                             & 17                                          & 40.00\%                            & 0                                      & 0.00\%                             & 22                                    & 100.00\%                           & 29                                          & 100.00\%                           & 50                                     & 46.15\%                            & 210                                   & 64.71\%                            & 24                                          & 40.00\%                             \\ 
\hline
{}\textbf{Business}   & 0                                      & 0.00\%                             & 44                                    & 40.00\%                            & 0                                           & 0.00\%                             & 0                                      & 0.00\%                             & 232                                   & 53.33\%                            & 0                                           & 0.00\%                             & 22                                     & 66.67\%                            & 21                                    & 40.00\%                            & 11                                          & 25.00\%                            & 24                                     & 100.00\%                           & 49                                    & 100.00\%                           & 46                                          & 100.00\%                           & 43                                     & 42.86\%                            & 154                                   & 69.23\%                            & 26                                          & 57.14\%                             \\ 
\hline
{}\textbf{Computers}  & 0                                      & 0.00\%                             & 28                                    & 20.00\%                            & 0                                           & 0.00\%                             & 15                                     & 100.00\%                           & 276                                   & 64.71\%                            & 9                                           & 100.00\%                           & 11                                     & 50.00\%                            & 19                                    & 66.67\%                            & 29                                          & 40.00\%                            & 29                                     & 100.00\%                           & 38                                    & 100.00\%                           & 20                                          & 100.00\%                           & 52                                     & 40.00\%                            & 192                                   & 58.82\%                            & 37                                          & 66.67\%                             \\ 
\hline
{}\textbf{Games}      & 0                                      & 0.00\%                             & 27                                    & 25.00\%                            & 0                                           & 0.00\%                             & 17                                     & 100.00\%                           & 247                                   & 50.00\%                            & 8                                           & 100.00\%                           & 15                                     & 50.00\%                            & 0                                     & 0.00\%                             & 15                                          & 25.00\%                            & 16                                     & 100.00\%                           & 22                                    & 100.00\%                           & 30                                          & 100.00\%                           & 61                                     & 50.00\%                            & 180                                   & 62.50\%                            & 20                                          & 50.00\%                             \\ 
\hline
{}\textbf{Health}     & 0                                      & 0.00\%                             & 36                                    & 40.00\%                            & 0                                           & 0.00\%                             & 0                                      & 0.00\%                             & 223                                   & 47.06\%                            & 13                                          & 50.00\%                            & 5                                      & 50.00\%                            & 5                                     & 33.33\%                            & 5                                           & 25.00\%                            & 1                                      & 100.00\%                           & 25                                    & 100.00\%                           & 21                                          & 100.00\%                           & 37                                     & 46.15\%                            & 141                                   & 57.14\%                            & 12                                          & 60.00\%                             \\ 
\hline
{}\textbf{Home}       & 0                                      & 0.00\%                             & 3                                     & 20.00\%                            & 0                                           & 0.00\%                             & 0                                      & 0.00\%                             & 153                                   & 53.85\%                            & 0                                           & 0.00\%                             & 0                                      & 0.00\%                             & 0                                     & 0.00\%                             & 6                                           & 33.33\%                            & 15                                     & 100.00\%                           & 8                                     & 100.00\%                           & 46                                          & 100.00\%                           & 45                                     & 53.33\%                            & 135                                   & 57.14\%                            & 27                                          & 50.00\%                             \\ 
\hline
{}\textbf{Kids}       & 0                                      & 0.00\%                             & 41                                    & 33.33\%                            & 0                                           & 0.00\%                             & 2                                      & 100.00\%                           & 252                                   & 56.25\%                            & 15                                          & 100.00\%                           & 7                                      & 50.00\%                            & 14                                    & 66.67\%                            & 13                                          & 25.00\%                            & 12                                     & 50.00\%                            & 27                                    & 100.00\%                           & 34                                          & 100.00\%                           & 52                                     & 40.00\%                            & 175                                   & 66.67\%                            & 41                                          & 71.43\%                             \\ 
\hline
{}\textbf{News}       & 3                                      & 25.00\%                            & 22                                    & 25.00\%                            & 0                                           & 0.00\%                             & 0                                      & 0.00\%                             & 251                                   & 60.00\%                            & 0                                           & 0.00\%                             & 5                                      & 50.00\%                            & 2                                     & 25.00\%                            & 13                                          & 50.00\%                            & 8                                      & 100.00\%                           & 27                                    & 100.00\%                           & 21                                          & 100.00\%                           & 36                                     & 46.15\%                            & 163                                   & 66.67\%                            & 25                                          & 71.43\%                             \\ 
\hline
{}\textbf{Recreation} & 0                                      & 0.00\%                             & 6                                     & 25.00\%                            & 0                                           & 0.00\%                             & 2                                      & 100.00\%                           & 208                                   & 52.94\%                            & 0                                           & 0.00\%                             & 9                                      & 66.67\%                            & 6                                     & 25.00\%                            & 5                                           & 33.33\%                            & 7                                      & 100.00\%                           & 13                                    & 50.00\%                            & 4                                           & 100.00\%                           & 42                                     & 50.00\%                            & 176                                   & 66.67\%                            & 23                                          & 50.00\%                             \\ 
\hline
{}\textbf{Reference}  & 0                                      & 0.00\%                             & 24                                    & 25.00\%                            & 0                                           & 0.00\%                             & 0                                      & 0.00\%                             & 221                                   & 52.94\%                            & 0                                           & 0.00\%                             & 20                                     & 66.67\%                            & 13                                    & 33.33\%                            & 22                                          & 50.00\%                            & 11                                     & 100.00\%                           & 45                                    & 100.00\%                           & 34                                          & 100.00\%                           & 46                                     & 46.67\%                            & 191                                   & 62.50\%                            & 31                                          & 60.00\%                             \\ 
\hline
{}\textbf{Regional}   & 0                                      & 0.00\%                             & 52                                    & 50.00\%                            & 0                                           & 0.00\%                             & 0                                      & 0.00\%                             & 203                                   & 50.00\%                            & 0                                           & 0.00\%                             & 13                                     & 50.00\%                            & 14                                    & 66.67\%                            & 21                                          & 50.00\%                            & 33                                     & 100.00\%                           & 30                                    & 100.00\%                           & 34                                          & 80.00\%                            & 49                                     & 38.46\%                            & 138                                   & 53.33\%                            & 37                                          & 60.00\%                             \\ 
\hline
{}\textbf{Science}    & 0                                      & 0.00\%                             & 26                                    & 25.00\%                            & 0                                           & 0.00\%                             & 0                                      & 0.00\%                             & 246                                   & 56.25\%                            & 0                                           & 0.00\%                             & 5                                      & 50.00\%                            & 0                                     & 0.00\%                             & 10                                          & 40.00\%                            & 1                                      & 100.00\%                           & 13                                    & 100.00\%                           & 16                                          & 100.00\%                           & 40                                     & 42.86\%                            & 191                                   & 64.71\%                            & 16                                          & 71.43\%                             \\ 
\hline
{}\textbf{Shopping}   & 0                                      & 0.00\%                             & 50                                    & 42.86\%                            & 0                                           & 0.00\%                             & 0                                      & 0.00\%                             & 223                                   & 50.00\%                            & 7                                           & 100.00\%                           & 23                                     & 66.67\%                            & 18                                    & 33.33\%                            & 16                                          & 25.00\%                            & 14                                     & 100.00\%                           & 14                                    & 100.00\%                           & 41                                          & 100.00\%                           & 47                                     & 45.45\%                            & 139                                   & 61.54\%                            & 25                                          & 66.67\%                             \\ 
\hline
{}\textbf{Society}    & 0                                      & 0.00\%                             & 5                                     & 20.00\%                            & 0                                           & 0.00\%                             & 0                                      & 0.00\%                             & 204                                   & 50.00\%                            & 0                                           & 0.00\%                             & 0                                      & 0.00\%                             & 0                                     & 0.00\%                             & 7                                           & 40.00\%                            & 10                                     & 100.00\%                           & 21                                    & 100.00\%                           & 54                                          & 100.00\%                           & 35                                     & 42.86\%                            & 126                                   & 69.23\%                            & 21                                          & 50.00\%                             \\ 
\hline
{}\textbf{Sports}     & 0                                      & 0.00\%                             & 43                                    & 40.00\%                            & 0                                           & 0.00\%                             & 3                                      & 100.00\%                           & 218                                   & 56.25\%                            & 0                                           & 0.00\%                             & 1                                      & 50.00\%                            & 0                                     & 0.00\%                             & 1                                           & 25.00\%                            & 20                                     & 100.00\%                           & 54                                    & 83.33\%                            & 41                                          & 100.00\%                           & 37                                     & 37.50\%                            & 189                                   & 64.71\%                            & 27                                          & 50.00\%                             \\ 
\hline
\textbf{Average}                                        & 0                                      & 1.56\%                             & 27                                    & 30.07\%                            & 0                                           & 0.00\%                             & 3                                      & 37.50\%                            & 223                                   & 53.35\%                            & 4                                           & 34.38\%                            & 10                                     & 47.92\%                            & 7                                     & 24.38\%                            & 13                                          & 35.00\%                            & 14                                     & 90.63\%                            & 27                                    & 95.83\%                            & 31                                          & 98.75\%                            & 45                                     & 44.62\%                            & 169                                   & 63.39\%                            & 26                                          & 57.80\%                             \\
\hline
\end{tabular}
\end{table*}

==> docs/pre-opt-out-interval.tex <==
\begin{table*}
\footnotesize
%\adjustbox{max width=\textwidth}{
    \centering
    \caption{\textcolor{blue}{Ad bidding under GDPR in Germany after 1 month since pre-opt-out and training. Avg. column represents the mean of all bid value. Std. represents the standard deviation of all bid value. Pre-opt-out represents the bids when we opt-out the usage of user data before we stimulate the persona, respectively.  Color \textcolor{pink}{pink} and \textcolor{cyan}{cyan} indicate bid values that are higher and lower than Control's avg., respectively. Color \textcolor{red}{red} and \textcolor{blue}{blue} indicate bid values that are Control's avg. $\pm$ std., respectively. --- represents the absence of bids.}}







\begin{tabular}{l?{0.3mm}ll?{0.3mm}ll?{0.3mm}ll?{0.3mm}ll|ll} 
    \toprule
                    & \multicolumn{10}{c}{\textbf{GDPR}}                                                                                                                                                                                                                                                                                                                                              \\ 

     & \multicolumn{2}{c?{0.3mm}}{\textbf{Cookiebot}} & \multicolumn{2}{c?{0.3mm}}{\textbf{Didomi}}& \multicolumn{2}{c?{0.3mm}}{\textbf{NAI}}&
     \multicolumn{2}{c?{0.3mm}}{\textbf{Onetrust}}& \multicolumn{2}{c}{\textbf{Quantcast}}      \\  

    \textbf{Persona}     & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c}{\textbf{Std.}} \\ 
    \toprule
\textbf{Adult}      & 0.48 {\cellcolor{cyan}}                                    & 0.17 & 0.07   {\cellcolor{pink}}                                                                             & 0.04 & 0.01    {\cellcolor{cyan}}                                 & 0.02 & 0.29    {\cellcolor{blue}}                                                                       & 0.22 & 0.17   {\cellcolor{pink}}                                                                                   & 0.11  \\
\textbf{Arts}       & 0.44   {\cellcolor{cyan}}                                  & 0.22 & 0.06   {\cellcolor{cyan}}                                  & 0.05 & 0.02    {\cellcolor{pink}}                                                                                  & 0.07 & 0.02  {\cellcolor{blue}}                                                                         & 0.00 & 0.16    {\cellcolor{cyan}}                                 & 0.09  \\
\textbf{Business}   & 0.44  {\cellcolor{cyan}}                                   & 0.22 & 0.07    {\cellcolor{pink}}                                                                                  & 0.04 & 0.01  {\cellcolor{pink}}                                                                                    & 0.04 & 0.09{\cellcolor{blue}}                                                                           & 0.13 & 0.16   {\cellcolor{cyan}}                                  & 0.10  \\
\textbf{Computers}  & 0.44 {\cellcolor{cyan}}                                    & 0.22 & 0.07 {\cellcolor{cyan}}                                    & 0.05 & 0.01   {\cellcolor{pink}}                                                                                   & 0.05 & 0.16    {\cellcolor{blue}}                                                                       & 0.25 & 0.16    {\cellcolor{cyan}}                                 & 0.10  \\
\textbf{Games}      & 0.44  {\cellcolor{cyan}}                                   & 0.22 & 0.07   {\cellcolor{pink}}                                                                                   & 0.04 & 0.02 {\cellcolor{pink}}                                                                                     & 0.06 & 0.07  {\cellcolor{blue}}                                                                         & 0.02 & 0.17   {\cellcolor{pink}}                                                                                   & 0.12  \\
\textbf{Health}     & 0.47    {\cellcolor{cyan}}                                 & 0.14 & 0.06 {\cellcolor{cyan}}                                    & 0.05 & 0.02  {\cellcolor{pink}}                                                                                    & 0.08 & 0.15  {\cellcolor{blue}}                                                                         & 0.15 & 0.22 {\cellcolor{pink}}                                                                                     & 0.83  \\
\textbf{Home}       & 0.36  {\cellcolor{cyan}}                                   & 0.26 & 0.07  {\cellcolor{cyan}}                                   & 0.05 & 3.81E-03  {\cellcolor{cyan}}                               & 0.02 & 0.05   {\cellcolor{blue}}                                                                        & 0.00 & 0.17  {\cellcolor{pink}}                                                                                    & 0.10  \\
\textbf{Kids}       & 0.48    {\cellcolor{cyan}}                                 & 0.17 & 0.07     {\cellcolor{cyan}}                                & 0.05 & 0.02   {\cellcolor{pink}}                                                                                   & 0.04 & 0.10   {\cellcolor{blue}}                                                                        & 0.00 & 0.18  {\cellcolor{pink}}                                                                                    & 0.26  \\
\textbf{News}       & 0.44   {\cellcolor{cyan}}                                  & 0.22 & 0.07  {\cellcolor{cyan}}                                   & 0.05 & 0.03  {\cellcolor{pink}}                                                                                    & 0.13 & 0.33          & 0.00 & 0.16  {\cellcolor{cyan}}                                   & 0.10  \\
\textbf{Recreation} & 0.48   {\cellcolor{cyan}}                                  & 0.17 & 0.06    {\cellcolor{cyan}}                                 & 0.05 & 0.01   {\cellcolor{pink}}                                                                                   & 0.06 & --            & --   & 0.16     {\cellcolor{cyan}}                                & 0.10  \\
\textbf{Reference}  & 0.44   {\cellcolor{cyan}}                                  & 0.22 & 0.07   {\cellcolor{cyan}}                                  & 0.05 & 2.71E-03  {\cellcolor{cyan}}                               & 0.01 & 0.03  {\cellcolor{blue}}                                                                         & 0.00 & 0.16    {\cellcolor{cyan}}                                 & 0.10  \\
\textbf{Regional}   & 0.48   {\cellcolor{cyan}}                                  & 0.17 & 0.06    {\cellcolor{cyan}}                                 & 0.05 & 0.02  {\cellcolor{pink}}                                                                                    & 0.05 & 0.05   {\cellcolor{blue}}                                                                        & 0.03 & 0.17  {\cellcolor{pink}}                                                                                    & 0.14  \\
\textbf{Science}    & 0.40    {\cellcolor{cyan}}                                 & 0.24 & 0.07  {\cellcolor{cyan}}                                   & 0.05 & 1.64E-03 {\cellcolor{cyan}}                                & 0.01 & 0.17  {\cellcolor{blue}}                                                                         & 0.12 & 0.16   {\cellcolor{cyan}}                                  & 0.09  \\
\textbf{Shopping}   & 0.40    {\cellcolor{cyan}}                                 & 0.24 & 0.07     {\cellcolor{cyan}}                                & 0.05 & 0.02   {\cellcolor{pink}}                                                                                   & 0.08 & 0.12  {\cellcolor{blue}}                                                                         & 0.22 & 0.17   {\cellcolor{pink}}                                                                                   & 0.13  \\
\textbf{Society}    & 0.13  {\cellcolor{blue}}                                                                         & 0.23 & 0.03   {\cellcolor{cyan}}                                  & 0.01 & 3.17E-03  {\cellcolor{cyan}}                               & 0.02 & 0.19         {\cellcolor{blue}}                                                                  & 0.16 & 0.15    {\cellcolor{cyan}}                                 & 0.08  \\
\textbf{Sports}     & 0.41    {\cellcolor{cyan}}                                 & 0.24 & 0.06   {\cellcolor{cyan}}                                  & 0.05 & 0.01   {\cellcolor{cyan}}                                  & 0.03 & 0.05 {\cellcolor{blue}}                                                                          & 0.02 & 0.17  {\cellcolor{pink}}                                                                                    & 0.11  \\

\midrule
\textbf{Control}    & 0.48          & 0.17 & 0.07          & 0.07 & 0.01          & 0.03 & 0.33          & 0.00 & 0.17          & 0.10 \\

\bottomrule
\end{tabular}
\label{table:GDPR-bidding-mean-pre-opt-out-interval}
\end{table*}


\begin{table*}
\footnotesize
%\adjustbox{max width=\textwidth}{
    \centering
    \caption{\textcolor{blue}{Ad bidding under CCPA in California after 1 month since pre-opt-out and training. Avg. column represents the mean of all bid value. Std. represents the standard deviation of all bid value. Pre-opt-out represents the bids when we opt-out the usage of user data before we stimulate the persona, respectively.  Color \textcolor{pink}{pink} and \textcolor{cyan}{cyan} indicate bid values that are higher and lower than Control's avg., respectively. Color \textcolor{red}{red} and \textcolor{blue}{blue} indicate bid values that are Control's avg. $\pm$ std., respectively. --- represents the absence of bids.}}







\begin{tabular}{l?{0.3mm}ll?{0.3mm}ll?{0.3mm}ll?{0.3mm}ll|ll} 
    \toprule
                    & \multicolumn{10}{c}{\textbf{CCPA}}                                                                                                                                                                                                                                                                                                                                              \\ 

     & \multicolumn{2}{c?{0.3mm}}{\textbf{Cookiebot}} & \multicolumn{2}{c?{0.3mm}}{\textbf{Didomi}}& \multicolumn{2}{c?{0.3mm}}{\textbf{NAI}}&
     \multicolumn{2}{c?{0.3mm}}{\textbf{Onetrust}}& \multicolumn{2}{c}{\textbf{Quantcast}}      \\  

    \textbf{Persona}     & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c}{\textbf{Std.}} \\ 
    \toprule
\textbf{Adult}      & 0.53   {\cellcolor{pink}}                                                                                           & 0.57 & 0.08  {\cellcolor{cyan}}                                                                                                  & 0.11 & 0.08  {\cellcolor{cyan}}                                                                                                         & 0.19 & 1.07          {\cellcolor{pink}}                                                                                    & 1.24 & 0.17   {\cellcolor{cyan}}                                                                                                        & 0.19  \\
\textbf{Arts}       & 0.40  {\cellcolor{pink}}                                                                                            & 0.24 & 0.18  {\cellcolor{cyan}}                                                                                                         & 0.31 & 0.06  {\cellcolor{cyan}}                                                                                                         & 0.08 & 1.20          {\cellcolor{pink}}                                                                                    & 1.38 & 0.19   {\cellcolor{cyan}}                                                                                                        & 0.19  \\
\textbf{Business}   & 0.42   {\cellcolor{pink}}                                                                                           & 0.20 & 0.16   {\cellcolor{cyan}}                                                                                                        & 0.26 & 0.09    {\cellcolor{pink}}                                                                                          & 0.23 & 1.08   {\cellcolor{pink}}                                                                                           & 1.35 & 0.21   {\cellcolor{cyan}}                                                                                                        & 0.33  \\
\textbf{Computers}  & 0.25   {\cellcolor{cyan}}                                                                                                        & 0.27 & 0.16    {\cellcolor{cyan}}                                                                                                       & 0.53 & 0.12   {\cellcolor{pink}}                                                                                           & 0.24 & 0.83   {\cellcolor{cyan}}                                                                                                        & 1.10 & 0.21   {\cellcolor{cyan}}                                                                                                        & 0.46  \\
\textbf{Games}      & 0.32    {\cellcolor{pink}}                                                                                          & 0.24 & 0.24   {\cellcolor{pink}}                                                                                           & 0.68 & 0.10    {\cellcolor{pink}}                                                                                          & 0.22 & 0.98     {\cellcolor{cyan}}                                                                                                      & 1.24 & 0.19     {\cellcolor{cyan}}                                                                                                      & 0.43  \\
\textbf{Health}     & 0.37     {\cellcolor{pink}}                                                                                         & 0.21 & 0.23    {\cellcolor{pink}}                                                                                          & 0.61 & 0.04    {\cellcolor{cyan}}                                                                                                       & 0.08 & 1.15     {\cellcolor{pink}}                                                                                         & 1.32 & 0.23    {\cellcolor{cyan}}                                                                                                       & 0.51  \\
\textbf{Home}       & 0.24     {\cellcolor{cyan}}                                                                                                      & 0.26 & 0.10    {\cellcolor{cyan}}                                                                                                       & 0.16 & 0.07    {\cellcolor{cyan}}                                                                                                       & 0.16 & 1.13  {\cellcolor{pink}}                                                                                            & 1.27 & 0.18    {\cellcolor{cyan}}                                                                                                       & 0.13  \\
\textbf{Kids}       & 0.41  {\cellcolor{pink}}                                                                                            & 0.21 & 0.14  {\cellcolor{cyan}}                                                                                                         & 0.18 & 0.03    {\cellcolor{cyan}}                                                                                                       & 0.08 & 1.06          {\cellcolor{pink}}                                                                                    & 1.20 & 0.21   {\cellcolor{cyan}}                                                                                                        & 0.30  \\
\textbf{News}       & 0.29    {\cellcolor{pink}}                                                                                          & 0.27 & 0.11 {\cellcolor{cyan}}                                                                                                          & 0.11 & 0.07   {\cellcolor{cyan}}                                                                                                        & 0.16 & 0.75  {\cellcolor{cyan}}                                                                                                         & 1.11 & 0.23    {\cellcolor{pink}}                                                                                          & 0.50  \\
\textbf{Recreation} & 0.40  {\cellcolor{pink}}                                                                                            & 0.20 & 0.14   {\cellcolor{cyan}}                                                                                                        & 0.29 & 0.08   {\cellcolor{cyan}}                                                                                                        & 0.12 & 1.16          {\cellcolor{pink}}                                                                                    & 1.56 & 0.24   {\cellcolor{pink}}                                                                                           & 0.57  \\
\textbf{Reference}  & 0.30   {\cellcolor{pink}}                                                                                           & 0.29 & 0.17    {\cellcolor{cyan}}                                                                                                       & 0.48 & 0.11  {\cellcolor{pink}}                                                                                            & 0.23 & 0.87   {\cellcolor{cyan}}                                                                                                        & 1.23 & 0.17 {\cellcolor{cyan}}                                                                                                          & 0.20  \\
\textbf{Regional}   & 0.34   {\cellcolor{pink}}                                                                                           & 0.26 & 0.10   {\cellcolor{cyan}}                                                                                                        & 0.14 & 0.08    {\cellcolor{cyan}}                                                                                                       & 0.19 & 1.24          {\cellcolor{pink}}                                                                                    & 1.61 & 0.26    {\cellcolor{pink}}                                                                                          & 0.61  \\
\textbf{Science}    & 0.26   {\cellcolor{cyan}}                                                                                                        & 0.27 & 0.14   {\cellcolor{cyan}}                                                                                                        & 0.44 & 0.06    {\cellcolor{cyan}}                                                                                                       & 0.17 & 0.78     {\cellcolor{cyan}}                                                                                                      & 1.07 & 0.23   {\cellcolor{pink}}                                                                                           & 0.49  \\
\textbf{Shopping}   & 0.31    {\cellcolor{pink}}                                                                                          & 0.27 & 0.19 {\cellcolor{cyan}}                                                                                                          & 0.54 & 0.08 {\cellcolor{cyan}}                                                                                                          & 0.22 & 1.00  {\cellcolor{cyan}}                                                                                                         & 1.17 & 0.20   {\cellcolor{cyan}}                                                                                                        & 0.24  \\
\textbf{Society}    & 0.32    {\cellcolor{pink}}                                                                                          & 0.26 & 0.07   {\cellcolor{cyan}}                                                                                                        & 0.07 & 0.06  {\cellcolor{cyan}}                                                                                                         & 0.08 & 1.02          {\cellcolor{pink}}                                                                                    & 1.28 & 0.23  {\cellcolor{cyan}}                                                                                                         & 0.64  \\
\textbf{Sports}     & 0.23   {\cellcolor{cyan}}                                                                                                        & 0.27 & 0.14   {\cellcolor{cyan}}                                                                                                        & 0.22 & 0.10    {\cellcolor{pink}}                                                                                          & 0.16 & 1.08    {\cellcolor{pink}}                                                                                          & 1.30 & 0.15  {\cellcolor{cyan}}                                                                                                         & 0.10  \\

\midrule
\textbf{Control}    & 0.28          & 0.27 & 0.22          & 0.54 & 0.08          & 0.15 & 1.01          & 1.12 & 0.23          & 0.62 \\

\bottomrule
\end{tabular}
\label{table:CCPA-bidding-mean-pre-opt-out-interval}
\end{table*}


==> docs/stats-test-table-new.tex <==
%\begin{table*}
%\centering
%\caption{\textcolor{blue}{Mann–Whitney U test to validate our hypothesis that the advertisers bidding behavior does not significantly change between opt-in and opt-out under GDPR. Column P and R represent p-value and effect size, respectively. Effect size is calculated only in cases when there is statistically significant difference (when p-value is smaller than 0.003125 after bonferroni correction). Otherwise, we use ``--'' in the table, to represent that we do not calculate this effect size.}}
%\begin{tabular}{l?{0.3mm}ll|ll|ll|ll|ll} 
%    \toprule
%
%
%\multicolumn{1}{c?{0.3mm}}{\multirow{2}{*}{\textbf{Persona}}}                       & \multicolumn{2}{c}{\textbf{Cookiebot}}                            & \multicolumn{2}{c}{\textbf{Didomi}}                           &  \multicolumn{2}{c}{\textbf{OneTrust}}                            & \multicolumn{2}{c}{\textbf{Quantcast}}                           & \multicolumn{2}{c}{\textbf{NAI}}                                  \\ 
%
%\multicolumn{1}{c?{0.3mm}}{}                         & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{E}} & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{E}} & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{E}} & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{E}} & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c}{\textbf{E}} \\ 
%\midrule
%\textbf{Adult}      & 0.115              & --         & 0.000           & inf        & 0.500             & --         & 0.019              & 0.073      & 0.430        & --          \\
%\textbf{Arts}       & 0.165              & --         & 0.375           & --         & 0.000             & inf        & 0.017              & 0.071      & 0.281        & --          \\
%\textbf{Business}   & 0.489              & --         & 0.000           & inf        & 0.018             & 0.423      & 6.11E-05              & 0.133      & 0.170        & --          \\
%\textbf{Computers}  & 0.232              & --         & 0.394           & --         & 0.126             & --         & 0.051              & --         & 0.374        & --          \\
%\textbf{Games}      & 0.464              & --         & 0.157           & --         & 0.500             & --         & 0.005              & 0.087      & 0.130        & --          \\
%\textbf{Health}     & 0.398              & --         & 0.000           & inf        & 0.007             & 0.775      & 0.124              & --         & 0.434        & --          \\
%\textbf{Home}       & 0.047              & --         & 0.465           & --         & 0.157             & --         & 0.263              & --         & --           & --          \\
%\textbf{Kids}       & 0.146              & --         & 0.470           & --         & 0.039             & --         & 0.172              & --         & 0.405        & --          \\
%\textbf{News}       & 0.144              & --         & 0.000           & inf        & 0.020             & 0.640      & 0.001              & 0.112      & 0.343        & --          \\
%\textbf{Recreation} & 0.277              & --         & 0.351           & --         & 0.001             & 0.812      & 0.005              & 0.092      & 0.439        & --          \\
%\textbf{Reference}  & 0.115              & --         & 0.000           & inf        & 0.192             & --         & 0.366              & --         & 0.099        & --          \\
%\textbf{Regional}   & 0.146              & --         & 0.000           & inf        & 0.152             & --         & 1.39E-05              & 0.144      & 0.116        & --          \\
%\textbf{Science}    & 0.092              & --         & 0.070           & --         & 0.109             & --         & 0.086              & --         & 0.262        & --          \\
%\textbf{Shopping}   & 0.458              & --         & 0.452           & --         & 0.240             & --         & 2.43E-04              & 0.135      & 0.304        & --          \\
%\textbf{Society}    & 0.495              & --         & 0.412           & --         & 0.140             & --         & 0.093              & --         & 0.089        & --          \\
%\textbf{Sports}     & 0.274              & --         & 0.499           & --         & 0.010             & 0.469      & 8.60E-05             & 0.128      & 0.215        & --       \\  
%
%\bottomrule
%\end{tabular}
%
%\label{table:u-test-gdpr}
%\end{table*}
%
%
%
%\begin{table*}
%\centering
%\caption{\textcolor{blue}{Mann–Whitney U test to validate our hypothesis that the advertisers bidding behavior does not significantly change between opt-in and opt-out under CCPA. Column P and R represent p-value and effect size, respectively. Effect size is calculated only in cases when there is statistically significant difference (when p-value is smaller than 0.003125 after bonferroni correction). Otherwise, we use ``--'' in the table, to represent that we do not calculate this effect size.}}
%\begin{tabular}{l?{0.3mm}ll|ll|ll|ll|ll} 
%    \toprule
%
%
%\multicolumn{1}{c?{0.3mm}}{\multirow{2}{*}{\textbf{Persona}}}                       & \multicolumn{2}{c}{\textbf{Cookiebot}}                            & \multicolumn{2}{c}{\textbf{Didomi}}                           &  \multicolumn{2}{c}{\textbf{OneTrust}}                            & \multicolumn{2}{c}{\textbf{Quantcast}}                           & \multicolumn{2}{c}{\textbf{NAI}}                                  \\ 
%
%\multicolumn{1}{c?{0.3mm}}{}                         & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{E}} & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{E}} & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{E}} & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{E}} & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c}{\textbf{E}} \\ 
%\midrule
%\textbf{Adult}      & 0.165     & --    & 4.70E-08  & 0.204 & 1.42E-07    & 0.354 & 4.17E-04     & 0.121 & 0.305 & --     \\
%\textbf{Arts}       & 0.040     & --    & 3.93E-19  & 0.309 & 0.289    & --    & 0.323     & --    & 0.008 & 0.154  \\
%\textbf{Business}   & 0.193     & --    & 2.39E-13  & 0.260 & 3.41E-12    & 0.496 & 0.115     & --    & 0.014 & 0.136  \\
%\textbf{Computers}  & 0.032     & --    & 2.61E-18  & 0.287 & 0.282    & --    & 0.311     & --    & 0.136 & --     \\
%\textbf{Games}      & 0.008     & 0.153 & 2.26E-11  & 0.245 & 0.030    & --    & 4.23E-04     & 0.109 & 0.014 & 0.136  \\
%\textbf{Health}     & 0.335     & --    & 1.17E-12  & 0.234 & 4.84E-07    & 0.310 & 0.025     & --    & 0.119 & --     \\
%\textbf{Home}       & 0.283     & --    & 5.74E-15  & 0.290 & 0.139    & --    & 0.004     & 0.093 & 0.407 & --     \\
%\textbf{Kids}       & 0.020     & 0.127 & 1.36E-06  & 0.154 & 7.40E-06    & 0.226 & 0.323     & --    & 0.118 & --     \\
%\textbf{News}       & 0.132     & --    & 2.49E-11  & 0.226 & 0.041    & --    & 0.039     & --    & 0.037 & --     \\
%\textbf{Recreation} & 0.107     & --    & 2.43E-13  & 0.270 & 2.24E-12    & 0.389 & 0.175     & --    & 0.010 & 0.166  \\
%\textbf{Reference}  & 0.056     & --    & 1.09E-10  & 0.226 & 2.31E-06    & 0.265 & 0.026     & --    & 0.003 & 0.175  \\
%\textbf{Regional}   & 0.058     & --    & 1.19E-28  & 0.372 & 3.78E-12    & 0.430 & 0.366     & --    & 0.493 & --     \\
%\textbf{Science}    & 0.139     & --    & 5.45E-15  & 0.265 & 0.010    & 0.170 & 0.004     & 0.097 & 0.223 & --     \\
%\textbf{Shopping}   & 0.318     & --    & 8.33E-13  & 0.233 & 0.036    & --    & 0.250     & --    & 0.496 & --     \\
%\textbf{Society}    & 0.082     & --    & 1.51E-13  & 0.261 & 1.14E-06    & 0.366 & 0.126     & --    & 0.014 & 0.145  \\
%\textbf{Sports}     & 0.486     & --    & 1.54E-13  & 0.233 & 0.038    & --    & 0.137     & --    & 0.015 & 0.148  \\
%
%
%\bottomrule
%\end{tabular}
%
%\label{table:u-test-ccpa}
%\end{table*}



\begin{table*}
\centering
\caption{\textcolor{blue}{Mann–Whitney U test to validate our hypothesis that the advertisers bidding behavior does not significantly change between opt-in and opt-out under GDPR. Column P and R represent p-value and effect size, respectively. Effect size is calculated only in cases when there is statistically significant difference (when p-value is smaller than 0.05 after bonferroni correction). Otherwise, we use ``--'' in the table, to represent that we do not calculate this effect size.}}
\begin{tabular}{l?{0.3mm}ll|ll|ll|ll|ll} 
    \toprule


\multicolumn{1}{c?{0.3mm}}{\multirow{2}{*}{\textbf{Persona}}}                       & \multicolumn{2}{c}{\textbf{Didomi}}                            & \multicolumn{2}{c}{\textbf{Quantcast}}                           &  \multicolumn{2}{c}{\textbf{OneTrust}}                            & \multicolumn{2}{c}{\textbf{Cookiebot}}                           & \multicolumn{2}{c}{\textbf{NAI}}                                  \\ 

\multicolumn{1}{c?{0.3mm}}{}                         & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{E}} & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{E}} & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{E}} & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{E}} & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c}{\textbf{E}} \\ 
\midrule
\textbf{Adult}      & 0.000 & inf      & 0.307    & 0.073 & 8.000 & 0.000 & 1.847 & 0.078 & 6.883 & 0.004  \\
\textbf{Arts}       & 5.996 & 0.011    & 0.271    & 0.071 & 0.000 & inf   & 2.645 & 0.063 & 4.498 & 0.022  \\
\textbf{Business}   & 0.000 & inf      & 0.001    & 0.133 & 0.284 & 0.423 & 7.822 & 0.002 & 2.719 & 0.039  \\
\textbf{Computers}  & 6.309 & 0.008    & 0.814    & 0.055 & 2.009 & 0.278 & 3.713 & 0.046 & 5.986 & 0.010  \\
\textbf{Games}      & 2.520 & 0.030    & 0.083    & 0.087 & 8.000 & 0.000 & 7.423 & 0.006 & 2.083 & 0.019  \\
\textbf{Health}     & 0.000 & inf      & 1.980    & 0.040 & 0.111 & 0.775 & 6.375 & 0.016 & 6.938 & 0.007  \\
\textbf{Home}       & 7.436 & 0.003    & 4.204    & 0.022 & 2.520 & 0.366 & 0.751 & 0.107 & --    & --     \\
\textbf{Kids}       & 7.522 & 0.003    & 2.758    & 0.032 & 0.619 & 0.439 & 2.331 & 0.068 & 6.484 & 0.009  \\
\textbf{News}       & 0.000 & inf      & 0.022    & 0.112 & 0.318 & 0.640 & 2.310 & 0.068 & 5.484 & 0.011  \\
\textbf{Recreation} & 5.615 & 0.012    & 0.085    & 0.092 & 0.018 & 0.812 & 4.431 & 0.039 & 7.024 & 0.006  \\
\textbf{Reference}  & 0.000 & inf      & 5.863    & 0.012 & 3.069 & 0.306 & 1.846 & 0.078 & 1.583 & 0.047  \\
\textbf{Regional}   & 0.000 & inf      & 2.22E-04 & 0.144 & 2.431 & 0.244 & 2.336 & 0.068 & 1.857 & 0.044  \\
\textbf{Science}    & 1.122 & 0.041    & 1.383    & 0.044 & 1.750 & 0.422 & 1.477 & 0.085 & 4.190 & 0.022  \\
\textbf{Shopping}   & 7.232 & 0.004    & 0.004    & 0.135 & 3.836 & 0.354 & 7.328 & 0.007 & 4.864 & 0.021  \\
\textbf{Society}    & 6.585 & 0.007    & 1.483    & 0.047 & 2.232 & 0.248 & 7.926 & 0.001 & 1.416 & 0.038  \\
\textbf{Sports}     & 7.978 & 1.08E-04 & 0.001    & 0.128 & 0.155 & 0.469 & 4.392 & 0.040 & 3.435 & 0.030  \\  

\bottomrule
\end{tabular}

\label{table:u-test-gdpr}
\end{table*}



\begin{table*}
\centering
\caption{\textcolor{blue}{Mann–Whitney U test to validate our hypothesis that the advertisers bidding behavior does not significantly change between opt-in and opt-out under CCPA. Column P and R represent p-value and effect size, respectively. Effect size is calculated only in cases when there is statistically significant difference (when p-value is smaller than 0.05 after bonferroni correction). Otherwise, we use ``--'' in the table, to represent that we do not calculate this effect size.}}
\begin{tabular}{l?{0.3mm}ll|ll|ll|ll|ll} 
    \toprule


\multicolumn{1}{c?{0.3mm}}{\multirow{2}{*}{\textbf{Persona}}}                       & \multicolumn{2}{c}{\textbf{Didomi}}                            & \multicolumn{2}{c}{\textbf{Quantcast}}                           &  \multicolumn{2}{c}{\textbf{OneTrust}}                            & \multicolumn{2}{c}{\textbf{Cookiebot}}                           & \multicolumn{2}{c}{\textbf{NAI}}                                  \\ 

\multicolumn{1}{c?{0.3mm}}{}                         & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{E}} & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{E}} & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{E}} & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{E}} & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c}{\textbf{E}} \\ 
\midrule
\textbf{Adult}      & 7.52E-07 & 0.204 & 0.007 & 0.121 & 2.27E-06 & 0.354 & 2.641 & 0.063 & 4.887 & 0.034  \\
\textbf{Arts}       & 6.28E-18 & 0.309 & 5.166 & 0.016 & 4.628    & 0.053 & 0.644 & 0.112 & 0.127 & 0.154  \\
\textbf{Business}   & 3.83E-12 & 0.260 & 1.839 & 0.042 & 5.46E-11 & 0.496 & 3.084 & 0.056 & 0.226 & 0.136  \\
\textbf{Computers}  & 4.17E-17 & 0.287 & 4.979 & 0.017 & 4.504    & 0.052 & 0.513 & 0.120 & 2.173 & 0.066  \\
\textbf{Games}      & 3.62E-10 & 0.245 & 0.007 & 0.109 & 0.473    & 0.106 & 0.136 & 0.153 & 0.218 & 0.136  \\
\textbf{Health}     & 1.86E-11 & 0.234 & 0.407 & 0.065 & 7.74E-06 & 0.310 & 5.359 & 0.028 & 1.901 & 0.079  \\
\textbf{Home}       & 9.18E-14 & 0.290 & 0.057 & 0.093 & 2.230    & 0.098 & 4.527 & 0.037 & 6.508 & 0.015  \\
\textbf{Kids}       & 2.17E-05 & 0.154 & 5.162 & 0.016 & 1.18E-04 & 0.226 & 0.323 & 0.127 & 1.886 & 0.075  \\
\textbf{News}       & 3.98E-10 & 0.226 & 0.620 & 0.067 & 0.657    & 0.099 & 2.119 & 0.071 & 0.595 & 0.114  \\
\textbf{Recreation} & 3.89E-12 & 0.270 & 2.805 & 0.034 & 3.58E-11 & 0.389 & 1.705 & 0.083 & 0.156 & 0.166  \\
\textbf{Reference}  & 1.74E-09 & 0.226 & 0.419 & 0.070 & 3.69E-05 & 0.265 & 0.890 & 0.102 & 0.049 & 0.175  \\
\textbf{Regional}   & 1.90E-27 & 0.372 & 5.855 & 0.012 & 6.05E-11 & 0.430 & 0.934 & 0.100 & 7.888 & 0.001  \\
\textbf{Science}    & 8.71E-14 & 0.265 & 0.061 & 0.097 & 0.161    & 0.170 & 2.218 & 0.070 & 3.562 & 0.040  \\
\textbf{Shopping}   & 1.33E-11 & 0.233 & 4.004 & 0.023 & 0.574    & 0.101 & 5.083 & 0.030 & 7.942 & 0.001  \\
\textbf{Society}    & 2.42E-12 & 0.261 & 2.017 & 0.041 & 1.83E-05 & 0.366 & 1.309 & 0.091 & 0.229 & 0.145  \\
\textbf{Sports}     & 2.46E-12 & 0.233 & 2.192 & 0.038 & 0.605    & 0.104 & 7.779 & 0.002 & 0.243 & 0.148  \\


\bottomrule
\end{tabular}

\label{table:u-test-ccpa}
\end{table*}

==> docs/stats-test-table.tex <==
\begin{table*}
\centering
\caption{Mann–Whitney U test to validate our hypothesis that the advertisers bidding behavior does not significantly change between opt-in and opt-out. Column P and R represent p-value and effect size, respectively. Effect size is calculated only in cases when there is statistically significant difference (when p-value is smaller than 0.05). Otherwise, we use ``--'' in the table, to represent that we do not calculate this effect size.}
\begin{tabular}{l?{0.3mm}rr|rr|rr?{0.3mm}rr|rr|rr} 
    \toprule
\multicolumn{1}{c?{0.3mm}}{\multirow{3}{*}{\textbf{Persona}}} & \multicolumn{6}{c?{0.3mm}}{\textbf{GDPR}}                                                                                                                                                                        & \multicolumn{6}{c}{\textbf{CCPA}}                                                                                                                                                                         \\ 

\multicolumn{1}{c?{0.3mm}}{}                         & \multicolumn{2}{c}{\textbf{OneTrust}}                            & \multicolumn{2}{c}{\textbf{CookieBot}}                           & \multicolumn{2}{c?{0.3mm}}{\textbf{NAI}}                                 & \multicolumn{2}{c}{\textbf{OneTrust}}                            & \multicolumn{2}{c}{\textbf{CookieBot}}                           & \multicolumn{2}{c}{\textbf{NAI}}                                  \\ 

\multicolumn{1}{c?{0.3mm}}{}                         & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{E}} & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{E}} & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c?{0.3mm}}{\textbf{E}} & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{E}} & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{E}} & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c}{\textbf{E}}  \\ 
\midrule
\textbf{Adult}                                          & 0.00                   & 0.29                   & 0.20                   & --                   & 0.34                   & --                   & 0.18                   & --                   & 0.00                   & 0.20                   & 0.34                   & --                    \\ 

\textbf{Arts}                                           & 0.13                   & -- & 0.91                   & --                   & 0.10                   & - & 0.68                   & --                   & 0.95                   & --                   & 0.10                   & --                    \\ 

\textbf{Business}                                       & 0.00                   & 0.53                   & 0.01                   & 0.47                   & 0.97                   & --                   & 0.03                   & 0.12                   & 0.00                   & 0.28                   & 0.97                   & --                   \\ 

\textbf{Computers}                                      & 0.00                   & 0.40                   & 0.71                   & --                   & 0.01                   & 0.11                   & 0.85                   & --                   & 0.85                   & --                   & 0.01                   & 0.11                    \\ 

\textbf{Games}                                          & 0.33                   & --                   & 0.32                   & --                                     & 0.00                   & 0.12                   & 0.26                   & --                                     & 0.05                   & 0.12                   & 0.00                   & 0.12                    \\ 

\textbf{Health}                                         & --                      & --                      & 0.95                   & --                                     & 0.00                   & 0.19                   & 0.00                   & 0.18                   & 0.11                   & --                                     & 0.00                   & 0.19                    \\ 

\textbf{Home}                                           & 0.00                   & 0.24                   & 1.00                   & --                                     & 0.00                   & 0.12                   & 0.00                   & 0.22                   & 0.48                   & --                                     & 0.00                   & 0.12                    \\ 

\textbf{Kids}                                           & 0.00                   & 0.40                   & 0.00                   & 0.41                   & 0.63                   & --                                     & 0.10                   & --                                     & 0.00                   & 0.18                   & 0.63                   & --                                      \\ 

\textbf{News}                                           & 0.00                   & 0.27                   & 0.93                   & --                                     & 0.29                   & --                                     & 0.01                   & 0.16                   & 0.01                   & 0.20                   & 0.29                   & --                                      \\ 

\textbf{Recreation}                                     & 0.00                   & 0.60                   & 0.34                   & --                                     & 0.06                   & --                                     & 0.00                   & 0.28                   & 0.26                   & --                                     & 0.06                   & --                                      \\ 

\textbf{Reference}                                      & 0.06                   & --                                     & 0.75                   & --                                     & 0.00                   & 0.11                   & 0.59                   & --                                     & 0.74                   & --                                     & 0.00                   & 0.11                    \\ 

\textbf{Regional}                                       & 0.00                   & 0.43                   & 0.66                   & --                                     & 0.43                   & --                                     & 0.45                   & --                                     & 0.27                   & --                                     & 0.43                   & --                                      \\ 

\textbf{Science}                                        & 0.62                   & --                                     & 0.53                   & --                                     & 0.45                   & --                                     & 0.02                   & 0.15                   & 0.52                   & --                                     & 0.45                   & --                                      \\ 

\textbf{Shopping}                                       & 0.92                   & --                                     & 0.02                   & 0.33                   & 0.41                   & --                                     & 0.00                   & 0.24                   & 0.01                   & 0.16                   & 0.41                   & --                                      \\ 

\textbf{Society}                                        & 0.00                   & 0.25                   & 0.20                   & --                                     & 0.00                   & 0.19                   & 0.03                   & 0.15                   & 0.58                   & --                                     & 0.00                   & 0.19                    \\ 

\textbf{Sports}                                         & 0.00                   & 0.39                   & 0.02                   & 0.29                   & 0.71                   & --                                     & 0.19                   & --                                     & 0.01                   & 0.15                   & 0.71                   & --                                      \\

\bottomrule
\end{tabular}

\label{table:u-test}
\end{table*}

==> stateless-ads-main_3/Makefile <==
extensions_to_clean := out aux log bbl blg fls fdb_latexmk glg gls lof glo glsdefs lot toc dvi ist acn acr synctex.gz alg xdy

all: paper

clean:
	@if [[ -f paper.pdf ]]; then \
		rm paper.pdf;\
	fi;
	@for extension in $(extensions_to_clean); do \
		find . -type f -name "*.$$extension" -delete;\
	done;

paper:
	latexmk -bibtex -pdf paper
	pdflatex -bibtex -interaction=nonstopmode paper

==> stateless-ads-main_3/docs/0_abstract.tex <==
\begin{abstract}
Data protection regulations, such as GDPR and CCPA, require websites and embedded third-parties, especially advertisers, to seek user consent before they can collect and process user data.
Only when the users opt in, can these entities collect, process, and share user data. 
Websites typically incorporate Consent Management Platforms (CMPs), such as OneTrust and CookieBot, to solicit and convey user consent to the embedded advertisers, with the expectation that the consent will be respected. 
However, neither the websites nor the regulators currently have any mechanism to audit advertisers' compliance with the user consent, i.e., to determine if advertisers indeed do not collect, process, and share user data when the user opts out. 

In this paper, we propose an auditing framework that leverages advertisers' bidding behavior to empirically assess the violations of data protection regulations. 
Using our framework, we conduct a measurement study to evaluate two of the most widely deployed CMPs, i.e., OneTrust and CookieBot, as well as advertiser-offered opt-out controls, i.e., National Advertising Initiative's opt-out, under GDPR and CCPA -- arguably two of the most mature data protection regulations.
Our results indicate that user data is unfortunately still being collected, processed, and shared even when users opt-out. 
Our findings suggest that several prominent advertisers (e.g., AppNexus, PubMatic) might be in potential violation of GDPR and CCPA. 
Overall, our work casts a doubt if regulations are effective at protecting users' online privacy. 


\end{abstract}


==> stateless-ads-main_3/docs/1_introduction.tex <==
\section{Introduction}
\label{sec:introduction}

There has been a recent increase in the promulgation of data protection regulations, such as General Data Protection Regulation (GDPR) \cite{GDPR}, California Consumer Privacy Act (CCPA) \cite{CCPA}, and General Personal Data Protection Act (LGPD) \cite{LGPD}, across the globe. 
%
At a high level, data protection regulations aim to protect user privacy by mandating online services to take user consent before collection, processing, and sharing of user data. 
%
Because of their mass deployment, automatic enforcement, and legal binding, data protection regulations are believed to guarantee user privacy; provided that users do not consent to data collection and processing.
%
In fact, infringement fines have amounted to billions. For example, in case of GDPR -- arguably the most mature data protection regulation -- the fines have accumulated to a total of \EUR 1.6 billion \cite{gdpr_fines_over_time}.
%

%
However, despite strict enforcement, prior research has found that online services often trick users into giving positive consent \cite{Matte20SPDoCookieBanners}, do not include controls to opt-out of data collection and processing \cite{dnsmpi}, or deploy user interfaces that are unintuitive to navigate in terms of providing consent \cite{alizadeh2020gdpr, habib19optout}.
%
In cases where users are indeed able to exercise their rights, user data is poorly handled. 
%
For example, online services often ignore or respond late to data access requests \cite{urban2019study} and even leak sensitive user data to unauthorized users because of weak authentication mechanisms \cite{bufalieri2020gdpr, di2019personal}.
While some negligence could be attributed to the complexity of the regulations, unpreparedness, or oversights of online services, a lot of it could be due to blatant inconsideration towards data protection regulations from online services. 



%
Regulators have mostly focused on auditing compliance of large well-known corporations, such as Amazon \cite{amazon_fine} and Google \cite{CNIL_google_fine}, perhaps because of the lack of systematic mechanisms to automatically detect infringements at scale \cite{google_amazon_fine}.
%
Prior research \cite{Matte20SPDoCookieBanners,dnsmpi, alizadeh2020gdpr, habib19optout} has focused on auditing the implementation deficiencies in consent management platforms/tools but it has largely ignored the instances where \textit{compliance is correctly conveyed but online services fail to comply}. 
%
Though, negligence in implementation raises doubts on the seriousness of online services in protecting users' privacy, it does not by itself imply non-compliance.
%


In this paper, we set out to fill this gap in the state-of-the-art research and deployed practice by regulatory bodies in assessing whether online services are actually compliant with the data regulations or not. To this end, we propose a framework to automatically audit regulatory compliance.
%
We focus on cases where user consent is correctly conveyed but online services may not necessarily comply. 
%
We evaluate our auditing framework on the web, whereby websites typically record user consent using consent management platforms (CMPs), e.g., OneTrust \cite{OneTrust}, and convey it to advertisers under GDPR and CCPA.
%
Our key idea is to leak user interest data in controlled A/B experiments, opt-out/in of processing and selling through CMPs, and leverage advertisers \textit{ bidding behavior} as a side channel in the advertising ecosystem to infer the processing and selling of user information.
%
Since the bidding behavior of advertisers is shaped up by their pre-existing knowledge of the user, we expect to receive higher bids when advertisers process or sell leaked user interest data, i.e., are non-compliant with the law, despite the user choosing to opt-out.   


We find that the most advertisers engage in data processing and selling activities, regardless of user consent. 
%
Overall, our results indicate that most advertisers and trackers might be in potential violation of GDPR and CCPA.
%

We summarize our key contributions as follows:

\begin{enumerate}
	\item We propose a framework to automatically audit regulatory compliance of online services. We implement our framework by extending OpenWPM \cite{Englehardt16MillionSiteMeasurementCCS}. The framework allows us to imitate real user, automatically opt-out/opt-in of data processing and selling, and capture advertisers bidding by advertisers. 
    
    \item As a case study, we use our proposed framework to audit regulatory compliance of online services under GDPR and CCPA with two consent management platforms, i.e, OneTrust \cite{OneTrust} and CookieBot \cite{Cookiebot}. Our results indicate that the advertisers do not necessarily comply with the user consent to opt-out of data processing and selling.

    \item We also pursue a comparative analysis between state-enforced regulations and advertiser-offered controls, i.e. National Advertising Initiative's (NAI) central opt-out \cite{naa_central_optout}, in reduction of collection and selling of user data. Our results indicate that the advertiser-offered NAI’s opt-out controls might be equally ineffective as state-enforced regulations. 
    
\end{enumerate}



\textit{Paper Organization:} 
The rest of the paper is outlined as follows. Section \ref{sec:background} presents an overview of online privacy threats and protection mechanisms. 
%
Section \ref{sec:methodology} describes the design of our framework to audit regulatory compliance of online services. 
%
Section \ref{sec:evaluation} presents the results of our auditing.
%
Section \ref{sec:discussion}  outlines limitations of our proposed auditing framework. 
%
Section \ref{sec:conclusion} offers the main conclusions from our work. 




==> stateless-ads-main_3/docs/2_background.tex <==
\section{Background \& Related Work}
\label{sec:background}


\subsection{Online Tracking}
Online trackers capture users browsing histories and activities across the web to facilitate risk mitigation, people search, and, perhaps most dominantly, advertising, among other services \cite{FTCDataBrokers}.
%
Online tracking is typically conducted through cookies that are set by third party resources loaded on websites, with the key idea being third parties having cross-site access to their cookies. 
%
Since most third parties are present on a limited number of websites, they often partner with each other to increase their coverage. 
%
Prior research has shown that trackers engage in data sharing partnerships and exchange cookies with \textit{as much as 118} other third parties \cite{Englehardt16MillionSiteMeasurementCCS}, which allows them to increase their coverage by as much as \textit{7 times} \cite{PapadopoulosCookieSynchronization19WWW}.  

%%
Online tracking, and especially tracking driven advertising, poses a serious threat to users' privacy both at the individual and the societal level. 
%
At the individual level, trackers collect sensitive personal information, for example, about health and sexual orientation, which is then used to hyper-target the individuals, for instance, through personalized ads \cite{targeted_ads_wp,targeted_ads_vox}.
%
At the societal level, tracking driven advertising has been leveraged to conduct mass surveillance \cite{mass_surveillance_ads}, increase political polarization \cite{AliAdDeliveryPolarization21WSDM}, spread misinformation \cite{misinformation_ads}, and discriminate \cite{discrimination_ads}.
%
Overall, people are frustrated by the privacy harms facilitated by online tracking.
%%
\subsection{Protection Mechanisms}
\subsubsection{Self-Regulations}
%
To tackle user privacy concerns and pressure from the regulatory bodies, such as the Federal Trade Commission (FTC), the online advertising industry has responded with self-regulations \cite{FTC_self_regulation_principles, FTC_congress}. 
%
However, prominent self-regulatory actions, such as the ones facilitated by browsers, for example, Platform for Privacy Preferences (P3P) \cite{p3p_w3c} and Do Not Track (DNT) \cite{dnt_w3c}, and the ones offered by the advertisers, for example, Digital Advertising Alliance's (DAA) AdChoices \cite{adchoices} and National Advertising Initiative's (NAI) central opt-out \cite{naa_central_optout}, are either not respected by majority of the vendors or they are too convoluted to be used or understood by the lay users.


%%
\textit{Browser-Facilitated Automated Controls.}
Browsers provide support to advertisers to enforce self-regulatory measures in an automated manner. 
%
To this end, browsers have provided two major controls, i.e., P3P and DNT request headers. 
%
P3P, now discontinued, was an automated mechanism for websites to communicate their privacy policies to web browsers.
%
It was implemented by major web browsers, such as Internet Explorer and Firefox \cite{p3p_internet_explorer,p3p_mozilla}, and supported by thousands of websites \cite{cranor2008p3pdeployment}.
%
However, P3P was often misrepresented by websites \cite{leon2010token,RaeyP3PTWEB09} likely because it was not enforced under any state regulation. 
%
Similarly, DNT was proposed to convey user's privacy preferences to the websites in an automated manner.
%
However, it also enjoyed limited adoption and it had practically no impact in limiting tracking. 
% 
Libert et al. \cite{libert2018automated} reported that only 7\% of the websites mentioned DNT in their privacy policies, and in majority of those cases specified that the DNT signal is not respected.
%
Miguel et al. \cite{Miguel15CoNEXTOBA}, conducted an A/B study and identified that the DNT signal essentially had no impact on ad targeting, experienced by users. 


%%
\textit{Advertiser-Offered Manual Controls.}
In response to the concerns from FTC, advertising networks formed National Advertising Initiative (NAI), which provides a central interface for users to opt-out from targeted advertising, i.e., if users opt-out through NAI's central opt-out interface, they will (supposedly) no longer be tracked for online advertising \cite{nai_opt_out}.
%
McDonald and Cranor \cite{mcdonald2010americans} conducted a user study and found that only 11\% of respondents understood NAI's opt-out mechanism, which indicates that its adoption is perhaps low.
%
Similarly, taking a step forward in self-regulations, several of the advertising consortiums, created Digital Advertising Alliance (DAA) with an aim to provide easy to access user transparency and control, with ``AdChoices'' icon, to opt-out of targeted advertisements \cite{adchoices}.
%
Unfortunately, similar to NAI's opt-out, only 9.9\% of ads shown on top websites had AdChoices icon \cite{tracking_the_trackers_adchoices}.



%%
\subsubsection{User-Managed Privacy Protections}
Currently, the most effective way for users to self-protect their privacy is to rely on off-the-shelf privacy-enhancing tools, such as AdBlock Plus \cite{adblockplus_web}, Privacy Badger \cite{privacybadger_web}, and Disconnect \cite{disconnect_me}.
%
However, privacy-enhancing tools are not available by default in browsers and need to be installed separately; which limits their adoptability to mostly tech-savvy users. 
%
Further, trackers engage in an arms-race with privacy-enhancing tools and try to come up with evasive tactics, for example, bounce tracking \cite{bounce_tracking_definition} and CNAME cloaking \cite{Dao20CNAME}, to evade privacy protections.

%%
The other likely more feasible alternative is to rely on default privacy protections offered by the mainstream browsers, which are available to a larger population.
%
However, these protections are too weak to completely protect user privacy. 
% 
For example, some main-stream browsers block third-party cookies, which makes them susceptible to new and sophisticated ways of tracking, such as browser fingerprinting \cite{Englehardt16MillionSiteMeasurementCCS,Iqbal21FPInspectorSP}.
% 
Further, some browsers, such as Google Chrome, are too cautious even in blocking third-party cookies because of website breakage concerns \cite{chrome_3p_cookie_blocking_delayed}.

\subsubsection{State-Enforced Regulations: The Focus of Our Work}
Both self-regulations and user-managed privacy protections do not have any legal binding and are thus blatantly bypassed by the advertisers and trackers. 
%
Only recently, legislators have promulgated regulations, such as General Data Protection Regulation (GDPR) \cite{GDPR} in EU and California Consumer Privacy Act (CCPA) \cite{CCPA} in California, that have potential to rein-in online advertising and tracking ecosystem. 
%
These regulations have clearly-stated frameworks that define protocols to collect, share, and use personal user information.
%
Most importantly, their infringements can be prosecuted; which can lead to heavy fines \cite{gdpr_faq, CCPA}.
%
For example, both Amazon and Google were recently fined for \EUR 746 \cite{amazon_fine, LuxembourgAmazonFine} and \EUR 50 millions \cite{CNIL_google_fine} under GDPR, respectively.
%
Essentially, these regulations possess the ability to keep advertising and tracking ecosystem in check. 

\begin{figure}
    \centering
        \subfloat[Consent management dialog for GDPR.]{
        \includegraphics[width=0.8\columnwidth]{figures/GDPR-OneTrust.png}
        \label{fig:GDPR-OneTrust}
        }
        \hfill
         \subfloat[Consent management dialog for CCPA.]{
        \includegraphics[width=0.8\columnwidth]{figures/CCPA-OneTrust.png}
        \label{fig:CCPA-OneTrust}
        }
        \caption{OneTrust's consent management dialog for GDPR and CCPA.}
    \label{fig:OneTrust-CMPs}
\end{figure}

%%
Both GDPR and CCPA guarantee a right for individuals to opt-out of processing and selling of their data. 
%
Under GDPR, online services need to take user consent (Articles 4 (11)) before they can process user data (Article 6 (1) (a)).
%
GDPR has a broad definition of data processing, that includes \textit{collection, recording, organization, structuring, storage, adaptation or alteration, retrieval, consultation, use, disclosure by transmission, dissemination or otherwise making available, alignment or combination, restriction, erasure or destruction} of user data (Article 4 (2)). 
%
Under CCPA, online services need to provide user control to opt-out of sale of personal user data (Section 1798 (a) (1)). 
%
CCPA has a broad definition of personal data selling, that includes \textit{selling, renting, releasing, disclosing, disseminating, making available, and transferring} data to another business or a third party for monetary or other valuable consideration (Section 178.140 (t) (1)).
%
Both GDPR's and CCPA's data processing and selling definition covers routine data exchanges, such as processing user data to serve personalized ads, e.g., through Real-Time Bidding (RTB) protocol \cite{RTB_protocol}, and sharing data with advertising partners under data sharing partnerships, e.g., with cookie syncing \cite{google_rtb_docs}. 
%
It is noteworthy that GDPR requires to obtain consent beforehand and CCPA requires to provide tools to opt-out, later.
%
CCPA does not require a beforehand consent because it only restricts the selling of personal data and not its collection. 


%
Both GDPR and CCPA require websites to provide \textit{privacy notices} with information and controls to opt-in/out of personal information collection and/or processing. 
%
To obtain user consent, websites typically embed off-the-shelf consent management platforms (CMPs), for example, OneTrust \cite{OneTrust} and Cookiebot \cite{Cookiebot}. 
%
CMPs scan websites and identify all cookies set by the HTTP headers and scripts, from both the first and third party resources. 
%
In case of GDPR, CMPs should ensure that only strictly necessary cookies are shared and consent is obtained before non-essential cookies, such as for advertising and analytics, are shared. 
%
In case of CCPA, CMPs should ensure that they provide controls to users to opt-out to sell their personal information.
%
Figure \ref{fig:GDPR-OneTrust} shows an example consent dialog displayed under GDPR, and Figure \ref{fig:CCPA-OneTrust} shows an example consent dialog displayed under CCPA. 
%


%%
\subsection{Related Work}
Prior research has identified that online services design unintuitive and hard to navigate interfaces \cite{alizadeh2020gdpr, habib19optout}, trick users into giving positive consent \cite{Matte20SPDoCookieBanners}, and do not include controls to opt-out of data selling \cite{dnsmpi}.
%
Alizadeh et al. \cite{alizadeh2020gdpr} conducted a user study to understand data rights under GDPR and identified that the participants find data access interfaces unintuitive and hard to navigate. 
%
Specifically, users prefer structured and easy-to-navigate data usage reports in contrast to data dumps, that are hard to explore. 
%
Habib et al. \cite{alizadeh2020gdpr} conducted a measurement study of 150 websites and identified that the privacy controls were hard to locate on the majority of websites.
%
Furthermore, in several instances, links to privacy control did not lead to stated choices.
%
Matte et al. \cite{Matte20SPDoCookieBanners} investigated CMPs and identified that the consent is often incorrectly conveyed.
%
Specifically, websites often register consent before the user has made any choice, register positive consent regardless of user's choice, or nudge users to give pre-selected positive consent. 
%
More recently, Nortwick and Wilson \cite{dnsmpi}, conducted a measurement study of top 500K English websites and identified that only 2\% of the websites provided controls to users to opt-out of data selling, i.e., ``Do Not Sell My Personal Information'' (DNSMPI), under CCPA. 



%%
Though negligence in obtaining consent and not providing easy-to-navigate opt-out controls raises doubts on online services' seriousness in protecting users' data and respecting their consent, it does not automatically imply non-compliance. 
%
Prior work, to the best of our knowledge, has not directly measured non-compliance, especially for the cases where consent is properly conveyed to the online services. 
%
To bridge that gap, in our work, we set out to audit the usage and selling of personal user data, where the user has directed online services to cease the processing and selling of their data, and their consent is properly recorded and conveyed by the CMPs.


==> stateless-ads-main_3/docs/3_methodology.tex <==
\section{Our Framework for Auditing Advertising \& Tracking Services}
\label{sec:methodology}

\begin{figure}[!t]
    \centering
        \subfloat[Consent management dialog for GDPR.]{
        \includegraphics[width=0.8\columnwidth]{figures/GDPR-Cookiebot-1.png}
        \label{fig:GDPR-CookieBot}
        }
        \hfill
         \subfloat[Consent management dialog for CCPA.]{
        \includegraphics[width=0.8\columnwidth]{figures/CCPA-Cookiebot-1.png}
        \label{fig:CCPA-CookieBot}
        }
        \caption{Cookiebot's consent management dialog for GDPR and CCPA.}
    \label{fig:CookieBot-CMPs}
\end{figure}

\begin{figure*}
    \centering

        \includegraphics[width=\textwidth]{figures/CMP_workflow.pdf}
     
        \caption{High level overview of our framework to audit regulatory compliance. (1) We use OpenWPM \cite{Englehardt16MillionSiteMeasurementCCS} to automatically visit top-50 websites from 16 different interest categories to simulate 16 user interest personas. (2) We filter top websites that support opt-outs through OneTrust \cite{OneTrust} and CookieBot \cite{Cookiebot} under GDPR and CCPA and also support header bidding through \texttt{prebid.js} \cite{prebid}. (3) We then visit the filtered websites with user interest personas, opt-out of data processing and selling, and collect bids and network requests from advertisers. (4) We then analyze the collected bids and network requests to infer data processing and selling from advertisers.} % to audit advertisers' compliance with user consent.}
        \label{fig:CMP}
\end{figure*}
%%
% \subsection{Overview}
In this section, we describe our framework to audit advertising and tracking services under GDPR and CCPA. % compliance with the user consent. 
%
At a high level, we simulate synthetic user personas (profiles) with specific interests, intentionally leak those interests to advertisers and trackers, opt-out of processing and selling of user data, and analyze advertisers bidding behavior to infer the usage and selling of leaked data. 
%
Figure \ref{fig:CMP} gives an overview of our approach. 
%%
\subsection{Inferring Non-Compliance}
\label{subsection:non-compliance}
Online services, including publishers, advertisers, and trackers, do not offer much transparency on the usage and sharing of collected data, which makes it challenging to directly assess non-compliance.
% %
Though prior work has not directly measured advertisers and trackers non-compliance, they have relied on side channel information to infer the usage and sharing of user data.
%
Specifically, a series of studies \cite{Cook20HeaderBiddingPETS,Olejnik14SellingPrivacyNDSS,Papadopoulos17IMCYouAreTheProduct} leaked user interest data, in controlled experiments, and leveraged advertisers bidding behavior as a side channel to infer the usage and sharing of user data. 
%
Their main insight is that the advertisers bidding behavior is shaped by their pre-existing knowledge of the user, which typically results in higher bid values.
Specifically, higher bids made by the advertiser to which the data was leaked indicates the usage of the leaked data for ad targeting.
%
Whereas, higher bids from the advertiser to which data was not leaked indicates the sharing of data from advertisers to which the data was leaked. 

We argue that analyzing advertisers bidding behavior, should also suffice in establishing whether advertisers comply with the user consent, when they opt-out of processing and selling of their data under GDPR and CCPA.
%
Specifically, if advertisers continuously bid higher despite user opting out of processing and selling of their data, it may indicate non-compliance with the user consent and potential violation of GDPR and CCPA. 
%
Thus, in this study, we leverage advertisers bidding behavior to audit regulatory compliance of advertisers under GDPR and CCPA. 

\subsection{Infrastructure}


\subsubsection{Web Crawling}
We rely on OpenWPM \cite{Englehardt16MillionSiteMeasurementCCS} to set up our auditing framework. 
%
OpenWPM is a widely used Firefox-based, open-source web measurement tool that has been used in numerous research studies \cite{openwpm_usage_stats}. 
%
OpenWPM by default provides functionality to automatically visit websites, capture network requests, and capture JavaScript API execution, among other things.
%
To adapt to our needs, we further extend OpenWPM to automatically opt-out of processing and selling of user data, and to capture advertisers bids on ad slots.\footnote{We will release our patch to OpenWPM at the time of publication.}



\subsubsection{Opting-out of Processing \& Selling of User Data}
\label{susub:opt-out}
We extend OpenWPM to programmatically opt-out of processing and selling of user data from OneTrust \cite{OneTrust} and CookieBot \cite{Cookiebot}, two of the widely used consent management platforms (CMPs) \cite{WebAlmanacStateofTheWebCMPs}.
%
To opt-out of processing/collection of user data under GDPR, for OneTrust, we traverse the DOM and click the \textit{Customize Settings} button, toggle the \textit{Targeting Cookies}, \textit{Analytics Cookies}, and \textit{Functionality Cookies} to disable them, and then click the \textit{Confirm My Choices} button. 
%
Figure \ref{fig:GDPR-OneTrust} represents the OneTrust's opt-out dialog under GDPR.
%
For CookieBot, we traverse the DOM and click the \textit{Customize} button, toggle the \textit{Marketing}, \textit{Statistics}, and \textit{Preferences} buttons to disable them, and then click the \textit{Allow selection} button.
%
Figure \ref{fig:GDPR-CookieBot} represents the CookieBot's opt-out dialog under GDPR.
%
To opt-out of selling of user data under CCPA, for OneTrust, we traverse the DOM and click the \textit{Do Not Sell My Personal Information} button, toggle the \textit{Sale of Personal Data} to disable it, and then click the \textit{Confirm My Choices} button. 
%
Figure \ref{fig:CCPA-OneTrust} represents the OneTrust's opt-out dialog under CCPA.
%
For CookieBot, we traverse the DOM and select the \textit{Do Not Sell My Personal Information} checkbox and then click the \textit{OK} button.
%
Figure \ref{fig:CCPA-CookieBot} represents the CookieBot's opt-out dialog under CCPA.





\subsubsection{Capturing Bidding by Advertisers}
We treat advertisers bidding behavior as an indication of advertisers and trackers non-compliance with the user consent (as discussed in $\S$ \ref{subsection:non-compliance}).
%
To this end, we audit advertisers and trackers on websites that support header bidding, more specifically \texttt{prebid.js} -- a widely used implementation of header bidding protocol \cite{HB_usage}, primarily because header bidding occurs at the client side and allows us to intercept the bidding process \cite{HB_protocol}. 
To capture the bids, we inject a script on header bidding supported websites, through OpenWPM that calls the \texttt{getBidResponses} method and returns the bids CPMs\footnote{The bid values are expressed in CPM (cost per mille); which is the amount that an advertiser pays a website per one thousand visitors who see its advertisements.}. 
%
In case, we do not get any bids, we request the bids ourselves by calling \texttt{requestBids} method.

\subsubsection{Simulating Measurements under GDPR \& CCPA}
We conduct our measurements from EU and California to audit third-party compliance under both GDPR and CCPA. 
We choose Frankfurt (Germany) and Northern California as representative jurisdictions under GDPR and CCPA, respectively.
%
We rely on web proxies to simulate web crawls through the respective locations.
%
Specifically, we set up Tinyproxy \cite{tinyproxy} servers on Amazon EC2 instances to funnel HTTP/HTTPS traffic. 
%
It is important to note that before visiting webpages, we connect each OpenWPM instance to a unique proxy server. 



\input{docs/bids-table-germany.tex}
\subsection{Methodology}

\subsubsection{Simulating Interest Personas}
Since advertisers bidding behavior is different for different user interests, we simulate 16 user interest personas to capture a wide spectrum of bidding behavior. 
%
User personas are based on 16\footnote{Adult, Art, Business, Computers, Games, Health, Home, Kids, News, Recreation, Reference, Regional, Science, Shopping, Society, and Sports.} Alexa top websites by categories lists \cite{alexa}.\footnote{As of September 2020, Alexa does not provide a pre-compiled list of websites by category but instead provides an alternate service to search websites by keywords.}
%
To simulate each persona, we initialize a fresh browser profile in an OpenWPM instance, connect it to a unique proxy server, iteratively visit top-50 websites in each category, and update browser profile after each visit.
%
Our rationale in simulating personas is to convince advertisers and trackers of each persona's interests, so that the advertisers bid higher when they target personalized ads to each persona. %
In addition to the above-mentioned 16 personas, we also include a control persona, i.e., an empty browser profile. 
%
Control persona acts as a baseline and allows us to measure differences in bidding behavior. 
%
It is noteworthy that we also enable OpenWPM's bot mitigation and randomly wait between 10--30 seconds after loading each website in order to more accurately simulate user behavior. 


\subsubsection{Measuring Targeting on Personas}
Next, we measure targeting received by our personas to infer compliance (or lack thereof) under GDPR and CCPA.
%
As mentioned earlier, we register negative user consent, i.e., opt-out of processing and selling of user data, through OneTrust and CookieBot and capture bids through \texttt{prebid.js}.
%
To this end, we shortlist websites that support opt-out through either OneTrust or CookieBot and also implement header bidding through \texttt{prebid.js}.
%
We identify such websites, by crawling Alexa top-10K websites, using OpenWPM, and probing for OneTrust or CookieBot and \texttt{prebid.js}.
%
Specifically, if a website loads a script from OneTrust or CookieBot, we treat it as OneTrust or CookieBot supported website, respectively. 
%
To identify the websites that support \texttt{prebid.js}, we inject a script that probes the \texttt{prebid.js} version; if we receive a response, we mark the website as \texttt{prebid.js} supported website.




We find that a total of 37 websites support OneTrust and also implement \texttt{prebid.js}, however, only 27 of them allow to opt-out of processing of data under GDPR and 11 of them allow to opt-out of selling data under CCPA.
%
In case of CookieBot, we only identify 2 websites that support CookieBot and also implement \texttt{prebid.js}. 
%
We increase the set of websites that support both CookieBot and also implement \texttt{prebid.js} to 13 by crawling Alexa top-100K websites, however, similar to OneTrust only 7 of them allow to opt-out of processing of data under GDPR and 5 of them allow to opt-out of selling data under CCPA. 
%
After filtering the websites, we iteratively visit each website four times from each of our 16 (+ control) personas.
%
We visit the websites first time to opt-out of processing or selling of data and the next three times to collect bids. 
%
We collect the bids from each website three times to reduce the chance of outliers biasing our measurements. 


%
To understand the impact of regulations, we also establish a baseline by opting in to the processing and selling of data. 
%
Our rationale for opting in is to get the upper bound on processing and selling of data, as inferred by advertisers bidding behavior.
%
It is noteworthy that to opt-in, we enable all cookie controls mentioned in $\S$ \ref{susub:opt-out}.
%
Similarly, we also compare state-enforced regulations, i.e., GDPR and CCPA, with advertisers offered controls, such as NAI's central opt-out \cite{nai_opt_out} in curbing the processing and selling of data.
%
We opt-out of NAI's offered controls by automatically navigating to their opt-out webpage \cite{nai_opt_out} and by clicking \textit{OPT OUT OF ALL} button.
%
To evaluate advertisers offered controls, we select a different set of websites that support \texttt{prebid.js} but do not support CMPs.
%
Specifically, we filter Alexa top-50 websites and identify 26 and 42 websites that support \texttt{prebid.js} but do not support any CMPs, under GDRP and CCPA, respectively. 
%
It is important to select websites that do not support CMPs, because otherwise we cannot differentiate between the impact of advertisers offered controls and state-enforced regulations. %facilitated by CMPs. 


==> stateless-ads-main_3/docs/3_methodology_backup.tex <==
\section{Methodology}
\label{sec:methodology}






\subsection{Experimental setup}
%We will do an initial crawl to find the persona and crawl configuration that triggers the most targeting. 
\textcolor{blue}{The purpose of the experiments is to figure out if the opt out really work.} So we will use that persona and crawl configuration to crawl a set of websites where we will opt out of tracking through consent management platforms. 
%We will also test the same set of websites by applying user controls (i.e. cookie blocking and fingerprint faking) to study their impact on targeting. 

We have 2 steps in our experiment setting. 

%\begin{figure}[]
%	\centering
%	\includegraphics[width=.9\linewidth]{figures/main/initial_fig.png}

%	\caption{Initial Crawl}
%	\label{initial}
%\end{figure}	

%\subsubsection{Initial Crawl} The first step is ``Initial crawl''. The purpose of this step is to find out which persona will be most affected by which human behaviors.  We selected 16 personas's key words in this step. For each persona, we have 4 behavior crawler settings. Each behavior crawler setting has 2 phrases: training phrase and testing phrase. Before training phrase, the crawler will create a new browser profile. Figure \ref{initial} shows how Initial Crawl works.


%\textbf{Training phrase: }The training phrase are different in 4 behavior crawler settings. In the 1st crawler setting ``vanilla crawl'', the crawler will visit one training site, wait 2-3 seconds, move to the next training site. In the 2nd crawler setting ``Interactive crawl 1'', the crawler only click subpages of each training site. In the 3rd crawler setting ``Interactive crawl 2'', the crawler click subpages of each training site, and the ads on the training site. In the 4th crawler setting ``Shopping cart crawl'', we only add products to the cart on each training site. After visiting all training websites, we will save the update browser profile as ``P''.

%\textbf{Testing phrase: }The testing phrase for 4 behavior crawler settings are same: visit each testing site three times, save all ads images, and use Prebid.js to collect bids value from each testing site. In creating the testing sites list, we filtered all websites that support header bidding from the Alexa top 10k website list. We chose top 25 websites from the filtered sites list as the testing sites. The crawler will load the profile ``P'' before visiting each testing website. And the profile ``P'' will not be updated after visiting each testing website.


%We ran those crawlers on the remote server at Iowa.


\begin{figure}[]
	\centering
	\includegraphics[width=.9\linewidth]{figures/main/opt_out_fig.png}

	\caption{Opt-Out Crawl: CMPs}
	\label{opt-out-cmp}
\end{figure}	


\begin{figure}[]
	\centering
	\includegraphics[width=.9\linewidth]{figures/main/opt_out_central_fig.png}

	\caption{Opt-Out Crawl: Central}
	\label{opt-out-cen}
\end{figure}	

\subsubsection{Opt-Out Crawl}The first step is ``opt-out crawl''. In this step, we will figure out if we can see the targeting ads after opting out from different CMPs. We will use the proxy in California and Europe to do this ``opt-out'' experiment. CCPA required websites providing ``Do not sell my information'' option for users when users are in California. GDPR in Europe protect EU residents' personal information before the residents giving consents to the websites. The purpose of this experiment is to verify if the websites followed CCPA or GDPR.  We implemented ``OpenWPM'' and used it as the crawling tool. We created 8 Amazon AWS EC2 instances and used ``tiny proxy'' as the proxy on those intances in training and testing phrases. We selected ``Onetrust'' and ``Cookiebot'' as the tested CMPs. The setting in this step also has 2 phrases: training phrase and testing phrase. Figure \ref{opt-out-cmp} and figure \ref{opt-out-cen} shows how Opt-Out Crawl works. \textcolor{blue}{Training will create a profile which meets the persona keyword. The data collected from the testing will display the feedback of this profile from the ads providers.}

\textbf{Training phrase: }
%In the first step ``Initial crawl'', we have selected one persona and one behavior. So in the training phrase, we will do what we did for this persona and behavior in the first step. 
\textcolor{blue}{At the beginning of this phrase, the crawler will create a new browser profile. Then the crawler will visit all assigned training websites sequentially, based on this persona keyword. Every time the browser finish visiting the training website, the browser profile will be updated. After visiting all training websites, the crawler will save the update browser profile as ``P'' on the server. This profile can be seen as a human profile who is interested in this persona keyword. This profile `P' will be used in Testing phrase.}

\textbf{Testing phrase: }In the testing phrase, all testing websites will use same CMPs and support header bidding. In creating Onetrust testing website list, we filtered the Alexa top 10k websites, and 37 of them support header biddings and use Onetrust service. After loading the CA proxy, 11 out of 37 provide opt out option. Under Germany IP, 27 out of 37 websites allow the users to give or not give consent. In creating Cookiebot testing website list, we also filtered Alexa top 10k websites. But only 2 websites use Cookiebot and header bidding. So I filtered Alexa top 100k websites, and 13 of thme use Cookiebot and support header bidding. Under CA IP, 5 out of 13 provide opt-out option to users. We will visit each testing website 4 times: in the first visit, we opt out the targeting/tracking cookie usage on CMPs. We call this visit "Opt-out visit". After opting out, we will visit this site again three times to collect ads images, and use Prebid.js to collect bids value from each testing site. We call it "Collecting visit". The crawler will load the profile ``P'' before visiting each testing website. And the profile ``P'' will not be updated after visiting each testing website. 

We will also do the central opting out in ``opt-out crawl''. After the training phrase, the crawler will visit the site ``https://optout.networkadvertising.org/?c=1'' to opt-out all of listed advertisers, then visit each testing site three times, save all ads images, \textcolor{blue}{and use Prebid.js to collect bids value from each testing site. In creating the testing sites list, we filtered all websites that support header bidding from the Alexa top 10k website list. We chose top 25 websites from the filtered sites list as the testing sites. The crawler will load the profile ``P'' before visiting each testing website. And the profile ``P'' will not be updated after visiting each testing website.}



\subsubsection{User-Control Crawl}
The third step is ``user-control crawl''

\subsection{Pre Experiment Preparation}

\subsubsection{Proxy Setting}
In ``opt-out'' experiment, we need proxy to change our IP to California, US and other Europe countries such as Germany, France and United Kingdom. \textcolor{blue}{We do not know if the bids data are modified by third party proxy service, which may increase the risk of data inaccuracy.} We would like to build our proxy, because we need to guarantee all the bids data we collected are accurate. 

Tinyproxy is a small, efficient HTTP/SSL proxy. We can deploy it on cloud instances. AWS can provide service locations in US West (N. California), Europe (Frankfurt), Europe (Paris) and Europe (London), which meets ``opt-out'' experiment setting. So we deploy Tinyproxy on AWS ec2 as the proxy instance in ``opt-out'' experiment. We will manually connect to those proxy instances before running crawlers to make sure the proxy can work well. All crawlers will auto connect to those proxy instances.

\subsubsection{Persona Designing}
\textcolor{blue}{The purpose of creating different personas is to compare the performance of header bidding under different personas. The keywords of 16 personas are ``Adult, Art, Business, Computers, Games, Health, Home, Kids, News, Recreation, Reference, Regional, Science, Shopping, Society, Sports''. Those personas covered most aspects of human life. For each persona, we selected Alexa top 50 websites by catogory. \cite{alexa}}

\subsubsection{Bids Collecting}
\textcolor{blue}{We need methods to collect bids in our crawlers. Prebid.js provides code to improve header bidding to display ads\cite{prebid}. We can used it to receive all of the bids from the ads providers.}
%\subsection{Initial crawl}
%\begin{enumerate}
%    \item Browser: Firefox 
%    \item Personas: Sports, Fashion (2-3 personas selected)
%    \item Location: Use any location
%        \begin{enumerate}
%            \item CCPA is by default opt-out and consent is only required if the data is intended to be sold. Selecting California as a crawl location may introduce a bias, we avoid that by selecting locations outside california.
%        \end{enumerate}
%    \item Targeting: Measured on the basis of bid values and ad images
 %   \item Testing website list: Alexa top 1K websites 
%        \begin{enumerate}
%            \item Select websites that support HB by checking the presence of bids on the website
%        \end{enumerate}
%        \item Crawling configurations for training (use 100 websites for training)
%            \begin{enumerate}
%                \item Vanilla crawl
 %                   \begin{enumerate}
  %                      \item Visit a website, wait 2-3 seconds, move to the next website
%                    \end{enumerate}
%                \item Interactive crawl 1
%                    \begin{enumerate}
%                        \item Open subpages only. People likely don't click ads frequently
%                        \item Random scrolls and mouse movements on the page
%                        \item Wait 20-30 seconds on each page 
%                    \end{enumerate}
%                \item Interactive crawl 2
%                    \begin{enumerate}
%                        \item Open subpages and ads.
%                        \item Random scrolls and mouse movements on the page
%                        \item Wait 20-30 seconds on each page 
%                    \end{enumerate}
%                \item Shopping cart crawl
%                    \begin{enumerate}
%                        \item Select 100 websites that support shopping cart
%                        \item Fill shopping cart with some items
%                        \item Random scrolls and mouse movements on the page
%                    \end{enumerate}
%            \end{enumerate}
%\end{enumerate}


%\subsection{Opt-out crawl}
%\begin{enumerate}
%    \item Browser: Firefox 
%    \item Personas: Use the persona that triggered the most targeting in the initial crawl.
%    \item Location: California and EU. If we crawl from both California and EU, we will also be able to quantify the effectiveness of GDPR and CCPA.
%    \item CMPs: CookieBot, ... (2-3)
%    \item Websites with the selected CMPs: Extract a list from nerdydata. Rank them on the basis of their Alexa ranking. Select top N for each CMP.
%    \item Crawl configuration: Use the crawl configuration that triggered the most targeting in the initial crawl.
%    \item Targeting: Measured on the basis of bid values and ad images
%\end{enumerate}

%\subsection{User control crawl:}
%\begin{enumerate}
%    \item Browser: Firefox 
%    \item Personas: Use the persona that triggered the most targeting in the initial crawl.
%    \item Location: California and EU.
%    \item Websites with the selected CMPs: Use the same list of websites that was extracted for opt-out crawl. 
%    \item Crawl configuration: Use the crawl configuration that triggered the most targeting in the initial crawl.
%    \item Targeting: Measured on the basis of bid values ad images
%    \item User controls: 
%        \begin{enumerate}
%            \item Blocked cookies, Fake fingerprint
%            \item Blocked cookies, Original fingerprint
%            \item Unblocked cookies, Fake fingerprint
%        \end{enumerate}
%\end{enumerate}




==> stateless-ads-main_3/docs/4_2_evaluation.tex <==

\subsection{Advertiser-Offered NAI's Opt-Out Controls are not very Effective Either}
We also analyze advertisers bidding behavior by exercising advertisers offered opt-out controls.
%
Specifically, we opt-out through National Advertising Initiative (NAI) -- an advertising consortium -- provided controls to opt-out of targeted advertising \cite{nai_opt_out}.
%
Similar to state-enforced regulations, i.e., GDPR and CCPA, we evaluate whether (a) opt-out through NAI reduces targeting, (b) whether the reduction is statistically different, and (c) whether advertisers share data without user consent. 


\textit{Similar to GDPR and CCPA, most personas receive higher bids as compared to control when user opt-out through NAI.}
%
NAI columns in Table \ref{table:GDPR-bidding-mean}  and \ref{table:CCPA-bidding-mean} present bids from advertisers who support opt-outs under the NAI's opt-out controls. 
%
To make a comparison with GDPR and CCPA, we opt-out of targeted advertising in both EU and California. 
%
In EU, when we opt-out of targeted advertising, 9 and 3 personas receive bids higher than the average and higher than the sum of average and standard deviation, respectively, as compared to the control persona. 
%
In California, when we opt-out of targeted advertising, 8 and 1 personas receive bids higher than the average and higher than the sum of average and standard deviation, respectively, as compared to the control persona. 
%
In comparison to the opt-out facilitated by OneTrust and CookieBot under GDPR, 4 and 7 few personas receive bid values that are higher than the average bid values of control.
%  
In comparison to the opt-out facilitated by OneTrust under CCPA, 2 personas receive bid values that are higher than the average bid values of control; for CookieBot in both cases equal number of personas receive bids that are higher than the average bid values of control.


\textit{Similar to GDPR and CCPA, opt-out is statistically similar to opt-in (no-action).}
%
Since advertisers assume default opt-in without explicit user consent to opt-out, we do not take any action to explicitly opt-in for NAI. 
%
It can be seen from the NAI columns in Table \ref{table:u-test}, that for 10 and 9 personas in EU and California, there is no significant difference in advertisers bidding behavior for opt-in and opt-out. 
%
For the remaining personas in both GDPR and CCPA, we note that bidding distributions are different for opt-out and opt-in configurations but the effect size is small.
%
In comparison to opt-out facilitated by OneTrust and CookieBot under GDPR, 5 more and 3 few personas are statistically similar to opt-in, respectively. 
%  
In comparison to opt-out facilitated by OneTrust under CCPA, 1 more persona is statistically similar to opt-in; for CookieBot in both cases equal number of personas are statistically similar. 

\input{docs/cookie-syncing-events-table_CCPA.tex}


\textit{Similar to GDPR and CCPA, advertisers share data without user consent.}
%
\textbf{\textit{(a) Server side sharing:}} Table \ref{table:in_test_not_in_train} presents the bids from NAI member advertisers who we did not explicitly leak user interests in both EU and California. 
%
In EU, when we opt-out of targeted advertising, 12 and 11 personas receive bids higher than the average and higher than the sum of average and standard deviation, respectively, as compared to the control persona. 
%
In California, when we opt-out of targeted advertising, 7 personas receive bids higher than the average and none of the personas receive higher than the sum of average and standard deviation as compared to the control persona. 
%
In comparison to the opt-out facilitated by OneTrust and CookieBot under GDPR, 4 few personas receive bid values that are higher than the average bid values of control.
%  
In comparison to the opt-out facilitated by OneTrust under CCPA, 1 more and 6 few personas personas receive bid values that are higher than the average bid values of control.


%%
\textbf{\textit{(b) Client side sharing:}}
Table \ref{tbl:GDPR_cookie_syncing} and \ref{tbl:CCPA_cookie_syncing} show cookie syncing statistics for NAI, under GDPR and CCPA, respectively.
%
When we opt-out, we note that the percentage of advertisers participating in cookie syncing decreases by 9.6\% under GDPR and increase by 0.7\% under CCPA.
%
In comparison to opt-out through OneTrust under GDPR, 8.2\% few advertisers participate in cookie syncing.
%
We do not make a comparison with CookieBot because cookie syncing increases when we opt-out through CookieBot under GDPR.
%
In comparison to opt-out through OneTrust and CookieBot under CCPA, 8.6\% few and 5.8\% more advertisers participate in cookie syncing.
%


%%
\textbf{\textit{Takeaway \#4:}}  
We note that the advertiser-offered opt-out controls are also ineffective in curbing the processing and selling of user data despite user consent to opt-out. 
%
While advertisers at large do not honor their own opt-out controls, they slightly reduce targeting and share less data as compared to the state-enforced regulations.
%


==> stateless-ads-main_3/docs/4_evaluation.tex <==
\section{Results and Analysis}
\label{sec:evaluation}
\input{docs/bids-table-california.tex}


\input{docs/bidders_appeared_percentage.tex}
 \input{docs/stats-test-table.tex}

In this section, we present and analyze our measurement results.
%
We compare and contrast advertisers bidding behavior across personas and configurations, make statistical observations, and draw conclusions from those observations about advertisers' compliance under GDPR and CCPA.

\subsection{Most Personas Receive Higher Bids Compared to Control}
Table \ref{table:GDPR-bidding-mean} and \ref{table:CCPA-bidding-mean} present advertisers average bidding for three iterations, under GDPR and CCPA.
%
We note that most personas in both GDPR and CCPA, for both OneTrust and CookieBot, receive higher bids as compared to control when we opt-out. 
%
Specifically, for GDPR (Table \ref{table:GDPR-bidding-mean}), 13 and 16 personas on average receive higher bids as compared to control for OneTrust and CookieBot across three iterations, respectively.
%
For CCPA (Table \ref{table:CCPA-bidding-mean}) 7 and 9 personas on average receive higher bids as compared to control for OneTrust and CookieBot across three iterations, respectively.
%
Bids are even higher than the sum of average and standard deviation for 5 and 16 personas for GDPR and 3 and 1 personas for CCPA, for OneTrust and CookieBot, respectively.


%%
Since GDPR applies to all EU countries, we simulate our experiment from France as well to evaluate whether the advertisers behavior is generalizable across the EU. 
%
Table \ref{table:GDPR-bidding-France-mean} (Appendix \ref{sec:appendix}) presents the advertisers bidding under GDPR in France. 
%
It can be seen from Table \ref{table:GDPR-bidding-France-mean}, that for both OneTrust and CookieBot, when we opt-out, 12 and 11 personas receive higher bids as compared to control, respectively. 
%
2 and 9 personas in OneTrust and CookieBot, receive bids that are higher than the sum of average bids in control and standard deviation.
%
As compared to Germany, 1 and 5 personas receive lower bids for OneTrust and CookieBot, respectively. 
%
Similarly, 3 and 7 personas receive bids that are lower than the difference of average and standard deviation. 
%
Note that the differences in bidding behavior could be explained by advertisers' perceived value of users' interests in these countries. 
%
Overall, we note that there are differences in advertiser's bidding behavior for some personas but the majority of personas still receive higher bids as compared to the control in both Germany and France. 

We further analyze the individual advertisers that participate in bidding when we opt-out through GDPR and CCPA.
%
Table \ref{tbl:prevalent-advertisers} presents the top 5 most prevalent advertisers. 
%
It can be seen from the table that the top advertisers do not shy away from bidding across most personas, when we opt-out. 


%%
\textbf{\textit{Takeaway \#1:}} The variability in bid values, particularly higher bids as compared to control, indicates that the leaked user interests are used to target ads to users, despite users' consent to opt-out of processing of data as part of the regulations. 


\subsection{Opt-out is not Statistically Different from Opt-in}


As compared to opt-in, the advertisers bidding behavior does not significantly change for opt-out (Table \ref{table:GDPR-bidding-mean} and \ref{table:CCPA-bidding-mean}). 
%
Specifically, as compared to opt-in in GDPR, 1 and 3 personas receive higher bids when we opt-out, for OneTrust and CookieBot, respectively.
%
As compared to opt-in in CCPA, 3 personas receive higher bids when we opt-out, for both OneTrust and CookieBot.
%
To validate our hypothesis that the advertisers bidding behavior does not significantly change between opt-in and opt-out, we conduct Mann-Whitney U test of statistical significance \cite{cohen1977statistical}.
%
Mann-Whitney U test is a nonparametric test to compare the differences between two distributions.
%
Our null hypothesis is that the bid distributions for opt-in and opt-out are similar to each other. 
%
We reject the null hypothesis, when the \textit{p-value} is less than 0.05 (reflecting a 95\% confidence interval), i.e., the distributions are statistically different. No Bonferroni correction was needed due to only a single pairwise comparison being performed.


%%
Table \ref{table:u-test} presents the results of the Mann-Whitney U test.
%
For 5 and 12 personas in OneTrust and CookieBot in GDPR, there is no significant difference in advertisers bidding behavior for opt-in and opt-out. 
%
Similarly, for 8 and 9 personas in OneTrust and CookieBot in CCPA, there is no significant difference in advertisers bidding behavior for opt-in and opt-out. 
%
It is noteworthy that for Business and Recreation, the bidding distributions are statistically different for opt-out and opt-in, in GDPR for OneTrust, and the effect size is large.\footnote{Effect size less than 0.3, between 0.3 and 0.5, and greater than 0.5 is considered small, medium, and larger, respectively \cite{cohen1977statistical}.} 
%
For the remaining personas in both GDPR and CCPA, we note that bidding distributions are different for opt-out and opt-in configurations but the effect size is either small or medium.


%%
\textbf{\textit{Takeaway \#2:}} The similarity in bid values for opt-in and opt-out indicates that the user consent has almost no effect on processing and selling of data, except for a few personas, such as Business and Recreation. 


\input{docs/bids-table-germany-california-non-appearing-advertisers.tex}
\input{docs/cookie-syncing-events-table_GDPR.tex}

\subsection{Advertisers are Sharing Data without User Consent}

Data sharing is an essential component of online advertising ecosystem and it is baked into ad delivery protocols, such as RTB \cite{RTB_protocol} and HB \cite{HB_protocol} protocols. 
%
Advertisers routinely share user data at the server \cite{Bashir16TrackingFlowsUsenix,Cook20HeaderBiddingPETS} and as well as at the client side \cite{Englehardt16MillionSiteMeasurementCCS,cookie_syncing}. 
%
We try to infer server side data sharing by analyzing advertisers bidding behavior and the client side data sharing by analyzing HTTP redirects between advertisers. 


\vspace{0.5em}
\noindent
\textit{(a) Server side data sharing:}
We  analyze bids from advertisers who we did not explicitly leak user interests to, i.e., the advertisers who did not appear in the persona simulation phase but appeared when we opted-out and measured targeting on those personas.
%
Higher bid values from advertisers, who we did not explicitly leak user interests to will highlight the potential selling and sharing of user data from at least one of the advertisers who we leaked user data in the persona simulation phase.
%
Table \ref{table:in_test_not_in_train} presents the bids from advertisers who we did not explicitly leak user interests to for both GDPR and CCPA. 
%
For GDPR, all 16 personas receive higher bids than the average and 3 and 16 personas receive bids that are higher than the sum of average and standard deviation, as compared to control for both OneTrust and CookieBot. 
%
For CCPA, 6 and 13 personas receive higher bids than the average and 1 persona receives bids that are higher than the sum of average and standard deviation, as compared to control for both OneTrust and CookieBot. 
%
In case of GDPR, as compared to bids from all the advertisers (Table \ref{table:GDPR-bidding-mean}), 2 and 3 few personas receive bid values that are higher than the sum of average and standard deviation for OneTrust and CookieBot, respectively.
%
In case of CCPA, as compared to bids from all the advertisers (Table \ref{table:CCPA-bidding-mean}), 2 few persona receives bid values that are higher than the sum of average and standard deviation for OneTrust; for CookieBot in both cases only 1 persona receives bids that are higher than the sum of average and standard deviation.



\vspace{0.5em}
\noindent
\textit{(b) Client side data sharing:}
Client side data sharing is a standard practice in the online advertising ecosystem.
%
Advertisers most commonly share data through cookie syncing \cite{cookie_syncing}.
%
We measure whether opt-outs, under GDPR and CCPA, reduce cookie syncing. 
%
We slightly tweak the heuristic proposed by prior work \cite{Englehardt16MillionSiteMeasurementCCS,PapadopoulosCookieSynchronization19WWW} to detect cookie syncing.\footnote{We consider identifiers from non-standard fields in the request and response header, in addition to the cookie header. We also consider Base64, SHA1, and SHA2, hashed versions of identifiers.} 


%%
Table \ref{tbl:GDPR_cookie_syncing} and \ref{tbl:CCPA_cookie_syncing} show cookie syncing statistics for OneTrust and CookieBot, under both GDPR and CCPA.
%
When we opt-out under GDPR (Table \ref{tbl:GDPR_cookie_syncing}), we note that the percentage of advertisers participating in cookie syncing decreases by 1.4\% for OneTrust but increases by 7.3\% for CookieBot. % under GDPR in Germany. 
%
When we opt-out under CCPA (Table \ref{tbl:CCPA_cookie_syncing}), we note that the percentage of advertisers participating in cookie syncing decreases by 6.5\% for CookieBot but increases by 9.3\% for OneTrust. % under GDPR in Germany. 
%
Since the frequency of advertisers participating in cookie syncing events, alternatively increases and decreases among CMPs for the same regulation, we suspect that the regulations do not have any impact on their increase/decrease. 

%%
We further investigate the cookie syncing frequency of individual advertisers. 
%
Table \ref{tbl:Advertisers_cookie_syncing} presents the top 5 most prevalent advertisers that participate in cookie syncing, when we opt-out under both GDPR and CCPA.
%
It can be seen from the table that advertisers participate in as many as 164 and 215 cookie syncing events when we opt-out under GDPR and CCPA with CMPs, respectively.
%
Our results corroborate with prior work, that found advertisers syncing their cookies with as many as 118 other advertisers  \cite{Englehardt16MillionSiteMeasurementCCS}.
%
However, it is important to note that the earlier study was conducted well before ($\sim$2016) the enforcement of GDPR and CCPA. 


\textbf{\textit{Takeaway \#3:}}
We note that advertisers participate in data sharing activities both at the server and the client side.
%
At the server side, we received higher bid values from advertisers, who we did not explicitly leak user interests; which indicates potential selling and sharing from advertisers who we leaked user data. 
%
However, we note that the bid values are comparatively lower than the bid values from all the advertisers (Table \ref{table:GDPR-bidding-mean} and \ref{table:CCPA-bidding-mean}). 
%
We surmise that it could be because of limited information gained from the data accessed through advertising partners.
%
At the client side, we notice that the advertisers share unique user identifiers in plain sight and share their data with as many as 215 other advertisers. 


==> stateless-ads-main_3/docs/5_discussion.tex <==
\section{Limitations}
\label{sec:discussion} 
%%
\textit{CCPA applicability criteria:} 
CCPA applies to online services that meet its broad applicability criteria. 
%
Specifically, as per Section 1798.140 (c) (1), CCPA applies to online services, that have an annual revenue of more than \$ 25 million, annually sell data of more than 50K California residents, or earn more than 50\% of their revenue from the sale of personal data of California residents. 
%
Since most information required to determine applicability is not publically available, it is challenging to determine the applicability criteria at scale \cite{dnsmpi}. 
%
Thus, for our study, we did not strictly follow the CCPA applicability criteria. 
%
However, it is noteworthy that the prevalent advertisers (Table \ref{tbl:Advertisers_cookie_syncing}) in our dataset are mostly large corporates with revenue exceeding hundreds of millions \cite{appnexux_revenue,pubmatic_revenue}.


\textit{Sample size:} 
We currently analyze advertisers on a small number, i.e., 37 and 13, of websites that support OneTrust and CookieBot, respectively. 
%
We repeat our measurements several times to reduce the chance of a small sample size biasing our results. 
%
Ideally, we could have increased the sample size by incorporating websites that support various CMPs; however, it is non-trivial to automate opt-outs because each CMP has a different workflow. 
%
We leave automated opt-outs at scale as future work. 



\textit{Automated data collection:} 
We rely on OpenWPM to automatically collect bids and use proxies to simulate crawls from Germany and California. 
%
In order to more accurately simulate real users, we enable bot mitigation in OpenWPM and also randomly wait between 10-–30 seconds after loading each website.
%
We also refrain from using public proxy servers, which may be black listed, and instead setup our own proxy servers. 
%

==> stateless-ads-main_3/docs/6_conclusion.tex <==
\section{Conclusions and Path Ahead}

In this paper, we proposed a framework to audit regulatory compliance of online services at scale. 
%
We used the proposed framework to audit online advertising services on popular websites under GDPR and CCPA.
%
Despite users exercising their rights under GDPR and CCPA to opt-out of processing and selling of their data, we find that advertisers process user data to possibly target them and also share it with their partners both at the server and the client side. 
%
We also audited advertisers' self-proposed opt-out controls, i.e., NAI's opt-out, and found that they might be equally ineffective at curbing processing and selling of user data. 
%
Overall, our measurements sadly indicate that the regulations may not protect user privacy, and advertisers might be in potential violation of GDPR and CCPA. 

%
We hope that our measurements will inform regulators and policy makers towards better auditing of online services. 
%
We envision our framework to be used by regulators to audit online services at scale. 
%
Specifically, it could be run periodically at several vantage points or deployed as a browser extension for volunteers (end users) to deploy, who periodically report violators to the regulatory bodies --- essentially to double verify potential violators. 
%
To foster follow-up research, we will also release our code and data set at the time of publication. 


\label{sec:conclusion}


==> stateless-ads-main_3/docs/ads_images.tex <==
\begin{figure}
    \centering
        \includegraphics[width=\columnwidth]{figures/ads_images/opt-out.png}
        
        \caption{ \textbf{Tower General Contractors} ads image in Opt-out in persona: Home, with setting: CCPA-Onetrust.}
        \label{fig:image_out}
\end{figure}

\begin{figure}
    \centering
        \includegraphics[width=\columnwidth]{figures/ads_images/opt-in.png}
          
        \caption{ \textbf{Framing With TimberStrand LSL} ads image in Opt-in in persona: Home, with setting: CCPA-Onetrust.}
        \label{fig:image_in}   
\end{figure}

\begin{figure}
    \centering
        \includegraphics[width=\columnwidth]{figures/ads_images/control.png}
        \caption{ \textbf{Buydrcleanspray.com} ads image in Control, with setting: CCPA-Onetrust.}
        \label{fig:image_control}     
\end{figure}

==> stateless-ads-main_3/docs/bid_tables.tex <==
\begin{table*}[!h]
    \centering
    \begin{tabular}{l?{0.3mm}rr|rr|rr?{0.3mm}rr|rr|rr?{0.3mm}rr|rr} 
    \toprule
     & \multicolumn{6}{c?{0.3mm}}{\textbf{OneTrust}} & \multicolumn{6}{c?{0.3mm}}{\textbf{CookieBot}}& \multicolumn{4}{c}{\textbf{NAI}}    \\ 
     & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c}{\textbf{Opt-in}}  & \multicolumn{2}{c?{0.3mm}}{\textbf{No-action}}   & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c}{\textbf{Opt-in}}  & \multicolumn{2}{c?{0.3mm}}{\textbf{No action}}   & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c}{\textbf{No action}}   \\ 
    \textbf{Personas}     & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c}{\textbf{Std.}}  \\ 
    \toprule
    \textbf{Adult}  & 0.45$^{\textcolor{red}{\uparrow}}$ & 0.89   & 1.80$^{\textcolor{red}{\uparrow}}$ 
    & 3.56   & 0.27$^{\textcolor{red}{\uparrow}}$ 
    & 0.14   & 2.5E-3$^{\textcolor{red}{\uparrow}}$   & 0.00   & 1.4E-5$^{\textcolor{red}{\downarrow}}$ & 0.00   & 1.4E-5$^{\textcolor{red}{\downarrow}}$ & 0.00   & 0.29$^{\downarrow}$  & 0.61   & 0.51$^{\textcolor{red}{\uparrow}}$  & 0.87    \\ 
    
    \textbf{Arts}  & 0.16$^{\textcolor{red}{\uparrow}}$& 0.22   & 0.36$^{\textcolor{red}{\uparrow}}$
    & 0.21   & 0.24$^{\textcolor{red}{\uparrow}}$   
    & 0.17   & 0.07$^{\textcolor{red}{\uparrow}}$  & 0.00   & 0.03$^{\textcolor{red}{\uparrow}}$ 
    & 0.03   & 0.01$^{\textcolor{red}{\downarrow}}$& 0.00   & 0.17$^{\downarrow}$  & 0.26   & 0.13$^{\downarrow}$    & 0.18    \\ 
    
    \textbf{Business}     & 0.05$^{\textcolor{red}{\uparrow}}$ & 0.04   & 0.28$^{\textcolor{red}{\uparrow}}$ 
    & 0.17   & 0.17$^{\uparrow}$    & 0.16   & 0.04$^{\textcolor{red}{\uparrow}}$  & 0.03   & 0.08$^{\textcolor{red}{\uparrow}}$ 
    & 0.06   & 1.3E-5$^{\textcolor{red}{\downarrow}}$& 0.00   & 0.56$^{\uparrow}$& 0.74   & 0.18$^{\downarrow}$   & 0.13    \\ 
    
    \textbf{Computers}    & 0.08$^{\textcolor{red}{\uparrow}}$  
    & 0.05   & 0.27$^{\textcolor{red}{\uparrow}}$ 
    & 0.13   & 0.04$^{\downarrow}$    & 0.00   & 0.12$^{\textcolor{red}{\uparrow}}$    & 0.06   & 0.15$^{\textcolor{red}{\uparrow}}$ 
    & 0.06   & 0.16$^{\textcolor{red}{\uparrow}}$   & 0.03   & 0.37$^{\uparrow}$& 0.69   & 0.57$^{\textcolor{red}{\uparrow}}$  & 0.86    \\ 
    
    \textbf{Games} & 0.16$^{\textcolor{red}{\uparrow}}$ & 0.00   & 1.6E-5$^{\textcolor{red}{\downarrow}}$ 
    & 0.00   & - $^{\downarrow}$ 
    & - & 1.3E-5
    & 0.00   & 1.3E-5$^{\textcolor{red}{\downarrow}}$& 0.00   & 0.04$^{\textcolor{red}{\downarrow}}$  & 0.03   & 0.42$^{\uparrow}$& 0.68   & 0.12$^{\downarrow}$    & 0.11    \\ 
    
    \textbf{Health}& 1.23$^{\textcolor{red}{\uparrow}}$  & 1.21   & -$^{\textcolor{red}{\downarrow}}$ 
    & - & - $^{\downarrow}$ 
    & - & 0.08$^{\textcolor{red}{\uparrow}}$   & 0.07   & 0.07$^{\textcolor{red}{\uparrow}}$ 
    & 0.05   & 1.3E-5$^{\textcolor{red}{\downarrow}}$  & 0.00   & 0.48$^{\uparrow}$& 0.89   & 0.47$^{\textcolor{red}{\uparrow}}$    & 0.85    \\ 
    
    \textbf{Home}  & 0.07$^{\textcolor{red}{\uparrow}}$ & 0.07   & 0.47$^{\textcolor{red}{\uparrow}}$ 
    & 0.51   & 0.25$^{\textcolor{red}{\uparrow}}$   & 0.18   & 0.69$^{\textcolor{red}{\uparrow}}$ 
    & 0.49   & 0.48$^{\textcolor{red}{\uparrow}}$ & 0.49   & 0.11$^{\uparrow}$  & 0.06   & 0.22$^{\downarrow}$  & 0.19   & 0.13$^{\downarrow}$  & 0.20    \\ 
    
    \textbf{Kids}  & 0.05$^{\textcolor{red}{\uparrow}}$ & 0.05   & 0.15$^{\textcolor{red}{\uparrow}}$ 
    & 0.10   & 0.04$^{\downarrow}$  & 0.02   & 0.11$^{\textcolor{red}{\uparrow}}$ 
    & 0.05   & 0.14$^{\textcolor{red}{\uparrow}}$& 0.05   & 0.12$^{\uparrow}$  & 0.06   & 0.18$^{\downarrow}$  & 0.17   & 0.37$^{\uparrow}$  & 0.69    \\ 
    
    \textbf{News}  & 0.04$^{\textcolor{red}{\uparrow}}$& 0.05   & 0.37$^{\textcolor{red}{\uparrow}}$ 
    & 0.46   & 0.24$^{\textcolor{red}{\uparrow}}$   & 0.16   & 0.17$^{\textcolor{red}{\uparrow}}$ 
    & 0.03   & 0.17$^{\textcolor{red}{\uparrow}}$& 0.03   & 0.15$^{\textcolor{red}{\uparrow}}$  & 0.04   & 0.42$^{\uparrow}$& 0.77   & 0.16$^{\downarrow}$    & 0.19    \\ 
    
    \textbf{Recreation}   & 0.04$^{\textcolor{red}{\uparrow}}$  & 0.04   & 0.29$^{\textcolor{red}{\uparrow}}$ 
    & 0.11   & 0.11$^{\downarrow}$& 0.00   & 0.05$^{\textcolor{red}{\uparrow}}$ 
    & 0.04   & 7.3E-4$^{\textcolor{red}{\downarrow}}$ & 0.00   & 1.3E-5$^{\textcolor{red}{\downarrow}}$ & 0.00   & 0.45$^{\uparrow}$& 0.68   & 0.13$^{\downarrow}$    & 0.20    \\ 
    
    \textbf{Reference}    & 0.04$^{\textcolor{red}{\uparrow}}$  & 0.04   & 0.42$^{\textcolor{red}{\uparrow}}$ 
    & 0.33   & 0.12$^{\uparrow}$ & 0.07   & 0.16$^{\textcolor{red}{\uparrow}}$
    & 0.03   & 0.17$^{\textcolor{red}{\uparrow}}$   & 0.05   & 0.16$^{\textcolor{red}{\uparrow}}$   & 0.02   & 0.71$^{\textcolor{red}{\uparrow}}$
    & 0.83   & 0.64$^{\textcolor{red}{\uparrow}}$& 0.88    \\ 
    
    \textbf{Regional}     & 0.03$^{\textcolor{red}{\uparrow}}$  & 0.03   & 0.21$^{\textcolor{red}{\uparrow}}$ 
    & 0.17   & 0.08$^{\downarrow}$      & 0.00   & 0.07$^{\textcolor{red}{\uparrow}}$ 
    & 0.01   & 0.11$^{\textcolor{red}{\uparrow}}$  & 0.05   & 0.01$^{\textcolor{red}{\downarrow}}$   & 0.00   & 0.88$^{\textcolor{red}{\uparrow}}$
    & 0.95   & 0.14$^{\downarrow}$      & 0.14    \\ 
    
    \textbf{Science}      & 0.07$^{\textcolor{red}{\uparrow}}$& 0.01   & 0.07$^{\uparrow}$ & 0.01   & 0.49$^{\textcolor{red}{\uparrow}}$  & 0.00   & 1.4E-5$^{\textcolor{red}{\uparrow}}$ & 0.00   & 0.04$^{\textcolor{red}{\uparrow}}$    & 0.04   & 1.4E-5$^{\textcolor{red}{\downarrow}}$   & 0.00   & 0.57$^{\uparrow}$& 0.85   & 0.31$^{\uparrow}$ & 0.31    \\ 
    
    \textbf{Shopping}     & 0.05$^{\textcolor{red}{\uparrow}}$ & 0.04   & 0.05$^{\uparrow}$ & 0.03   & 0.07$^{\downarrow}$ & 3.8E-3   & 1.3E-5   & 0.00   & 0.06$^{\textcolor{red}{\uparrow}}$ & 0.04   & 0.10$^{\uparrow}$    & 0.09   & 0.26$^{\downarrow}$  & 0.29   & 0.64$^{\textcolor{red}{\uparrow}}$  & 0.87    \\ 
    
    \textbf{Society}      & 0.19$^{\textcolor{red}{\uparrow}}$    & 0.15   & 0.38$^{\textcolor{red}{\uparrow}}$ 
    & 0.15   & 0.32$^{\textcolor{red}{\uparrow}}$ & 0.17   & 0.17$^{\textcolor{red}{\uparrow}}$ 
    & 0.03   & 0.16$^{\textcolor{red}{\uparrow}}$& 0.02   & 0.17$^{\textcolor{red}{\uparrow}}$    & 0.03   & 0.14$^{\downarrow}$  & 0.19   & 0.16$^{\downarrow}$  & 0.19    \\ 
    
    \textbf{Sports}& 0.16$^{\textcolor{red}{\uparrow}}$ & 0.29   & 0.17$^{\textcolor{red}{\uparrow}}$ 
    & 0.13   & 0.09$^{\downarrow}$  & 0.03   & 0.12$^{\textcolor{red}{\uparrow}}$ 
    & 0.04   & 0.10$^{\textcolor{red}{\uparrow}}$& 0.08   & 0.09$^{\downarrow}$  & 0.04   & 0.39$^{\uparrow}$& 0.71   & 0.26$^{\uparrow}$   & 0.25    \\
    
    \midrule
    \textbf{Control} & 1.4E-5   & 0.00   & 0.06   & 0.05   & 0.12   & 0.08   & 1.3E-5   & 0.00   & 0.0014   & 0.00   & 0.10   & 0.03   & 0.29   & 0.29   & 0.19   & 0.19    \\ 
    
    \bottomrule
    % \hline
    % \textbf{Avg.}   & 0.177     & 0.080     & 0.168     & 0.187     & 0.334     & 0.382     & 0.071     & 0.025     & 0.109     & 0.052     & 0.104     & 0.062     & 0.300     & 0.418     & 0.400     & 0.576      \\ 
    % \hline
    % \textbf{Std.}   & 0.124     & 0.076     & 0.292     & 0.337     & 0.418     & 0.859     & 0.067     & 0.026     & 0.161     & 0.116     & 0.115     & 0.113     & 0.193     & 0.325     & 0.201     & 0.276      \\
    % \hline
\end{tabular}
\caption{Ad bidding under GDPR in Germany. Avg. column represents the average of each advertiser's median bid value. Std. represents the standard deviation of each advertiser's median bid value. Opt-out, opt-in, and no action represent the bids when we opt-out, opt-in, and do no take any action on selling of user data, respectively.  $\uparrow$ and $\downarrow$ indicate bid values that are higher and lower than Control's avg., respectively. $\textcolor{red}{\uparrow}$ and $\textcolor{red}{\downarrow}$ indicate bid values that are Control's avg. $\pm$ std., respectively.}
\label{table:GDPR-bidding}
\end{table*}


\begin{table*}[!h]
    \centering
    \begin{tabular}{l?{0.3mm}rr|rr|rr?{0.3mm}rr|rr|rr?{0.3mm}rr|rr} 
    \toprule
    \multirow{3}{*}{\textbf{Personas}}
     & \multicolumn{6}{c?{0.3mm}}{\textbf{OneTrust}} & \multicolumn{6}{c?{0.3mm}}{\textbf{CookieBot}}& \multicolumn{4}{c}{\textbf{NAI}}    \\ 
     & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c}{\textbf{Opt-in}}  & \multicolumn{2}{c?{0.3mm}}{\textbf{No-action}}   & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c}{\textbf{Opt-in}}  & \multicolumn{2}{c?{0.3mm}}{\textbf{No action}}   & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c}{\textbf{No action}}   \\ 
    
        & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c}{\textbf{Std.}}  \\ 
    \toprule
    \textbf{Adult}& 0.38$^{\textcolor{red}{\uparrow}}$ 
    & 0.60   & 0.51$^{\textcolor{red}{\uparrow}}$    & 0.69   & 0.09$^{\downarrow}$    & 0.02   & 0.26$^{\uparrow}$    & 0.26   & 0.12$^{\downarrow}$ & 0.15   & 0.67$^{\textcolor{red}{\uparrow}}$ & 1.69   & 0.32$^{\downarrow}$& 0.26   & 0.54$^{\uparrow}$& 0.66    \\ 
    
    \textbf{Arts} & 0.27$^{\uparrow}$    & 0.30   & 0.20$^{\downarrow}$    & 0.12   & 0.22$^{\uparrow}$    & 0.24   & 0.22$^{\uparrow}$    & 0.29   & 0.33$^{\uparrow}$ & 0.33   & 0.30$^{\uparrow}$ & 0.31   & 0.35$^{\downarrow}$& 0.28   & 0.47$^{\downarrow}$  & 0.59    \\ 
    
    \textbf{Business}    & 0.36$^{\textcolor{red}{\uparrow}}$    & 0.31   & 0.62$^{\textcolor{red}{\uparrow}}$    & 0.47   & 0.60$^{\textcolor{red}{\uparrow}}$    & 0.40   & 0.21$^{\uparrow}$    & 0.26   & 0.27$^{\uparrow}$ & 0.24   & 0.15$^{\downarrow}$& 0.16   & 0.46$^{\downarrow}$& 0.51   & 0.24$^{\downarrow}$  & 0.23    \\ 
    
    \textbf{Computers}   & 0.34$^{\uparrow}$    & 0.29   & 0.65$^{\textcolor{red}{\uparrow}}$    & 0.86   & 0.30$^{\uparrow}$    & 0.32   & 0.26$^{\uparrow}$    & 0.29   & 0.16$^{\downarrow}$ & 0.16   & 0.15$^{\downarrow}$& 0.15   & 0.41$^{\downarrow}$& 0.57   & 0.29$^{\downarrow}$  & 0.52    \\ 
    
    \textbf{Games}& 0.55$^{\textcolor{red}{\uparrow}}$    & 0.39   & 0.32$^{\uparrow}$    & 0.32   & 0.39$^{\uparrow}$    & 0.19   & 0.24$^{\uparrow}$    & 0.35   & 0.23$^{\uparrow}$ & 0.29   & 0.14$^{\downarrow}$& 0.16   & 0.64$^{\uparrow}$& 1.02   & 0.46$^{\downarrow}$  & 0.57    \\ 
    
    \textbf{Health}      & 0.35$^{\uparrow}$    & 0.35   & 0.83$^{\textcolor{red}{\uparrow}}$    & 0.90   & 0.44$^{\textcolor{red}{\uparrow}}$    & 0.38   & 0.97$^{\textcolor{red}{\uparrow}}$    & 1.84   & 0.22$^{\uparrow}$ & 0.34   & 0.18$^{\uparrow}$ & 0.22   & 0.51$^{\uparrow}$& 0.83   & 0.31$^{\downarrow}$  & 0.27    \\ 
    
    \textbf{Home} & 0.97$^{\textcolor{red}{\uparrow}}$    & 1.63   & 0.38$^{\uparrow}$    & 0.30   & 0.41$^{\textcolor{red}{\uparrow}}$    & 0.32   & 0.18$^{\downarrow}$    & 0.25   & 0.22$^{\uparrow}$ & 0.23   & 0.14$^{\downarrow}$& 0.17   & 0.71$^{\uparrow}$& 0.88   & 0.42$^{\downarrow}$  & 0.58    \\ 
    
    \textbf{Kids} & 0.30$^{\uparrow}$    & 0.38   & 0.41$^{\uparrow}$    & 0.33   & 0.61$^{\textcolor{red}{\uparrow}}$    & 0.72   & 0.27$^{\uparrow}$    & 0.25   & 0.22$^{\uparrow}$ & 0.26   & 0.20$^{\uparrow}$ & 0.27   & 0.19$^{\downarrow}$& 0.21   & 0.40$^{\downarrow}$  & 0.95    \\ 
    
    \textbf{News} & 0.31$^{\uparrow}$    & 0.27   & 0.37$^{\uparrow}$    & 0.41   & 0.44$^{\textcolor{red}{\uparrow}}$    & 0.34   & 0.25$^{\uparrow}$    & 0.22   & 0.20$^{\uparrow}$ & 0.21   & 0.17$^{\uparrow}$ & 0.20   & 0.66$^{\uparrow}$& 0.67   & 0.96$^{\uparrow}$& 1.62    \\ 
    
    \textbf{Recreation}  & 0.29$^{\uparrow}$    & 0.43   & 0.68$^{\textcolor{red}{\uparrow}}$    & 1.04   & 0.25$^{\uparrow}$    & 0.32   & 0.16$^{\downarrow}$ & 0.20   & 0.14$^{\downarrow}$ & 0.19   & 0.16$^{\uparrow}$ & 0.18   & 0.35$^{\downarrow}$ & 0.50   & 0.16$^{\downarrow}$  & 0.20    \\ 
    
    \textbf{Reference}   & 1.52$^{\textcolor{red}{\uparrow}}$    & 2.68   & 0.32$^{\uparrow}$    & 0.28   & 0.36$^{\uparrow}$    & 0.19   & 0.79$^{\textcolor{red}{\uparrow}}$    & 1.38   & 0.22$^{\uparrow}$ & 0.26   & 0.23$^{\uparrow}$ & 0.29   & 0.68$^{\uparrow}$& 0.96   & 0.38$^{\downarrow}$  & 0.27    \\ 
    
    \textbf{Regional}    & 0.82$^{\textcolor{red}{\uparrow}}$    & 1.14   & 0.29$^{\uparrow}$    & 0.32   & 0.59$^{\textcolor{red}{\uparrow}}$    & 0.58   & 0.17$^{\downarrow}$ & 0.18   & 0.20$^{\uparrow}$ & 0.18   & 0.16$^{\uparrow}$ & 0.18   & 0.33$^{\downarrow}$& 0.26   & 0.82$^{\uparrow}$& 0.91    \\ 
    
    \textbf{Science}     & 0.35$^{\uparrow}$    & 0.22   & 0.31$^{\uparrow}$    & 0.24   & 0.37$^{\uparrow}$    & 0.38   & 0.27$^{\uparrow}$    & 0.27   & 0.16$^{\downarrow}$ & 0.17   & 0.16$^{\uparrow}$ & 0.23   & 0.35$^{\downarrow}$& 0.35   & 0.45$^{\downarrow}$  & 0.41    \\ 
    
    \textbf{Shopping}    & 0.32$^{\uparrow}$    & 0.23   & 1.35$^{\textcolor{red}{\uparrow}}$    & 1.43   & 0.30$^{\uparrow}$    & 0.20   & 0.16$^{\downarrow}$ & 0.17   & 0.27$^{\uparrow}$ & 0.36   & 0.15$^{\downarrow}$& 0.15   & 0.63$^{\uparrow}$& 0.83   & 0.36$^{\downarrow}$  & 0.26    \\ 
    
    \textbf{Society}     & 0.43$^{\textcolor{red}{\uparrow}}$    & 0.31   & 0.45$^{\uparrow}$    & 0.29   & 0.62$^{\textcolor{red}{\uparrow}}$    & 0.77   & 0.13$^{\downarrow}$    & 0.16   & 0.17$^{\uparrow}$ & 0.17   & 0.12$^{\downarrow}$& 0.15   & 0.54$^{\uparrow}$& 0.46   & 0.43$^{\downarrow}$  & 0.56    \\ 
    
    \textbf{Sports}      & 0.37$^{\textcolor{red}{\uparrow}}$    & 0.30   & 0.38$^{\uparrow}$    & 0.33   & 0.40$^{\textcolor{red}{\uparrow}}$    & 0.31   & 0.19$^{\uparrow}$    & 0.17   & 0.14$^{\downarrow}$ & 0.15   & 0.20$^{\uparrow}$ & 0.27   & 0.23$^{\downarrow}$& 0.25   & 0.55$^{\uparrow}$  & 0.86    \\ 
    
    
    \midrule
    \textbf{Control} & 0.23   & 0.13   & 0.26   & 0.21   & 0.19   & 0.20   & 0.19   & 0.18   & 0.16   & 0.18   & 0.15   & 0.17   & 0.47   & 0.59   & 0.49   & 0.61    \\ 
    
    \bottomrule
    % \textbf{Avg.}   & 0.388     & 0.346     & 0.481     & 0.587     & 0.490     & 0.501     & 0.203     & 0.290     & 0.290     & 0.395     & 0.202     & 0.228     & 0.454     & 0.592     & 0.461     & 0.554      \\ 
    % \textbf{Std.}   & 0.157     & 0.191     & 0.333     & 0.657     & 0.279     & 0.357     & 0.128     & 0.364     & 0.227     & 0.467     & 0.055     & 0.069     & 0.195     & 0.354     & 0.162     & 0.269      \\
    % \bottomrule
    \end{tabular}
    \caption{Ad bidding under CCPA. Avg. column represents the average of each advertiser's median bid value. Std. represents the standard deviation of each advertiser's median bid value. Opt-out, opt-in, and no action represent the bids when we opt-out, opt-in, and do no take any action on selling of user data, respectively. $\uparrow$ and $\downarrow$ indicate bid values that are higher and lower than Control's avg., respectively. $\textcolor{red}{\uparrow}$ and $\textcolor{red}{\downarrow}$ indicate bid values that are Control's avg. $\pm$ std., respectively.}
    \label{table:CCPA-bidding}
    \end{table*}


\begin{table*}
    \centering
    \begin{tabular}{l?{0.3mm}ll|ll|ll?{0.3mm}ll|ll|ll} 
    \toprule

    & \multicolumn{6}{c?{0.3mm}}{\textbf{GDPR}} & \multicolumn{6}{c}{\textbf{CCPA}} \\ 
    
    \textbf{Personas} & \multicolumn{2}{c}{\textbf{OneTrsut}}& \multicolumn{2}{c}{\textbf{CookieBot}}  & \multicolumn{2}{c?{0.3mm}}{\textbf{NAI}}  & \multicolumn{2}{c}{\textbf{OneTrsut}}& \multicolumn{2}{c}{\textbf{CookieBot}}  & \multicolumn{2}{c}{\textbf{NAI}}  \\ 

    \multicolumn{1}{c?{0.3mm}}{}  & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \textbf{Avg.} & \textbf{Std.}   & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c}{\textbf{Std.}}  \\ 
    \toprule
    \textbf{Adult}  & 0.08$^{\textcolor{red}{\uparrow}}$      & 0.00  & \multicolumn{1}{c}{---}& \multicolumn{1}{c|}{---}& 0.66$^{\textcolor{red}{\uparrow}}$ & 0.96& 0.16$^{\downarrow}$    & 0.00  & 0.27$^{\uparrow}$    & 0.20  & 0.29$^{\downarrow}$    & 0.30     \\ 
    
    \textbf{Arts}  & 0.07$^{\textcolor{red}{\uparrow}}$      & 0.00  & \multicolumn{1}{c}{---}& \multicolumn{1}{c|}{---}& 0.05$^{\downarrow}$      & 0.00 & \multicolumn{1}{c}{---}   & \multicolumn{1}{c|}{---} & 0.28$^{\uparrow}$    & 0.20  & 0.18$^{\downarrow}$    & 0.22     \\ 
    
    \textbf{Business}  & 0.08$^{\textcolor{red}{\uparrow}}$      & 0.00  & 0.07$^{\textcolor{red}{\uparrow}}$    & 0.00 & 0.33$^{\uparrow}$ & 0.28& 0.22$^{\downarrow}$    & 0.00  & 0.25$^{\uparrow}$    & 0.22  & 0.25$^{\downarrow}$    & 0.28     \\ 
    
    \textbf{Computers} & \multicolumn{1}{c}{---}   & \multicolumn{1}{c|}{---} & 0.06$^{\textcolor{red}{\uparrow}}$    & 0.00 & 1.20$^{\textcolor{red}{\uparrow}}$ & 1.13& 0.41$^{\textcolor{red}{\uparrow}}$    & 0.00  & 0.38$^{\textcolor{red}{\uparrow}}$    & 0.17  & 0.72$^{\uparrow}$      & 0.87     \\ 
    
    \textbf{Games}  & 0.16$^{\textcolor{red}{\uparrow}}$      & 0.00  & \multicolumn{1}{c}{---}& \multicolumn{1}{c|}{---}& 0.92$^{\textcolor{red}{\uparrow}}$ & 0.84& 0.68$^{\textcolor{red}{\uparrow}}$    & 0.49  & 0.25$^{\uparrow}$    & 0.22  & 0.23$^{\downarrow}$    & 0.22     \\ 
    
    \textbf{Health} & 2.43$^{\textcolor{red}{\uparrow}}$      & 0.00  & 0.05$^{\textcolor{red}{\uparrow}}$    & 0.00 & 0.74$^{\textcolor{red}{\uparrow}}$ & 1.03& 0.09$^{\textcolor{red}{\downarrow}}$    & 0.01  & 2.27$^{\textcolor{red}{\uparrow}}$    & 2.68  & 0.89$^{\uparrow}$      & 1.07     \\ 
    
    \textbf{Home}   & \multicolumn{1}{c}{---}   & \multicolumn{1}{c|}{---} & \multicolumn{1}{c}{---}    & \multicolumn{1}{c|}{---}    & 0.33$^{\uparrow}$ & 0.28& 0.58$^{\textcolor{red}{\uparrow}}$    & 0.37  & 0.25$^{\uparrow}$    & 0.22  & 0.69$^{\uparrow}$      & 0.72     \\ 
    
    \textbf{Kids}   & 0.07$^{\textcolor{red}{\uparrow}}$      & 0.00  & 0.05$^{\textcolor{red}{\uparrow}}$    & 0.00 & 0.07$^{\downarrow}$      & 0.00& 0.30$^{\uparrow}$    & 0.21  & 0.44$^{\textcolor{red}{\uparrow}}$    & 0.17  & 0.06$^{\downarrow}$    & 0.05     \\ 
    
    \textbf{News}   & \multicolumn{1}{c}{---}   & \multicolumn{1}{c|}{---} & \multicolumn{1}{c}{---}& \multicolumn{1}{c|}{---}& 1.53$^{\textcolor{red}{\uparrow}}$ & 0.86& 0.32$^{\uparrow}$    & 0.30  & 0.19$^{\downarrow}$      & 0.00  & 0.74$^{\uparrow}$      & 0.80     \\ 
    
    \textbf{Recreation}& \multicolumn{1}{c}{---}   & \multicolumn{1}{c|}{---} & 0.05$^{\textcolor{red}{\uparrow}}$    & 0.00 & 1.02$^{\textcolor{red}{\uparrow}}$ & 0.77& 0.14$^{\downarrow}$      & 0.00  & 0.37$^{\uparrow}$    & 0.18  & 0.05$^{\downarrow}$    & 0.02     \\ 
    
    \textbf{Reference} & 0.08$^{\textcolor{red}{\uparrow}}$      & 0.01  & \multicolumn{1}{c}{---}& \multicolumn{1}{c|}{---}& 1.47$^{\textcolor{red}{\uparrow}}$ & 0.85& 1.16$^{\textcolor{red}{\uparrow}}$    & 1.12  & 0.37$^{\uparrow}$    & 0.17  & 0.65$^{\uparrow}$      & 0.74     \\ 
    
    \textbf{Regional}  & 0.08$^{\textcolor{red}{\uparrow}}$      & 0.00  & 0.06$^{\textcolor{red}{\uparrow}}$    & 0.00 & 1.78$^{\textcolor{red}{\uparrow}}$ & 0.82& 0.14$^{\downarrow}$      & 0.00  & 0.37$^{\uparrow}$    & 0.18  & 0.62$^{\uparrow}$      & 0.00     \\ 
    
    \textbf{Science}& 0.07$^{\textcolor{red}{\uparrow}}$      & 0.00  & \multicolumn{1}{c}{---}& \multicolumn{1}{c|}{---}& 0.67$^{\textcolor{red}{\uparrow}}$ & 0.90& 0.35$^{\uparrow}$      & 0.28  & 0.39$^{\textcolor{red}{\uparrow}}$    & 0.14  & 0.33$^{\downarrow}$    & 0.20     \\ 
    
    \textbf{Shopping}  & 0.09$^{\textcolor{red}{\uparrow}}$      & 0.02  & \multicolumn{1}{c}{---}& \multicolumn{1}{c|}{---}& 0.75$^{\textcolor{red}{\uparrow}}$ & 0.00& 0.19$^{\downarrow}$      & 0.02  & 0.19$^{\downarrow}$      & 0.22  & 1.11$^{\textcolor{red}{\uparrow}}$      & 1.03     \\ 
    
    \textbf{Society}& \multicolumn{1}{c}{---}   & \multicolumn{1}{c|}{---} & \multicolumn{1}{c}{---}& \multicolumn{1}{c|}{---}& 0.08$^{\downarrow}$      & 0.03& 0.52$^{\textcolor{red}{\uparrow}}$      & 0.42  & 0.25$^{\uparrow}$    & 0.22  & 0.57$^{\uparrow}$      & 0.45     \\ 
    
    \textbf{Sports} & 0.09$^{\textcolor{red}{\uparrow}}$      & 0.02  & \multicolumn{1}{c}{---}& \multicolumn{1}{c|}{---}& 1.01$^{\textcolor{red}{\uparrow}}$ & 0.96& 0.27$^{\uparrow}$      & 0.11  & 0.31$^{\uparrow}$    & 0.17  & 0.22$^{\downarrow}$    & 0.27     \\ 
    
    \midrule

    \textbf{Control}& 0.00    & 0.00  & 0.00 & 0.00 & 0.29    & 0.29& 0.23    & 0.13  & 0.19    & 0.18  & 0.47    & 0.59     \\
    
    \bottomrule

\end{tabular}
\caption{Ad bidding under CCPA and GDPR from advertisers who did not bid or appear when we simulated personas but appeared and bid after we opted opt-out under of processing and selling of data. Avg. column represents the average of each advertiser's median bid value. Std. represents the standard deviation of each advertiser's median bid value. $\uparrow$ and $\downarrow$ indicate bid values that are higher and lower than Control's avg., respectively. $\textcolor{red}{\uparrow}$ and $\textcolor{red}{\downarrow}$ indicate bid values that are Control's avg. $\pm$ std., respectively. \hl{@Zengrui, please swap GDPR and CCPA columns. We discuss GDPR first.}}
\label{table:in_test_not_in_train}
\end{table*}
    





==> stateless-ads-main_3/docs/bidders_appeared_percentage.tex <==


\begin{table}[h]
\centering
\caption{Top 5 most prevalent advertisers that participate in bidding when we opt-out through OneTrust and CookieBot under GDPR and CCPA. GDPR and CCPA columns represent the average number of personas in which the advertiser appear as a bidder across both OneTrust and CookieBot, under GDPR and CCPA, respectively.}
    \begin{tabular}{l?{0.3mm}r?{0.3mm}r} 
    \toprule
     \textbf{Advertisers}& \textbf{GDPR} & \textbf{CCPA}    \\ 
    \toprule


\textbf{AppNexus}      & 93.75\%       & 71.88\%  \\
\textbf{PubMatic}      & 62.50\%       & 100.00\%   \\
\textbf{IndexExchange} & 46.88\%    & 90.63\%   \\
\textbf{Rubicon}       & 34.38\% &  78.13\%   \\
% \textbf{Nobid}         & 21.88\% & 31.25\%       \\
\textbf{TripleLift} &6.25\% & 81.25\% \\
\bottomrule
\end{tabular}
\vspace{-3mm}
\label{tbl:prevalent-advertisers}
\end{table}


% Most prevalent advertisers that participate in cookie syncing, when we opt-out under GDPR and CCPA. These advertiser appear in all personas across OneTrust, CookieBot, and NAI configurations. OT, CB, and NAI columns represent the count of cookie syncing events under OneTrust, CookieBot, and NAI for each advertiser.

==> stateless-ads-main_3/docs/bids-table-california.tex <==
\begin{table*}
%\adjustbox{max width=\textwidth}{
    \centering
    \caption{Ad bidding under CCPA in California. Avg. column represents the mean of all bid value. Std. represents the standard deviation of all bid value. Opt-out and opt-in represent the bids when we opt-out and opt-in the selling of user data, respectively.  $\uparrow$ and $\downarrow$ indicate bid values that are higher and lower than Control's avg., respectively. $\textcolor{red}{\uparrow}$ and $\textcolor{red}{\downarrow}$ indicate bid values that are Control's avg. $\pm$ std., respectively.}
    \begin{tabular}{l?{0.3mm}rr|rr?{0.3mm}rr|rr?{0.3mm}rr|rr} 
    \toprule
     & \multicolumn{4}{c?{0.3mm}}{\textbf{OneTrust}} & \multicolumn{4}{c?{0.3mm}}{\textbf{CookieBot}}& \multicolumn{4}{c}{\textbf{NAI}}    \\ 
     & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c?{0.3mm}}{\textbf{Opt-in}}     & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c?{0.3mm}}{\textbf{Opt-in}}    & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c}{\textbf{Opt-in}}   \\ 
    \textbf{Persona}     & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}}  & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c}{\textbf{Std.}}  \\ 
    \toprule
    
    
    
\textbf{Adult}      & 0.29$^{\downarrow}$                     & 0.35                     & 0.21$^{\downarrow}$                          & 0.31                     &  0.32$^{\uparrow}$                          & 0.19                     & 0.29$^{\uparrow}$                     & 0.53                     &  0.27$^{\downarrow}$                          & 0.42                     & 0.37$^{\uparrow}$                     & 0.47                      \\ 

\textbf{Arts}       & 0.33$^{\downarrow}$                     & 0.41                     & 0.26$^{\downarrow}$                     & 0.28                     &  0.37$^{\uparrow}$                     & 0.55                     & 0.34$^{\uparrow}$                     & 0.30                     &  0.40$^{\downarrow}$                     & 0.46                     & 0.41$^{\uparrow}$                     & 0.43                      \\ 

\textbf{Business}   & 0.40$^{\uparrow}$                     & 0.49                     & 0.70$^{\uparrow}$                     & 0.78                      & 0.25$^{\downarrow}$                       & 0.19                     & 0.32$^{\uparrow}$                     & 0.17                     &  0.40$^{\downarrow}$                       & 0.59                     & 0.31$^{\downarrow}$                       & 0.41                      \\ 

\textbf{Computers}  & 0.32$^{\downarrow}$                     & 0.31                     & 0.47$^{\uparrow}$                     & 0.74                     &  0.34$^{\uparrow}$                     & 0.23                     & 0.35$^{\uparrow}$                     & 0.31                     &  0.48$^{\uparrow}$                     & 0.78                     & 0.51$^{\uparrow}$                     & 0.97                      \\ 

\textbf{Games}      & 0.44$^{\uparrow}$                     & 0.42                     & 0.42$^{\downarrow}$                      & 0.55                     &  0.28$^{\downarrow}$                      & 0.21                     & 0.32$^{\uparrow}$                     & 0.18                     &  0.94$^{\uparrow}$                     & 1.57                     & 0.31$^{\downarrow}$                      & 0.48                      \\ 

\textbf{Health}     & 0.36$^{\downarrow}$                      & 0.40                     & 0.56$^{\uparrow}$                      & 0.63                     &  0.64$^{\textcolor{red}{\uparrow}}$                      & 1.11                     & 0.48$^{\textcolor{red}{\uparrow}}$                      & 0.44                     & 0.28$^{\downarrow}$                      & 0.56                     & 0.50$^{\uparrow}$                      & 0.48                      \\ 

\textbf{Home}       & 1.69$^{\textcolor{red}{\uparrow}}$                      & 2.58                     & 0.39$^{\downarrow}$                     & 0.50                     &  0.26$^{\downarrow}$                     & 0.19                     & 0.28$^{\uparrow}$                      & 0.20                     &  1.18$^{\textcolor{red}{\uparrow}}$                      & 2.82                     & 0.46$^{\uparrow}$                      & 0.90                      \\ 

\textbf{Kids}       & 0.31$^{\downarrow}$                     & 0.36                     & 0.45$^{\uparrow}$                       & 0.59                     &  0.37$^{\uparrow}$                       & 0.55                     & 0.30$^{\uparrow}$                       & 0.53                     &  0.30$^{\downarrow}$                     & 0.58                     & 0.35$^{\uparrow}$                       & 0.65                      \\ 

\textbf{News}       & 0.35$^{\downarrow}$                      & 0.40                     & 0.51$^{\uparrow}$                       & 0.61                     &  0.34$^{\uparrow}$                       & 0.17                     & 0.25$^{\downarrow}$                      & 0.15                     &  0.90$^{\uparrow}$                       & 1.57                     & 0.83$^{\uparrow}$                       & 1.83                      \\ 

\textbf{Recreation} & 0.21$^{\downarrow}$                      & 0.29                     & 0.45$^{\uparrow}$                      & 0.55                     &  0.29$^{\downarrow}$                      & 0.19                     & 0.25$^{\downarrow}$                      & 0.19                     &  0.46$^{\uparrow}$                      & 0.98                     & 0.24$^{\downarrow}$                      & 0.43                      \\ 

\textbf{Reference}  & 0.70$^{\textcolor{red}{\uparrow}}$                      & 1.50                     & 0.54$^{\uparrow}$                      & 0.96                                          & 0.36$^{\uparrow}$                      & 0.42                     & 0.33$^{\uparrow}$                      & 0.20                     &  0.66$^{\uparrow}$                      & 1.06                     & 0.35$^{\uparrow}$                      & 0.45                      \\ 

\textbf{Regional}   & 0.78$^{\textcolor{red}{\uparrow}}$                      & 1.82                     & 0.41$^{\downarrow}$                      & 0.57                                          & 0.30$^{\downarrow}$                      & 0.18                     & 0.26$^{\downarrow}$                      & 0.20                     &  0.58$^{\uparrow}$                      & 0.47                     & 0.33$^{\uparrow}$                      & 0.11                      \\ 

\textbf{Science}    & 0.45$^{\uparrow}$                      & 0.38                     & 0.37$^{\downarrow}$                      & 0.48                                          & 0.34$^{\uparrow}$                      & 0.35                     & 0.28$^{\uparrow}$                      & 0.20                     &  0.33$^{\downarrow}$                      & 0.49                     & 1.04$^{\textcolor{red}{\uparrow}}$                      & 2.11                      \\ 

\textbf{Shopping}   & 0.27$^{\downarrow}$                     & 0.24                     & 0.62$^{\uparrow}$                      & 0.81                     &  0.30$^{\downarrow}$                     & 0.18                     & 0.27$^{\uparrow}$                      & 0.23                     &  0.26$^{\downarrow}$                     & 0.15                     & 0.54$^{\uparrow}$                      & 0.77                      \\ 

\textbf{Society}    & 0.37$^{\uparrow}$                     & 0.40                     & 0.54$^{\uparrow}$                     & 0.64                     &  0.29$^{\downarrow}$                     & 0.19                     & 0.28$^{\uparrow}$                     & 0.19                     &  0.61$^{\uparrow}$                     & 0.86                     & 0.24$^{\downarrow}$                     & 0.36                      \\ 

\textbf{Sports}     & 0.31$^{\downarrow}$                     & 0.31                     & 0.52$^{\uparrow}$                      & 0.63                     &  0.32$^{\uparrow}$                      & 0.17                     & 0.27$^{\downarrow}$                     & 0.17                     & 0.24$^{\downarrow}$                     & 0.40                     & 0.23$^{\downarrow}$                     & 0.44                      \\ 
\midrule
\textbf{Control}    & 0.36                     & 0.34                     & 0.45                     & 0.39                                          & 0.30                     & 0.16                     & 0.27                     & 0.18                                          & 0.44                     & 0.60                     & 0.31                     & 0.53                      \\

    \bottomrule

\end{tabular}

%\vspace{-5mm}
\label{table:CCPA-bidding-mean}
\end{table*}



==> stateless-ads-main_3/docs/bids-table-france.tex <==
\begin{table*}[!h]
%\adjustbox{max width=\textwidth}{
    \centering
        \caption{Ad bidding under GDPR in France. Avg. column represents the mean of all bid value. Std. represents the standard deviation of all bid value. Opt-out and opt-in represent the bids when we opt-out and opt-in the selling of user data, respectively.  $\uparrow$ and $\downarrow$ indicate bid values that are higher and lower than Control's avg., respectively. $\textcolor{red}{\uparrow}$ and $\textcolor{red}{\downarrow}$ indicate bid values that are Control's avg. $\pm$ std., respectively.}
    \begin{tabular}{l?{0.3mm}rr|rr?{0.3mm}rr|rr?{0.3mm}rr|rr} 
    \toprule
     & \multicolumn{4}{c?{0.3mm}}{\textbf{OneTrust}} & \multicolumn{4}{c?{0.3mm}}{\textbf{CookieBot}}& \multicolumn{4}{c}{\textbf{NAI}}    \\ 
     & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c?{0.3mm}}{\textbf{Opt-in}}     & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c?{0.3mm}}{\textbf{Opt-in}}    & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c}{\textbf{Opt-in}}   \\ 
    \textbf{Persona}     & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}}  & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c}{\textbf{Std.}}  \\ 
    \toprule
        
        
        
    \textbf{Adult}                                                              & 0.21$^{\uparrow}$                                           & 0.21                                          & 0.16$^{\downarrow}$                                          & 0.16                                                                                   & 0.10$^{\uparrow}$                                           & 0.00                                          & 0.02$^{\downarrow}$                                          & 0.01                                                                                  & 0.31$^{\uparrow}$                                           & 0.32                                          & 0.19$^{\uparrow}$                                           & 0.18                                           \\ 
    
    \textbf{Arts}                                                               & 0.05$^{\downarrow}$                                          & 0.07                                          & 0.50$^{\uparrow}$                                           & 0.45                                                                                    & 0.04$^{\downarrow}$                                          & 0.03                                          & 0.03$^{\downarrow}$                                          & 0.05                                           & 0.29$^{\uparrow}$                                           & 0.17                                          & 0.24$^{\textcolor{red}{\uparrow}}$                                           & 0.17                                           \\ 
    
    \textbf{Business}                                                           & 0.03$^{\downarrow}$                                          & 0.05                                          & 0.56$^{\uparrow}$                                           & 0.50                                           & 0.27$^{\textcolor{red}{\uparrow}}$                                           & 0.16                                          & 0.17$^{\uparrow}$                                           & 0.17                                           & 0.03$^{\textcolor{red}{\downarrow}}$                                          & 0.02                                          & 0.03$^{\textcolor{red}{\downarrow}}$                                          & 0.01                                           \\ 
    
    \textbf{Computers}                                                          & 0.33$^{\uparrow}$                                           & 0.52                                          & 0.67$^{\uparrow}$                                           & 0.88                                           & 0.23$^{\textcolor{red}{\uparrow}}$                                           & 0.12                                          & 0.11$^{\uparrow}$                                           & 0.07                                                                                    & 0.08$^{\textcolor{red}{\downarrow}}$                                          & 0.08                                          & 0.34$^{\textcolor{red}{\uparrow}}$                                           & 0.46                                           \\ 
    
    \textbf{Games}                                                              & 0.25$^{\uparrow}$                                          & 0.20                                          & 0.96$^{\uparrow}$                                          & 0.92                                                                                  & 0.21$^{\textcolor{red}{\uparrow}}$                                          & 0.22                                          & 0.20$^{\uparrow}$                                          & 0.23                                           & 0.13$^{\downarrow}$                                          & 0.15                                          & - & -  \\ 
    
    \textbf{Health}                                                             & 0.33$^{\uparrow}$                                          & 0.34                                          & 0.74$^{\uparrow}$                                          & 0.55                                                                                    & 0.28$^{\textcolor{red}{\uparrow}}$                                          & 0.41                                          & 0.32$^{\textcolor{red}{\uparrow}}$                                          & 0.18                                                                                   & - & - & - & -  \\ 
    
    \textbf{Home}                                                               & 0.30$^{\uparrow}$                                          & 0.40                                          & 0.85$^{\uparrow}$                                          & 1.28                                                                                    & 0.03$^{\downarrow}$                                          & 0.02                                          & 0.03$^{\downarrow}$                                          & 0.02                                           & 0.07$^{\textcolor{red}{\downarrow}}$                                          & 0.05                                          & 0.04$^{\textcolor{red}{\downarrow}}$                                          & 0.02                                           \\ 
    
    \textbf{Kids}                                                               & 0.33$^{\uparrow}$                                          & 0.34                                          & 0.54$^{\uparrow}$                                          & 0.76                                                                                    & 0.31$^{\textcolor{red}{\uparrow}}$                                          & 0.15                                          & 0.05$^{\downarrow}$                                          & 0.06                                                                                   & 0.14$^{\downarrow}$                                          & 0.18                                          & 0.17$^{\uparrow}$                                          & 0.45                                           \\ 
    
    \textbf{News}                                                               & 0.17$^{\downarrow}$                                          & 0.19                                          & 0.41$^{\downarrow}$                                          & 0.72                                           & 0.26$^{\textcolor{red}{\uparrow}}$                                          & 0.22                                          & 0.31$^{\textcolor{red}{\uparrow}}$                                          & 0.19                                                                                    & 0.07$^{\textcolor{red}{\downarrow}}$                                          & 0.05                                          & 0.05$^{\textcolor{red}{\downarrow}}$                                          & 0.04                                           \\ 
    
    \textbf{Recreation}                                                         & 0.23$^{\uparrow}$                                          & 0.22                                          & 0.22$^{\downarrow}$                                          & 0.27                                           & 0.33$^{\textcolor{red}{\uparrow}}$                                          & 0.18                                          & 0.06$^{\downarrow}$                                          & 0.00                                                                                    & 0.02$^{\textcolor{red}{\downarrow}}$                                          & 0.02                                          & 0.01$^{\textcolor{red}{\downarrow}}$                                          & 0.01                                           \\ 
    
    \textbf{Reference}                                                          & 0.29$^{\uparrow}$                                          & 0.18                                          & 0.68$^{\uparrow}$                                          & 0.86                                                                                    & 0.08$^{\downarrow}$                                          & 0.14                                          & 0.14$^{\uparrow}$                                          & 0.20                                                                                   & 0.24$^{\uparrow}$                                          & 0.18                                          & 0.23$^{\uparrow}$                                          & 0.15                                           \\ 
    
    \textbf{Regional}                                                           & 0.08$^{\downarrow}$                                          & 0.12                                          & 0.65$^{\uparrow}$                                          & 0.54                                                                                    & 0.14$^{\uparrow}$                                          & 0.19                                          & 0.04$^{\downarrow}$                                          & 0.03                                           & 0.30$^{\uparrow}$                                          & 0.29                                          & 0.21$^{\uparrow}$                                          & 0.15                                           \\ 
    
    \textbf{Science}                                                            & 0.21$^{\uparrow}$                                          & 0.22                                          & 0.77$^{\uparrow}$                                          & 1.13                                                                                    & 0.09$^{\downarrow}$                                          & 0.08                                          & 0.09$^{\downarrow}$                                          & 0.08                                           & 0.05$^{\textcolor{red}{\downarrow}}$                                          & 0.03                                          & 0.04$^{\textcolor{red}{\downarrow}}$                                          & 0.03                                           \\ 
    
    \textbf{Shopping}                                                           & 0.38$^{\textcolor{red}{\uparrow}}$                                          & 0.56                                          & 0.67$^{\uparrow}$                                          & 1.10                                           & 0.19$^{\textcolor{red}{\uparrow}}$                                          & 0.07                                          & 0.27$^{\textcolor{red}{\uparrow}}$                                          & 0.13                                                                                    & 0.07$^{\textcolor{red}{\downarrow}}$                                          & 0.15                                          & 0.34$^{\textcolor{red}{\uparrow}}$                                          & 0.68                                           \\ 
    
    \textbf{Society}                                                            & 0.34$^{\uparrow}$                                          & 0.36                                          & 0.50$^{\uparrow}$                                          & 0.63                                           & 0.27$^{\textcolor{red}{\uparrow}}$                                          & 0.26                                          & 0.19$^{\uparrow}$                                          & 0.19                                                                                    & 0.07$^{\textcolor{red}{\downarrow}}$                                          & 0.07                                          & 0.05$^{\textcolor{red}{\downarrow}}$                                          & 0.04                                           \\ 
    
    \textbf{Sports}                                                             & 0.48$^{\textcolor{red}{\uparrow}}$                                          & 0.38                                          & 0.80$^{\uparrow}$                                          & 0.99                                                                                   & 0.01$^{\textcolor{red}{\downarrow}}$                                          & 0.00                                          & 0.02$^{\downarrow}$                                          & 0.00                                           & 0.09$^{\downarrow}$                                          & 0.09                                          & 0.08$^{\textcolor{red}{\downarrow}}$                                          & 0.12                                           \\ 
    
    \midrule
    \textbf{Control}                                                            & 0.18                                          & 0.18                                          & 0.42                                          & 0.63                                                                                    & 0.09                                          & 0.07                                          & 0.09                                          & 0.15                                          &  0.22                                          & 0.14                                          & 0.16                                          & 0.07                                           \\
    
        \bottomrule
    
    \end{tabular}

    \label{table:GDPR-bidding-France-mean}
    \end{table*}
    

==> stateless-ads-main_3/docs/bids-table-germany-california-non-appearing-advertisers.tex <==


\begin{table*}[htb!]
    \centering
    \caption{Ad bidding under CCPA and GDPR from advertisers who did not bid or appear when we simulated personas but appeared and bid after we opted opt-out under of processing and selling of data. Avg. column represents the average of each advertiser's median bid value. Std. represents the standard deviation of each advertiser's median bid value. $\uparrow$ and $\downarrow$ indicate bid values that are higher and lower than Control's avg., respectively. $\textcolor{red}{\uparrow}$ and $\textcolor{red}{\downarrow}$ indicate bid values that are Control's avg. $\pm$ std., respectively.}
    \begin{tabular}{l?{0.3mm}ll|ll|ll?{0.3mm}ll|ll|ll} 
    \toprule

    & \multicolumn{6}{c?{0.3mm}}{\textbf{GDPR}} & \multicolumn{6}{c}{\textbf{CCPA}} \\ 
    
    \textbf{Persona} & \multicolumn{2}{c}{\textbf{OneTrust}}& \multicolumn{2}{c}{\textbf{CookieBot}}  & \multicolumn{2}{c?{0.3mm}}{\textbf{NAI}}  & \multicolumn{2}{c}{\textbf{OneTrust}}& \multicolumn{2}{c}{\textbf{CookieBot}}  & \multicolumn{2}{c}{\textbf{NAI}}  \\ 

    \multicolumn{1}{c?{0.3mm}}{}  & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \textbf{Avg.} & \textbf{Std.}   & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c}{\textbf{Std.}}  \\ 
    \toprule
\textbf{Adult}                              														& 0.08$^{\uparrow}$                                                           & 0.00                                          & 0.02$^{\textcolor{red}{\uparrow}}$                                                           & 0.03                                          & 0.68$^{\textcolor{red}{\uparrow}}$                                                           & 0.96                                          & 0.16$\downarrow$                                                        & 0.00                                          & 0.36$^{\uparrow}$                                                           & 0.16                                          & 0.34$\downarrow$                                                        & 0.42                                           \\ 

\textbf{Arts}                                                                                                          & 0.07$^{\uparrow}$                                                           & 0.00                                          & 0.08$^{\textcolor{red}{\uparrow}}$                                                           & 0.08                                          & 0.05$\downarrow$                                                        & 0.01                                          & 0.33$\downarrow$                                                        & 0.41                                          & 0.40$^{\uparrow}$                                                           & 0.61                                          & 0.22$\downarrow$                                                        & 0.27                                           \\ 

\textbf{Business}                                                                                                      & 0.08$^{\uparrow}$                                                           & 0.00                                          & 0.07$^{\textcolor{red}{\uparrow}}$                                                           & 0.00                                          & 0.30$^{\uparrow}$                                                           & 0.28                                          & 0.38$^{\uparrow}$                                                           & 0.37                                          & 0.27$\downarrow$                                                        & 0.16                                          & 0.32$\downarrow$                                                        & 0.43                                           \\ 

\textbf{Computers}                                                                                                     & 0.09$^{\uparrow}$                                                           & 0.11                                          & 0.11$^{\textcolor{red}{\uparrow}}$                                                           & 0.09                                          & 1.11$^{\textcolor{red}{\uparrow}}$                                                           & 1.12                                          & 0.43$^{\uparrow}$                                                           & 0.22                                          & 0.34$^{\uparrow}$                                                           & 0.16                                          & 0.43$\downarrow$                                                        & 0.65                                           \\ 

\textbf{Games}                                                                                                         & 0.16$^{\textcolor{red}{\uparrow}}$                                                           & 0.01                                          & 3E-3$^{\textcolor{red}{\uparrow}}$                                                           & 0.01                                          & 0.74$^{\textcolor{red}{\uparrow}}$                                                           & 0.83                                          & 0.39$^{\uparrow}$                                                           & 0.49                                          & 0.31$^{\uparrow}$                                                           & 0.16                                          & 0.56$^{\uparrow}$                                                           & 0.74                                           \\ 

\textbf{Health}                                                                                                        & 2.43$^{\textcolor{red}{\uparrow}}$                                                           & 0.00                                          & 0.05$^{\textcolor{red}{\uparrow}}$                                                           & 0.00                                          & 0.68$^{\textcolor{red}{\uparrow}}$                                                           & 0.97                                          & 0.36$\downarrow$                                                        & 0.47                                          & 0.47$^{\textcolor{red}{\uparrow}}$                                                           & 1.32                                          & 0.79$^{\uparrow}$                                                           & 0.96                                           \\ 

\textbf{Home}                                                                                                          & 0.13$^{\uparrow}$                                                           & 0.16                                          & 1.00$^{\textcolor{red}{\uparrow}}$                                                           & 1.37                                          & 0.11$\downarrow$                                                        & 0.18                                          & 0.53$^{\uparrow}$                                                           & 0.45                                          & 0.27$\downarrow$                                                        & 0.17                                          & 0.50$\downarrow$                                                        & 0.63                                           \\ 

\textbf{Kids}                                                                                                          & 0.07$^{\uparrow}$                                                           & 0.00                                          & 0.06$^{\textcolor{red}{\uparrow}}$                                                           & 0.01                                          & 0.07$\downarrow$                                                        & 0.01                                          & 0.31$\downarrow$                                                        & 0.34                                          & 0.41$^{\uparrow}$                                                           & 0.61                                          & 0.27$\downarrow$                                                        & 0.51                                           \\ 

\textbf{News}                                                                                                          & 0.12$^{\uparrow}$                                                           & 0.14                                          & 0.17$^{\textcolor{red}{\uparrow}}$                                                           & 0.03                                          & 0.85$^{\textcolor{red}{\uparrow}}$                                                           & 0.71                                          & 0.35$\downarrow$                                                        & 0.41                                          & 0.20$\downarrow$                                                        & 0.01                                          & 0.84$^{\uparrow}$                                                           & 1.02                                           \\ 

\textbf{Recreation}                                                                                                    & 0.10$^{\uparrow}$                                                           & 0.17                                          & 0.05$^{\textcolor{red}{\uparrow}}$                                                           & 0.00                                          & 1.07$^{\textcolor{red}{\uparrow}}$                                                           & 0.95                                          & 0.12$\downarrow$                                                        & 0.06                                          & 0.34$^{\uparrow}$                                                           & 0.16                                          & 0.13$\downarrow$                                                        & 0.18                                           \\ 

\textbf{Reference}                                                                                                     & 0.07$^{\uparrow}$                                                           & 0.01                                          & 0.18$^{\textcolor{red}{\uparrow}}$                                                           & 0.05                                          & 1.10$^{\textcolor{red}{\uparrow}}$                                                           & 0.77                                          & 1.34$^{\textcolor{red}{\uparrow}}$                                                           & 2.47                                          & 0.33$^{\uparrow}$                                                           & 0.16                                          & 0.59$^{\uparrow}$                                                           & 0.93                                           \\ 

\textbf{Regional}                                                                                                      & 0.08$^{\uparrow}$                                                           & 0.01                                          & 0.06$^{\textcolor{red}{\uparrow}}$                                                           & 0.01                                          & 1.67$^{\textcolor{red}{\uparrow}}$                                                           & 0.84                                          & 0.31$\downarrow$                                                        & 0.37                                          & 0.35$^{\uparrow}$                                                           & 0.16                                          & 0.61$^{\uparrow}$                                                           & 0.01                                           \\ 

\textbf{Science}                                                                                                       & 0.07$^{\uparrow}$                                                           & 0.00                                          & 0.01$^{\textcolor{red}{\uparrow}}$                                                           & 0.03                                          & 0.56$^{\textcolor{red}{\uparrow}}$                                                           & 0.69                                          & 0.46$^{\uparrow}$                                                           & 0.33                                          & 0.34$^{\uparrow}$                                                           & 0.24                                          & 0.36$\downarrow$                                                        & 0.35                                           \\ 

\textbf{Shopping}                                                                                                      & 0.09$^{\uparrow}$                                                           & 0.02                                          & 0.01$^{\textcolor{red}{\uparrow}}$                                                           & 0.05                                          & 0.75$^{\textcolor{red}{\uparrow}}$                                                           & 0.00                                          & 0.28$\downarrow$                                                        & 0.17                                          & 0.32$^{\uparrow}$                                                           & 0.18                                          & 0.78$^{\uparrow}$                                                           & 0.72                                           \\ 

\textbf{Society}                                                                                                       & 0.23$^{\textcolor{red}{\uparrow}}$                                                           & 0.14                                          & 0.16$^{\textcolor{red}{\uparrow}}$                                                           & 0.03                                          & 0.05$\downarrow$                                                        & 0.02                                          & 0.30$\downarrow$                                                        & 0.35                                          & 0.33$^{\uparrow}$                                                           & 0.17                                          & 0.71$^{\uparrow}$                                                           & 0.99                                           \\ 

\textbf{Sports}                                                                                                        & 0.10$^{\uparrow}$                                                           & 0.02                                          & 0.69$^{\textcolor{red}{\uparrow}}$                                                           & 0.97                                          & 0.54$^{\textcolor{red}{\uparrow}}$                                                           & 0.83                                          & 0.32$\downarrow$                                                        & 0.33                                          & 0.33$^{\uparrow}$                                                           & 0.16                                          & 0.40$\downarrow$                                                        & 0.54                                           \\ 

    
    \midrule

\textbf{Control}                                                                                                       & 0.04                                                        & 0.11                                          & 5E-4                                                        & 1.9E-3                                          & 0.16                                                        & 0.20                                          & 0.36                                                        & 0.34                                          & 0.30                                                        & 0.16                                          & 0.53                                                        & 0.61                                           \\

    \bottomrule

\end{tabular}

\label{table:in_test_not_in_train}
\end{table*}

==> stateless-ads-main_3/docs/bids-table-germany.tex <==
\begin{table*}
%\adjustbox{max width=\textwidth}{
    \centering
    \caption{Ad bidding under GDPR in Germany. Avg. column represents the mean of all bid value. Std. represents the standard deviation of all bid value. Opt-out and opt-in represent the bids when we opt-out and opt-in the selling of user data, respectively.  $\uparrow$ and $\downarrow$ indicate bid values that are higher and lower than Control's avg., respectively. $\textcolor{red}{\uparrow}$ and $\textcolor{red}{\downarrow}$ indicate bid values that are Control's avg. $\pm$ std., respectively. --- represents the absence of bids.}
    \begin{tabular}{l?{0.3mm}rr|rr?{0.3mm}rr|rr?{0.3mm}rr|rr} 
    \toprule
     & \multicolumn{4}{c?{0.3mm}}{\textbf{OneTrust}} & \multicolumn{4}{c?{0.3mm}}{\textbf{CookieBot}}& \multicolumn{4}{c}{\textbf{NAI}}    \\ 
     & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c?{0.3mm}}{\textbf{Opt-in}}     & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c?{0.3mm}}{\textbf{Opt-in}}    & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c}{\textbf{Opt-in}}   \\ 
    \textbf{Persona}     & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}}  & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c|}{\textbf{Std.}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c}{\textbf{Std.}}  \\ 
    \toprule


\textbf{Adult}      & 0.25$^{\textcolor{red}{\uparrow}}$                      & 0.60                     & 1.02$^{\textcolor{red}{\uparrow}}$                      & 2.53                      & 0.02$^{\textcolor{red}{\uparrow}}$                      & 0.03                     & 0.01$^{\uparrow}$                      & 0.02                                          & 0.07$^{\downarrow}$                      & 0.07                     & 0.10$^{\uparrow}$                      & 0.08                      \\ 

\textbf{Arts}       & 0.39$^{\textcolor{red}{\uparrow}}$                      & 0.41                     & 0.65$^{\textcolor{red}{\uparrow}}$                      & 1.54                      & 0.08$^{\textcolor{red}{\uparrow}}$                      & 0.08                     & 0.08$^{\textcolor{red}{\uparrow}}$                      & 0.09                      & 0.06$^{\downarrow}$                      & 0.07                     & 0.07$^{\downarrow}$                      & 0.13                      \\ 

\textbf{Business}   & 0.03$^{\downarrow}$                       & 0.04                     & 0.33$^{\uparrow}$                      & 0.79                                          & 0.01$^{\textcolor{red}{\uparrow}}$                      & 0.02                     & 0.02$^{\textcolor{red}{\uparrow}}$                      & 0.05                                          & 1.80$^{\textcolor{red}{\uparrow}}$                      & 2.15                     & 0.30$^{\textcolor{red}{\uparrow}}$                      & 0.65                      \\ 

\textbf{Computers}  & 0.09$^{\uparrow}$                     & 0.11                     & 0.80$^{\textcolor{red}{\uparrow}}$                     & 2.07                                          & 0.16$^{\textcolor{red}{\uparrow}}$                     & 0.05                     & 0.17$^{\textcolor{red}{\uparrow}}$                     & 0.04                                          & 0.21$^{\uparrow}$                     & 1.06                     & 0.54$^{\textcolor{red}{\uparrow}}$                     & 1.56                      \\ 

\textbf{Games}      & 0.16$^{\textcolor{red}{\uparrow}}$                     & 0.01                     & 1.6E-5$^{\downarrow}$                      & 0.00                     & 3E-3$^{\textcolor{red}{\uparrow}}$                     & 0.01                     & 1.3E-5$^{\downarrow}$                      & 1.7E-21                      & 0.09$^{\downarrow}$                      & 0.12                     & 0.12$^{\uparrow}$                     & 0.19                      \\ 

\textbf{Health}     & 0.74$^{\textcolor{red}{\uparrow}}$                      & 1.11                     & --& --& 0.06$^{\textcolor{red}{\uparrow}}$                      & 0.15                     & 0.03$^{\textcolor{red}{\uparrow}}$                      & 0.05                                          & 0.04$^{\downarrow}$                      & 0.05                     & 0.05$^{\downarrow}$                      & 0.10                      \\ 

\textbf{Home}       & 0.13$^{\uparrow}$                      & 0.16                     & 0.43$^{\textcolor{red}{\uparrow}}$                      & 0.71                      & 1.00$^{\textcolor{red}{\uparrow}}$                      & 1.37                     & 0.97$^{\textcolor{red}{\uparrow}}$                      & 1.27                                         & 1.18$^{\textcolor{red}{\uparrow}}$                      & 2.38                     & 0.60$^{\textcolor{red}{\uparrow}}$                      & 1.64                      \\ 

\textbf{Kids}       & 0.05$^{\uparrow}$                      & 0.11                     & 0.16$^{\uparrow}$                      & 0.18                                          & 0.15$^{\textcolor{red}{\uparrow}}$                      & 0.04                     & 0.25$^{\textcolor{red}{\uparrow}}$                      & 0.19                                          & 0.23$^{\textcolor{red}{\uparrow}}$                      & 0.92                     & 0.37$^{\textcolor{red}{\uparrow}}$                      & 1.14                      \\ 

\textbf{News}       & 0.12$^{\uparrow}$                     & 0.14                     & 0.86$^{\textcolor{red}{\uparrow}}$                     & 1.66                                          & 0.17$^{\textcolor{red}{\uparrow}}$                     & 0.03                     & 0.17$^{\textcolor{red}{\uparrow}}$                     & 0.03                                          & 0.06$^{\downarrow}$                      & 0.12                     & 0.04$^{\downarrow}$                      & 0.05                      \\ 

\textbf{Recreation} & 0.10$^{\uparrow}$                     & 0.17                     & 0.41$^{\textcolor{red}{\uparrow}}$                     & 0.74                                          & 0.02$^{\textcolor{red}{\uparrow}}$                     & 0.03                     & 7.3E-4$^{\downarrow}$                     & 7.2E-4                     &  0.07$^{\downarrow}$                     & 0.11                     & 0.17$^{\uparrow}$                     & 0.39                      \\ 

\textbf{Reference}  & 0.04$^{\downarrow}$                     & 0.04                     & 0.17$^{\uparrow}$                      & 0.22                     &  0.18$^{\textcolor{red}{\uparrow}}$                      & 0.05                     & 0.17$^{\textcolor{red}{\uparrow}}$                      & 0.04                     & 0.06$^{\downarrow}$                     & 0.09                     & 0.04$^{\downarrow}$                     & 0.06                      \\ 

\textbf{Regional}   & 0.02$^{\downarrow}$                      & 0.03                     & 0.71$^{\textcolor{red}{\uparrow}}$                      & 1.29                                         & 0.09$^{\textcolor{red}{\uparrow}}$                      & 0.08                     & 0.09$^{\textcolor{red}{\uparrow}}$                      & 0.09                                          & 0.13$^{\uparrow}$                     & 0.20                     & 0.10$^{\uparrow}$                  & 0.06                      \\ 

\textbf{Science}    & 0.09$^{\uparrow}$                     & 0.11                     & 0.11$^{\downarrow}$                     & 0.12                                          & 0.01$^{\textcolor{red}{\uparrow}}$                     & 0.03                     & 3.3E-3$^{\downarrow}$                     & 0.01                                         & 0.13$^{\uparrow}$                     & 0.08                     & 0.12$^{\uparrow}$                     & 0.06                      \\ 

\textbf{Shopping}   & 0.07$^{\uparrow}$                      & 0.12                     & 0.06$^{\downarrow}$                     & 0.09                     &  0.01$^{\textcolor{red}{\uparrow}}$                      & 0.05                     & 0.02$^{\uparrow}$                      & 0.03                     &  0.15$^{\uparrow}$                      & 0.14                     & 0.10$^{\uparrow}$ 	                     & 0.07                      \\ 

\textbf{Society}    & 0.23$^{\textcolor{red}{\uparrow}}$                      & 0.14                     & 0.49$^{\textcolor{red}{\uparrow}}$                      & 0.55                      & 0.16$^{\textcolor{red}{\uparrow}}$                      & 0.03                     & 0.16$^{\textcolor{red}{\uparrow}}$                      & 0.02                      & 0.10$^{\uparrow}$                      & 0.12                     & 0.10$^{\uparrow}$                      & 0.26                      \\ 

\textbf{Sports}     & 0.09$^{\uparrow}$                      & 0.28                     & 0.68$^{\textcolor{red}{\uparrow}}$                      & 1.77                                          & 0.69$^{\textcolor{red}{\uparrow}}$                      & 0.97                     & 0.11$^{\textcolor{red}{\uparrow}}$                      & 0.07                                         & 0.14$^{\uparrow}$                      & 0.25                     & 0.13$^{\uparrow}$                      & 0.17                      \\ 



\midrule
\textbf{Control}    & 0.04                     & 0.11                     & 0.13                     & 0.20                                         & 5.0E-4 & 1.9E-3                     & 0.01                     & 0.01                      & 0.09                     & 0.12                     & 0.09                     & 0.10                      \\

    \bottomrule

\end{tabular}

\label{table:GDPR-bidding-mean}
\end{table*}

==> stateless-ads-main_3/docs/cookie-syncing-events-table.tex <==

\begin{table*}[!htpb]
\centering
    \begin{tabular}{l?{0.3mm}rr|rr?{0.3mm}rr|rr?{0.3mm}rr|rr} 
    \toprule
     & \multicolumn{4}{c?{0.3mm}}{\textbf{OneTrust}} & \multicolumn{4}{c?{0.3mm}}{\textbf{CookieBot}}& \multicolumn{4}{c}{\textbf{NAI}}    \\ 
     & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c?{0.3mm}}{\textbf{Opt-in}}     & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c?{0.3mm}}{\textbf{Opt-in}}    & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c}{\textbf{Opt-in}}   \\ 
    \textbf{Persona}     & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Pct.}} & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Pct.}}  & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c}{\textbf{Pct.}}  \\ 
    \toprule
    
\textbf{Adult}      & 24 & 75\%  & 91  & 66.7\%    & 2 & 100\% & 1  & 100\% & 47 & 45.5\%  & 54 & 54.5\%   \\ 

\textbf{Arts}       & 4  & 50\%  & 49  & 83.3\%    & 1 & 100\% & -- & --   & 32 & 83.3\%  & 41 & 66.7\%   \\ 

\textbf{Business}   & 16 & 50\%  & 106 & 85.7\%    & 2 & 50\%  & 2  & 33.3\%  & 21 & 42.9\%  & 28 & 57.1\%   \\ 

\textbf{Computers}  & 22 & 75\%  & 69  & 80\%    & 1 & 50\%  & 5  & 33.3\%  & 27 & 55.6\%  & 41 & 54.5\%   \\ 

\textbf{Games}      & 2  & 100\% & 12  & 100\%   & --& --   & 1  & 100\% & 29 & 40\%  & 24 & 75\%   \\ 

\textbf{Health}     & 8  & 50\%  & --   & -- & 6 & 50\%  & 5  & 66.7\%  & 42 & 45.5\%  & 35 & 41.7\%   \\ 

\textbf{Home}       & 5  & 75\%  & 57  & 87.5\%    & --& --   & 1  & 33.3\%  & 14 & 28.6\%  & 28 & 50\%   \\ 

\textbf{Kids}       & 28 & 80\%  & 69  & 80\%    & 4 & 33.3\%  & -- & --   & 29 & 57.1\%  & 23 & 44.4\%   \\ 

\textbf{News}       & 8  & 100\% & 67  & 66.7\%    & --& --   & -- & --   & 32 & 62.5\%  & 31 & 66.7\%   \\ 

\textbf{Recreation} & 28 & 100\% & 59  & 75\%    & 5 & 66.7\%  & 1  & 100\% & 42 & 50\%  & 46 & 62.5\%   \\ 

\textbf{Reference}  & 6  & 50\%  & 41  & 60\%    & 1 & 50\%  & 3  & 50\%  & 18 & 40\%  & 28 & 80\%   \\ 

\textbf{Regional}   & 9  & 75\%  & 55  & 75\%    & --& --   & -- & --   & 22 & 57.1\%  & 14 & 66.7\%   \\ 

\textbf{Science}    & 7  & 66.7\%  & 32  & 66.7\%    & 1 & 100\% & 1  & 50\%  & 22 & 50\%  & 22 & 100\%  \\ 

\textbf{Shopping}   & 22 & 50\%  & 40  & 60\%    & 1 & 100\% & 10 & 66.7\%  & 32 & 100\% & 32 & 60\%   \\ 

\textbf{Society}    & 22 & 66.7\%  & 69  & 83.3\%    & 7 & 100\% & -- & --   & 34 & 50\%  & 34 & 66.7\%   \\ 

\textbf{Sports}     & 14 & 50\%  & 49  & 66.7\%    & --& --   & 2  & 50\%  & 31 & 55.6\%  & 35 & 71.4\%   \\
\midrule
\textbf{Average} & 14 & 69.6\% & 54 & 71\% & 2 & 50\% & 2 & 42.7\% & 30 & 54\% & 32 & 63.6\%  \\

\bottomrule
\end{tabular}
\caption{Cookie syncing events by advertisers under GDPR in Germany. Evt. column represents the number of cookie syncing events. Pct. represents the percentage of advertisers that participate in cookie syncing. Opt-out, opt-in represent the configurations when we opt-out and opt-in on selling of user data, respectively.}
\label{tbl:GDPR_cookie_syncing}
\end{table*}



\begin{table*}[!htpb]
\centering
    \begin{tabular}{l?{0.3mm}rr|rr?{0.3mm}rr|rr?{0.3mm}rr|rr} 
    \toprule
     & \multicolumn{4}{c?{0.3mm}}{\textbf{OneTrust}} & \multicolumn{4}{c?{0.3mm}}{\textbf{CookieBot}}& \multicolumn{4}{c}{\textbf{NAI}}    \\ 
     & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c?{0.3mm}}{\textbf{Opt-in}}     & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c?{0.3mm}}{\textbf{Opt-in}}    & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c}{\textbf{Opt-in}}   \\ 
    \textbf{Persona}     & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Pct.}} & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Pct.}}  & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c}{\textbf{Pct.}}  \\ 
    \toprule
\textbf{Adult}      & 61 & 88.9\%  & 41 & 83.3\% & 26 & 42.9\% & 40 & 60\% & 78  & 50\% & 110 & 64.3\%  \\ 

\textbf{Arts}       & 23 & 100\% & 22 & 71.4\% & 29 & 55.6\% & 7  & 50\% & 29  & 54.5\% & 51  & 66.7\%  \\ 

\textbf{Business}   & 24 & 57.1\%  & 33 & 57.1\% & 54 & 50\% & 37 & 50\% & 68  & 53.3\% & 70  & 57.1\%  \\ 

\textbf{Computers}  & 52 & 77.8\%  & 33 & 71.4\% & 13 & 50\% & 35 & 62.5\% & 46  & 43.8\% & 58  & 54.5\%  \\ 

\textbf{Games}      & 32 & 66.7\%  & 26 & 55.6\% & 31 & 55.6\% & 11 & 28.6\% & 61  & 66.7\% & 38  & 38.5\%  \\ 

\textbf{Health}     & 54 & 71.4\%  & 51 & 66.7\% & 18 & 28.6\% & 20 & 50\% & 74  & 53.3\% & 26  & 50\%  \\ 

\textbf{Home}       & 46 & 80\%  & 38 & 62.5\% & 30 & 44.4\% & 24 & 50\% & 77  & 55.6\% & 50  & 50\%  \\ 

\textbf{Kids}       & 32 & 50\%  & 35 & 62.5\% & 34 & 44.4\% & 28 & 50\% & 46  & 50\% & 68  & 60\%  \\ 

\textbf{News}       & 20 & 60\%  & 13 & 55.6\% & 3  & 33.3\% & 6  & 50\% & 37  & 40\% & 61  & 42.9\%  \\ 

\textbf{Recreation} & 34 & 71.4\%  & 45 & 75\% & 10 & 50\% & 12 & 66.7\% & 52  & 58.3\% & 66  & 66.7\%  \\ 

\textbf{Reference}  & 29 & 77.8\%  & 32 & 63.6\% & 27 & 50\% & 19 & 50\% & 61  & 46.7\% & 65  & 50\%  \\ 

\textbf{Regional}   & 50 & 77.8\%  & 41 & 70\% & 5  & 40\% & 20 & 50\% & 10  & 66.7\% & 11  & 37.5\%  \\ 

\textbf{Science}    & 54 & 71.4\%  & 70 & 66.7\% & 33 & 50\% & 45 & 60\% & 103 & 50\% & 65  & 50\%  \\ 

\textbf{Shopping}   & 84 & 80\%  & 63 & 66.7\% & 56 & 50\% & 46 & 66.7\% & 58  & 45.5\% & 32  & 60\%  \\ 

\textbf{Society}    & 33 & 66.7\%  & 32 & 44.4\% & 38 & 50\% & 36 & 42.9\% & 74  & 56.3\% & 58  & 42.9\%  \\ 

\textbf{Sports}     & 33 & 75\%  & 18 & 50\% & 22 & 37.5\% & 23 & 50\% & 45  & 61.5\% & 65  & 50\%  \\
\midrule
\textbf{Average} & 41 & 73.2\% & 37 & 63.9\% & 27 & 45.8\% & 26 & 52.3\% & 57 & 53.3\% & 56 & 52.6\%  \\

\bottomrule
\end{tabular}
\caption{Cookie syncing events by advertisers under CCPA in California. Evt. column represents the number of cookie syncing events. Pct. represents the percentage of advertisers that participate in cookie syncing. Opt-out, opt-in represent the configurations when we opt-out and opt-in on selling of user data, respectively.}
\label{tbl:CCPA_cookie_syncing}
\end{table*}






\begin{table}[!h]
\centering
    \begin{tabular}{l?{0.3mm}rrr?{0.3mm}rrr} 
    \toprule
     & \multicolumn{3}{c?{0.3mm}}{\textbf{GDPR}} & \multicolumn{3}{c}{\textbf{CCPA}}    \\ 
     \textbf{Advertisers}& \multicolumn{1}{c}{\textbf{OT}} & \multicolumn{1}{c}{\textbf{CB}}& \multicolumn{1}{c?{0.3mm}}{\textbf{NAI}}& \multicolumn{1}{c}{\textbf{OT}} & \multicolumn{1}{c}{\textbf{CB}}& \multicolumn{1}{c}{\textbf{NAI}}    \\ 
    \toprule


\textbf{AppNexus}           & 87 & 12 & 183 & 214 & 201& 311 \\ 
\textbf{Conversant} & 32                                                      & 7                                                       & 81                                                       & 215                                                      & 161                                                      & 326                                                       \\ 
\textbf{PubMatic}        & 164                                                     & 43                                                      & 188                                                      & 131                                                      & 94                                                       & 131                                                       \\ 
\textbf{TripleLift}      & 13                                                      & 1                                                       & 159                                                      & 86                                                       & 120                                                      & 139                                                       \\
\textbf{Rubicon}  & 51                                                      & 23                                                      & 68                                                       & 130                                                      & 127                                                      & 115                                                       \\
\bottomrule
\end{tabular}
\caption{Most prevalent advertisers that participate in cookie syncing, when we opt-out under GDPR and CCPA. These advertiser appear in all personas across OneTrust, CookieBot, and NAI configurations. OT, CB, and NAI columns represent the count of cookie syncing events under OneTrust, CookieBot, and NAI for each advertiser.}
\label{tbl:Advertisers_cookie_syncing}
\end{table}

==> stateless-ads-main_3/docs/cookie-syncing-events-table_CCPA.tex <==



\begin{table*}[!htpb]
\centering
\caption{Cookie syncing events by advertisers under CCPA in California. Evt. column represents the number of cookie syncing events. Pct. represents the percentage of advertisers that participate in cookie syncing. Opt-out, opt-in represent the configurations when we opt-out and opt-in on selling of user data, respectively.}
    \begin{tabular}{l?{0.3mm}rr|rr?{0.3mm}rr|rr?{0.3mm}rr|rr} 
    \toprule
     & \multicolumn{4}{c?{0.3mm}}{\textbf{OneTrust}} & \multicolumn{4}{c?{0.3mm}}{\textbf{CookieBot}}& \multicolumn{4}{c}{\textbf{NAI}}    \\ 
     & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c?{0.3mm}}{\textbf{Opt-in}}     & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c?{0.3mm}}{\textbf{Opt-in}}    & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c}{\textbf{Opt-in}}   \\ 
    \textbf{Persona}     & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Pct.}} & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Pct.}}  & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c}{\textbf{Pct.}}  \\ 
    \toprule
\textbf{Adult}      & 61 & 88.9\%  & 41 & 83.3\% & 26 & 42.9\% & 40 & 60\% & 78  & 50\% & 110 & 64.3\%  \\ 

\textbf{Arts}       & 23 & 100\% & 22 & 71.4\% & 29 & 55.6\% & 7  & 50\% & 29  & 54.5\% & 51  & 66.7\%  \\ 

\textbf{Business}   & 24 & 57.1\%  & 33 & 57.1\% & 54 & 50\% & 37 & 50\% & 68  & 53.3\% & 70  & 57.1\%  \\ 

\textbf{Computers}  & 52 & 77.8\%  & 33 & 71.4\% & 13 & 50\% & 35 & 62.5\% & 46  & 43.8\% & 58  & 54.5\%  \\ 

\textbf{Games}      & 32 & 66.7\%  & 26 & 55.6\% & 31 & 55.6\% & 11 & 28.6\% & 61  & 66.7\% & 38  & 38.5\%  \\ 

\textbf{Health}     & 54 & 71.4\%  & 51 & 66.7\% & 18 & 28.6\% & 20 & 50\% & 74  & 53.3\% & 26  & 50\%  \\ 

\textbf{Home}       & 46 & 80\%  & 38 & 62.5\% & 30 & 44.4\% & 24 & 50\% & 77  & 55.6\% & 50  & 50\%  \\ 

\textbf{Kids}       & 32 & 50\%  & 35 & 62.5\% & 34 & 44.4\% & 28 & 50\% & 46  & 50\% & 68  & 60\%  \\ 

\textbf{News}       & 20 & 60\%  & 13 & 55.6\% & 3  & 33.3\% & 6  & 50\% & 37  & 40\% & 61  & 42.9\%  \\ 

\textbf{Recreation} & 34 & 71.4\%  & 45 & 75\% & 10 & 50\% & 12 & 66.7\% & 52  & 58.3\% & 66  & 66.7\%  \\ 

\textbf{Reference}  & 29 & 77.8\%  & 32 & 63.6\% & 27 & 50\% & 19 & 50\% & 61  & 46.7\% & 65  & 50\%  \\ 

\textbf{Regional}   & 50 & 77.8\%  & 41 & 70\% & 5  & 40\% & 20 & 50\% & 10  & 66.7\% & 11  & 37.5\%  \\ 

\textbf{Science}    & 54 & 71.4\%  & 70 & 66.7\% & 33 & 50\% & 45 & 60\% & 103 & 50\% & 65  & 50\%  \\ 

\textbf{Shopping}   & 84 & 80\%  & 63 & 66.7\% & 56 & 50\% & 46 & 66.7\% & 58  & 45.5\% & 32  & 60\%  \\ 

\textbf{Society}    & 33 & 66.7\%  & 32 & 44.4\% & 38 & 50\% & 36 & 42.9\% & 74  & 56.3\% & 58  & 42.9\%  \\ 

\textbf{Sports}     & 33 & 75\%  & 18 & 50\% & 22 & 37.5\% & 23 & 50\% & 45  & 61.5\% & 65  & 50\%  \\
\midrule
\textbf{Average} & 41 & 73.2\% & 37 & 63.9\% & 27 & 45.8\% & 26 & 52.3\% & 57 & 53.3\% & 56 & 52.6\%  \\

\bottomrule
\end{tabular}

\label{tbl:CCPA_cookie_syncing}
\end{table*}






\begin{table}[!h]
\centering
\caption{Most prevalent advertisers that participate in cookie syncing, when we opt-out under GDPR and CCPA. These advertiser appear in all personas across OneTrust, CookieBot, and NAI configurations. OT, CB, and NAI columns represent the count of cookie syncing events under OneTrust, CookieBot, and NAI for each advertiser.}
    \begin{tabular}{l?{0.3mm}rrr?{0.3mm}rrr} 
    \toprule
     & \multicolumn{3}{c?{0.3mm}}{\textbf{GDPR}} & \multicolumn{3}{c}{\textbf{CCPA}}    \\ 
     \textbf{Advertisers}& \multicolumn{1}{c}{\textbf{OT}} & \multicolumn{1}{c}{\textbf{CB}}& \multicolumn{1}{c?{0.3mm}}{\textbf{NAI}}& \multicolumn{1}{c}{\textbf{OT}} & \multicolumn{1}{c}{\textbf{CB}}& \multicolumn{1}{c}{\textbf{NAI}}    \\ 
    \toprule


\textbf{AppNexus}           & 87 & 12 & 183 & 214 & 201& 311 \\ 
\textbf{Conversant} & 32                                                      & 7                                                       & 81                                                       & 215                                                      & 161                                                      & 326                                                       \\ 
\textbf{PubMatic}        & 164                                                     & 43                                                      & 188                                                      & 131                                                      & 94                                                       & 131                                                       \\ 
\textbf{TripleLift}      & 13                                                      & 1                                                       & 159                                                      & 86                                                       & 120                                                      & 139                                                       \\
\textbf{Rubicon}  & 51                                                      & 23                                                      & 68                                                       & 130                                                      & 127                                                      & 115                                                       \\
\bottomrule
\end{tabular}

\label{tbl:Advertisers_cookie_syncing}
\end{table}

==> stateless-ads-main_3/docs/cookie-syncing-events-table_GDPR.tex <==

\begin{table*}[!htpb]
\centering
\caption{Cookie syncing events by advertisers under GDPR in Germany. Evt. column represents the number of cookie syncing events. Pct. represents the percentage of advertisers that participate in cookie syncing. Opt-out, opt-in represent the configurations when we opt-out and opt-in on selling of user data, respectively.}
    \begin{tabular}{l?{0.3mm}rr|rr?{0.3mm}rr|rr?{0.3mm}rr|rr} 
    \toprule
     & \multicolumn{4}{c?{0.3mm}}{\textbf{OneTrust}} & \multicolumn{4}{c?{0.3mm}}{\textbf{CookieBot}}& \multicolumn{4}{c}{\textbf{NAI}}    \\ 
     & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c?{0.3mm}}{\textbf{Opt-in}}     & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c?{0.3mm}}{\textbf{Opt-in}}    & \multicolumn{2}{c}{\textbf{Opt-out}}& \multicolumn{2}{c}{\textbf{Opt-in}}   \\ 
    \textbf{Persona}     & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Pct.}} & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Pct.}}  & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c|}{\textbf{Pct.}} & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c}{\textbf{Pct.}}  \\ 
    \toprule
    
\textbf{Adult}      & 24 & 75\%  & 91  & 66.7\%    & 2 & 100\% & 1  & 100\% & 47 & 45.5\%  & 54 & 54.5\%   \\ 

\textbf{Arts}       & 4  & 50\%  & 49  & 83.3\%    & 1 & 100\% & -- & --   & 32 & 83.3\%  & 41 & 66.7\%   \\ 

\textbf{Business}   & 16 & 50\%  & 106 & 85.7\%    & 2 & 50\%  & 2  & 33.3\%  & 21 & 42.9\%  & 28 & 57.1\%   \\ 

\textbf{Computers}  & 22 & 75\%  & 69  & 80\%    & 1 & 50\%  & 5  & 33.3\%  & 27 & 55.6\%  & 41 & 54.5\%   \\ 

\textbf{Games}      & 2  & 100\% & 12  & 100\%   & --& --   & 1  & 100\% & 29 & 40\%  & 24 & 75\%   \\ 

\textbf{Health}     & 8  & 50\%  & --   & -- & 6 & 50\%  & 5  & 66.7\%  & 42 & 45.5\%  & 35 & 41.7\%   \\ 

\textbf{Home}       & 5  & 75\%  & 57  & 87.5\%    & --& --   & 1  & 33.3\%  & 14 & 28.6\%  & 28 & 50\%   \\ 

\textbf{Kids}       & 28 & 80\%  & 69  & 80\%    & 4 & 33.3\%  & -- & --   & 29 & 57.1\%  & 23 & 44.4\%   \\ 

\textbf{News}       & 8  & 100\% & 67  & 66.7\%    & --& --   & -- & --   & 32 & 62.5\%  & 31 & 66.7\%   \\ 

\textbf{Recreation} & 28 & 100\% & 59  & 75\%    & 5 & 66.7\%  & 1  & 100\% & 42 & 50\%  & 46 & 62.5\%   \\ 

\textbf{Reference}  & 6  & 50\%  & 41  & 60\%    & 1 & 50\%  & 3  & 50\%  & 18 & 40\%  & 28 & 80\%   \\ 

\textbf{Regional}   & 9  & 75\%  & 55  & 75\%    & --& --   & -- & --   & 22 & 57.1\%  & 14 & 66.7\%   \\ 

\textbf{Science}    & 7  & 66.7\%  & 32  & 66.7\%    & 1 & 100\% & 1  & 50\%  & 22 & 50\%  & 22 & 100\%  \\ 

\textbf{Shopping}   & 22 & 50\%  & 40  & 60\%    & 1 & 100\% & 10 & 66.7\%  & 32 & 100\% & 32 & 60\%   \\ 

\textbf{Society}    & 22 & 66.7\%  & 69  & 83.3\%    & 7 & 100\% & -- & --   & 34 & 50\%  & 34 & 66.7\%   \\ 

\textbf{Sports}     & 14 & 50\%  & 49  & 66.7\%    & --& --   & 2  & 50\%  & 31 & 55.6\%  & 35 & 71.4\%   \\
\midrule
\textbf{Average} & 14 & 69.6\% & 54 & 71\% & 2 & 50\% & 2 & 42.7\% & 30 & 54\% & 32 & 63.6\%  \\

\bottomrule
\end{tabular}

\label{tbl:GDPR_cookie_syncing}
\end{table*}





==> stateless-ads-main_3/docs/cookie-syncing-events-table_old.tex <==




\begin{table*}[!h]
\centering
\begin{tabular}{l?{0.3mm}rrrrr?{0.3mm}rrrrr} 
\toprule
 & \multicolumn{5}{c?{0.3mm}}{\textbf{Opt-out}}                                                                                                                                                                                                           & \multicolumn{5}{c}{\textbf{Opt-in}}                                                                                                                                                                                                             \\ 

     \textbf{Persona}     & \multicolumn{1}{l}{\textbf{Requests}} & \multicolumn{1}{l}{\textbf{Http cookies}} & \multicolumn{1}{l}{\textbf{Syncing}} & \multicolumn{1}{l}{\textbf{From}} & \multicolumn{1}{l?{0.3mm}}{\textbf{To}} & \multicolumn{1}{l}{\textbf{Requests}} & \multicolumn{1}{l}{\textbf{Http cookies}} & \multicolumn{1}{l}{\textbf{Syncing}} & \multicolumn{1}{l}{\textbf{From}} & \multicolumn{1}{l}{\textbf{To}}  \\ 
\toprule
\textbf{Adult    }                         & 13743                                            & 1808                                                 & 158                                                           & 138                                & 152                              & 10708                                            & 1310                                                 & 97                                                            & 83                                 & 86                                \\ 

\textbf{Arts}                              & 12800                                            & 1895                                                 & 115                                                           & 99                                 & 102                              & 11551                                            & 1128                                                 & 74                                                            & 66                                 & 65                                \\ 

\textbf{Business}                          & 14420                                            & 1521                                                 & 114                                                           & 103                                & 106                              & 11981                                            & 1553                                                 & 173                                                           & 154                                & 146                               \\ 

\textbf{Computers}                         & 14336                                            & 2358                                                 & 180                                                           & 157                                & 170                              & 12997                                            & 1264                                                 & 105                                                           & 91                                 & 92                                \\ 

\textbf{Games}                             & 13986                                            & 1579                                                 & 138                                                           & 126                                & 130                              & 11796                                            & 1433                                                 & 90                                                            & 80                                 & 83                                \\ 

\textbf{Health}                            & 13543                                            & 2374                                                 & 171                                                           & 151                                & 160                              & 13190                                            & 1537                                                 & 126                                                           & 108                                & 117                               \\ 

\textbf{Home}                              & 13242                                            & 1583                                                 & 133                                                           & 119                                & 126                              & 11587                                            & 1558                                                 & 110                                                           & 98                                 & 103                               \\ 

\textbf{Kids}                              & 11700                                            & 1434                                                 & 97                                                            & 82                                 & 90                               & 12311                                            & 1431                                                 & 98                                                            & 84                                 & 87                                \\ 

\textbf{News}                              & 13884                                            & 1570                                                 & 80                                                            & 73                                 & 75                               & 13775                                            & 1488                                                 & 82                                                            & 76                                 & 74                                \\ 

\textbf{Recreation}                        & 14196                                            & 1533                                                 & 126                                                           & 109                                & 122                              & 14391                                            & 1613                                                 & 133                                                           & 121                                & 129                               \\ 

\textbf{Reference}                         & 13317                                            & 1217                                                 & 95                                                            & 83                                 & 88                               & 15293                                            & 1702                                                 & 71                                                            & 61                                 & 61                                \\ 

\textbf{Regional}                          & 12542                                            & 1660                                                 & 159                                                           & 145                                & 151                              & 12460                                            & 1639                                                 & 148                                                           & 135                                & 132                               \\ 

\textbf{Science}                           & 14038                                            & 1619                                                 & 160                                                           & 140                                & 153                              & 14080                                            & 1752                                                 & 145                                                           & 129                                & 135                               \\ 

\textbf{Shopping}                          & 13458                                            & 2100                                                 & 216                                                           & 194                                & 208                              & 13784                                            & 2017                                                 & 173                                                           & 158                                & 159                               \\ 

\textbf{Society}                           & 14090                                            & 2254                                                 & 125                                                           & 108                                & 118                              & 12759                                            & 1557                                                 & 102                                                           & 90                                 & 96                                \\ 

\textbf{Sports}                            & 12923                                            & 1348                                                 & 131                                                           & 118                                & 119                              & 13728                                            & 1626                                                 & 122                                                           & 107                                & 107                               \\
\bottomrule
\end{tabular}
\caption{Cookie syncing events of Onetrust in CCPA.}
\label{tbl:cookie_CCPA_onetrust}
\end{table*}

\begin{table*}[!h]
\centering
\begin{tabular}{l?{0.3mm}rrrrr?{0.3mm}rrrrr} 
\toprule
 & \multicolumn{5}{c?{0.3mm}}{\textbf{Opt-out}}                                                                                                                                                                                                           & \multicolumn{5}{c}{\textbf{Opt-in}}                                                                                                                                                                                                             \\ 

     \textbf{Persona}     & \multicolumn{1}{l}{\textbf{Requests}} & \multicolumn{1}{l}{\textbf{Http cookies}} & \multicolumn{1}{l}{\textbf{Syncing}} & \multicolumn{1}{l}{\textbf{From}} & \multicolumn{1}{l?{0.3mm}}{\textbf{To}} & \multicolumn{1}{l}{\textbf{Requests}} & \multicolumn{1}{l}{\textbf{Http cookies}} & \multicolumn{1}{l}{\textbf{Syncing}} & \multicolumn{1}{l}{\textbf{From}} & \multicolumn{1}{l}{\textbf{To}}  \\ 
\toprule
\textbf{Adult}                    & 21354                                   & 1555                                        & 92                                                   & 76                        & 84                      & 34857                                   & 3827                                        & 221                                                  & 200                       & 197                      \\ 

\textbf{Arts}                     & 18392                                   & 1311                                        & 36                                                   & 28                        & 34                      & 31319                                   & 3232                                        & 116                                                  & 106                       & 101                      \\ 

\textbf{Business}                 & 17686                                   & 1169                                        & 54                                                   & 48                        & 51                      & 30442                                   & 2558                                        & 206                                                  & 183                       & 184                      \\ 

\textbf{Computers}                & 19727                                   & 1604                                        & 72                                                   & 61                        & 68                      & 32518                                   & 3231                                        & 163                                                  & 147                       & 140                      \\ 

\textbf{Games}                    & 16864                                   & 1603                                        & 47                                                   & 37                        & 45                      & 25319                                   & 1691                                        & 117                                                  & 108                       & 103                      \\ 

\textbf{Health}                   & 14810                                   & 681                                         & 25                                                   & 21                        & 23                      & 31816                                   & 2771                                        & 174                                                  & 154                       & 155                      \\ 

\textbf{Home}                     & 18057                                   & 1031                                        & 33                                                   & 28                        & 31                      & 33273                                   & 3422                                        & 129                                                  & 116                       & 109                      \\ 

\textbf{Kids}                     & 16694                                   & 964                                         & 64                                                   & 54                        & 58                      & 33859                                   & 4046                                        & 214                                                  & 183                       & 186                      \\ 

\textbf{News}                     & 18930                                   & 1149                                        & 43                                                   & 36                        & 36                      & 32084                                   & 3228                                        & 166                                                  & 145                       & 135                      \\ 

\textbf{Recreation}               & 17975                                   & 1083                                        & 82                                                   & 67                        & 76                      & 32981                                   & 3365                                        & 195                                                  & 172                       & 163                      \\ 

\textbf{Reference}                & 17881                                   & 1149                                        & 76                                                   & 67                        & 72                      & 32966                                   & 3579                                        & 212                                                  & 190                       & 184                      \\ 

\textbf{Regional}                 & 17647                                   & 1068                                        & 49                                                   & 38                        & 43                      & 32818                                   & 3771                                        & 191                                                  & 172                       & 167                      \\ 

\textbf{Science}                  & 18830                                   & 1221                                        & 80                                                   & 62                        & 70                      & 36463                                   & 4246                                        & 186                                                  & 158                       & 163                      \\ 

\textbf{Shopping}                 & 20349                                   & 1951                                        & 80                                                   & 64                        & 74                      & 32999                                   & 3732                                        & 178                                                  & 160                       & 163                      \\ 

\textbf{Society}                  & 19812                                   & 1332                                        & 94                                                   & 75                        & 79                      & 30157                                   & 3073                                        & 168                                                  & 146                       & 149                      \\ 

\textbf{Sports}                   & 19200                                   & 1239                                        & 84                                                   & 67                        & 74                      & 33772                                   & 3598                                        & 142                                                  & 121                       & 121                      \\


\bottomrule
\end{tabular}
\caption{Cookie syncing events of Onetrust in GDPR.}
\label{tbl:cookie_GDPR_onetrust}
\end{table*}



==> stateless-ads-main_3/docs/stats-test-table.tex <==
\begin{table*}
\centering
\caption{Mann–Whitney U test to validate our hypothesis that the advertisers bidding behavior does not significantly change between opt-in and opt-out. Column P and R represent p-value and effect size, respectively. Effect size is calculated only in cases when there is statistically significant difference (when p-value is smaller than 0.05). Otherwise, we use ``--'' in the table, to represent that we do not calculate this effect size.}
\begin{tabular}{l?{0.3mm}rr|rr|rr?{0.3mm}rr|rr|rr} 
    \toprule
\multicolumn{1}{c?{0.3mm}}{\multirow{3}{*}{\textbf{Persona}}} & \multicolumn{6}{c?{0.3mm}}{\textbf{GDPR}}                                                                                                                                                                        & \multicolumn{6}{c}{\textbf{CCPA}}                                                                                                                                                                         \\ 

\multicolumn{1}{c?{0.3mm}}{}                         & \multicolumn{2}{c}{\textbf{OneTrust}}                            & \multicolumn{2}{c}{\textbf{CookieBot}}                           & \multicolumn{2}{c?{0.3mm}}{\textbf{NAI}}                                 & \multicolumn{2}{c}{\textbf{OneTrust}}                            & \multicolumn{2}{c}{\textbf{CookieBot}}                           & \multicolumn{2}{c}{\textbf{NAI}}                                  \\ 

\multicolumn{1}{c?{0.3mm}}{}                         & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{E}} & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{E}} & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c?{0.3mm}}{\textbf{E}} & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{E}} & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{E}} & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c}{\textbf{E}}  \\ 
\midrule
\textbf{Adult}                                          & 0.00                   & 0.29                   & 0.20                   & --                   & 0.34                   & --                   & 0.18                   & --                   & 0.00                   & 0.20                   & 0.34                   & --                    \\ 

\textbf{Arts}                                           & 0.13                   & -- & 0.91                   & --                   & 0.10                   & - & 0.68                   & --                   & 0.95                   & --                   & 0.10                   & --                    \\ 

\textbf{Business}                                       & 0.00                   & 0.53                   & 0.01                   & 0.47                   & 0.97                   & --                   & 0.03                   & 0.12                   & 0.00                   & 0.28                   & 0.97                   & --                   \\ 

\textbf{Computers}                                      & 0.00                   & 0.40                   & 0.71                   & --                   & 0.01                   & 0.11                   & 0.85                   & --                   & 0.85                   & --                   & 0.01                   & 0.11                    \\ 

\textbf{Games}                                          & 0.33                   & --                   & 0.32                   & --                                     & 0.00                   & 0.12                   & 0.26                   & --                                     & 0.05                   & 0.12                   & 0.00                   & 0.12                    \\ 

\textbf{Health}                                         & --                      & --                      & 0.95                   & --                                     & 0.00                   & 0.19                   & 0.00                   & 0.18                   & 0.11                   & --                                     & 0.00                   & 0.19                    \\ 

\textbf{Home}                                           & 0.00                   & 0.24                   & 1.00                   & --                                     & 0.00                   & 0.12                   & 0.00                   & 0.22                   & 0.48                   & --                                     & 0.00                   & 0.12                    \\ 

\textbf{Kids}                                           & 0.00                   & 0.40                   & 0.00                   & 0.41                   & 0.63                   & --                                     & 0.10                   & --                                     & 0.00                   & 0.18                   & 0.63                   & --                                      \\ 

\textbf{News}                                           & 0.00                   & 0.27                   & 0.93                   & --                                     & 0.29                   & --                                     & 0.01                   & 0.16                   & 0.01                   & 0.20                   & 0.29                   & --                                      \\ 

\textbf{Recreation}                                     & 0.00                   & 0.60                   & 0.34                   & --                                     & 0.06                   & --                                     & 0.00                   & 0.28                   & 0.26                   & --                                     & 0.06                   & --                                      \\ 

\textbf{Reference}                                      & 0.06                   & --                                     & 0.75                   & --                                     & 0.00                   & 0.11                   & 0.59                   & --                                     & 0.74                   & --                                     & 0.00                   & 0.11                    \\ 

\textbf{Regional}                                       & 0.00                   & 0.43                   & 0.66                   & --                                     & 0.43                   & --                                     & 0.45                   & --                                     & 0.27                   & --                                     & 0.43                   & --                                      \\ 

\textbf{Science}                                        & 0.62                   & --                                     & 0.53                   & --                                     & 0.45                   & --                                     & 0.02                   & 0.15                   & 0.52                   & --                                     & 0.45                   & --                                      \\ 

\textbf{Shopping}                                       & 0.92                   & --                                     & 0.02                   & 0.33                   & 0.41                   & --                                     & 0.00                   & 0.24                   & 0.01                   & 0.16                   & 0.41                   & --                                      \\ 

\textbf{Society}                                        & 0.00                   & 0.25                   & 0.20                   & --                                     & 0.00                   & 0.19                   & 0.03                   & 0.15                   & 0.58                   & --                                     & 0.00                   & 0.19                    \\ 

\textbf{Sports}                                         & 0.00                   & 0.39                   & 0.02                   & 0.29                   & 0.71                   & --                                     & 0.19                   & --                                     & 0.01                   & 0.15                   & 0.71                   & --                                      \\

\bottomrule
\end{tabular}

\label{table:u-test}
\end{table*}

==> stateless-ads-main_3/includes/packages.tex <==
\usepackage{marvosym}
\usepackage{colortbl}
\newcommand{\hi}[1]{\textcolor{red}{#1}}
\newcolumntype{?}[1]{!{\vrule width #1}}
\usepackage{url}
\usepackage{booktabs}
\usepackage{xspace}
\def\UrlBreaks{\do\/\do-}
\usepackage{breakurl}
\usepackage{subfig}
\usepackage{multirow}
\usepackage{color,soul}
\usepackage{enumitem}
\usepackage{tikz}
\usepackage{listings}
% \usepackage[colorlinks]{hyperref}
% \usepackage[flushleft]{threeparttable}
\usepackage{adjustbox}

==> tables/appear-after-out/NAI.tex <==

\begin{table}[htb!]
\centering

\caption{Ad bidding under GDPR and CCPA from advertisers who did not bid or appear when we simulated personas but appeared and bid after we opted opt-out under of processing and selling of data in NAI. Avg. column represents the mean of all bid value. Std. represents the standard deviation of all bid value. \textcolor{highbids}{Light red} and \textcolor{lowbids}{Light blue} indicate bid values that are higher and lower than Control's avg., respectively. \textcolor{higherbids}{Dark red} and \textcolor{lowerbids}{Dark blue} indicate bid values that are Control's avg. $\pm$ std., respectively.}





    \begin{tabular}{l?{0.3mm}ll?{0.3mm}ll} 
    \toprule

    & \multicolumn{2}{c?{0.3mm}}{\textbf{GDPR}} & \multicolumn{2}{c}{\textbf{CCPA}} \\ 
    


    \multicolumn{1}{c?{0.3mm}}{}  & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}} &  \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c}{\textbf{Std.}}  \\ 
    \toprule
    
\textbf{Adult}      & 1.42E-03 {\cellcolor{higherbids}}& 0.01     & 2.26E-03 {\cellcolor{lowerbids}}& 0.01  \\
\textbf{Arts}       & 0.00     & 0.00     & 1.25E-03 {\cellcolor{lowerbids}}& 0.01  \\
\textbf{Business}   & 0.00     & 0.00     & 0.00     {\cellcolor{lowerbids}}& 0.00  \\
\textbf{Computers}  & 4.09E-03 {\cellcolor{higherbids}}& 0.03     & 0.00   {\cellcolor{lowerbids}}  & 0.00  \\
\textbf{Games}      & 0.00     & 0.00     & 0.00   {\cellcolor{lowerbids}}  & 0.00  \\
\textbf{Health}     & 1.00E-03 {\cellcolor{higherbids}}& 4.36E-03 & 0.01   {\cellcolor{lowerbids}}  & 0.05  \\
\textbf{Home}       & 0.00     & 0.00     & 0.00  {\cellcolor{lowerbids}}   & 0.00  \\
\textbf{Kids}       & 0.00     & 0.00     & 0.00  {\cellcolor{lowerbids}}   & 0.00  \\
\textbf{News}       & 0.00     & 0.00     & 1.92E-03 {\cellcolor{lowerbids}}& 0.01  \\
\textbf{Recreation} & 0.00     & 0.00     & 2.26E-03 {\cellcolor{lowerbids}}& 0.01  \\
\textbf{Reference}  & 1.37E-03 {\cellcolor{higherbids}}& 0.01     & 3.97E-03 {\cellcolor{lowerbids}} & 0.01  \\
\textbf{Regional}   & 0.00     & 0.00     & 0.03   {\cellcolor{lowerbids}}  & 0.12  \\
\textbf{Science}    & 0.00     & 0.00     & 0.00  {\cellcolor{lowerbids}}   & 0.00  \\
\textbf{Shopping}   & 0.00     & 0.00     & 0.00   {\cellcolor{lowerbids}}  & 0.00  \\
\textbf{Society}    & 0.00     & 0.00     & 0.00  {\cellcolor{lowerbids}}   & 0.00  \\
\textbf{Sports}     & 0.00     & 0.00     & 3.47E-03 {\cellcolor{lowerbids}}& 0.02  \\
\midrule

\textbf{Control}    & 0.00 & 0.00 & 0.07 & 0.15 \\
\bottomrule             
\end{tabular}
\label{table:NAI-appear-after-out}
\end{table}

==> tables/appear-after-out/cookiebot.tex <==

\begin{table}[htb!]
\centering

\caption{Ad bidding under GDPR and CCPA from advertisers who did not bid or appear when we simulated personas but appeared and bid after we opted opt-out under of processing and selling of data in Cookiebot. Avg. column represents the mean of all bid value. Std. represents the standard deviation of all bid value. \textcolor{highbids}{Light red} and \textcolor{lowbids}{Light blue} indicate bid values that are higher and lower than Control's avg., respectively. \textcolor{higherbids}{Dark red} and \textcolor{lowerbids}{Dark blue} indicate bid values that are Control's avg. $\pm$ std., respectively.}





    \begin{tabular}{l?{0.3mm}ll?{0.3mm}ll} 
    \toprule

    & \multicolumn{2}{c?{0.3mm}}{\textbf{GDPR}} & \multicolumn{2}{c}{\textbf{CCPA}} \\ 
    


    \multicolumn{1}{c?{0.3mm}}{}  & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}} &  \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c}{\textbf{Std.}}  \\ 
    \toprule
\textbf{Adult}      & 0.37 {\cellcolor{highbids}}& 0.20 & 0.37 {\cellcolor{highbids}}& 0.20  \\
\textbf{Arts}       & 0.35 {\cellcolor{highbids}}& 0.21 & 0.37 {\cellcolor{highbids}}& 0.20  \\
\textbf{Business}   & 0.35 {\cellcolor{highbids}}& 0.21 & 0.37 {\cellcolor{highbids}}& 0.20  \\
\textbf{Computers}  & 0.35 {\cellcolor{highbids}}& 0.21 & 0.37 {\cellcolor{highbids}}& 0.20  \\
\textbf{Games}      & 0.38 {\cellcolor{highbids}}& 0.20 & 0.36 {\cellcolor{highbids}}& 0.20  \\
\textbf{Health}     & 0.35 {\cellcolor{highbids}} & 0.21 & 0.37 {\cellcolor{highbids}}& 0.20  \\
\textbf{Home}       & 0.38 {\cellcolor{highbids}}& 0.20 & 0.36 {\cellcolor{highbids}}& 0.20  \\
\textbf{Kids}       & 0.37 {\cellcolor{highbids}}& 0.20 & 0.36 {\cellcolor{highbids}}& 0.21  \\
\textbf{News}       & 0.35 {\cellcolor{highbids}}& 0.21 & 0.37 {\cellcolor{highbids}}& 0.20  \\
\textbf{Recreation} & 0.37 {\cellcolor{highbids}}& 0.20 & 0.36 {\cellcolor{highbids}}& 0.20  \\
\textbf{Reference}  & 0.37 {\cellcolor{highbids}}& 0.20 & 0.37 {\cellcolor{highbids}}& 0.20  \\
\textbf{Regional}   & 0.38 {\cellcolor{highbids}}& 0.19 & 0.36 {\cellcolor{highbids}}& 0.21  \\
\textbf{Science}    & 0.35 {\cellcolor{highbids}}& 0.21 & 0.37 {\cellcolor{highbids}}& 0.20  \\
\textbf{Shopping}   & 0.37 {\cellcolor{highbids}}& 0.20 & 0.31 {\cellcolor{lowbids}}& 0.23  \\
\textbf{Society}    & 0.37 {\cellcolor{highbids}}& 0.20 & 0.37 {\cellcolor{highbids}}& 0.20  \\
\textbf{Sports}     & 0.37 {\cellcolor{highbids}}& 0.20 & 0.33 {\cellcolor{highbids}}& 0.22  \\    
                                  
\midrule
\textbf{Control}    & 0.33 & 0.22 & 0.32 & 0.22 \\

\bottomrule             
\end{tabular}
\label{table:cookiebot-appear-after-out}
\end{table}

==> tables/appear-after-out/didomi.tex <==

\begin{table}[htb!]
\centering

\caption{Ad bidding under GDPR and CCPA from advertisers who did not bid or appear when we simulated personas but appeared and bid after we opted opt-out under of processing and selling of data in Didomi. Avg. column represents the mean of all bid value. Std. represents the standard deviation of all bid value. \textcolor{highbids}{Light red} and \textcolor{lowbids}{Light blue} indicate bid values that are higher and lower than Control's avg., respectively. \textcolor{higherbids}{Dark red} and \textcolor{lowerbids}{Dark blue} indicate bid values that are Control's avg. $\pm$ std., respectively.}





    \begin{tabular}{l?{0.3mm}ll?{0.3mm}ll} 
    \toprule

    & \multicolumn{2}{c?{0.3mm}}{\textbf{GDPR}} & \multicolumn{2}{c}{\textbf{CCPA}} \\ 
    


    \multicolumn{1}{c?{0.3mm}}{}  & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}} &  \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c}{\textbf{Std.}}  \\ 
    \toprule
\textbf{Adult}      & --   & --   & 0.12 {\cellcolor{lowbids}}& 0.08  \\
\textbf{Arts}       & 0.05 & 0.00 & 0.45 {\cellcolor{higherbids}}& 1.34  \\
\textbf{Business}   & --   & --   & 0.15 {\cellcolor{lowbids}} & 0.09  \\
\textbf{Computers}  & 0.05 & 0.00 & 0.45 {\cellcolor{higherbids}}& 1.08  \\
\textbf{Games}      & 0.03 {\cellcolor{lowerbids}}& 0.02 & 0.15 {\cellcolor{lowbids}}& 0.10  \\
\textbf{Health}     & --   & --   & 0.16 {\cellcolor{lowbids}}& 0.12  \\
\textbf{Home}       & 0.05 & 0.00 & 0.23 {\cellcolor{highbids}}& 0.44  \\
\textbf{Kids}       & 0.06 {\cellcolor{higherbids}}& 0.00 & 0.04 {\cellcolor{lowbids}}& 0.09  \\
\textbf{News}       & --   & --   & 0.18 & 0.25  \\
\textbf{Recreation} & 0.06 {\cellcolor{higherbids}}& 0.00 & 0.14 {\cellcolor{lowbids}}& 0.12  \\
\textbf{Reference}  & --   & --   & 0.17 {\cellcolor{lowbids}}& 0.22  \\
\textbf{Regional}   & --   & --   & 0.22 {\cellcolor{highbids}}& 0.58  \\
\textbf{Science}    & 0.41 {\cellcolor{higherbids}}& 0.00 & 0.16 {\cellcolor{lowbids}}& 0.09  \\
\textbf{Shopping}   & 0.03 {\cellcolor{lowerbids}}& 0.00 & 0.19 {\cellcolor{highbids}}& 0.35  \\
\textbf{Society}    & 0.05 & 0.00 & 0.24 {\cellcolor{highbids}}& 1.10  \\
\textbf{Sports}     & 0.05 & 0.00 & 0.18 & 0.15  \\    
                                  
\midrule

\textbf{Control}    & 0.05 & 3E-3 & 0.18 & 0.16 \\
\bottomrule             
\end{tabular}
\label{table:didomi-appear-after-out}
\end{table}

==> tables/appear-after-out/onetrust.tex <==

\begin{table}[htb!]
\centering

\caption{Ad bidding under GDPR and CCPA from advertisers who did not bid or appear when we simulated personas but appeared and bid after we opted opt-out under of processing and selling of data in Onetrust. Avg. column represents the mean of all bid value. Std. represents the standard deviation of all bid value. \textcolor{highbids}{Light red} and \textcolor{lowbids}{Light blue} indicate bid values that are higher and lower than Control's avg., respectively. \textcolor{higherbids}{Dark red} and \textcolor{lowerbids}{Dark blue} indicate bid values that are Control's avg. $\pm$ std., respectively.}





    \begin{tabular}{l?{0.3mm}ll?{0.3mm}ll} 
    \toprule

    & \multicolumn{2}{c?{0.3mm}}{\textbf{GDPR}} & \multicolumn{2}{c}{\textbf{CCPA}} \\ 
    


    \multicolumn{1}{c?{0.3mm}}{}  & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}} &  \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c}{\textbf{Std.}}  \\ 
    \toprule
\textbf{Adult}      & 0.02 & 4.95E-03 & 1.64 {\cellcolor{highbids}}& 0.85  \\
\textbf{Arts}       & --   & --   & 1.43 {\cellcolor{highbids}}& 1.03  \\
\textbf{Business}   & 0.01 {\cellcolor{lowerbids}}& 0.01 & 1.29 {\cellcolor{highbids}}& 1.22  \\
\textbf{Computers}  & 0.02 & 0.00 & 1.78 {\cellcolor{highbids}}& 0.94  \\
\textbf{Games}      & 0.02 & 0.00 & 1.50 {\cellcolor{highbids}}& 0.87  \\
\textbf{Health}     & 0.03 {\cellcolor{higherbids}}& 0.02 & 1.37 {\cellcolor{highbids}}& 0.77  \\
\textbf{Home}       & 0.31 {\cellcolor{higherbids}}& 0.25 & 1.63 {\cellcolor{highbids}}& 0.87  \\
\textbf{Kids}       & 0.02 & 0.01 & 1.95 {\cellcolor{highbids}}& 1.14  \\
\textbf{News}       & 0.02 & 0.00 & 1.76 {\cellcolor{highbids}}& 1.00  \\
\textbf{Recreation} & 0.02 & 0.01 & 1.55 {\cellcolor{highbids}}& 0.70  \\
\textbf{Reference}  & 0.03 {\cellcolor{higherbids}}& 0.01 & 1.86 {\cellcolor{highbids}}& 1.05  \\
\textbf{Regional}   & 0.01 {\cellcolor{lowerbids}}& 4.79E-03 & 1.36 {\cellcolor{highbids}}& 0.50  \\
\textbf{Science}    & 0.03 {\cellcolor{higherbids}}& 0.02 & 2.05 {\cellcolor{higherbids}}& 1.16  \\
\textbf{Shopping}   & 1.10 {\cellcolor{higherbids}}& 0.00 & 1.77 {\cellcolor{highbids}}& 1.31  \\
\textbf{Society}    & 0.01 {\cellcolor{lowerbids}}& 3.97E-03 & 1.83 {\cellcolor{highbids}}& 1.28  \\
\textbf{Sports}     & 0.02 & 0.00 & 1.51 {\cellcolor{highbids}}& 1.00  \\    
                                  
\midrule
\textbf{Control}    & 0.02 & 4.00E-03 & 0.88 & 1.18 \\

\bottomrule             
\end{tabular}
\label{table:onetrust-appear-after-out}
\end{table}

==> tables/appear-after-out/quantcast.tex <==

\begin{table}[htb!]
\centering

\caption{Ad bidding under GDPR and CCPA from advertisers who did not bid or appear when we simulated personas but appeared and bid after we opted opt-out under of processing and selling of data in Quantcast. Avg. column represents the mean of all bid value. Std. represents the standard deviation of all bid value. \textcolor{highbids}{Light red} and \textcolor{lowbids}{Light blue} indicate bid values that are higher and lower than Control's avg., respectively. \textcolor{higherbids}{Dark red} and \textcolor{lowerbids}{Dark blue} indicate bid values that are Control's avg. $\pm$ std., respectively.}





    \begin{tabular}{l?{0.3mm}ll?{0.3mm}ll} 
    \toprule

    & \multicolumn{2}{c?{0.3mm}}{\textbf{GDPR}} & \multicolumn{2}{c}{\textbf{CCPA}} \\ 
    


    \multicolumn{1}{c?{0.3mm}}{}  & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}} &  \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c}{\textbf{Std.}}  \\ 
    \toprule
\textbf{Adult}      & 0.19 {\cellcolor{highbids}}& 0.55 & 0.20  {\cellcolor{highbids}}& 0.22  \\
\textbf{Arts}       & 0.16 & 0.20 & 0.29  {\cellcolor{highbids}}& 1.51  \\
\textbf{Business}   & 0.14 {\cellcolor{lowbids}}& 0.19 & 0.19  {\cellcolor{highbids}}& 0.46  \\
\textbf{Computers}  & 0.28 {\cellcolor{higherbids}}& 0.66 & 0.21  {\cellcolor{highbids}}& 0.57  \\
\textbf{Games}      & 0.44 {\cellcolor{higherbids}}& 0.97 & 0.24  {\cellcolor{highbids}}& 0.69  \\
\textbf{Health}     & 0.17 {\cellcolor{highbids}}& 0.20 & 0.52 {\cellcolor{higherbids}}& 1.19  \\
\textbf{Home}       & 0.16 & 0.18 & 0.18  {\cellcolor{highbids}}& 0.16  \\
\textbf{Kids}       & 0.25 {\cellcolor{higherbids}}& 0.55 & 0.23  {\cellcolor{highbids}}& 0.53  \\
\textbf{News}       & 0.20 {\cellcolor{highbids}}& 0.38 & 0.17 & 0.14  \\
\textbf{Recreation} & 0.18 {\cellcolor{highbids}}& 0.33 & 0.16 {\cellcolor{lowbids}}& 0.11  \\
\textbf{Reference}  & 0.18 {\cellcolor{highbids}}& 0.29 & 0.22  {\cellcolor{highbids}}& 0.63  \\
\textbf{Regional}   & 0.13 {\cellcolor{lowbids}}& 0.18 & 0.23  {\cellcolor{highbids}}& 0.81  \\
\textbf{Science}    & 0.37 {\cellcolor{higherbids}}& 0.79 & 0.23  {\cellcolor{highbids}}& 0.64  \\
\textbf{Shopping}   & 0.15 {\cellcolor{lowbids}}& 0.08 & 0.22  {\cellcolor{highbids}}& 0.62  \\
\textbf{Society}    & 0.12 {\cellcolor{lowbids}}& 0.08 & 0.16 {\cellcolor{lowbids}}& 0.13  \\
\textbf{Sports}     & 0.18 {\cellcolor{highbids}}& 0.30 & 0.19  {\cellcolor{highbids}}& 0.58  \\    
                                  
\midrule
\textbf{Control}    & 0.16 & 0.08 & 0.17 & 0.18 \\

\bottomrule             
\end{tabular}
\label{table:quantcast-appear-after-out}
\end{table}

==> tables/bids-opt-in/NAI.tex <==

\begin{table}[htb!]
\centering

\caption{Ad bidding under GDPR and CCPA in NAI after opt-in. Avg. column represents the mean of all bid value. Std. represents the standard deviation of all bid value. \textcolor{highbids}{Light red} and \textcolor{lowbids}{Light blue} indicate bid values that are higher and lower than Control's avg., respectively. \textcolor{higherbids}{Dark red} and \textcolor{lowerbids}{Dark blue} indicate bid values that are Control's avg. $\pm$ std., respectively.}





    \begin{tabular}{l?{0.3mm}ll?{0.3mm}ll} 
    \toprule

    & \multicolumn{2}{c?{0.3mm}}{\textbf{GDPR}} & \multicolumn{2}{c}{\textbf{CCPA}} \\ 
    


    \multicolumn{1}{c?{0.3mm}}{}  & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}} &  \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c}{\textbf{Std.}}  \\ 
    \toprule
    
\textbf{Adult}      & 3.91E-03  {\cellcolor{highbids}}                                     & 0.03     & 0.07 {\cellcolor{highbids}}                                    & 0.12  \\
\textbf{Arts}       & 1.61E-03  {\cellcolor{lowbids}}                                     & 0.01     & 0.07 {\cellcolor{highbids}}                                    & 0.15  \\
\textbf{Business}   & 0.01     {\cellcolor{highbids}}                                      & 0.04     & 0.08 {\cellcolor{highbids}}                                    & 0.21  \\
\textbf{Computers}  & 0.01    {\cellcolor{highbids}}                                       & 0.03     & 0.03 {\cellcolor{lowbids}}                                    & 0.07  \\
\textbf{Games}      & 0.00     {\cellcolor{lowbids}}                                    & 0.00     & 0.03 {\cellcolor{lowbids}}                                    & 0.07  \\
\textbf{Health}     & 0.01   {\cellcolor{highbids}}                                        & 0.04     & 0.20 {\cellcolor{higherbids}}                                    & 0.40  \\
\textbf{Home}       & 0.00   {\cellcolor{lowbids}}                                      & 0.00     & 0.05 {\cellcolor{highbids}}                                    & 0.11  \\
\textbf{Kids}       & 4.32E-03  {\cellcolor{highbids}}                                     & 0.03     & 0.08 {\cellcolor{highbids}}                                     & 0.16  \\
\textbf{News}       & 1.34E-03 {\cellcolor{lowbids}}                                    & 0.01     & 0.06 {\cellcolor{highbids}}                                    & 0.15  \\
\textbf{Recreation} & 2.28E-03 {\cellcolor{lowbids}}                                    & 0.01     & 0.08 {\cellcolor{highbids}}                                    & 0.12  \\
\textbf{Reference}  & 1.92E-04 {\cellcolor{lowbids}}                                    & 1.37E-03 & 0.07 {\cellcolor{highbids}}                                    & 0.17  \\
\textbf{Regional}   & 2.00E-04 {\cellcolor{lowbids}}                                    & 1.40E-03 & 0.09 {\cellcolor{highbids}}                                    & 0.21  \\
\textbf{Science}    & 0.01    {\cellcolor{highbids}}                                       & 0.04     & 0.03 {\cellcolor{lowbids}}                                    & 0.07  \\
\textbf{Shopping}   & 1.09E-03 {\cellcolor{lowbids}}                                    & 4.78E-03 & 0.07 {\cellcolor{highbids}}                                    & 0.16  \\
\textbf{Society}    & 0.01    {\cellcolor{highbids}}                                       & 0.04     & 0.11 {\cellcolor{highbids}}                                    & 0.21  \\
\textbf{Sports}     & 0.01    {\cellcolor{highbids}}                                       & 0.04     & 0.14 {\cellcolor{highbids}}                                    & 0.23  \\
                                  
\midrule

\textbf{Control}    & 3.84E-03 & 0.02     & 0.05 & 0.12 \\

\bottomrule             
\end{tabular}
\label{table:NAI-opt-in}
\end{table}

==> tables/bids-opt-in/cookiebot.tex <==

\begin{table}[htb!]
\centering

\caption{Ad bidding under GDPR and CCPA in Cookiebot after opt-in. Avg. column represents the mean of all bid value. Std. represents the standard deviation of all bid value. \textcolor{highbids}{Light red} and \textcolor{lowbids}{Light blue} indicate bid values that are higher and lower than Control's avg., respectively. \textcolor{higherbids}{Dark red} and \textcolor{lowerbids}{Dark blue} indicate bid values that are Control's avg. $\pm$ std., respectively.}





    \begin{tabular}{l?{0.3mm}ll?{0.3mm}ll} 
    \toprule

    & \multicolumn{2}{c?{0.3mm}}{\textbf{GDPR}} & \multicolumn{2}{c}{\textbf{CCPA}} \\ 
    


    \multicolumn{1}{c?{0.3mm}}{}  & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}} &  \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c}{\textbf{Std.}}  \\ 
    \toprule
\textbf{Adult}      & 0.33 {\cellcolor{highbids}}                                       & 0.21 & 0.34 {\cellcolor{highbids}}                                      & 0.21  \\
\textbf{Arts}       & 0.32 {\cellcolor{highbids}}                                      & 0.22 & 0.31 {\cellcolor{highbids}}                                      & 0.22  \\
\textbf{Business}   & 0.35 {\cellcolor{highbids}}                                      & 0.21 & 0.32 {\cellcolor{highbids}}                                      & 0.23  \\
\textbf{Computers}  & 0.36 {\cellcolor{highbids}}                                      & 0.24 & 0.30 & 0.22  \\
\textbf{Games}      & 0.38 {\cellcolor{highbids}}                                      & 0.22 & 0.28 {\cellcolor{lowbids}}                                        & 0.22  \\
\textbf{Health}     & 0.34 {\cellcolor{highbids}}                                      & 0.22 & 0.38 {\cellcolor{highbids}}                                      & 0.31  \\
\textbf{Home}       & 0.31 {\cellcolor{highbids}}                                      & 0.22 & 0.34 {\cellcolor{highbids}}                                      & 0.21  \\
\textbf{Kids}       & 0.34 {\cellcolor{highbids}}                                      & 0.21 & 0.29 {\cellcolor{lowbids}}                                       & 0.21  \\
\textbf{News}       & 0.39 {\cellcolor{highbids}}                                      & 0.26 & 0.33 {\cellcolor{highbids}}                                      & 0.23  \\
\textbf{Recreation} & 0.35 {\cellcolor{highbids}}                                      & 0.21 & 0.31 {\cellcolor{highbids}}                                      & 0.22  \\
\textbf{Reference}  & 0.33 {\cellcolor{highbids}}                                      & 0.22 & 0.32 {\cellcolor{highbids}}                                      & 0.23  \\
\textbf{Regional}   & 0.34 {\cellcolor{highbids}}                                      & 0.22 & 0.30 & 0.23  \\
\textbf{Science}    & 0.39 {\cellcolor{highbids}}                                      & 0.23 & 0.32 {\cellcolor{highbids}}                                      & 0.22  \\
\textbf{Shopping}   & 0.35 {\cellcolor{highbids}}                                      & 0.22 & 0.32 {\cellcolor{highbids}}                                      & 0.22  \\
\textbf{Society}    & 0.37 {\cellcolor{highbids}}                                      & 0.22 & 0.33 {\cellcolor{highbids}}                                      & 0.21  \\
\textbf{Sports}     & 0.35 {\cellcolor{highbids}}                                      & 0.22 & 0.31 {\cellcolor{highbids}}                                      & 0.22  \\    
                                  
\midrule

\textbf{Control}    & 0.26 & 0.24 & 0.30 & 0.23\\
\bottomrule             
\end{tabular}
\vspace{-1em}
\label{table:cookiebot-opt-in}
\end{table}

==> tables/bids-opt-in/didomi.tex <==

\begin{table}[htb!]
\centering

\caption{Ad bidding under GDPR and CCPA in Didomi after opt-in. Avg. column represents the mean of all bid value. Std. represents the standard deviation of all bid value. \textcolor{highbids}{Light red} and \textcolor{lowbids}{Light blue} indicate bid values that are higher and lower than Control's avg., respectively. \textcolor{higherbids}{Dark red} and \textcolor{lowerbids}{Dark blue} indicate bid values that are Control's avg. $\pm$ std., respectively.}





    \begin{tabular}{l?{0.3mm}ll?{0.3mm}ll} 
    \toprule

    & \multicolumn{2}{c?{0.3mm}}{\textbf{GDPR}} & \multicolumn{2}{c}{\textbf{CCPA}} \\ 
    


    \multicolumn{1}{c?{0.3mm}}{}  & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}} &  \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c}{\textbf{Std.}}  \\ 
    \toprule
\textbf{Adult}      & 0.11 & 0.17 & 0.17 & 0.35  \\
\textbf{Arts}       & 0.16 {\cellcolor{highbids}}                                      & 0.29 & 0.18 {\cellcolor{highbids}}                                      & 0.51  \\
\textbf{Business}   & 0.11 & 0.17 & 0.19 {\cellcolor{highbids}}                                      & 0.42  \\
\textbf{Computers}  & 0.11 & 0.16 & 0.15 {\cellcolor{lowbids}}                                     & 0.34  \\
\textbf{Games}      & 0.12 {\cellcolor{highbids}}                                      & 0.21 & 0.16 {\cellcolor{lowbids}}                                     & 0.34  \\
\textbf{Health}     & 0.11 & 0.19 & 0.20 {\cellcolor{highbids}}                                      & 0.40  \\
\textbf{Home}       & 0.12 {\cellcolor{highbids}}                                      & 0.27 & 0.16 {\cellcolor{lowbids}}                                     & 0.34  \\
\textbf{Kids}       & 0.14 {\cellcolor{highbids}}                                      & 0.19 & 0.18 {\cellcolor{highbids}}                                      & 0.59  \\
\textbf{News}       & 0.09 {\cellcolor{lowbids}}                                      & 0.17 & 0.17 & 0.36  \\
\textbf{Recreation} & 0.11 & 0.21 & 0.27 {\cellcolor{highbids}}                                      & 0.91  \\
\textbf{Reference}  & 0.13 {\cellcolor{highbids}}                                      & 0.26 & 0.16 {\cellcolor{lowbids}}                                     & 0.31  \\
\textbf{Regional}   & 0.13 {\cellcolor{highbids}}                                      & 0.19 & 0.14 {\cellcolor{lowbids}}                                     & 0.38  \\
\textbf{Science}    & 0.12 {\cellcolor{highbids}}                                      & 0.24 & 0.23 {\cellcolor{highbids}}                                      & 0.63  \\
\textbf{Shopping}   & 0.10 {\cellcolor{lowbids}}                                      & 0.21 & 0.18 {\cellcolor{highbids}}                                      & 0.41  \\
\textbf{Society}    & 0.12 {\cellcolor{highbids}}                                      & 0.23 & 0.17 & 0.34  \\
\textbf{Sports}     & 0.13 {\cellcolor{highbids}}                                      & 0.23 & 0.18 {\cellcolor{highbids}}                                      & 0.39  \\    
                                  
\midrule

\textbf{Control}    & 0.11 & 0.31 & 0.17 & 0.36\\
\bottomrule             
\end{tabular}
\vspace{-1em}
\label{table:didomi-opt-in}
\end{table}

==> tables/bids-opt-in/onetrust.tex <==

\begin{table}[htb!]
\centering

\caption{Ad bidding under GDPR and CCPA in Onetrust after opt-in. Avg. column represents the mean of all bid value. Std. represents the standard deviation of all bid value. \textcolor{highbids}{Light red} and \textcolor{lowbids}{Light blue} indicate bid values that are higher and lower than Control's avg., respectively. \textcolor{higherbids}{Dark red} and \textcolor{lowerbids}{Dark blue} indicate bid values that are Control's avg. $\pm$ std., respectively.}





    \begin{tabular}{l?{0.3mm}ll?{0.3mm}ll} 
    \toprule

    & \multicolumn{2}{c?{0.3mm}}{\textbf{GDPR}} & \multicolumn{2}{c}{\textbf{CCPA}} \\ 
    


    \multicolumn{1}{c?{0.3mm}}{}  & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}} &  \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c}{\textbf{Std.}}  \\ 
    \toprule
\textbf{Adult}      & 0.01 {\cellcolor{lowerbids}}                                    & 0.00 & 0.46 {\cellcolor{lowbids}}                                  & 0.64  \\
\textbf{Arts}       & 0.04 {\cellcolor{higherbids}}                                   & 0.04 & 1.14  {\cellcolor{highbids}}   & 1.39  \\
\textbf{Business}   & 0.06 {\cellcolor{higherbids}}                                   & 0.06 & 0.19  {\cellcolor{lowbids}}   & 0.22  \\
\textbf{Computers}  & 0.01 {\cellcolor{lowerbids}}                                   & 4E-3 & 1.40  {\cellcolor{highbids}} & 1.42  \\
\textbf{Games}      & 0.03 {\cellcolor{higherbids}}                                  & 0.02 & 0.81  {\cellcolor{highbids}} & 1.24  \\
\textbf{Health}     & 0.15 {\cellcolor{higherbids}}                                  & 0.08 & 0.70  {\cellcolor{highbids}} & 1.07  \\
\textbf{Home}       & 0.05 {\cellcolor{higherbids}}                                  & 0.04 & 1.61  {\cellcolor{highbids}} & 1.50  \\
\textbf{Kids}       & 0.02 & 0.00 & 0.66  {\cellcolor{lowbids}}   & 1.03  \\
\textbf{News}       & 0.46 {\cellcolor{higherbids}}                                  & 0.30 & 0.75  {\cellcolor{highbids}} & 1.03  \\
\textbf{Recreation} & 0.14 {\cellcolor{higherbids}}                                  & 0.03 & 0.46  {\cellcolor{lowbids}}   & 0.76  \\
\textbf{Reference}  & 0.20 {\cellcolor{higherbids}}                                  & 0.26 & 0.72  {\cellcolor{highbids}} & 1.10  \\
\textbf{Regional}   & 0.02  & 4E-3 & 0.35  {\cellcolor{lowbids}}   & 0.59  \\
\textbf{Science}    & 0.09 {\cellcolor{higherbids}}                                  & 0.05 & 0.68  {\cellcolor{lowbids}}   & 1.05  \\
\textbf{Shopping}   & 0.13 {\cellcolor{higherbids}}                                  & 0.00 & 0.77  {\cellcolor{highbids}} & 1.06  \\
\textbf{Society}    & 0.02 & 3E-3 & 0.20  {\cellcolor{lowbids}}   & 0.22  \\
\textbf{Sports}     & 0.11 {\cellcolor{higherbids}}                                  & 0.09 & 0.77  {\cellcolor{highbids}} & 1.12  \\    
                                  
\midrule

\textbf{Control}    & 0.02 & 4E-3 & 0.69 & 1.11\\
\bottomrule             
\end{tabular}
\vspace{-1em}
\label{table:onetrust-opt-in}
\end{table}

==> tables/bids-opt-in/quantcast.tex <==

\begin{table}[htb!]
\centering

\caption{Ad bidding under GDPR and CCPA in Quantcast after opt-in. Avg. column represents the mean of all bid value. Std. represents the standard deviation of all bid value. \textcolor{highbids}{Light red} and \textcolor{lowbids}{Light blue} indicate bid values that are higher and lower than Control's avg., respectively. \textcolor{higherbids}{Dark red} and \textcolor{lowerbids}{Dark blue} indicate bid values that are Control's avg. $\pm$ std., respectively.}





    \begin{tabular}{l?{0.3mm}ll?{0.3mm}ll} 
    \toprule

    & \multicolumn{2}{c?{0.3mm}}{\textbf{GDPR}} & \multicolumn{2}{c}{\textbf{CCPA}} \\ 
    


    \multicolumn{1}{c?{0.3mm}}{}  & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}} &  \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c}{\textbf{Std.}}  \\ 
    \toprule
\textbf{Adult}      & 0.15 & 0.15 & 0.16 {\cellcolor{lowbids}}& 0.18  \\
\textbf{Arts}       & 0.14  {\cellcolor{lowbids}} & 0.14 & 0.18 & 0.13  \\
\textbf{Business}   & 0.15 & 0.12 & 0.21 {\cellcolor{highbids}}& 0.46  \\
\textbf{Computers}  & 0.16  {\cellcolor{highbids}} & 0.17 & 0.33 {\cellcolor{higherbids}}& 2.35  \\
\textbf{Games}      & 0.14 {\cellcolor{lowbids}}& 0.14 & 0.23 {\cellcolor{highbids}} & 0.73  \\
\textbf{Health}     & 0.15 & 0.14 & 0.38 {\cellcolor{higherbids}}& 0.81  \\
\textbf{Home}       & 0.14 {\cellcolor{lowbids}}& 0.14 & 0.28 {\cellcolor{highbids}}& 0.89  \\
\textbf{Kids}       & 0.14 {\cellcolor{lowbids}}& 0.12 & 0.19 {\cellcolor{highbids}} & 0.21  \\
\textbf{News}       & 0.14 {\cellcolor{lowbids}}& 0.15 & 0.18 & 0.19  \\
\textbf{Recreation} & 0.15 & 0.13 & 0.21 {\cellcolor{highbids}}& 0.41  \\
\textbf{Reference}  & 0.14 {\cellcolor{lowbids}}& 0.16 & 0.17 {\cellcolor{lowbids}}& 0.22  \\
\textbf{Regional}   & 0.16  {\cellcolor{highbids}} & 0.18 & 0.19 {\cellcolor{highbids}}& 0.32  \\
\textbf{Science}    & 0.15 & 0.19 & 0.15 {\cellcolor{lowbids}}& 0.14  \\
\textbf{Shopping}   & 0.12 {\cellcolor{lowbids}}& 0.14 & 0.21 {\cellcolor{highbids}}& 0.69  \\
\textbf{Society}    & 0.16  {\cellcolor{highbids}} & 0.18 & 0.16 {\cellcolor{lowbids}}& 0.19  \\
\textbf{Sports}     & 0.16  {\cellcolor{highbids}} & 0.20 & 0.18 & 0.21  \\    
                                  
\midrule

\textbf{Control}    & 0.15 & 0.11 & 0.18 & 0.14 \\
\bottomrule             
\end{tabular}
\label{table:quantcast-opt-in}
\end{table}

==> tables/bids-opt-out/NAI.tex <==

\begin{table}[htb!]
\centering

\caption{Ad bidding under GDPR and CCPA in NAI after opt-out. Avg. column represents the mean of all bid value. Std. represents the standard deviation of all bid value. \textcolor{highbids}{Light red} and \textcolor{lowbids}{Light blue} indicate bid values that are higher and lower than Control's avg., respectively. \textcolor{higherbids}{Dark red} and \textcolor{lowerbids}{Dark blue} indicate bid values that are Control's avg. $\pm$ std., respectively.}





    \begin{tabular}{l?{0.3mm}ll?{0.3mm}ll} 
    \toprule

    & \multicolumn{2}{c?{0.3mm}}{\textbf{GDPR}} & \multicolumn{2}{c}{\textbf{CCPA}} \\ 
    


    \multicolumn{1}{c?{0.3mm}}{}  & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}} &  \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c}{\textbf{Std.}}  \\ 
    \toprule
\textbf{Adult}      & 1.42E-03  {\cellcolor{higherbids}}& 0.01     & 0.10  {\cellcolor{highbids}}& 0.26  \\
\textbf{Arts}       & 1.28E-03  {\cellcolor{higherbids}}& 4.97E-03 & 0.06 {\cellcolor{lowbids}}& 0.14  \\
\textbf{Business}   & 1.94E-03  {\cellcolor{higherbids}}& 0.01     & 0.02 {\cellcolor{lowbids}}& 0.06  \\
\textbf{Computers}  & 4.09E-03  {\cellcolor{higherbids}}& 0.03     & 0.03 {\cellcolor{lowbids}}& 0.14  \\
\textbf{Games}      & 4.44E-04  {\cellcolor{higherbids}}& 2.95E-03 & 0.09 {\cellcolor{highbids}}& 0.18  \\
\textbf{Health}     & 1.00E-03  {\cellcolor{higherbids}}& 4.36E-03 & 0.16 {\cellcolor{highbids}}& 0.33  \\
\textbf{Home}       & 0.00     & 0.00     & 0.03 {\cellcolor{lowbids}}& 0.10  \\
\textbf{Kids}       & 7.32E-04  {\cellcolor{higherbids}}& 3.41E-03 & 0.07 & 0.12  \\
\textbf{News}       & 4.08E-04  {\cellcolor{higherbids}}& 2.83E-03 & 0.03 {\cellcolor{lowbids}}& 0.09  \\
\textbf{Recreation} & 9.99E-04  {\cellcolor{higherbids}}& 0.01     & 0.02 {\cellcolor{lowbids}}& 0.05  \\
\textbf{Reference}  & 2.28E-03  {\cellcolor{higherbids}}& 0.01     & 0.02 {\cellcolor{lowbids}}& 0.04  \\
\textbf{Regional}   & 1.75E-03  {\cellcolor{higherbids}}& 0.01     & 0.22 {\cellcolor{higherbids}}& 0.57  \\
\textbf{Science}    & 5.00E-04  {\cellcolor{higherbids}}& 3.12E-03 & 0.02 {\cellcolor{lowbids}}& 0.07  \\
\textbf{Shopping}   & 2.47E-03  {\cellcolor{higherbids}}& 0.01     & 0.07 & 0.16  \\
\textbf{Society}    & 0.00     & 0.00     & 0.05 {\cellcolor{lowbids}}& 0.12  \\
\textbf{Sports}     & 0.01      {\cellcolor{higherbids}}& 0.04     & 0.09 {\cellcolor{highbids}}& 0.17  \\  
                                  
\midrule

\textbf{Control}    & 0.00 & 0.00 & 0.07 & 0.15\\
\bottomrule             
\end{tabular}
\label{table:NAI-opt-out}
\end{table}

==> tables/bids-opt-out/cookiebot.tex <==

\begin{table}[htb!]
    \centering
\caption{Ad bidding under GDPR and CCPA in Cookiebot after opt-out. Avg. column represents the mean of all bid value. Std. represents the standard deviation of all bid value. \textcolor{highbids}{Light red} and \textcolor{lowbids}{Light blue} indicate bid values that are higher and lower than Control's avg., respectively. \textcolor{higherbids}{Dark red} and \textcolor{lowerbids}{Dark blue} indicate bid values that are Control's avg. $\pm$ std., respectively.}

\adjustbox{max width=\columnwidth}{



    \begin{tabular}{l?{0.3mm}ll?{0.3mm}llllll} 
    \toprule

    & \multicolumn{2}{c?{0.3mm}}{\textbf{GDPR}} & \multicolumn{2}{c}{\textbf{CCPA}} && && \\ 
    


    \multicolumn{1}{c?{0.3mm}}{}  & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}} &  \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c}{\textbf{Std.}} && &&  \\ 
    \toprule
\textbf{Adult}      & 0.37 {\cellcolor{highbids}}& 0.20 & 0.37 {\cellcolor{highbids}}& 0.20  & - {\cellcolor{highbids}}& - & - {\cellcolor{highbids}}& - \\
\textbf{Arts}       & 0.35 {\cellcolor{highbids}}& 0.21 & 0.38 {\cellcolor{highbids}}& 0.21  \\
\textbf{Business}   & 0.35 {\cellcolor{highbids}}& 0.21 & 0.36 {\cellcolor{highbids}}& 0.22  \\
\textbf{Computers}  & 0.35 {\cellcolor{highbids}}& 0.21 & 0.37 {\cellcolor{highbids}}& 0.20  \\
\textbf{Games}      & 0.38 {\cellcolor{highbids}}& 0.20 & 0.36 {\cellcolor{highbids}}& 0.20  \\
\textbf{Health}     & 0.35 {\cellcolor{highbids}}& 0.21 & 0.38 {\cellcolor{highbids}}& 0.21  \\
\textbf{Home}       & 0.38 {\cellcolor{highbids}}& 0.20 & 0.36 {\cellcolor{highbids}}& 0.21  \\
\textbf{Kids}       & 0.37 {\cellcolor{highbids}}& 0.20 & 0.35 {\cellcolor{highbids}}& 0.21  \\
\textbf{News}       & 0.35 {\cellcolor{highbids}}& 0.21 & 0.37 {\cellcolor{highbids}}& 0.20  \\
\textbf{Recreation} & 0.37 {\cellcolor{highbids}}& 0.20 & 0.36 {\cellcolor{highbids}}& 0.20  \\
\textbf{Reference}  & 0.37 {\cellcolor{highbids}}& 0.20 & 0.37 {\cellcolor{highbids}}& 0.20  \\
\textbf{Regional}   & 0.38 {\cellcolor{highbids}}& 0.19 & 0.35 {\cellcolor{highbids}}& 0.21  \\
\textbf{Science}    & 0.35 {\cellcolor{highbids}}& 0.21 & 0.36 {\cellcolor{highbids}}& 0.20  \\
\textbf{Shopping}   & 0.37 {\cellcolor{highbids}}& 0.20 & 0.32 & 0.23  \\
\textbf{Society}    & 0.37 {\cellcolor{highbids}}& 0.20 & 0.37 {\cellcolor{highbids}}& 0.20  \\
\textbf{Sports}     & 0.37 {\cellcolor{highbids}}& 0.20 & 0.33 {\cellcolor{highbids}}& 0.23  \\    
                                  
\midrule
\textbf{Control}    & 0.33 & 0.22 & 0.32 & 0.22 \\

\bottomrule             
\end{tabular}
    }
    \vspace{-1em}
\label{table:cookiebot-opt-out}
    
\end{table}

==> tables/bids-opt-out/didomi.tex <==

\begin{table}[htb!]
\centering

\caption{Ad bidding under GDPR and CCPA in Didomi after opt-out. Avg. column represents the mean of all bid value. Std. represents the standard deviation of all bid value. \textcolor{highbids}{Light red} and \textcolor{lowbids}{Light blue} indicate bid values that are higher and lower than Control's avg., respectively. \textcolor{higherbids}{Dark red} and \textcolor{lowerbids}{Dark blue} indicate bid values that are Control's avg. $\pm$ std., respectively.}





    \begin{tabular}{l?{0.3mm}ll?{0.3mm}ll} 
    \toprule

    & \multicolumn{2}{c?{0.3mm}}{\textbf{GDPR}} & \multicolumn{2}{c}{\textbf{CCPA}} \\ 
    


    \multicolumn{1}{c?{0.3mm}}{}  & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}} &  \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c}{\textbf{Std.}}  \\ 
    \toprule
    
\textbf{Adult}      & --   & --   & 0.17 {\cellcolor{lowbids}}& 0.28  \\
\textbf{Arts}       & 0.05 & 0.00 & 0.39  {\cellcolor{higherbids}}& 1.20  \\
\textbf{Business}   & --   & --   & 0.16 {\cellcolor{lowbids}}& 0.12  \\
\textbf{Computers}  & 0.05 & 4E-3 & 0.45  {\cellcolor{higherbids}}& 1.08  \\
\textbf{Games}      & 0.03 {\cellcolor{lowerbids}}& 0.02 & 0.15 {\cellcolor{lowbids}}& 0.13  \\
\textbf{Health}     & --   & --   & 0.22  {\cellcolor{highbids}}& 0.38  \\
\textbf{Home}       & 0.05 & 0.00 & 0.23  {\cellcolor{highbids}}& 0.42  \\
\textbf{Kids}       & 0.06  {\cellcolor{higherbids}}& 0.00 & 0.18 & 0.51  \\
\textbf{News}       & --   & --   & 0.17 {\cellcolor{lowbids}}& 0.25  \\
\textbf{Recreation} & 0.06 {\cellcolor{higherbids}} & 0.00 & 0.16 {\cellcolor{lowbids}}& 0.15  \\
\textbf{Reference}  & --   & --   & 0.17 {\cellcolor{lowbids}}& 0.22  \\
\textbf{Regional}   & --   & --   & 0.23 {\cellcolor{highbids}}& 0.54  \\
\textbf{Science}    & 0.41 {\cellcolor{higherbids}} & 0.00 & 0.18 & 0.16  \\
\textbf{Shopping}   & 0.03  {\cellcolor{lowerbids}}& 0.00 & 0.20 {\cellcolor{highbids}}& 0.34  \\
\textbf{Society}    & 0.05 & 0.00 & 0.24 {\cellcolor{highbids}}& 1.05  \\
\textbf{Sports}     & 0.05 & 0.00 & 0.17 {\cellcolor{lowbids}}& 0.29  \\                                  
\midrule
\textbf{Control}    & 0.05 & 3E-3 & 0.18 & 0.16\\

\bottomrule             
\end{tabular}
\vspace{-1em}
\label{table:didomi-opt-out}
\end{table}

==> tables/bids-opt-out/onetrust.tex <==

\begin{table}[htb!]
\centering

\caption{Ad bidding under GDPR and CCPA in Onetrust after opt-out. Avg. column represents the mean of all bid value. Std. represents the standard deviation of all bid value. \textcolor{highbids}{Light red} and \textcolor{lowbids}{Light blue} indicate bid values that are higher and lower than Control's avg., respectively. \textcolor{higherbids}{Dark red} and \textcolor{lowerbids}{Dark blue} indicate bid values that are Control's avg. $\pm$ std., respectively.}





    \begin{tabular}{l?{0.3mm}ll?{0.3mm}ll} 
    \toprule

    & \multicolumn{2}{c?{0.3mm}}{\textbf{GDPR}} & \multicolumn{2}{c}{\textbf{CCPA}} \\ 
    


    \multicolumn{1}{c?{0.3mm}}{}  & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}} &  \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c}{\textbf{Std.}}  \\ 
    \toprule
\textbf{Adult}      & 0.02 & 0.00 & 1.09 {\cellcolor{highbids}}& 0.98  \\
\textbf{Arts}       & --   & --   & 1.06 {\cellcolor{highbids}}& 1.14  \\
\textbf{Business}   & 0.01 {\cellcolor{lowerbids}}& 0.01 & 0.61 {\cellcolor{lowbids}}& 0.73  \\
\textbf{Computers}  & 0.02 & 0.01 & 1.02 {\cellcolor{highbids}}& 1.11  \\
\textbf{Games}      & 0.02 & 0.00 & 0.99 {\cellcolor{highbids}}& 0.95  \\
\textbf{Health}     & 0.03 {\cellcolor{higherbids}}& 0.02 & 0.98 {\cellcolor{highbids}}& 0.85  \\
\textbf{Home}       & 0.31 {\cellcolor{higherbids}}& 0.25 & 1.03 {\cellcolor{highbids}}& 1.01  \\
\textbf{Kids}       & 0.01 {\cellcolor{lowerbids}}& 0.00 & 0.91 {\cellcolor{highbids}}& 1.07  \\
\textbf{News}       & 0.03 {\cellcolor{higherbids}}& 0.02 & 0.95 {\cellcolor{highbids}}& 0.97  \\
\textbf{Recreation} & 0.02 & 0.01 & 1.03 {\cellcolor{highbids}}& 0.89  \\
\textbf{Reference}  & 0.03 {\cellcolor{higherbids}}& 0.01 & 1.10 {\cellcolor{highbids}}& 1.09  \\
\textbf{Regional}   & 0.01 {\cellcolor{lowerbids}}& 0.00 & 0.91 {\cellcolor{highbids}}& 0.69  \\
\textbf{Science}    & 0.03 {\cellcolor{higherbids}}& 0.02 & 1.05 {\cellcolor{highbids}}& 1.23  \\
\textbf{Shopping}   & 1.10 {\cellcolor{higherbids}}& 0.00 & 1.00 {\cellcolor{highbids}}& 1.21  \\
\textbf{Society}    & 0.01 {\cellcolor{lowerbids}}& 0.00 & 0.85 {\cellcolor{lowbids}}& 1.06  \\
\textbf{Sports}     & 0.01 {\cellcolor{lowerbids}}& 0.00 & 0.94 {\cellcolor{highbids}}& 1.01  \\    
                                  
\midrule

\textbf{Control}    & 0.02 & 0.00 & 0.88 & 1.18\\
\bottomrule             
\end{tabular}
\label{table:onetrust-opt-out}
\end{table}

==> tables/bids-opt-out/quantcast.tex <==

\begin{table}[htb!]
\centering

\caption{Ad bidding under GDPR and CCPA in Quantcast after opt-out. Avg. column represents the mean of all bid value. Std. represents the standard deviation of all bid value. \textcolor{highbids}{Light red} and \textcolor{lowbids}{Light blue} indicate bid values that are higher and lower than Control's avg., respectively. \textcolor{higherbids}{Dark red} and \textcolor{lowerbids}{Dark blue} indicate bid values that are Control's avg. $\pm$ std., respectively.}





    \begin{tabular}{l?{0.3mm}ll?{0.3mm}ll} 
    \toprule

    & \multicolumn{2}{c?{0.3mm}}{\textbf{GDPR}} & \multicolumn{2}{c}{\textbf{CCPA}} \\ 
    


    \multicolumn{1}{c?{0.3mm}}{}  & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Std.}} &  \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c}{\textbf{Std.}}  \\ 
    \toprule
\textbf{Adult}      & 0.22 {\cellcolor{highbids}}& 0.82 & 0.25 {\cellcolor{highbids}}& 0.58  \\
\textbf{Arts}       & 0.22 {\cellcolor{highbids}}& 1.03 & 0.30 {\cellcolor{highbids}}& 1.31  \\
\textbf{Business}   & 0.19 {\cellcolor{highbids}}& 0.82 & 0.20 {\cellcolor{highbids}}& 0.40  \\
\textbf{Computers}  & 0.28 {\cellcolor{higherbids}}& 0.97 & 0.31 {\cellcolor{highbids}}& 1.24  \\
\textbf{Games}      & 0.43 {\cellcolor{higherbids}}& 1.36 & 0.23 {\cellcolor{highbids}}& 0.62  \\
\textbf{Health}     & 0.41 {\cellcolor{higherbids}}& 1.31 & 0.51 {\cellcolor{higherbids}}& 1.17  \\
\textbf{Home}       & 0.23 {\cellcolor{highbids}}& 0.93 & 0.21 {\cellcolor{highbids}}& 0.52  \\
\textbf{Kids}       & 0.30 {\cellcolor{higherbids}}& 0.96 & 0.23 {\cellcolor{highbids}}& 0.53  \\
\textbf{News}       & 0.22 {\cellcolor{highbids}}& 0.79 & 0.20 {\cellcolor{highbids}}& 0.50  \\
\textbf{Recreation} & 0.31 {\cellcolor{higherbids}}& 1.38 & 0.27 {\cellcolor{highbids}}& 0.66  \\
\textbf{Reference}  & 0.26 {\cellcolor{higherbids}}& 1.20 & 0.22 {\cellcolor{highbids}}& 0.54  \\
\textbf{Regional}   & 0.27 {\cellcolor{higherbids}}& 1.23 & 0.24 {\cellcolor{highbids}}& 0.74  \\
\textbf{Science}    & 0.36 {\cellcolor{higherbids}}& 1.17 & 0.23 {\cellcolor{highbids}}& 0.55  \\
\textbf{Shopping}   & 0.18 {\cellcolor{highbids}}& 0.74 & 0.22 {\cellcolor{highbids}}& 0.58  \\
\textbf{Society}    & 0.30 {\cellcolor{higherbids}}& 1.00 & 0.18 {\cellcolor{highbids}}& 0.24  \\
\textbf{Sports}     & 0.21 {\cellcolor{highbids}}& 0.82 & 0.23 {\cellcolor{highbids}}& 0.57  \\    
                                  
\midrule

\textbf{Control}    & 0.16 & 0.08 & 0.17 & 0.18\\

\bottomrule             
\end{tabular}
\label{table:quantcast-opt-out}
\end{table}

==> tables/cookie-syncing-opt-in/NAI.tex <==

\begin{table}[htb!]
\centering

\caption{Cookie syncing events by advertisers under GDPR and CCPA in NAI after opt-in. Evt. column represents the number of cookie syncing events. Pct. represents the percentage of advertisers that participate in cookie syncing.}





    \begin{tabular}{l?{0.3mm}ll?{0.3mm}ll} 
    \toprule

    & \multicolumn{2}{c?{0.3mm}}{\textbf{GDPR}} & \multicolumn{2}{c}{\textbf{CCPA}} \\ 
    


    \multicolumn{1}{c?{0.3mm}}{}  & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Pct.}} &  \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c}{\textbf{Pct.}}  \\  
    \toprule
\textbf{Adult}      & 0  & 0.00\%  & 23 & 60.00\%  \\
\textbf{Arts}       & 0  & 0.00\%  & 86 & 62.50\%  \\
\textbf{Business}   & 21 & 40.00\% & 27 & 60.00\%  \\
\textbf{Computers}  & 19 & 66.67\% & 33 & 66.67\%  \\
\textbf{Games}      & 0  & 0.00\%  & 20 & 75.00\%  \\
\textbf{Health}     & 5  & 33.33\% & 71 & 83.33\%  \\
\textbf{Home}       & 0  & 0.00\%  & 31 & 80.00\%  \\
\textbf{Kids}       & 14 & 66.67\% & 67 & 83.33\%  \\
\textbf{News}       & 2  & 25.00\% & 18 & 75.00\%  \\
\textbf{Recreation} & 6  & 25.00\% & 49 & 83.33\%  \\
\textbf{Reference}  & 13 & 33.33\% & 27 & 83.33\%  \\
\textbf{Regional}   & 14 & 66.67\% & 49 & 80.00\%  \\
\textbf{Science}    & 0  & 0.00\%  & 22 & 75.00\%  \\
\textbf{Shopping}   & 18 & 33.33\% & 74 & 71.43\%  \\
\textbf{Society}    & 0  & 0.00\%  & 93 & 83.33\%  \\
\textbf{Sports}     & 0  & 0.00\%  & 78 & 80.00\%  \\    
                                  
\midrule

\textbf{Average}    & 7  & 24.38\% & 48 & 75.14\% \\
\bottomrule             
\end{tabular}
\label{table:NAI-opt-in-syncing}
\end{table}

==> tables/cookie-syncing-opt-in/cookiebot.tex <==

\begin{table}[htb!]
\centering

\caption{Cookie syncing events by advertisers under GDPR and CCPA in Cookiebot after opt-in. Evt. column represents the number of cookie syncing events. Pct. represents the percentage of advertisers that participate in cookie syncing.}





    \begin{tabular}{l?{0.3mm}ll?{0.3mm}ll} 
    \toprule

    & \multicolumn{2}{c?{0.3mm}}{\textbf{GDPR}} & \multicolumn{2}{c}{\textbf{CCPA}} \\ 
    


    \multicolumn{1}{c?{0.3mm}}{}  & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Pct.}} &  \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c}{\textbf{Pct.}}  \\ 
    \toprule

\textbf{Adult}      & 25 & 25.00\% & 11 & 20.00\%  \\
\textbf{Arts}       & 7  & 25.00\% & 3  & 20.00\%  \\
\textbf{Business}   & 44 & 40.00\% & 3  & 20.00\%  \\
\textbf{Computers}  & 28 & 20.00\% & 4  & 20.00\%  \\
\textbf{Games}      & 27 & 25.00\% & 4  & 14.29\%  \\
\textbf{Health}     & 36 & 40.00\% & 25 & 40.00\%  \\
\textbf{Home}       & 3  & 20.00\% & 14 & 33.33\%  \\
\textbf{Kids}       & 41 & 33.33\% & 26 & 40.00\%  \\
\textbf{News}       & 22 & 25.00\% & 3  & 20.00\%  \\
\textbf{Recreation} & 6  & 25.00\% & 13 & 20.00\%  \\
\textbf{Reference}  & 24 & 25.00\% & 5  & 20.00\%  \\
\textbf{Regional}   & 52 & 50.00\% & 16 & 28.57\%  \\
\textbf{Science}    & 26 & 25.00\% & 18 & 16.67\%  \\
\textbf{Shopping}   & 50 & 42.86\% & 12 & 20.00\%  \\
\textbf{Society}    & 5  & 20.00\% & 5  & 25.00\%  \\
\textbf{Sports}     & 43 & 40.00\% & 7  & 20.00\%  \\    
                                  
\midrule

\textbf{Average}    & 27 & 30.07\% & 11 & 23.62\% \\

\bottomrule             
\end{tabular}
\label{table:cookiebot-opt-in-syncing}
\end{table}

==> tables/cookie-syncing-opt-in/didomi.tex <==

\begin{table}[htb!]
\centering

\caption{Cookie syncing events by advertisers under GDPR and CCPA in Cookiebot after opt-in. Evt. column represents the number of cookie syncing events. Pct. represents the percentage of advertisers that participate in cookie syncing.}





    \begin{tabular}{l?{0.3mm}ll?{0.3mm}ll} 
    \toprule

    & \multicolumn{2}{c?{0.3mm}}{\textbf{GDPR}} & \multicolumn{2}{c}{\textbf{CCPA}} \\ 
    


    \multicolumn{1}{c?{0.3mm}}{}  & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Pct.}} &  \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c}{\textbf{Pct.}}  \\ 
    \toprule
    
\textbf{Adult}      & 205 & 53.33\% & 136 & 50.00\%  \\
\textbf{Arts}       & 209 & 46.67\% & 163 & 57.14\%  \\
\textbf{Business}   & 232 & 53.33\% & 129 & 46.15\%  \\
\textbf{Computers}  & 276 & 64.71\% & 161 & 61.54\%  \\
\textbf{Games}      & 247 & 50.00\% & 178 & 46.67\%  \\
\textbf{Health}     & 223 & 47.06\% & 222 & 60.00\%  \\
\textbf{Home}       & 153 & 53.85\% & 155 & 46.15\%  \\
\textbf{Kids}       & 252 & 56.25\% & 169 & 53.33\%  \\
\textbf{News}       & 251 & 60.00\% & 162 & 60.00\%  \\
\textbf{Recreation} & 208 & 52.94\% & 232 & 58.82\%  \\
\textbf{Reference}  & 221 & 52.94\% & 143 & 50.00\%  \\
\textbf{Regional}   & 203 & 50.00\% & 144 & 61.54\%  \\
\textbf{Science}    & 246 & 56.25\% & 219 & 58.33\%  \\
\textbf{Shopping}   & 223 & 50.00\% & 185 & 50.00\%  \\
\textbf{Society}    & 204 & 50.00\% & 161 & 41.67\%  \\
\textbf{Sports}     & 218 & 56.25\% & 162 & 50.00\%  \\                                  
\midrule
\textbf{Average}    & 223 & 53.35\% & 170 & 53.21\% \\

\bottomrule             
\end{tabular}
\label{table:didomi-opt-in-syncing}
\end{table}

==> tables/cookie-syncing-opt-in/onetrust.tex <==

\begin{table}[htb!]
\centering

\caption{Cookie syncing events by advertisers under GDPR and CCPA in Onetrust after opt-in. Evt. column represents the number of cookie syncing events. Pct. represents the percentage of advertisers that participate in cookie syncing.}





    \begin{tabular}{l?{0.3mm}ll?{0.3mm}ll} 
    \toprule

    & \multicolumn{2}{c?{0.3mm}}{\textbf{GDPR}} & \multicolumn{2}{c}{\textbf{CCPA}} \\ 
    


    \multicolumn{1}{c?{0.3mm}}{}  & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Pct.}} &  \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c}{\textbf{Pct.}}  \\ 
    \toprule
    
\textbf{Adult}      & 20 & 100.00\% & 128 & 71.43\%  \\
\textbf{Arts}       & 22 & 100.00\% & 71  & 80.00\%  \\
\textbf{Business}   & 49 & 100.00\% & 77  & 80.00\%  \\
\textbf{Computers}  & 38 & 100.00\% & 84  & 85.71\%  \\
\textbf{Games}      & 22 & 100.00\% & 58  & 57.14\%  \\
\textbf{Health}     & 25 & 100.00\% & 120 & 71.43\%  \\
\textbf{Home}       & 8  & 100.00\% & 56  & 80.00\%  \\
\textbf{Kids}       & 27 & 100.00\% & 116 & 87.50\%  \\
\textbf{News}       & 27 & 100.00\% & 47  & 66.67\%  \\
\textbf{Recreation} & 13 & 50.00\%  & 77  & 75.00\%  \\
\textbf{Reference}  & 45 & 100.00\% & 89  & 71.43\%  \\
\textbf{Regional}   & 30 & 100.00\% & 53  & 60.00\%  \\
\textbf{Science}    & 13 & 100.00\% & 106 & 83.33\%  \\
\textbf{Shopping}   & 14 & 100.00\% & 76  & 80.00\%  \\
\textbf{Society}    & 21 & 100.00\% & 87  & 83.33\%  \\
\textbf{Sports}     & 54 & 83.33\%  & 57  & 57.14\%  \\                                  
\midrule
\textbf{Average}    & 27 & 95.83\%  & 81  & 74.38\% \\

\bottomrule             
\end{tabular}
\label{table:onetrust-opt-in-syncing}
\end{table}

==> tables/cookie-syncing-opt-in/quantcast.tex <==

\begin{table}[htb!]
\centering

\caption{Cookie syncing events by advertisers under GDPR and CCPA in Quantcast after opt-in. Evt. column represents the number of cookie syncing events. Pct. represents the percentage of advertisers that participate in cookie syncing.}





    \begin{tabular}{l?{0.3mm}ll?{0.3mm}ll} 
    \toprule

    & \multicolumn{2}{c?{0.3mm}}{\textbf{GDPR}} & \multicolumn{2}{c}{\textbf{CCPA}} \\ 
    


    \multicolumn{1}{c?{0.3mm}}{}  & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Pct.}} &  \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c}{\textbf{Pct.}}  \\ 
    \toprule
\textbf{Adult}      & 204 & 68.75\% & 161 & 55.56\%  \\
\textbf{Arts}       & 210 & 64.71\% & 149 & 50.00\%  \\
\textbf{Business}   & 154 & 69.23\% & 179 & 60.00\%  \\
\textbf{Computers}  & 192 & 58.82\% & 125 & 47.06\%  \\
\textbf{Games}      & 180 & 62.50\% & 184 & 57.89\%  \\
\textbf{Health}     & 141 & 57.14\% & 252 & 68.42\%  \\
\textbf{Home}       & 135 & 57.14\% & 210 & 70.59\%  \\
\textbf{Kids}       & 175 & 66.67\% & --  & --       \\
\textbf{News}       & 163 & 66.67\% & 179 & 68.75\%  \\
\textbf{Recreation} & 176 & 66.67\% & 160 & 60.00\%  \\
\textbf{Reference}  & 191 & 62.50\% & 142 & 52.94\%  \\
\textbf{Regional}   & 138 & 53.33\% & 215 & 70.59\%  \\
\textbf{Science}    & 191 & 64.71\% & 170 & 56.25\%  \\
\textbf{Shopping}   & 139 & 61.54\% & 158 & 55.56\%  \\
\textbf{Society}    & 126 & 69.23\% & 166 & 56.25\%  \\
\textbf{Sports}     & 189 & 64.71\% & 162 & 64.71\%  \\    
                                  
\midrule

\textbf{Average}    & 169 & 63.39\% & 174 & 59.64\% \\
\bottomrule             
\end{tabular}
\label{table:quantcast-opt-in-syncing}
\end{table}

==> tables/cookie-syncing-opt-out/NAI.tex <==

\begin{table}[htb!]
\centering

\caption{Cookie syncing events by advertisers under GDPR and CCPA in NAI after opt-out. Evt. column represents the number of cookie syncing events. Pct. represents the percentage of advertisers that participate in cookie syncing.}





    \begin{tabular}{l?{0.3mm}ll?{0.3mm}ll} 
    \toprule

    & \multicolumn{2}{c?{0.3mm}}{\textbf{GDPR}} & \multicolumn{2}{c}{\textbf{CCPA}} \\ 
    


    \multicolumn{1}{c?{0.3mm}}{}  & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Pct.}} &  \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c}{\textbf{Pct.}}  \\ 
    \toprule
    
\textbf{Arts}       & 13 & 50.00\% & 5  & 33.33\%  \\
\textbf{Business}   & 22 & 66.67\% & 18 & 66.67\%  \\
\textbf{Computers}  & 11 & 50.00\% & 20 & 66.67\%  \\
\textbf{Games}      & 15 & 50.00\% & 10 & 50.00\%  \\
\textbf{Health}     & 5  & 50.00\% & 57 & 83.33\%  \\
\textbf{Home}       & 0  & 0.00\%  & 18 & 66.67\%  \\
\textbf{Kids}       & 7  & 50.00\% & 38 & 75.00\%  \\
\textbf{News}       & 5  & 50.00\% & 16 & 66.67\%  \\
\textbf{Recreation} & 9  & 66.67\% & 19 & 50.00\%  \\
\textbf{Reference}  & 20 & 66.67\% & 25 & 50.00\%  \\
\textbf{Regional}   & 13 & 50.00\% & 22 & 50.00\%  \\
\textbf{Science}    & 5  & 50.00\% & 54 & 66.67\%  \\
\textbf{Shopping}   & 23 & 66.67\% & 27 & 50.00\%  \\
\textbf{Society}    & 0  & 0.00\%  & 17 & 66.67\%  \\
\textbf{Sports}     & 1  & 50.00\% & 46 & 80.00\%  \\                                  
\midrule

\textbf{Average}    & 10 & 47.92\% & 26 & 60.73\% \\
\bottomrule             
\end{tabular}
\label{table:NAI-opt-out-syncing}
\end{table}

==> tables/cookie-syncing-opt-out/cookiebot.tex <==

\begin{table}[htb!]
\centering

\caption{Cookie syncing events by advertisers under GDPR and CCPA in Cookiebot after opt-out. Evt. column represents the number of cookie syncing events. Pct. represents the percentage of advertisers that participate in cookie syncing.}





    \begin{tabular}{l?{0.3mm}ll?{0.3mm}ll} 
    \toprule

    & \multicolumn{2}{c?{0.3mm}}{\textbf{GDPR}} & \multicolumn{2}{c}{\textbf{CCPA}} \\ 
    


    \multicolumn{1}{c?{0.3mm}}{}  & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Pct.}} &  \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c}{\textbf{Pct.}}  \\ 
    \toprule
    
\textbf{Adult}      & 0 & 0.00\%  & 0  & 0.00\%   \\
\textbf{Arts}       & 0 & 0.00\%  & 4  & 25.00\%  \\
\textbf{Business}   & 0 & 0.00\%  & 3  & 33.33\%  \\
\textbf{Computers}  & 0 & 0.00\%  & 0  & 0.00\%   \\
\textbf{Games}      & 0 & 0.00\%  & 0  & 0.00\%   \\
\textbf{Health}     & 0 & 0.00\%  & 28 & 40.00\%  \\
\textbf{Home}       & 0 & 0.00\%  & 6  & 16.67\%  \\
\textbf{Kids}       & 0 & 0.00\%  & 5  & 20.00\%  \\
\textbf{News}       & 3 & 25.00\% & 3  & 25.00\%  \\
\textbf{Recreation} & 0 & 0.00\%  & 21 & 20.00\%  \\
\textbf{Reference}  & 0 & 0.00\%  & 14 & 20.00\%  \\
\textbf{Regional}   & 0 & 0.00\%  & 28 & 33.33\%  \\
\textbf{Science}    & 0 & 0.00\%  & 29 & 40.00\%  \\
\textbf{Shopping}   & 0 & 0.00\%  & 37 & 28.57\%  \\
\textbf{Society}    & 0 & 0.00\%  & 0  & 0.00\%   \\
\textbf{Sports}     & 0 & 0.00\%  & 5  & 20.00\%  \\    
                                  
\midrule

\textbf{Average}    & 1 & 1.56\%  & 11 & 20.12\% \\

\bottomrule             
\end{tabular}
\label{table:cookiebot-opt-out-syncing}
\end{table}

==> tables/cookie-syncing-opt-out/didomi.tex <==

\begin{table}[htb!]
\centering

\caption{Cookie syncing events by advertisers under GDPR and CCPA in Didomi after opt-out. Evt. column represents the number of cookie syncing events. Pct. represents the percentage of advertisers that participate in cookie syncing.}





    \begin{tabular}{l?{0.3mm}ll?{0.3mm}ll} 
    \toprule

    & \multicolumn{2}{c?{0.3mm}}{\textbf{GDPR}} & \multicolumn{2}{c}{\textbf{CCPA}} \\ 
    


    \multicolumn{1}{c?{0.3mm}}{}  & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Pct.}} &  \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c}{\textbf{Pct.}}  \\ 
    \toprule
\textbf{Adult}      & 0  & 0.00\%   & 36 & 75.00\%   \\
\textbf{Arts}       & 1  & 100.00\% & 43 & 71.43\%   \\
\textbf{Business}   & 0  & 0.00\%   & 21 & 75.00\%   \\
\textbf{Computers}  & 15 & 100.00\% & 38 & 100.00\%  \\
\textbf{Games}      & 17 & 100.00\% & 30 & 60.00\%   \\
\textbf{Health}     & 0  & 0.00\%   & 86 & 83.33\%   \\
\textbf{Home}       & 0  & 0.00\%   & 19 & 75.00\%   \\
\textbf{Kids}       & 2  & 100.00\% & 65 & 75.00\%   \\
\textbf{News}       & 0  & 0.00\%   & 31 & 83.33\%   \\
\textbf{Recreation} & 2  & 100.00\% & 47 & 57.14\%   \\
\textbf{Reference}  & 0  & 0.00\%   & 32 & 66.67\%   \\
\textbf{Regional}   & 0  & 0.00\%   & 36 & 57.14\%   \\
\textbf{Science}    & 0  & 0.00\%   & 52 & 75.00\%   \\
\textbf{Shopping}   & 0  & 0.00\%   & 69 & 66.67\%   \\
\textbf{Society}    & 0  & 0.00\%   & 31 & 80.00\%   \\
\textbf{Sports}     & 3  & 100.00\% & 37 & 80.00\%   \\    
                                  
\midrule

\textbf{Average}    & 3  & 37.50\%  & 42 & 73.79\%  \\
\bottomrule             
\end{tabular}
\label{table:didomi-opt-out-syncing}
\end{table}

==> tables/cookie-syncing-opt-out/onetrust.tex <==

\begin{table}[htb!]
\centering

\caption{Cookie syncing events by advertisers under GDPR and CCPA in Onetrust after opt-out. Evt. column represents the number of cookie syncing events. Pct. represents the percentage of advertisers that participate in cookie syncing.}





    \begin{tabular}{l?{0.3mm}ll?{0.3mm}ll} 
    \toprule

    & \multicolumn{2}{c?{0.3mm}}{\textbf{GDPR}} & \multicolumn{2}{c}{\textbf{CCPA}} \\ 
    


    \multicolumn{1}{c?{0.3mm}}{}  & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Pct.}} &  \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c}{\textbf{Pct.}}  \\ 
    \toprule
\textbf{Adult}      & 19 & 100.00\% & 85  & 50.00\%  \\
\textbf{Arts}       & 0  & 0.00\%   & 53  & 42.86\%  \\
\textbf{Business}   & 24 & 100.00\% & 125 & 87.50\%  \\
\textbf{Computers}  & 29 & 100.00\% & 86  & 62.50\%  \\
\textbf{Games}      & 16 & 100.00\% & 95  & 71.43\%  \\
\textbf{Health}     & 1  & 100.00\% & 115 & 60.00\%  \\
\textbf{Home}       & 15 & 100.00\% & 110 & 70.00\%  \\
\textbf{Kids}       & 12 & 50.00\%  & 124 & 62.50\%  \\
\textbf{News}       & 8  & 100.00\% & 98  & 62.50\%  \\
\textbf{Recreation} & 7  & 100.00\% & 86  & 71.43\%  \\
\textbf{Reference}  & 11 & 100.00\% & 67  & 55.56\%  \\
\textbf{Regional}   & 33 & 100.00\% & 85  & 66.67\%  \\
\textbf{Science}    & 1  & 100.00\% & 114 & 62.50\%  \\
\textbf{Shopping}   & 14 & 100.00\% & 136 & 60.00\%  \\
\textbf{Society}    & 10 & 100.00\% & 89  & 80.00\%  \\
\textbf{Sports}     & 20 & 100.00\% & 74  & 75.00\%  \\    
                                  
\midrule
\textbf{Average}    & 14 & 90.63\%  & 96  & 65.03\% \\

\bottomrule             
\end{tabular}
\label{table:onetrust-opt-out-syncing}
\end{table}

==> tables/cookie-syncing-opt-out/quantcast.tex <==

\begin{table}[htb!]
\centering

\caption{Cookie syncing events by advertisers under GDPR and CCPA in Quantcast after opt-out. Evt. column represents the number of cookie syncing events. Pct. represents the percentage of advertisers that participate in cookie syncing.}





    \begin{tabular}{l?{0.3mm}ll?{0.3mm}ll} 
    \toprule

    & \multicolumn{2}{c?{0.3mm}}{\textbf{GDPR}} & \multicolumn{2}{c}{\textbf{CCPA}} \\ 
    


    \multicolumn{1}{c?{0.3mm}}{}  & \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c?{0.3mm}}{\textbf{Pct.}} &  \multicolumn{1}{c}{\textbf{Evt.}} & \multicolumn{1}{c}{\textbf{Pct.}}  \\ 
    \toprule
\textbf{Adult}      & 54 & 45.45\% & 128 & 57.89\%  \\
\textbf{Arts}       & 50 & 46.15\% & 108 & 52.94\%  \\
\textbf{Business}   & 43 & 42.86\% & 118 & 58.82\%  \\
\textbf{Computers}  & 52 & 40.00\% & 122 & 60.00\%  \\
\textbf{Games}      & 61 & 50.00\% & 120 & 63.16\%  \\
\textbf{Health}     & 37 & 46.15\% & 184 & 68.18\%  \\
\textbf{Home}       & 45 & 53.33\% & 101 & 61.11\%  \\
\textbf{Kids}       & 52 & 40.00\% & 136 & 50.00\%  \\
\textbf{News}       & 36 & 46.15\% & 89  & 64.29\%  \\
\textbf{Recreation} & 42 & 50.00\% & 137 & 63.16\%  \\
\textbf{Reference}  & 46 & 46.67\% & 145 & 65.00\%  \\
\textbf{Regional}   & 49 & 38.46\% & 163 & 63.16\%  \\
\textbf{Science}    & 40 & 42.86\% & 146 & 52.94\%  \\
\textbf{Shopping}   & 47 & 45.45\% & 189 & 68.18\%  \\
\textbf{Society}    & 35 & 42.86\% & 109 & 52.94\%  \\
\textbf{Sports}     & 37 & 37.50\% & 83  & 55.56\%  \\    
                                  
\midrule

\textbf{Average}    & 45 & 44.62\% & 130 & 59.83\% \\
\bottomrule             
\end{tabular}
\label{table:quantcast-opt-out-syncing}
\end{table}

==> tables/new/cookiebot-3.tex <==
\begin{table}[!htpb]
    \scriptsize
\centering
\footnotesize
\caption{Ad bidding and cookie syncing under GDPR and CCPA after Pre-opt-out with Cookiebot. Avg. column represents the mean of all bid value after we pre-opt-out. Evt. under C-Sync. represent number of cookie syncing events after pre-opt-out, respectively.}
% \adjustbox{max width=\columnwidth}{
\begin{tabular}{l?{0.3mm}c|c?{0.3mm}c|c} 
\toprule
                    & \multicolumn{2}{c?{0.3mm}}{\textbf{GDPR}}                              & \multicolumn{2}{c}{\textbf{CCPA}}                               \\ 

                    & \textbf{Bids} & \multicolumn{1}{c?{0.3mm}}{\textbf{C-Sync.}} & \textbf{Bids} & \multicolumn{1}{c}{\textbf{C-Sync.}}  \\ 

\textbf{Persona}    & \textbf{Avg.}    & \textbf{Evt.}           & \textbf{Avg.}    & \textbf{Evt.}           \\ 
\toprule

\textbf{Adult}      & 0.37 {\cellcolor{highbids}}& 0  & 0.38 {\cellcolor{highbids}}& 17  \\
\textbf{Arts}       & 0.37 {\cellcolor{highbids}}& 0  & 0.37 {\cellcolor{highbids}}& 27  \\
\textbf{Business}   & 0.37 {\cellcolor{highbids}}& 0  & 0.36 {\cellcolor{highbids}}& 23  \\
\textbf{Computers}  & 0.38 {\cellcolor{highbids}}& 0  & 0.36 {\cellcolor{highbids}}& 16  \\
\textbf{Games}      & 0.37 {\cellcolor{highbids}}& 0  & 0.37 {\cellcolor{highbids}}& 15  \\
\textbf{Health}     & 0.37 {\cellcolor{highbids}}& 0  & 0.38 {\cellcolor{highbids}}& 13  \\
\textbf{Home}       & 0.37 {\cellcolor{highbids}}& 0  & 0.37 {\cellcolor{highbids}}& 0   \\
\textbf{Kids}       & 0.37 {\cellcolor{highbids}}& 0  & 0.38 {\cellcolor{highbids}}& 26  \\
\textbf{News}       & 0.37 {\cellcolor{highbids}}& 0  & 0.37 {\cellcolor{highbids}}& 37  \\
\textbf{Recreation} & 0.37 {\cellcolor{highbids}}& 0  & 0.36 {\cellcolor{highbids}}& 21  \\
\textbf{Reference}  & 0.37 {\cellcolor{highbids}}& 0  & 0.37 {\cellcolor{highbids}}& 0   \\
\textbf{Regional}   & 0.37 {\cellcolor{highbids}}& 0  & 0.37 {\cellcolor{highbids}}& 18  \\
\textbf{Science}    & 0.36 {\cellcolor{highbids}}& 0  & 0.38 {\cellcolor{highbids}}& 0   \\
\textbf{Shopping}   & 0.37 {\cellcolor{highbids}}& 0  & 0.36 {\cellcolor{highbids}}& 13  \\
\textbf{Society}    & 0.38 {\cellcolor{highbids}}& 0  & 0.35 & 47  \\
\textbf{Sports}     & 0.37 {\cellcolor{highbids}}& 0  & 0.37 {\cellcolor{highbids}}& 18  \\
\midrule
\textbf{Control}    & 0.31 & -- & 0.35 & --  \\
\midrule
\textbf{Average}    & --   & 0  & --   & 18  \\
\bottomrule
\end{tabular}
% }
\vspace{-1em}
\label{table:cookiebot-table3}
\end{table}

% \textcolor{highbids}{Light red} and \textcolor{lowbids}{Light blue} indicate bid values that are higher and lower than Control's avg., respectively. \textcolor{higherbids}{Dark red} and \textcolor{lowerbids}{Dark blue} indicate bid values that are Control's avg. $\pm$ std., respectively.

==> tables/new/didomi-3.tex <==
\begin{table}[!htpb]
    \scriptsize
\centering
\footnotesize
\caption{Ad bidding and cookie syncing under GDPR and CCPA after Pre-opt-out with Didomi. Avg. column represents the mean of all bid value after we pre-opt-out. Evt. under C-Sync. represent number of cookie syncing events after pre-opt-out, respectively.}
% \adjustbox{max width=\columnwidth}{
\begin{tabular}{l?{0.3mm}c|c?{0.3mm}c|c} 
\toprule
                    & \multicolumn{2}{c?{0.3mm}}{\textbf{GDPR}}                              & \multicolumn{2}{c}{\textbf{CCPA}}                               \\ 

                    & \textbf{Bids} & \multicolumn{1}{c?{0.3mm}}{\textbf{C-Sync.}} & \textbf{Bids} & \multicolumn{1}{c}{\textbf{C-Sync.}}  \\ 

\textbf{Persona}    & \textbf{Avg.}    & \textbf{Evt.}           & \textbf{Avg.}    & \textbf{Evt.}           \\ 
\toprule
\textbf{Adult}      & 0.02 {\cellcolor{higherbids}}& 6  & 0.13 {\cellcolor{lowbids}}& 39  \\
\textbf{Arts}       & 0.11 {\cellcolor{higherbids}}& 0  & 0.11 {\cellcolor{lowbids}}& 35  \\
\textbf{Business}   & --   & 0  & 0.10 {\cellcolor{lowbids}}& 36  \\
\textbf{Computers}  & 0.01 & 9  & 0.11 {\cellcolor{lowbids}}& 34  \\
\textbf{Games}      & 0.01 & 8  & 0.15 & 45  \\
\textbf{Health}     & 0.13 {\cellcolor{higherbids}}& 13 & 0.09 {\cellcolor{lowbids}}& 41  \\
\textbf{Home}       & --   & 0  & 0.16 {\cellcolor{highbids}}& 37  \\
\textbf{Kids}       & 0.01 & 15 & 0.06 {\cellcolor{lowbids}}& 57  \\
\textbf{News}       & 0.06 {\cellcolor{higherbids}}& 0  & 0.12 {\cellcolor{lowbids}}& 34  \\
\textbf{Recreation} & --   & 0  & 0.10 {\cellcolor{lowbids}}& 57  \\
\textbf{Reference}  & --   & 0  & 0.09 {\cellcolor{lowbids}}& 35  \\
\textbf{Regional}   & --   & 0  & 0.10 {\cellcolor{lowbids}}& 32  \\
\textbf{Science}    & --   & 0  & 0.13 {\cellcolor{lowbids}}& 46  \\
\textbf{Shopping}   & 0.02 {\cellcolor{higherbids}}& 7  & 0.12 {\cellcolor{lowbids}}& 37  \\
\textbf{Society}    & --   & 0  & 0.13 {\cellcolor{lowbids}}& 54  \\
\textbf{Sports}     & --   & 0  & 0.08 {\cellcolor{lowbids}}& 34  \\
\midrule
\textbf{Control}    & 0.01 & -- & 0.15 & --  \\
\midrule
\textbf{Average}    & --   & 4  & --   & 41 \\


\bottomrule
\end{tabular}
% }
\label{table:didomi-table3}
\end{table}

% \textcolor{highbids}{Light red} and \textcolor{lowbids}{Light blue} indicate bid values that are higher and lower than Control's avg., respectively. \textcolor{higherbids}{Dark red} and \textcolor{lowerbids}{Dark blue} indicate bid values that are Control's avg. $\pm$ std., respectively.

==> tables/new/nai-3.tex <==
\begin{table}[!htpb]
    \scriptsize
\centering
\footnotesize
\caption{Ad bidding and cookie syncing under GDPR and CCPA after Pre-opt-out with NAI. Avg. column represents the mean of all bid value after we pre-opt-out. Evt. under C-Sync. represent number of cookie syncing events after pre-opt-out, respectively.}
% \adjustbox{max width=\columnwidth}{
\begin{tabular}{l?{0.3mm}c|c?{0.3mm}c|c} 
\toprule
                    & \multicolumn{2}{c?{0.3mm}}{\textbf{GDPR}}                              & \multicolumn{2}{c}{\textbf{CCPA}}                               \\ 

                    & \textbf{Bids} & \multicolumn{1}{c?{0.3mm}}{\textbf{C-Sync.}} & \textbf{Bids} & \multicolumn{1}{c}{\textbf{C-Sync.}}  \\ 

\textbf{Persona}    & \textbf{Avg.}    & \textbf{Evt.}           & \textbf{Avg.}    & \textbf{Evt.}           \\ 
\toprule
\textbf{Adult}      & 3.3E-4 {\cellcolor{lowbids}}& 16 & 0.07 & 31  \\
\textbf{Arts}       & 4.6E-3 {\cellcolor{higherbids}}& 17 & 0.05 {\cellcolor{lowbids}}& 24  \\
\textbf{Business}   & 0.04   {\cellcolor{higherbids}}  & 11 & 0.05 {\cellcolor{lowbids}}& 27  \\
\textbf{Computers}  & 0.01  {\cellcolor{higherbids}}   & 29 & 0.05 {\cellcolor{lowbids}}& 32  \\
\textbf{Games}      & 6E-4 {\cellcolor{highbids}}& 15 & 0.04 {\cellcolor{lowbids}}& 25  \\
\textbf{Health}     & 0.01  {\cellcolor{higherbids}}   & 5  & 0.52 {\cellcolor{higherbids}}& 71  \\
\textbf{Home}       & 1.7E-3 {\cellcolor{highbids}}& 6  & 0.06 {\cellcolor{lowbids}}& 29  \\
\textbf{Kids}       & 5E-3 {\cellcolor{higherbids}}& 13 & 0.10 {\cellcolor{highbids}}& 59  \\
\textbf{News}       & 3E-4 {\cellcolor{lowbids}}& 13 & 0.04 {\cellcolor{lowbids}}& 31  \\
\textbf{Recreation} & 3.6E-4 {\cellcolor{lowbids}}& 5  & 0.17 {\cellcolor{highbids}}& 45  \\
\textbf{Reference}  & 1.4E-3 {\cellcolor{highbids}}& 22 & 0.02 {\cellcolor{lowbids}}& 30  \\
\textbf{Regional}   & 0.01  {\cellcolor{higherbids}}   & 21 & 0.06 {\cellcolor{lowbids}}& 43  \\
\textbf{Science}    & 0.01  {\cellcolor{higherbids}}   & 10 & 0.05 {\cellcolor{lowbids}}& 49  \\
\textbf{Shopping}   & 0.01  {\cellcolor{higherbids}}   & 16 & 0.05 {\cellcolor{lowbids}}& 50  \\
\textbf{Society}    & 0.01  {\cellcolor{higherbids}}   & 7  & 0.03 {\cellcolor{lowbids}}& 56  \\
\textbf{Sports}     & 0.01  {\cellcolor{higherbids}}   & 1  & 0.10 {\cellcolor{highbids}}& 31  \\
\midrule
\textbf{Control}    & 3.7E-4     & -- & 0.07 & --  \\
\midrule
\textbf{Average}    & --       & 13 & --   & 40 \\


\bottomrule
\end{tabular}
% }
\label{table:nai-table3}
\end{table}

% \textcolor{highbids}{Light red} and \textcolor{lowbids}{Light blue} indicate bid values that are higher and lower than Control's avg., respectively. \textcolor{higherbids}{Dark red} and \textcolor{lowerbids}{Dark blue} indicate bid values that are Control's avg. $\pm$ std., respectively.

==> tables/new/new.tex <==
\begin{table}
\centering
\caption{table1-cookiebot}
\adjustbox{max width=\columnwidth}{
\begin{tabular}{l|l|l|l|l|l|l|l|l} 

                    & \multicolumn{4}{c|}{\textbf{GDPR}}                                                  & \multicolumn{4}{c|}{\textbf{CCPA}}                                                   \\ 

                    & \textbf{Out} & \textbf{In} & \multicolumn{2}{l|}{\textbf{Statistical}} & \textbf{Out} & \textbf{In} & \multicolumn{2}{l|}{\textbf{Statistical}}  \\ 

\textbf{Persona}    & \textbf{Avg.}    & \textbf{Avg.}   & \textbf{p-val} & \textbf{Eff}        & \textbf{Avg.}    & \textbf{Avg.}   & \textbf{p-val} & \textbf{Eff}         \\ 

\textbf{Adult}      & 0.37             & 0.33            & 1.847            & 0.078                       & 0.37             & 0.34            & 2.641            & 0.063                        \\ 

\textbf{Arts}       & 0.35             & 0.32            & 2.645            & 0.063                       & 0.38             & 0.31            & 0.644            & 0.112                        \\ 

\textbf{Business}   & 0.35             & 0.35            & 7.822            & 0.002                       & 0.36             & 0.32            & 3.084            & 0.056                        \\ 

\textbf{Computers}  & 0.35             & 0.36            & 3.713            & 0.046                       & 0.37             & 0.30            & 0.513            & 0.120                        \\ 

\textbf{Games}      & 0.38             & 0.38            & 7.423            & 0.006                       & 0.36             & 0.28            & 0.136            & 0.153                        \\ 

\textbf{Health}     & 0.35             & 0.34            & 6.375            & 0.016                       & 0.38             & 0.38            & 5.359            & 0.028                        \\ 

\textbf{Home}       & 0.38             & 0.31            & 0.751            & 0.107                       & 0.36             & 0.34            & 4.527            & 0.037                        \\ 

\textbf{Kids}       & 0.37             & 0.34            & 2.331            & 0.068                       & 0.35             & 0.29            & 0.323            & 0.127                        \\ 

\textbf{News}       & 0.35             & 0.39            & 2.310            & 0.068                       & 0.37             & 0.33            & 2.119            & 0.071                        \\ 

\textbf{Recreation} & 0.37             & 0.35            & 4.431            & 0.039                       & 0.36             & 0.31            & 1.705            & 0.083                        \\ 

\textbf{Reference}  & 0.37             & 0.33            & 1.846            & 0.078                       & 0.37             & 0.32            & 0.890            & 0.102                        \\ 

\textbf{Regional}   & 0.38             & 0.34            & 2.336            & 0.068                       & 0.35             & 0.30            & 0.934            & 0.100                        \\ 

\textbf{Science}    & 0.35             & 0.39            & 1.477            & 0.085                       & 0.36             & 0.32            & 2.218            & 0.070                        \\ 

\textbf{Shopping}   & 0.37             & 0.35            & 7.328            & 0.007                       & 0.32             & 0.32            & 5.083            & 0.030                        \\ 

\textbf{Society}    & 0.37             & 0.37            & 7.926            & 0.001                       & 0.37             & 0.33            & 1.309            & 0.091                        \\ 

\textbf{Sports}     & 0.37             & 0.35            & 4.392            & 0.040                       & 0.33             & 0.31            & 7.779            & 0.002                        \\ 

\textbf{Control}    & 0.33             & 0.26            & 0.529            & 0.114                       & 0.32             & 0.30            & 6.770            & 0.012                        \\

\end{tabular}
}
\end{table}




\begin{table}
\centering
\caption{table2-cookiebot}
\adjustbox{max width=\columnwidth}{
\begin{tabular}{l|l|l|l|l|l|l} 

                    & \multicolumn{3}{c|}{\textbf{GDPR}}                              & \multicolumn{3}{c|}{\textbf{CCPA}}                               \\ 

                    & \textbf{Opt-out} & \multicolumn{2}{l|}{\textbf{C-Sync}} & \textbf{Opt-out} & \multicolumn{2}{l|}{\textbf{C-Sync}}  \\ 

\textbf{Persona}    & \textbf{Avg.}    & \textbf{out} & \textbf{in}           & \textbf{Avg.}    & \textbf{out} & \textbf{in}            \\ 

\textbf{Adult}      & 0.37             & 0                & 25                        & 0.37             & 0                & 11                         \\ 

\textbf{Arts}       & 0.35             & 0                & 7                         & 0.37             & 4                & 3                          \\ 

\textbf{Business}   & 0.35             & 0                & 44                        & 0.37             & 3                & 3                          \\ 

\textbf{Computers}  & 0.35             & 0                & 28                        & 0.37             & 0                & 4                          \\ 

\textbf{Games}      & 0.38             & 0                & 27                        & 0.36             & 0                & 4                          \\ 

\textbf{Health}     & 0.35             & 0                & 36                        & 0.37             & 28               & 25                         \\ 

\textbf{Home}       & 0.38             & 0                & 3                         & 0.36             & 6                & 14                         \\ 

\textbf{Kids}       & 0.37             & 0                & 41                        & 0.36             & 5                & 26                         \\ 

\textbf{News}       & 0.35             & 3                & 22                        & 0.37             & 3                & 3                          \\ 

\textbf{Recreation} & 0.37             & 0                & 6                         & 0.36             & 21               & 13                         \\ 

\textbf{Reference}  & 0.37             & 0                & 24                        & 0.37             & 14               & 5                          \\ 

\textbf{Regional}   & 0.38             & 0                & 52                        & 0.36             & 28               & 16                         \\ 

\textbf{Science}    & 0.35             & 0                & 26                        & 0.37             & 29               & 18                         \\ 

\textbf{Shopping}   & 0.37             & 0                & 50                        & 0.31             & 37               & 12                         \\ 

\textbf{Society}    & 0.37             & 0                & 5                         & 0.37             & 0                & 5                          \\ 

\textbf{Sports}     & 0.37             & 0                & 43                        & 0.33             & 5                & 7                          \\ 

\textbf{Control}    & 0.33             & --               & --                        & 0.32             & --               & --                         \\

\end{tabular}
}
\end{table}

==> tables/new/onetrust-3.tex <==
\begin{table}[!htpb]
    \scriptsize
\centering
\footnotesize
\caption{Ad bidding and cookie syncing under GDPR and CCPA after Pre-opt-out with Onetrust. Avg. column represents the mean of all bid value after we pre-opt-out. Evt. under C-Sync. represent number of cookie syncing events after pre-opt-out, respectively.}
% \adjustbox{max width=\columnwidth}{
\begin{tabular}{l?{0.3mm}c|c?{0.3mm}c|c} 
\toprule
                    & \multicolumn{2}{c?{0.3mm}}{\textbf{GDPR}}                              & \multicolumn{2}{c}{\textbf{CCPA}}                               \\ 

                    & \textbf{Bids} & \multicolumn{1}{c?{0.3mm}}{\textbf{C-Sync.}} & \textbf{Bids} & \multicolumn{1}{c}{\textbf{C-Sync.}}  \\ 

\textbf{Persona}    & \textbf{Avg.}    & \textbf{Evt.}           & \textbf{Avg.}    & \textbf{Evt.}           \\ 
\toprule
\textbf{Adult}      & 0.08 {\cellcolor{highbids}}& 19 & 0.38 {\cellcolor{lowbids}}& 107  \\
\textbf{Arts}       & 0.16 {\cellcolor{higherbids}}& 29 & 1.05 {\cellcolor{highbids}}& 90   \\
\textbf{Business}   & 0.09 {\cellcolor{highbids}}& 46 & 1.26 {\cellcolor{highbids}}& 77   \\
\textbf{Computers}  & 0.05 {\cellcolor{lowbids}}& 20 & 1.12 {\cellcolor{highbids}}& 79   \\
\textbf{Games}      & 0.07 & 30 & 0.73 {\cellcolor{lowbids}}& 109  \\
\textbf{Health}     & 0.11 {\cellcolor{highbids}}& 21 & 0.61 {\cellcolor{lowbids}}& 134  \\
\textbf{Home}       & 0.08 {\cellcolor{highbids}}& 46 & 0.80 {\cellcolor{highbids}}& 46   \\
\textbf{Kids}       & 0.13 {\cellcolor{highbids}}& 34 & 0.59 {\cellcolor{lowbids}}& 111  \\
\textbf{News}       & 0.08 {\cellcolor{highbids}}& 21 & 0.66 {\cellcolor{lowbids}}& 100  \\
\textbf{Recreation} & 0.02 {\cellcolor{lowbids}}& 4  & 0.50 {\cellcolor{lowbids}}& 61   \\
\textbf{Reference}  & 0.06 {\cellcolor{lowbids}}& 34 & 0.67 {\cellcolor{lowbids}}& 64   \\
\textbf{Regional}   & 0.04 {\cellcolor{lowbids}}& 34 & 0.50 {\cellcolor{lowbids}}& 106  \\
\textbf{Science}    & 0.12 {\cellcolor{highbids}}& 16 & 0.81 {\cellcolor{highbids}}& 71   \\
\textbf{Shopping}   & 0.17 {\cellcolor{higherbids}}& 41 & 0.86 {\cellcolor{highbids}}& 62   \\
\textbf{Society}    & 0.14 {\cellcolor{highbids}}& 54 & 0.31 {\cellcolor{lowbids}}& 94   \\
\textbf{Sports}     & 0.07 & 41 & 0.75 {\cellcolor{highbids}}& 112  \\
\midrule
\textbf{Control}    & 0.07 & -- & 0.74 & --   \\
\midrule
\textbf{Average}    & --   & 31 & --   & 89  \\

\bottomrule
\end{tabular}
% }
\label{table:onetrust-table3}
\end{table}

% \textcolor{highbids}{Light red} and \textcolor{lowbids}{Light blue} indicate bid values that are higher and lower than Control's avg., respectively. \textcolor{higherbids}{Dark red} and \textcolor{lowerbids}{Dark blue} indicate bid values that are Control's avg. $\pm$ std., respectively.

==> tables/new/quantcast-3.tex <==
\begin{table}[!htpb]
    \scriptsize
\centering
\footnotesize
\caption{Ad bidding and cookie syncing under GDPR and CCPA after Pre-opt-out with Quantcast. Avg. column represents the mean of all bid value after we pre-opt-out. Evt. under C-Sync. represent number of cookie syncing events after pre-opt-out, respectively.}
% \adjustbox{max width=\columnwidth}{
\begin{tabular}{l?{0.3mm}c|c?{0.3mm}c|c} 
\toprule
                    & \multicolumn{2}{c?{0.3mm}}{\textbf{GDPR}}                              & \multicolumn{2}{c}{\textbf{CCPA}}                               \\ 

                    & \textbf{Bids} & \multicolumn{1}{c?{0.3mm}}{\textbf{C-Sync.}} & \textbf{Bids} & \multicolumn{1}{c}{\textbf{C-Sync.}}  \\ 

\textbf{Persona}    & \textbf{Avg.}    & \textbf{Evt.}           & \textbf{Avg.}    & \textbf{Evt.}           \\ 
\toprule
\textbf{Adult}      & 0.58 {\cellcolor{higherbids}}& 27 & 0.18 {\cellcolor{lowbids}}& 125  \\
\textbf{Arts}       & 0.16 {\cellcolor{highbids}}& 24 & 0.22 {\cellcolor{highbids}}& 90   \\
\textbf{Business}   & 0.58 {\cellcolor{higherbids}}& 26 & 0.17 {\cellcolor{lowbids}}& 94   \\
\textbf{Computers}  & 0.16 {\cellcolor{highbids}}& 37 & 0.32 {\cellcolor{highbids}}& 73   \\
\textbf{Games}      & 0.16 {\cellcolor{highbids}}& 20 & 0.19 {\cellcolor{lowbids}}& 96   \\
\textbf{Health}     & 0.16 {\cellcolor{highbids}}& 12 & 0.44 {\cellcolor{highbids}}& 89   \\
\textbf{Home}       & 0.23 {\cellcolor{higherbids}}& 27 & 0.18 {\cellcolor{lowbids}}& 104  \\
\textbf{Kids}       & 0.60 {\cellcolor{higherbids}}& 41 & 0.17 {\cellcolor{lowbids}}& 90   \\
\textbf{News}       & 0.55 {\cellcolor{higherbids}}& 25 & 0.17 {\cellcolor{lowbids}}& 66   \\
\textbf{Recreation} & 0.64 {\cellcolor{higherbids}}& 23 & 0.17 {\cellcolor{lowbids}}& 83   \\
\textbf{Reference}  & 0.16 {\cellcolor{highbids}}& 31 & 0.16 {\cellcolor{lowbids}}& 95   \\
\textbf{Regional}   & 0.15 {\cellcolor{highbids}}& 37 & 0.22 {\cellcolor{highbids}}& 137  \\
\textbf{Science}    & 0.55 {\cellcolor{higherbids}}& 16 & 0.20 {\cellcolor{lowbids}}& 86   \\
\textbf{Shopping}   & 0.60 {\cellcolor{higherbids}}& 25 & 0.21 & 98   \\
\textbf{Society}    & 0.16 {\cellcolor{highbids}}& 21 & 0.20 {\cellcolor{lowbids}}& 91   \\
\textbf{Sports}     & 0.16 {\cellcolor{highbids}}& 27 & 0.16 {\cellcolor{lowbids}}& 107  \\
\midrule
\textbf{Control}    & 0.14 & -- & 0.21 & --   \\
\midrule
\textbf{Average}    & --   & 26 & --   & 95  \\

\bottomrule
\end{tabular}
% }
\label{table:quantcast-table3}
\end{table}

% \textcolor{highbids}{Light red} and \textcolor{lowbids}{Light blue} indicate bid values that are higher and lower than Control's avg., respectively. \textcolor{higherbids}{Dark red} and \textcolor{lowerbids}{Dark blue} indicate bid values that are Control's avg. $\pm$ std., respectively.

==> tables/statistical-analysis-out-vs-in/NAI.tex <==

\begin{table}[htb!]
\centering

\caption{Mann–Whitney U test to validate our hypothesis that the advertisers bidding behavior does not significantly change between opt-in and opt-out under GDPR and CCPA in NAI. Column P and R represent p-value and effect size, respectively. Effect size is calculated only in cases when there is statistically significant difference (when p-value is smaller than 0.05 after bonferroni correction). Otherwise, we use “–” in the table, to represent that we do not calculate this effect size.}





    \begin{tabular}{l?{0.3mm}ll?{0.3mm}ll} 
    \toprule

    & \multicolumn{2}{c?{0.3mm}}{\textbf{GDPR}} & \multicolumn{2}{c}{\textbf{CCPA}} \\ 
    


    \multicolumn{1}{c?{0.3mm}}{}  & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c?{0.3mm}}{\textbf{E}} &  \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c}{\textbf{E}}  \\ 
    \toprule
\textbf{Adult}      & 6.883 & 0.004 & 4.887 & 0.034  \\
\textbf{Arts}       & 4.498 & 0.022 & 0.127 & 0.154  \\
\textbf{Business}   & 2.719 & 0.039 & 0.226 & 0.136  \\
\textbf{Computers}  & 5.986 & 0.010 & 2.173 & 0.066  \\
\textbf{Games}      & 2.083 & 0.019 & 0.218 & 0.136  \\
\textbf{Health}     & 6.938 & 0.007 & 1.901 & 0.079  \\
\textbf{Home}       & --    & --    & 6.508 & 0.015  \\
\textbf{Kids}       & 6.484 & 0.009 & 1.886 & 0.075  \\
\textbf{News}       & 5.484 & 0.011 & 0.595 & 0.114  \\
\textbf{Recreation} & 7.024 & 0.006 & 0.156 & 0.166  \\
\textbf{Reference}  & 1.583 & 0.047 & 0.049 & 0.175  \\
\textbf{Regional}   & 1.857 & 0.044 & 7.888 & 0.001  \\
\textbf{Science}    & 4.190 & 0.022 & 3.562 & 0.040  \\
\textbf{Shopping}   & 4.864 & 0.021 & 7.942 & 0.001  \\
\textbf{Society}    & 1.416 & 0.038 & 0.229 & 0.145  \\
\textbf{Sports}     & 3.435 & 0.030 & 0.243 & 0.148  \\
\bottomrule             
\end{tabular}
\label{table:NAI-mann}
\end{table}

==> tables/statistical-analysis-out-vs-in/cookiebot.tex <==

\begin{table}[htb!]
\centering

\caption{Mann–Whitney U test to validate our hypothesis that the advertisers bidding behavior does not significantly change between opt-in and opt-out under GDPR and CCPA in Cookiebot. Column P and R represent p-value and effect size, respectively. Effect size is calculated only in cases when there is statistically significant difference (when p-value is smaller than 0.05 after bonferroni correction). Otherwise, we use “–” in the table, to represent that we do not calculate this effect size.}





    \begin{tabular}{l?{0.3mm}ll?{0.3mm}ll} 
    \toprule

    & \multicolumn{2}{c?{0.3mm}}{\textbf{GDPR}} & \multicolumn{2}{c}{\textbf{CCPA}} \\ 
    


    \multicolumn{1}{c?{0.3mm}}{}  & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c?{0.3mm}}{\textbf{E}} &  \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c}{\textbf{E}}  \\ 
    \toprule
    
\textbf{Adult}      & 1.847 & 0.078 & 2.641 & 0.063  \\
\textbf{Arts}       & 2.645 & 0.063 & 0.644 & 0.112  \\
\textbf{Business}   & 7.822 & 0.002 & 3.084 & 0.056  \\
\textbf{Computers}  & 3.713 & 0.046 & 0.513 & 0.120  \\
\textbf{Games}      & 7.423 & 0.006 & 0.136 & 0.153  \\
\textbf{Health}     & 6.375 & 0.016 & 5.359 & 0.028  \\
\textbf{Home}       & 0.751 & 0.107 & 4.527 & 0.037  \\
\textbf{Kids}       & 2.331 & 0.068 & 0.323 & 0.127  \\
\textbf{News}       & 2.310 & 0.068 & 2.119 & 0.071  \\
\textbf{Recreation} & 4.431 & 0.039 & 1.705 & 0.083  \\
\textbf{Reference}  & 1.846 & 0.078 & 0.890 & 0.102  \\
\textbf{Regional}   & 2.336 & 0.068 & 0.934 & 0.100  \\
\textbf{Science}    & 1.477 & 0.085 & 2.218 & 0.070  \\
\textbf{Shopping}   & 7.328 & 0.007 & 5.083 & 0.030  \\
\textbf{Society}    & 7.926 & 0.001 & 1.309 & 0.091  \\
\textbf{Sports}     & 4.392 & 0.040 & 7.779 & 0.002 \\
\bottomrule             
\end{tabular}
\label{table:cookiebot-mann}
\end{table}

==> tables/statistical-analysis-out-vs-in/didomi.tex <==

\begin{table}[htb!]
\centering

\caption{Mann–Whitney U test to validate our hypothesis that the advertisers bidding behavior does not significantly change between opt-in and opt-out under GDPR and CCPA in Didomi. Column P and R represent p-value and effect size, respectively. Effect size is calculated only in cases when there is statistically significant difference (when p-value is smaller than 0.05 after bonferroni correction). Otherwise, we use “–” in the table, to represent that we do not calculate this effect size.}





    \begin{tabular}{l?{0.3mm}ll?{0.3mm}ll} 
    \toprule

    & \multicolumn{2}{c?{0.3mm}}{\textbf{GDPR}} & \multicolumn{2}{c}{\textbf{CCPA}} \\ 
    


    \multicolumn{1}{c?{0.3mm}}{}  & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c?{0.3mm}}{\textbf{E}} &  \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c}{\textbf{E}}  \\ 
    \toprule
    
\textbf{Adult}      & 0.000 & inf      & 7.52E-07 & 0.204  \\
\textbf{Arts}       & 5.996 & 0.011    & 6.28E-18 & 0.309  \\
\textbf{Business}   & 0.000 & inf      & 3.83E-12 & 0.260  \\
\textbf{Computers}  & 6.309 & 0.008    & 4.17E-17 & 0.287  \\
\textbf{Games}      & 2.520 & 0.030    & 3.62E-10 & 0.245  \\
\textbf{Health}     & 0.000 & inf      & 1.86E-11 & 0.234  \\
\textbf{Home}       & 7.436 & 0.003    & 9.18E-14 & 0.290  \\
\textbf{Kids}       & 7.522 & 0.003    & 2.17E-05 & 0.154  \\
\textbf{News}       & 0.000 & inf      & 3.98E-10 & 0.226  \\
\textbf{Recreation} & 5.615 & 0.012    & 3.89E-12 & 0.270  \\
\textbf{Reference}  & 0.000 & inf      & 1.74E-09 & 0.226  \\
\textbf{Regional}   & 0.000 & inf      & 1.90E-27 & 0.372  \\
\textbf{Science}    & 1.122 & 0.041    & 8.71E-14 & 0.265  \\
\textbf{Shopping}   & 7.232 & 0.004    & 1.33E-11 & 0.233  \\
\textbf{Society}    & 6.585 & 0.007    & 2.42E-12 & 0.261  \\
\textbf{Sports}     & 7.978 & 1.08E-04 & 2.46E-12 & 0.233  \\
\bottomrule             
\end{tabular}
\label{table:didomi-mann}
\end{table}

==> tables/statistical-analysis-out-vs-in/onetrust.tex <==

\begin{table}[htb!]
\centering

\caption{Mann–Whitney U test to validate our hypothesis that the advertisers bidding behavior does not significantly change between opt-in and opt-out under GDPR and CCPA in Onetrust. Column P and R represent p-value and effect size, respectively. Effect size is calculated only in cases when there is statistically significant difference (when p-value is smaller than 0.05 after bonferroni correction). Otherwise, we use “–” in the table, to represent that we do not calculate this effect size.}





    \begin{tabular}{l?{0.3mm}ll?{0.3mm}ll} 
    \toprule

    & \multicolumn{2}{c?{0.3mm}}{\textbf{GDPR}} & \multicolumn{2}{c}{\textbf{CCPA}} \\ 
    


    \multicolumn{1}{c?{0.3mm}}{}  & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c?{0.3mm}}{\textbf{E}} &  \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c}{\textbf{E}}  \\ 
    \toprule
    
\textbf{Adult}      & 8.000 & 0.000 & 2.27E-06 & 0.354  \\
\textbf{Arts}       & 0.000 & inf   & 4.628    & 0.053  \\
\textbf{Business}   & 0.284 & 0.423 & 5.46E-11 & 0.496  \\
\textbf{Computers}  & 2.009 & 0.278 & 4.504    & 0.052  \\
\textbf{Games}      & 8.000 & 0.000 & 0.473    & 0.106  \\
\textbf{Health}     & 0.111 & 0.775 & 7.74E-06 & 0.310  \\
\textbf{Home}       & 2.520 & 0.366 & 2.230    & 0.098  \\
\textbf{Kids}       & 0.619 & 0.439 & 1.18E-04 & 0.226  \\
\textbf{News}       & 0.318 & 0.640 & 0.657    & 0.099  \\
\textbf{Recreation} & 0.018 & 0.812 & 3.58E-11 & 0.389  \\
\textbf{Reference}  & 3.069 & 0.306 & 3.69E-05 & 0.265  \\
\textbf{Regional}   & 2.431 & 0.244 & 6.05E-11 & 0.430  \\
\textbf{Science}    & 1.750 & 0.422 & 0.161    & 0.170  \\
\textbf{Shopping}   & 3.836 & 0.354 & 0.574    & 0.101  \\
\textbf{Society}    & 2.232 & 0.248 & 1.83E-05 & 0.366  \\
\textbf{Sports}     & 0.155 & 0.469 & 0.605    & 0.104  \\

\bottomrule             
\end{tabular}
\label{table:onetrust-mann}
\end{table}

==> tables/statistical-analysis-out-vs-in/quantcast.tex <==

\begin{table}[htb!]
\centering

\caption{Mann–Whitney U test to validate our hypothesis that the advertisers bidding behavior does not significantly change between opt-in and opt-out under GDPR and CCPA in Quantcast. Column P and R represent p-value and effect size, respectively. Effect size is calculated only in cases when there is statistically significant difference (when p-value is smaller than 0.05 after bonferroni correction). Otherwise, we use “–” in the table, to represent that we do not calculate this effect size.}





    \begin{tabular}{l?{0.3mm}ll?{0.3mm}ll} 
    \toprule

    & \multicolumn{2}{c?{0.3mm}}{\textbf{GDPR}} & \multicolumn{2}{c}{\textbf{CCPA}} \\ 
    


    \multicolumn{1}{c?{0.3mm}}{}  & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c?{0.3mm}}{\textbf{E}} &  \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c}{\textbf{E}}  \\ 
    \toprule
    
\textbf{Adult}      & 0.307    & 0.073 & 0.007 & 0.121  \\
\textbf{Arts}       & 0.271    & 0.071 & 5.166 & 0.016  \\
\textbf{Business}   & 0.001    & 0.133 & 1.839 & 0.042  \\
\textbf{Computers}  & 0.814    & 0.055 & 4.979 & 0.017  \\
\textbf{Games}      & 0.083    & 0.087 & 0.007 & 0.109  \\
\textbf{Health}     & 1.980    & 0.040 & 0.407 & 0.065  \\
\textbf{Home}       & 4.204    & 0.022 & 0.057 & 0.093  \\
\textbf{Kids}       & 2.758    & 0.032 & 5.162 & 0.016  \\
\textbf{News}       & 0.022    & 0.112 & 0.620 & 0.067  \\
\textbf{Recreation} & 0.085    & 0.092 & 2.805 & 0.034  \\
\textbf{Reference}  & 5.863    & 0.012 & 0.419 & 0.070  \\
\textbf{Regional}   & 2.22E-04 & 0.144 & 5.855 & 0.012  \\
\textbf{Science}    & 1.383    & 0.044 & 0.061 & 0.097  \\
\textbf{Shopping}   & 0.004    & 0.135 & 4.004 & 0.023  \\
\textbf{Society}    & 1.483    & 0.047 & 2.017 & 0.041  \\
\textbf{Sports}     & 0.001    & 0.128 & 2.192 & 0.038  \\

\bottomrule             
\end{tabular}
\label{table:quantcast-mann}
\end{table}
